Structure and Melting of Fe, MgO, SiO2, and MgSiO3 in Planets: Database, Inversion, and Phase Diagram

We present globally inverted pressure-temperature (P-T) phase diagrams up to 5,000 GPa for four fundamental planetary materials, Fe, MgO, SiO2, and MgSiO3, derived from logistic regression and supervised learning, together with an experimental phase equilibria database. These new P-T phase diagrams provide a solution to long-standing disputes about their melting curves. Their implications extend to the melting and freezing of rocky materials in the interior of giant planets and super-Earth exoplanets, contributing to the refinement of their internal structure models.

==> ref.tex <==
%%%%%%%%%%%%%%%%%%%%
INTRODUCTION
%%%%%%%%%%%%%%%%%%%%
@article{kojitani_precise_2016,
	title = {Precise measurements of enthalpy of postspinel transition in {Mg2SiO4} and application to the phase boundary calculation},
	volume = {121},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1002/2015JB012211},
	doi = {https://doi.org/10.1002/2015JB012211},
	abstract = {Abstract Drop solution enthalpies (ΔH°d-s) of Mg2SiO4 ringwoodite, Mg2SiO4 forsterite, perovskite-type MgSiO3 (bridgmanite), and MgSiO3 enstatite were measured using a single batch of 2PbO · B2O3 solvent at 978 K. From the obtained ΔH°d-s values of Mg2SiO4 ringwoodite, MgSiO3 bridgmanite, and MgO, an enthalpy of the postspinel phase transition, Mg2SiO4 ringwoodite = MgSiO3 bridgmanite + MgO, was determined to be 78.54 ± 2.28 kJ/mol. Thermodynamic calculations using the obtained phase transition enthalpy and available thermochemical and thermoelastic data provided the phase transition pressure of 23.1 ± 1.4 GPa at 298 K. This value is comparable to those at about 2000 K determined by previous experimental and theoretical studies, implying a considerably gentle Clapeyron slope. Thermodynamic calculations of the postspinel boundary at high temperatures in the anhydrous condition by changing thermochemical and thermoelastic parameters within the uncertainties suggested that the postspinel transition pressure of Mg2SiO4 at high temperature is lower than the pressure corresponding to the global average depth of the “660 km” seismic discontinuity in the Earth's mantle ( 23.5 GPa) estimated from one-dimensional reference Earth models and that a most likely Clapeyron slope is about −1 MPa/K. The postspinel transition in the hydrous condition with about 2 wt \% H2O, which shows higher transition pressure and steeper Clapeyron slope than those in the anhydrous condition, gives a plausible explanation for seismic observations on the 660 km discontinuity, and therefore, hydrous mantle transition zone would be required.},
	number = {2},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Kojitani, Hiroshi and Inoue, Toru and Akaogi, Masaki},
	year = {2016},
	note = {\_eprint: https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1002/2015JB012211},
	keywords = {660 km seismic discontinuity, calorimetry, Clapeyron slope, phase transition enthalpy, postspinel phase boundary, thermodynamic calculation},
	pages = {729--742},
}

@book{young_phase_1991,
	address = {Berkeley, Calif.},
	title = {Phase diagrams of the elements},
	isbn = {978-0-520-07483-5},
	language = {eng},
	publisher = {Univ. of California Press},
	author = {Young, David A.},
	year = {1991},
	annote = {Includes bibliographical references and index},
}

@book{lewis_physics_2004,
	address = {Amsterdam ; Boston},
	edition = {2nd ed},
	series = {This is volume 87 in the {International} geophysics series},
	title = {Physics and chemistry of the solar system},
	isbn = {978-0-12-446744-6},
	publisher = {Elsevier Academic Press},
	author = {Lewis, John S.},
	year = {2004},
	keywords = {Astrophysics, Cosmochemistry, Planetary science, Solar system},
}
@book{seager_exoplanets_2010,
	address = {Tucson},
	series = {The {University} of {Arizona} space science series},
	title = {Exoplanets},
	isbn = {978-0-8165-2945-2},
	language = {eng},
	publisher = {University of Arizona press},
	author = {Seager, Sara and Dotson, Renée},
	year = {2010},
}
@book{perryman_exoplanet_2018,
	edition = {2},
	title = {The {Exoplanet} {Handbook}},
	isbn = {978-1-108-41977-2 978-1-108-30416-0},
	shorttitle = {The {Exoplanet} {Handbook}},
	url = {https://www.cambridge.org/core/product/identifier/9781108304160/type/book},
	urldate = {2024-07-31},
	publisher = {Cambridge University Press},
	author = {Perryman, Michael},
	month = aug,
	year = {2018},
	doi = {10.1017/9781108304160},
}

@techreport{simon_uranus_2021,
	title = {Uranus {Orbiter} and {Probe}: {Journey} to an {Ice} {Giant} {System}},
	url = {https://smd-cms.nasa.gov/wp-content/uploads/2023/10/uranus-orbiter-and-probe.pdf},
	institution = {National Aeronautics and Space Administration (NASA)},
	author = {Simon, Amy and Nimmo, Francis and Anderson, Richard C.},
	year = {2021},
	file = {uranus-orbiter-and-probe.pdf:/Users/jdong/Zotero/storage/JXJ6ZFGE/uranus-orbiter-and-probe.pdf:application/pdf},
}

@techreport{rymer_neptune_2021,
	title = {Neptune {Odyssey}: {Mission} to the {Neptune}-{Triron} {System}},
	url = {https://smd-cms.nasa.gov/wp-content/uploads/2023/05/NeptuneOdyssey.pdf},
	language = {en},
	institution = {National Aeronautics and Space Administration (NASA)},
	author = {Rymer, Abigail and Clyde, Brenda and Runyon, Kirby},
	year = {2021},
	file = {Rymer et al. - We are enormously proud to be part of a large nati.pdf:/Users/jdong/Zotero/storage/GP8ZHCGQ/Rymer et al. - We are enormously proud to be part of a large nati.pdf:application/pdf},
}
@article{helled_revelations_2022,
	title = {Revelations on {Jupiter}'s formation, evolution and interior: {Challenges} from {Juno} results},
	volume = {378},
	issn = {00191035},
	shorttitle = {Revelations on {Jupiter}'s formation, evolution and interior},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0019103522000586},
	doi = {10.1016/j.icarus.2022.114937},
	language = {en},
	urldate = {2024-07-22},
	journal = {Icarus},
	author = {Helled, Ravit and Stevenson, David J. and Lunine, Jonathan I. and Bolton, Scott J. and Nettelmann, Nadine and Atreya, Sushil and Guillot, Tristan and Militzer, Burkhard and Miguel, Yamila and Hubbard, William B.},
	month = may,
	year = {2022},
	pages = {114937},
	file = {Full Text:/Users/jdong/Zotero/storage/RN7Z894L/Helled et al. - 2022 - Revelations on Jupiter's formation, evolution and .pdf:application/pdf},
}
@incollection{baines_interior_2018,
	edition = {1},
	title = {The {Interior} of {Saturn}},
	isbn = {978-1-316-22722-0 978-1-107-10677-2 978-1-107-51446-1},
	url = {https://www.cambridge.org/core/product/identifier/9781316227220%23CN-bp-3/type/book_part},
	urldate = {2024-07-31},
	booktitle = {Saturn in the 21st {Century}},
	publisher = {Cambridge University Press},
	author = {Fortney, Jonathan J. and Helled, Ravit and Nettelmann, Nadine and Stevenson, David J. and Marley, Mark S. and Hubbard, William B. and Iess, Luciano},
	editor = {Baines, Kevin H. and Flasar, F. Michael and Krupp, Norbert and Stallard, Tom},
	month = nov,
	year = {2018},
	doi = {10.1017/9781316227220.003},
	pages = {44--68},
	file = {Fortney et al. - 2018 - The Interior of Saturn.pdf:/Users/jdong/Zotero/storage/Y5SPYXFV/Fortney et al. - 2018 - The Interior of Saturn.pdf:application/pdf},
}
@article{boujibar_superearth_2020,
	title = {Super‐{Earth} {Internal} {Structures} and {Initial} {Thermal} {States}},
	volume = {125},
	issn = {2169-9097, 2169-9100},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2019JE006124},
	doi = {10.1029/2019JE006124},
	abstract = {Abstract
            
              The presence of a planetary magnetic field is an important ingredient for habitability. The coexistence of a solid and a liquid core can facilitate the maintenance of a compositionally driven dynamo; however, the likelihood of such a configuration in super‐Earths is unknown. Recently, shock experiments and ab initio calculations have constrained the stability, equations of state, and melting properties of ultrahigh pressure core and mantle phases. Here, we investigate the internal structure of super‐Earth exoplanets with a range of total masses and core mass fractions ranging from that of Mars (0.2) to Mercury (0.68), including an Earth‐like bulk composition. We examine the effect of the initial core‐mantle boundary temperature (
              T
              CMB
              ) on their internal structure and identify regimes with coexisting solid and liquid cores, and deep mantle melting. We find that the range of
              T
              CMB
              for which an inner core is growing increases with the total planet mass and even more with the core mass fraction. Therefore, our results suggest that super‐Earths should have a crystallizing core over a large temperature range. We also find that the presence of a growing inner core is likely to be accompanied by a partially liquid lower mantle, which will likely influence planetary thermal evolution. We estimate the initial CMB temperature after super‐Earth accretion by assuming an accretional heat retention efficiency similar to Earth. We find that massive super‐Earths are expected to have an initial internal temperature consistent with a partially liquid core, allowing for the possibility of thermal and compositional dynamo action.
            
          , 
            Plain Language Summary
            The presence of a magnetic field in a planetary body is an important criterion for habitability, since it may reduce atmospheric loss and shield planetary surfaces from high‐energy charged particles. In terrestrial planets, when an inner iron‐rich core crystallizes, it releases light elements in the residual liquid outer core, which can facilitate liquid iron alloy convection and contribute to the maintenance of a magnetic field. In this study, we investigate the optimal conditions for the presence of a crystallizing core in super‐Earths (i.e., large rocky exoplanets), by modeling their internal structure and using recent data on the melting properties of materials at ultrahigh pressure. We find that cores of super‐Earths of large sizes have a greater likelihood to be partially molten, which may aid in maintaining a magnetic field. In addition, the lowermost mantle of massive super‐Earths are likely to experience prolonged partial melting. Increasing the size of their core relative to their mantle increases even more the probability of a growing inner core. In addition, we calculate the initial heat retained during planetary formation, which confirms that large super‐Earths are likely to have an initial crystallizing core.
          , 
            Key Points
            
              
                
                  We modeled the internal structure of super‐Earths and investigated the likelihood that an inner core exists
                
                
                  Super‐Earths with a large core have a wide range of temperature at the core mantle boundary over which a solid and a liquid core coexist
                
                
                  Increasing the size of super‐Earths iron core increases the likelihood of maintaining an inner core and deep mantle melting},
	language = {en},
	number = {5},
	urldate = {2024-07-22},
	journal = {Journal of Geophysical Research: Planets},
	author = {Boujibar, A. and Driscoll, P. and Fei, Y.},
	month = may,
	year = {2020},
	pages = {e2019JE006124},
}
@article{militzer_relation_2023,
	title = {Relation of {Gravity}, {Winds}, and the {Moment} of {Inertia} of {Jupiter} and {Saturn}},
	volume = {4},
	issn = {2632-3338},
	url = {https://iopscience.iop.org/article/10.3847/PSJ/acd2cd},
	doi = {10.3847/PSJ/acd2cd},
	abstract = {Abstract
            
              We study the relationship of zonal gravity coefficients,
              J
              
                2
                n
              
              , zonal winds, and axial moment of inertia (MoI) by constructing models for the interiors of giant planets. We employ the nonperturbative concentric Maclaurin spheroid method to construct both physical (realistic equation of state and barotropes) and abstract (small number of constant-density spheroids) interior models. We find that accurate gravity measurements of Jupiter’s and Saturn’s
              J
              2
              ,
              J
              4
              , and
              J
              6
              by the Juno and Cassini spacecraft do not uniquely determine the MoI of either planet but do constrain it to better than 1\%. Zonal winds (or differential rotation (DR)) then emerge as the leading source of uncertainty. For Saturn they are predicted to decrease the MoI by 0.4\% because they reach a depth of ∼9000 km, while on Jupiter they appear to reach only ∼3000 km. We thus predict DR to affect Jupiter’s MoI by only 0.01\%, too small by one order of magnitude to be detectable by the Juno spacecraft. We find that winds primarily affect the MoI indirectly via the gravity harmonic
              J
              6
              , while direct contributions are much smaller because the effects of pro- and retrograde winds cancel. DR contributes +6\% and −0.8\% to Saturn’s and Jupiter’s
              J
              6
              value, respectively. This changes the
              J
              6
              contribution that comes from the uniformly rotating bulk of the planet that correlates most strongly with the predicted MoI. With our physical models, we predict Jupiter’s MoI to be 0.26393 ± 0.00001. For Saturn, we predict 0.2181 ± 0.0002, assuming a rotation period of 10:33:34 hr that matches the observed polar radius.},
	number = {5},
	urldate = {2024-07-22},
	journal = {The Planetary Science Journal},
	author = {Militzer, Burkhard and Hubbard, William B.},
	month = may,
	year = {2023},
	pages = {95},
	file = {Full Text:/Users/jdong/Zotero/storage/PIQMD6VE/Militzer and Hubbard - 2023 - Relation of Gravity, Winds, and the Moment of Iner.pdf:application/pdf},
}

@article{militzer_study_2024,
	title = {Study of {Jupiter}’s interior: {Comparison} of 2, 3, 4, 5, and 6 layer models},
	volume = {411},
	issn = {00191035},
	shorttitle = {Study of {Jupiter}’s interior},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0019103524000137},
	doi = {10.1016/j.icarus.2024.115955},
	language = {en},
	urldate = {2024-07-22},
	journal = {Icarus},
	author = {Militzer, Burkhard and Hubbard, William B.},
	month = mar,
	year = {2024},
	pages = {115955},
	file = {Submitted Version:/Users/jdong/Zotero/storage/LT9KW4VP/Militzer and Hubbard - 2024 - Study of Jupiter’s interior Comparison of 2, 3, 4.pdf:application/pdf},
}


@article{soderlund_underexplored_2020,
	title = {The underexplored frontier of ice giant dynamos},
	volume = {378},
	issn = {1364-503X, 1471-2962},
	url = {https://royalsocietypublishing.org/doi/10.1098/rsta.2019.0479},
	doi = {10.1098/rsta.2019.0479},
	abstract = {The
              Voyager 2
              flybys of Uranus and Neptune revealed the first multipolar planetary magnetic fields and highlighted how much we have yet to learn about ice giant planets. In this review, we summarize observations of Uranus’ and Neptune’s magnetic fields and place them in the context of other planetary dynamos. The ingredients for dynamo action in general, and for the ice giants in particular, are discussed, as are the factors thought to control magnetic field strength and morphology. These ideas are then applied to Uranus and Neptune, where we show that no models are yet able to fully explain their observed magnetic fields. We then propose future directions for missions, modelling, experiments and theory necessary to answer outstanding questions about the dynamos of ice giant planets, both within our solar system and beyond.
            
            This article is part of a discussion meeting issue ‘Future exploration of ice giant systems’.},
	language = {en},
	number = {2187},
	urldate = {2024-07-20},
	journal = {Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
	author = {Soderlund, K. M. and Stanley, S.},
	month = dec,
	year = {2020},
	pages = {20190479},
	file = {Full Text:/Users/jdong/Zotero/storage/7BWCVW72/Soderlund and Stanley - 2020 - The underexplored frontier of ice giant dynamos.pdf:application/pdf},
}
@article{grasselli_heat_2020,
	title = {Heat and charge transport in {H2O} at ice-giant conditions from ab initio molecular dynamics simulations},
	volume = {11},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-020-17275-5},
	doi = {10.1038/s41467-020-17275-5},
	abstract = {Abstract
            The impact of the inner structure and thermal history of planets on their observable features, such as luminosity or magnetic field, crucially depends on the poorly known heat and charge transport properties of their internal layers. The thermal and electric conductivities of different phases of water (liquid, solid, and super-ionic) occurring in the interior of ice giant planets, such as Uranus or Neptune, are evaluated from equilibrium ab initio molecular dynamics, leveraging recent progresses in the theory and data analysis of transport in extended systems. The implications of our findings on the evolution models of the ice giants are briefly discussed.},
	language = {en},
	number = {1},
	urldate = {2024-07-20},
	journal = {Nature Communications},
	author = {Grasselli, Federico and Stixrude, Lars and Baroni, Stefano},
	month = jul,
	year = {2020},
	pages = {3605},
	file = {Full Text:/Users/jdong/Zotero/storage/SBHVVKYM/Grasselli et al. - 2020 - Heat and charge transport in H2O at ice-giant cond.pdf:application/pdf},
}
@article{james_thermal_2024,
	title = {Thermal and {Tidal} {Evolution} of {Ice} {Giants} with {Growing} {Frozen} {Cores}: {The} {Case} of {Neptune}},
	volume = {220},
	issn = {0038-6308, 1572-9672},
	shorttitle = {Thermal and {Tidal} {Evolution} of {Ice} {Giants} with {Growing} {Frozen} {Cores}},
	url = {https://link.springer.com/10.1007/s11214-024-01053-6},
	doi = {10.1007/s11214-024-01053-6},
	abstract = {The contrasting internal luminosity of Uranus and Neptune present a challenge to our understanding of the origin and evolution of these bodies, as well as extra-solar ice giants. The thermal evolution of Neptune is known to be nearly consistent with an entirely ﬂuid interior, but this is not a unique solution, and does not account for the tidal dissipation required by the migration of its moons. We examine a model that has been previously shown to explain the thermal and tidal evolution of Uranus: one that features a growing, frozen core. The core traps heat in the interior, affecting the cooling time scale, and provides a source of tidal dissipation. We review the growing, frozen core model, and the computation of thermal and tidal evolution. We then apply this model to Neptune. We ﬁnd that the growing frozen core model can account for the observed internal luminosity of Neptune and the migration of its moons, in the form of resonances that were either encountered or avoided in the past. We discuss prospects for observational tests of the growing frozen core model and possible implications for understanding the gas giants.},
	language = {en},
	number = {2},
	urldate = {2024-07-20},
	journal = {Space Science Reviews},
	author = {James, David A. and Stixrude, Lars},
	month = mar,
	year = {2024},
	pages = {21},
	file = {James and Stixrude - 2024 - Thermal and Tidal Evolution of Ice Giants with Gro.pdf:/Users/jdong/Zotero/storage/TPYQ9M3H/James and Stixrude - 2024 - Thermal and Tidal Evolution of Ice Giants with Gro.pdf:application/pdf},
}
@article{vazan_explaining_2020,
	title = {Explaining the low luminosity of {Uranus}: a self-consistent thermal and structural evolution},
	volume = {633},
	copyright = {https://www.edpsciences.org/en/authors/copyright-and-licensing},
	issn = {0004-6361, 1432-0746},
	shorttitle = {Explaining the low luminosity of {Uranus}},
	url = {https://www.aanda.org/10.1051/0004-6361/201936588},
	doi = {10.1051/0004-6361/201936588},
	abstract = {The low luminosity of Uranus is a long-standing challenge in planetary science. Simple adiabatic models are inconsistent with the measured luminosity, which indicates that Uranus is non-adiabatic because it has thermal boundary layers and/or conductive regions. A gradual composition distribution acts as a thermal boundary to suppress convection and slow down the internal cooling. Here we investigate whether composition gradients in the deep interior of Uranus can explain its low luminosity, the required composition gradient, and whether it is stable for convective mixing on a timescale of some billion years. We varied the primordial composition distribution and the initial energy budget of the planet, and chose the models that fit the currently measured properties (radius, luminosity, and moment of inertia) of Uranus. We present several alternative non-adiabatic internal structures that fit the Uranus measurements. We found that convective mixing is limited to the interior of Uranus, and a composition gradient is stable and sufficient to explain its current luminosity. As a result, the interior of Uranus might still be very hot, in spite of its low luminosity. The stable composition gradient also indicates that the current internal structure of Uranus is similar to its primordial structure. Moreover, we suggest that the initial energy content of Uranus cannot be greater than 20\% of its formation (accretion) energy. We also find that an interior with a mixture of ice and rock, rather than separated ice and rock shells, is consistent with measurements, suggesting that Uranus might not be “differentiated”. Our models can explain the luminosity of Uranus, and they are also consistent with its metal-rich atmosphere and with the predictions for the location where its magnetic field is generated.},
	urldate = {2024-07-20},
	journal = {Astronomy \& Astrophysics},
	author = {Vazan, Allona and Helled, Ravit},
	month = jan,
	year = {2020},
	pages = {A50},
	file = {Full Text:/Users/jdong/Zotero/storage/M2H4BNH2/Vazan and Helled - 2020 - Explaining the low luminosity of Uranus a self-co.pdf:application/pdf},
}
@article{podolak_effect_2019,
	title = {Effect of non-adiabatic thermal profiles on the inferred compositions of {Uranus} and {Neptune}},
	volume = {487},
	copyright = {https://academic.oup.com/journals/pages/open\_access/funder\_policies/chorus/standard\_publication\_model},
	issn = {0035-8711, 1365-2966},
	url = {https://academic.oup.com/mnras/article/487/2/2653/5505844},
	doi = {10.1093/mnras/stz1467},
	language = {en},
	number = {2},
	urldate = {2024-07-20},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Podolak, Morris and Helled, Ravit and Schubert, Gerald},
	month = aug,
	year = {2019},
	pages = {2653--2664},
	file = {Full Text:/Users/jdong/Zotero/storage/LZJPXQJ6/Podolak et al. - 2019 - Effect of non-adiabatic thermal profiles on the in.pdf:application/pdf},
}
@article{huo_methane_2003,
	title = {Methane hydrate nonstoichiometry and phase diagram},
	volume = {49},
	copyright = {http://onlinelibrary.wiley.com/termsAndConditions\#vor},
	issn = {0001-1541, 1547-5905},
	url = {https://aiche.onlinelibrary.wiley.com/doi/10.1002/aic.690490521},
	doi = {10.1002/aic.690490521},
	abstract = {Abstract
            
              A previous study discovered that, when formed from different ethylene oxide (EO) feed solutions, hydrates had different small‐cage occupancies with essentially total occupation of the large cavities of sI hydrate. An EO + H
              2
              O isobaric phase diagram was proposed with a solid solution range to explain this phenomenon. Since methane and CO
              2
              also occupy both small cages and large cages of sI hydrate, new phase diagrams were proposed which allowed the methane or CO
              2
              hydrate composition to vary as a function of feed composition at fixed p‐T conditions. Raman spectroscopy experiments now show that H
              2
              O + CH
              4
              hydrates formed at the vapor–liquid interface have a different composition than dendrites growing into the water below the interface. Interfacial hydrates were typical laboratory samples formed with excess gas, while dendrites coexisted with excess water and were similar to seafloor hydrate. Integrated peak intensities were used to calculate relative cage occupancies in Raman data analysis. Interfacial hydrates had an average of 95.4\% small cages occupied at 30 MPa and 275.15 K, while dendrite hydrates had only 82.8\% small‐cage occupancy at the same conditions. This result suggests that hydrates in the ocean floor may have lower methane concentrations than hydrates formed under normal laboratory conditions at the same pressure and temperature.},
	language = {en},
	number = {5},
	urldate = {2024-07-20},
	journal = {AIChE Journal},
	author = {Huo, Zhongxin and Hester, Keith and Sloan, E. Dendy and Miller, Kelly T.},
	month = may,
	year = {2003},
	pages = {1300--1306},
}
@misc{neuenschwander_uranus_2024,
	title = {Uranus' {Complex} {Internal} {Structure}},
	copyright = {arXiv.org perpetual, non-exclusive license},
	url = {https://arxiv.org/abs/2401.11769},
	doi = {10.48550/ARXIV.2401.11769},
	abstract = {Uranus' bulk composition remains unknown. Although there are clear indications that Uranus' interior is not fully convective, and therefore has a non-adiabatic temperature profile, many interior models continue to assume an adiabatic interior. In this paper we present a new method to interpret empirical structure models in terms of composition and for identifying non-convective regions. We also explore how the uncertainty in Uranus' rotation period and winds affect the inferred composition and temperature profile. We use Uranus' density profiles from previous work where the density is represented by up to three polytropes. Using our new method, we find that these empirical models imply that Uranus' interior includes non-adiabatic regions. This leads to significantly hotter internal temperatures that can reach a few 10\${\textasciicircum}3\$ K and higher bulk heavy-element abundances (up to 1 M\$\_{\textbackslash}oplus\$) compared to standard adiabatic models. We find that the assumed rotation period strongly affects the inferred composition while the winds have a negligible effect. Although solutions with only H-He and rock are possible, we find that the maximum water-to-rock ratio in Uranus for our models ranges between 2.6 and 21. This is significantly lower compared to standard adiabatic models. We conclude that it is important to include non-adiabatic regions in Uranus structure models as they significantly affect the inferred temperature profile, and therefore the inferred bulk heavy-element abundance. In addition, we suggest that it is of great value to measure Uranus' gravitational field and determine its rotation period in order to decrease the uncertainty in Uranus' bulk composition.},
	urldate = {2024-07-20},
	publisher = {arXiv},
	author = {Neuenschwander, Benno A. and Müller, Simon and Helled, Ravit},
	year = {2024},
	note = {Version Number: 1},
	keywords = {Earth and Planetary Astrophysics (astro-ph.EP), FOS: Physical sciences},
	annote = {Other
15 pages, 15 figures, 2 tables, accepted for publication in A\&A;},
}

@article{cheng_phase_2021,
	title = {Phase behaviours of superionic water at planetary conditions},
	volume = {17},
	issn = {1745-2473, 1745-2481},
	url = {https://www.nature.com/articles/s41567-021-01334-9},
	doi = {10.1038/s41567-021-01334-9},
	language = {en},
	number = {11},
	urldate = {2024-07-20},
	journal = {Nature Physics},
	author = {Cheng, Bingqing and Bethkenhagen, Mandy and Pickard, Chris J. and Hamel, Sebastien},
	month = nov,
	year = {2021},
	pages = {1228--1232},
	file = {Cheng et al. - 2021 - Phase behaviours of superionic water at planetary .pdf:/Users/jdong/Zotero/storage/6KXX86GY/Cheng et al. - 2021 - Phase behaviours of superionic water at planetary .pdf:application/pdf},
}

@article{prakapenka_structure_2021,
	title = {Structure and properties of two superionic ice phases},
	volume = {17},
	issn = {1745-2473, 1745-2481},
	url = {https://www.nature.com/articles/s41567-021-01351-8},
	doi = {10.1038/s41567-021-01351-8},
	language = {en},
	number = {11},
	urldate = {2024-07-20},
	journal = {Nature Physics},
	author = {Prakapenka, Vitali B. and Holtgrewe, Nicholas and Lobanov, Sergey S. and Goncharov, Alexander F.},
	month = nov,
	year = {2021},
	pages = {1233--1238},
	file = {Prakapenka et al. - 2021 - Structure and properties of two superionic ice pha.pdf:/Users/jdong/Zotero/storage/A67SCYD6/Prakapenka et al. - 2021 - Structure and properties of two superionic ice pha.pdf:application/pdf},
}

@article{millot_nanosecond_2019,
	title = {Nanosecond {X}-ray diffraction of shock-compressed superionic water ice},
	volume = {569},
	issn = {0028-0836, 1476-4687},
	url = {https://www.nature.com/articles/s41586-019-1114-6},
	doi = {10.1038/s41586-019-1114-6},
	language = {en},
	number = {7755},
	urldate = {2024-07-20},
	journal = {Nature},
	author = {Millot, Marius and Coppari, Federica and Rygg, J. Ryan and Correa Barrios, Antonio and Hamel, Sebastien and Swift, Damian C. and Eggert, Jon H.},
	month = may,
	year = {2019},
	pages = {251--255},
	file = {Millot et al. - 2019 - Nanosecond X-ray diffraction of shock-compressed s.pdf:/Users/jdong/Zotero/storage/8KBN2K69/Millot et al. - 2019 - Nanosecond X-ray diffraction of shock-compressed s.pdf:application/pdf},
}

@article{huang_stability_2020,
	title = {Stability of {H} $_{\textrm{3}}$ {O} at extreme conditions and implications for the magnetic fields of {Uranus} and {Neptune}},
	volume = {117},
	issn = {0027-8424, 1091-6490},
	url = {https://pnas.org/doi/full/10.1073/pnas.1921811117},
	doi = {10.1073/pnas.1921811117},
	abstract = {Significance
            
              Understanding the interior structure and dynamics of outer Solar System planets in terms of their component materials is a major scientific challenge. A highly intriguing case concerns the anomalous nondipolar and nonaxisymmetric magnetic fields of Uranus and Neptune. A thin-shell dynamo model has been shown to capture observed phenomena but leaves unexplained its origin and materials basis. We report extensive theoretical calculations that indicate the stability of trihydrogen oxide (H
              3
              O) in solid, superionic, and fluid metallic states at the deep interior conditions of these planets. The fluid metallic phase is stable in a thin-shell zone near their cores and exhibits the properties required to produce the observed enigmatic magnetic fields. These findings have implications for other planets, including related exoplanets.
            
          , 
            
              The anomalous nondipolar and nonaxisymmetric magnetic fields of Uranus and Neptune have long challenged conventional views of planetary dynamos. A thin-shell dynamo conjecture captures the observed phenomena but leaves unexplained the fundamental material basis and underlying mechanism. Here we report extensive quantum-mechanical calculations of polymorphism in the hydrogen–oxygen system at the pressures and temperatures of the deep interiors of these ice giant planets (to {\textgreater}600 GPa and 7,000 K). The results reveal the surprising stability of solid and fluid trihydrogen oxide (H
              3
              O) at these extreme conditions. Fluid H
              3
              O is metallic and calculated to be stable near the cores of Uranus and Neptune. As a convecting fluid, the material could give rise to the magnetic field consistent with the thin-shell dynamo model proposed for these planets. H
              3
              O could also be a major component in both solid and superionic forms in other (e.g., nonconvecting) layers. The results thus provide a materials basis for understanding the enigmatic magnetic-field anomalies and other aspects of the interiors of Uranus and Neptune. These findings have direct implications for the internal structure, composition, and dynamos of related exoplanets.},
	language = {en},
	number = {11},
	urldate = {2024-07-20},
	journal = {Proceedings of the National Academy of Sciences},
	author = {Huang, Peihao and Liu, Hanyu and Lv, Jian and Li, Quan and Long, Chunhong and Wang, Yanchao and Chen, Changfeng and Hemley, Russell J. and Ma, Yanming},
	month = mar,
	year = {2020},
	pages = {5638--5643},
	file = {Huang et al. - 2020 - Stability of H 3 O at extreme condition.pdf:/Users/jdong/Zotero/storage/NCBJD5Z8/Huang et al. - 2020 - Stability of H 3 O at extreme condition.pdf:application/pdf},
}

@article{weck_evidence_2022,
	title = {Evidence and {Stability} {Field} of fcc {Superionic} {Water} {Ice} {Using} {Static} {Compression}},
	volume = {128},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.128.165701},
	doi = {10.1103/PhysRevLett.128.165701},
	language = {en},
	number = {16},
	urldate = {2024-07-20},
	journal = {Physical Review Letters},
	author = {Weck, Gunnar and Queyroux, Jean-Antoine and Ninet, Sandra and Datchi, Frédéric and Mezouar, Mohamed and Loubeyre, Paul},
	month = apr,
	year = {2022},
	pages = {165701},
	file = {Weck et al. - 2022 - Evidence and Stability Field of fcc Superionic Wat.pdf:/Users/jdong/Zotero/storage/ARDTUGAU/Weck et al. - 2022 - Evidence and Stability Field of fcc Superionic Wat.pdf:application/pdf},
}

@incollection{bindi_mineralogy_2023,
	address = {Cham},
	title = {Mineralogy of {Planetary} {Cores}},
	isbn = {978-3-031-28804-3 978-3-031-28805-0},
	url = {https://link.springer.com/10.1007/978-3-031-28805-0_9},
	language = {en},
	urldate = {2024-07-20},
	booktitle = {Celebrating the {International} {Year} of {Mineralogy}},
	publisher = {Springer Nature Switzerland},
	author = {Zurkowski, C. C. and Fei, Y.},
	editor = {Bindi, Luca and Cruciani, Giuseppe},
	year = {2023},
	doi = {10.1007/978-3-031-28805-0_9},
	note = {Series Title: Springer Mineralogy},
	pages = {207--247},
}
@article{helled_understanding_2020,
	title = {Understanding dense hydrogen at planetary conditions},
	volume = {2},
	issn = {2522-5820},
	url = {https://www.nature.com/articles/s42254-020-0223-3},
	doi = {10.1038/s42254-020-0223-3},
	language = {en},
	number = {10},
	urldate = {2024-07-20},
	journal = {Nature Reviews Physics},
	author = {Helled, Ravit and Mazzola, Guglielmo and Redmer, Ronald},
	month = sep,
	year = {2020},
	pages = {562--574},
	file = {Submitted Version:/Users/jdong/Zotero/storage/TLNM6PLU/Helled et al. - 2020 - Understanding dense hydrogen at planetary conditio.pdf:application/pdf},
}

@article{stixrude_structure_2012,
	title = {Structure of {Iron} to 1 {Gbar} and 40 000 {K}},
	volume = {108},
	copyright = {http://link.aps.org/licenses/aps-default-license},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.108.055505},
	doi = {10.1103/PhysRevLett.108.055505},
	language = {en},
	number = {5},
	urldate = {2024-07-20},
	journal = {Physical Review Letters},
	author = {Stixrude, Lars},
	month = feb,
	year = {2012},
	pages = {055505},
}

@inproceedings{francis_dragulet_electrical_2023,
	address = {San Francisco},
	title = {Electrical and {Thermal} {Conductivity} of {Iron}-enriched {Basal} {Magma} {Oceans} in {Early} {Earth} and {Super}-{Earths}},
	booktitle = {American {Geophysical} {Union} 2023 {Annual} {Meeting} {Abstracts}},
	author = {Dragulet, Francis and Stxirude, Lars P},
	year = {2023},
}

@article{mazevet_fate_2019,
	title = {The fate of planetary cores in giant and ice-giant planets},
	volume = {631},
	copyright = {http://creativecommons.org/licenses/by/4.0},
	issn = {0004-6361, 1432-0746},
	url = {https://www.aanda.org/10.1051/0004-6361/201936288},
	doi = {10.1051/0004-6361/201936288},
	abstract = {Context.
              The Juno probe that currently orbits Jupiter measures its gravitational moments with great accuracy. Preliminary results suggest that the core of the planet may be eroded. While great attention has been paid to the material properties of elements constituting the envelope, little is known about those that constitute the core. This situation clutters our interpretation the Juno data and modeling of giant planets and exoplanets in general.
            
            
              Aims.
              We calculate the high-pressure melting temperatures of three potential components of the cores of giant planets, water, iron, and a simple silicate, MgSiO3, to investigate the state of the deep inner core.
            
            
              Methods.
              We used ab initio molecular dynamics simulations to calculate the high-pressure melting temperatures of the three potential core components. The planetary adiabats were obtained by solving the hydrostatic equations in a three-layer model adjusted to reproduce the measured gravitational moments. Recently developed ab initio equations of state were used for the envelope and the core.
            
            
              Results.
              We find that the cores of the giant and ice-giant planets of the solar system differ because the pressure–temperature conditions encountered in each object correspond to different regions of the phase diagrams. For Jupiter and Saturn, the results are compatible with a diffuse core and mixing of a significant fraction of metallic elements in the envelope, leading to a convective and/or a double-diffusion regime. We also find that their solid cores vary in nature and size throughout the lifetimes of these planets. The solid cores of the two giant planets are not primordial and nucleate and grow as the planets cool. We estimate that the solid core of Jupiter is 3 Gyr old and that of Saturn is 1.5 Gyr old. The situation is less extreme for Uranus and Neptune, whose cores are only partially melted.
            
            
              Conclusions.
              To model Jupiter, the time evolution of the interior structure of the giant planets and exoplanets in general, their luminosity, and the evolution of the tidal effects over their lifetimes, the core should be considered as crystallizing and growing rather than gradually mixing into the envelope due to the solubility of its components.},
	urldate = {2024-07-21},
	journal = {Astronomy \& Astrophysics},
	author = {Mazevet, S. and Musella, R. and Guyot, F.},
	month = nov,
	year = {2019},
	pages = {L4},
	file = {Full Text:/Users/jdong/Zotero/storage/KGL3Q52A/Mazevet et al. - 2019 - The fate of planetary cores in giant and ice-giant.pdf:application/pdf},
}

@article{stixrude_thermodynamics_2024,
	title = {Thermodynamics of mantle minerals – {III}: the role of iron},
	volume = {237},
	copyright = {https://creativecommons.org/licenses/by/4.0/},
	issn = {0956-540X, 1365-246X},
	shorttitle = {Thermodynamics of mantle minerals – {III}},
	url = {https://academic.oup.com/gji/article/237/3/1699/7640845},
	doi = {10.1093/gji/ggae126},
	abstract = {SUMMARY
            We expand the scope of HeFESTo by encompassing the rich physics of iron in the mantle, including the existence of multiple valence and spin states. In our previous papers, we considered iron only in its most common state in the mantle: the high-spin divalent (ferrous) cation. We now add ferric iron end-members to six phases, as well as the three phases of native iron. We also add low-spin states of ferrous and ferric iron and capture the behaviour of the high-spin to low-spin transition. Consideration of the multi-state nature of iron, unique among the major elements, leads to developments of our theory, including generalization of the chemical potential to account for the possibility of multiple distinguishable states of iron co-existing on a single crystallographic site, the effect of the high-spin to low-spin transition on seismic wave velocities in multiphase systems, and computation of oxygen fugacity. Consideration of ferric iron also motivates the addition of the chromia component to several phases, so that we now consider the set of components: Ca, Na, Fe, Mg, Al, Si, O and Cr (CNFMASO+Cr). We present the results of a new global inversion of mineral properties and compare our results to experimental observations over the entire pressure–temperature range of the mantle and over a wide range of oxygen fugacity. Applications of our method illustrate how it might be used to better understand the seismic structure, dynamics and oxygen fugacity of the mantle.},
	language = {en},
	number = {3},
	urldate = {2024-05-25},
	journal = {Geophysical Journal International},
	author = {Stixrude, Lars and Lithgow-Bertelloni, Carolina},
	month = apr,
	year = {2024},
	pages = {1699--1733},
	file = {Full Text:/Users/jdong/Zotero/storage/EC9TU5X9/Stixrude and Lithgow-Bertelloni - 2024 - Thermodynamics of mantle minerals – III the role .pdf:application/pdf;Screenshot 2024-08-28 at 5.34.47 PM.png:/Users/jdong/Zotero/storage/VRBCFZKP/Screenshot 2024-08-28 at 5.34.47 PM.png:image/png},
}


@article{stixrude_thermodynamics_2011,
	title = {Thermodynamics of mantle minerals - {II}. {Phase} equilibria},
	volume = {184},
	issn = {1365-246X, 0956-540X},
	url = {https://academic.oup.com/gji/article/184/3/1180/625783},
	doi = {10.1111/j.1365-246X.2010.04890.x},
	language = {en},
	number = {3},
	urldate = {2024-01-19},
	journal = {Geophysical Journal International},
	author = {Stixrude, Lars and Lithgow-Bertelloni, Carolina},
	year = {2011},
	pages = {1180--1213},
	file = {Full Text:/Users/dong2j/Zotero/storage/Y5JGKZRJ/Stixrude and Lithgow-Bertelloni - 2011 - Thermodynamics of mantle minerals - II. Phase equi.pdf:application/pdf},
}

@article{stixrude_thermal_2021,
	title = {Thermal expansivity, heat capacity and bulk modulus of the mantle},
	volume = {228},
	issn = {0956-540X, 1365-246X},
	url = {https://academic.oup.com/gji/article/228/2/1119/6375416},
	doi = {10.1093/gji/ggab394},
	abstract = {SUMMARY
            We derive exact expressions for the thermal expansivity, heat capacity and bulk modulus for assemblages with arbitrarily large numbers of components and phases, including the influence of phase transformations and chemical exchange. We illustrate results in simple two-component, two-phase systems, including Mg–Fe olivine-wadsleyite and Ca–Mg clinopyroxene-orthopyroxene and for a multicompontent model of mantle composition in the form of pyrolite. For the latter we show results for the thermal expansivity and heat capacity over the entire mantle pressure–temperature regime to 40 GPa, or a depth of 1000 km. From the thermal expansivity, we derive a new expression for the phase buoyancy parameter that is valid for arbitrarily large numbers of phases and components and which is defined at every point in pressure–temperature space. Results reveal regions of the mantle where the magnitude of the phase buoyancy parameter is larger in magnitude than for those phase transitions that are most commonly included in mantle convection simulations. These regions include the wadsleyite to garnet and ferropericlase transition, which is encountered along hot isentropes (e.g. 2000 K potential temperature) in the transition zone, and the ferropericlase and stishovite to bridgmanite transition, which is encountered along cold isentropes (e.g. 1000 K potential temperature) in the shallow lower mantle. We also show the bulk modulus along a typical mantle isentrope and relate it to the Bullen inhomogeneity parameter. All results are computed with our code HeFESTo, updates and improvements to which we discuss, including the implementation of the exact expressions for the thermal expansivity, heat capacity and bulk modulus, generalization to allow for pressure dependence of non-ideal solution parameters and an improved numerical scheme for minimizing the Gibbs free energy. Finally, we present the results of a new global inversion of parameters updated to incorporate more recent results from experiment and first principles theory, as well as a new phase (nal phase), and new species: Na-majorite and the NaAlO2 end-member of ferropericlase.},
	language = {en},
	number = {2},
	urldate = {2024-01-19},
	journal = {Geophysical Journal International},
	author = {Stixrude, Lars and Lithgow-Bertelloni, Carolina},
	year = {2021},
	pages = {1119--1149},
	file = {Full Text:/Users/dong2j/Zotero/storage/MJFNHMRT/Stixrude and Lithgow-Bertelloni - 2021 - Thermal expansivity, heat capacity and bulk modulu.pdf:application/pdf},
}

@article{stixrude_thermodynamics_2005,
	title = {Thermodynamics of mantle minerals - {I}. {Physical} properties},
	volume = {162},
	issn = {0956540X, 1365246X},
	url = {https://academic.oup.com/gji/article-lookup/doi/10.1111/j.1365-246X.2005.02642.x},
	doi = {10.1111/j.1365-246X.2005.02642.x},
	language = {en},
	number = {2},
	urldate = {2024-01-19},
	journal = {Geophysical Journal International},
	author = {Stixrude, Lars and Lithgow-Bertelloni, Carolina},
	year = {2005},
	pages = {610--632},
	file = {Full Text:/Users/dong2j/Zotero/storage/LP9NQ6QG/Stixrude and Lithgow-Bertelloni - 2005 - Thermodynamics of mantle minerals - I. Physical pr.pdf:application/pdf},
}

@book{schubert_mantle_2001,
	edition = {1},
	title = {Mantle {Convection} in the {Earth} and {Planets}},
	isbn = {978-0-521-35367-0 978-0-521-79836-5 978-0-511-61287-9},
	url = {https://www.cambridge.org/core/product/identifier/9780511612879/type/book},
	abstract = {Mantle Convection in the Earth and Planets is a comprehensive synthesis of all aspects of mantle convection within the Earth, the terrestrial planets, the Moon, and the Galilean satellites of Jupiter. The book includes up-to-date discussions of the latest research developments that have revolutionized our understanding of the Earth and the planets. It is suitable as a text for graduate courses in geophysics and planetary physics, and as a supplementary reference for use at the undergraduate level. It is also an invaluable review for researchers in the broad fields of the Earth and planetary sciences including seismologists, tectonophysicists, geodesists, mineral physicists, volcanologists, geochemists, geologists, mineralogists, petrologists, paleomagnetists, planetary geologists, and meteoriticists. The book features a comprehensive index, an extensive reference list, numerous illustrations (many in color) and major questions that focus the discussion and suggest avenues of future research.},
	urldate = {2024-01-19},
	publisher = {Cambridge University Press},
	author = {Schubert, Gerald and Turcotte, Donald L. and Olson, Peter},
	year = {2001},
	doi = {10.1017/CBO9780511612879},
}

@article{dziewonski_preliminary_1981,
	title = {Preliminary reference {Earth} model},
	volume = {25},
	issn = {00319201},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0031920181900467},
	doi = {10.1016/0031-9201(81)90046-7},
	language = {en},
	number = {4},
	urldate = {2024-01-19},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Dziewonski, Adam M. and Anderson, Don L.},
	year = {1981},
	pages = {297--356},
}

@article{khan_upper_2021,
	title = {Upper mantle structure of {Mars} from {InSight} seismic data},
	volume = {373},
	issn = {0036-8075, 1095-9203},
	url = {https://www.science.org/doi/10.1126/science.abf2966},
	doi = {10.1126/science.abf2966},
	abstract = {Single seismometer structure
            
              Because of the lack of direct seismic observations, the interior structure of Mars has been a mystery. Khan
              et al.
              , Knapmeyer-Endrun
              et al.
              , and Stähler
              et al.
              used recently detected marsquakes from the seismometer deployed during the InSight mission to map the interior of Mars (see the Perspective by Cottaar and Koelemeijer). Mars likely has a 24- to 72-kilometer-thick crust with a very deep lithosphere close to 500 kilometers. Similar to the Earth, a low-velocity layer probably exists beneath the lithosphere. The crust of Mars is likely highly enriched in radioactive elements that help to heat this layer at the expense of the interior. The core of Mars is liquid and large, ∼1830 kilometers, which means that the mantle has only one rocky layer rather than two like the Earth has. These results provide a preliminary structure of Mars that helps to constrain the different theories explaining the chemistry and internal dynamics of the planet.
            
            
              Science
              , abf2966, abf8966, abi7730, this issue p.
              434
              , p.
              438
              , p.
              443
              see also abj8914, p.
              388
            
          , 
            Data from the InSight mission on Mars help constrain the structure and properties of the martian interior.
          , 
            
              For 2 years, the InSight lander has been recording seismic data on Mars that are vital to constrain the structure and thermochemical state of the planet. We used observations of direct (
              P
              and
              S
              ) and surface-reflected (
              PP
              ,
              PPP
              ,
              SS
              , and
              SSS
              ) body-wave phases from eight low-frequency marsquakes to constrain the interior structure to a depth of 800 kilometers. We found a structure compatible with a low-velocity zone associated with a thermal lithosphere much thicker than on Earth that is possibly related to a weak
              S
              -wave shadow zone at teleseismic distances. By combining the seismic constraints with geodynamic models, we predict that, relative to the primitive mantle, the crust is more enriched in heat-producing elements by a factor of 13 to 20. This enrichment is greater than suggested by gamma-ray surface mapping and has a moderate-to-elevated surface heat flow.},
	language = {en},
	number = {6553},
	urldate = {2024-01-19},
	journal = {Science},
	author = {Khan, Amir and Ceylan, Savas and Van Driel, Martin and Giardini, Domenico and Lognonné, Philippe and Samuel, Henri and Schmerr, Nicholas C. and Stähler, Simon C. and Duran, Andrea C. and Huang, Quancheng and Kim, Doyeon and Broquet, Adrien and Charalambous, Constantinos and Clinton, John F. and Davis, Paul M. and Drilleau, Mélanie and Karakostas, Foivos and Lekic, Vedran and McLennan, Scott M. and Maguire, Ross R. and Michaut, Chloé and Panning, Mark P. and Pike, William T. and Pinot, Baptiste and Plasman, Matthieu and Scholz, John-Robert and Widmer-Schnidrig, Rudolf and Spohn, Tilman and Smrekar, Suzanne E. and Banerdt, William B.},
	year = {2021},
	pages = {434--438},
	file = {Submitted Version:/Users/dong2j/Zotero/storage/C22CE79C/Khan et al. - 2021 - Upper mantle structure of Mars from InSight seismi.pdf:application/pdf},
}

@article{huang_seismic_2022,
	title = {Seismic detection of a deep mantle discontinuity within {Mars} by {InSight}},
	volume = {119},
	issn = {0027-8424, 1091-6490},
	url = {https://pnas.org/doi/10.1073/pnas.2204474119},
	doi = {10.1073/pnas.2204474119},
	abstract = {Constraining the thermal and compositional state of the mantle is crucial for deciphering the formation and evolution of Mars. Mineral physics predicts that Mars’ deep mantle is demarcated by a seismic discontinuity arising from the pressure-induced phase transformation of the mineral olivine to its higher-pressure polymorphs, making the depth of this boundary sensitive to both mantle temperature and composition. Here, we report on the seismic detection of a midmantle discontinuity using the data collected by NASA’s InSight Mission to Mars that matches the expected depth and sharpness of the postolivine transition. In five teleseismic events, we observed triplicated P and S waves and constrained the depth of this discontinuity to be 1,006
              
                
                  ±
                
              
              40 km by modeling the triplicated waveforms. From this depth range, we infer a mantle potential temperature of 1,605
              
                
                  ±
                
              
              100 K, a result consistent with a crust that is 10 to 15 times more enriched in heat-producing elements than the underlying mantle. Our waveform fits to the data indicate a broad gradient across the boundary, implying that the Martian mantle is more enriched in iron compared to Earth. Through modeling of thermochemical evolution of Mars, we observe that only two out of the five proposed composition models are compatible with the observed boundary depth. Our geodynamic simulations suggest that the Martian mantle was relatively cold 4.5 Gyr ago (1,720 to 1,860 K) and are consistent with a present-day surface heat flow of 21 to 24 mW/m
              2
              .},
	language = {en},
	number = {42},
	urldate = {2024-01-19},
	journal = {Proceedings of the National Academy of Sciences},
	author = {Huang, Quancheng and Schmerr, Nicholas C. and King, Scott D. and Kim, Doyeon and Rivoldini, Attilio and Plesa, Ana-Catalina and Samuel, Henri and Maguire, Ross R. and Karakostas, Foivos and Lekić, Vedran and Charalambous, Constantinos and Collinet, Max and Myhill, Robert and Antonangeli, Daniele and Drilleau, Mélanie and Bystricky, Misha and Bollinger, Caroline and Michaut, Chloé and Gudkova, Tamara and Irving, Jessica C. E. and Horleston, Anna and Fernando, Benjamin and Leng, Kuangdai and Nissen-Meyer, Tarje and Bejina, Frederic and Bozdağ, Ebru and Beghein, Caroline and Waszek, Lauren and Siersch, Nicki C. and Scholz, John-Robert and Davis, Paul M. and Lognonné, Philippe and Pinot, Baptiste and Widmer-Schnidrig, Rudolf and Panning, Mark P. and Smrekar, Suzanne E. and Spohn, Tilman and Pike, William T. and Giardini, Domenico and Banerdt, W. Bruce},
	year = {2022},
	pages = {e2204474119},
	file = {Full Text:/Users/dong2j/Zotero/storage/T7ZKE4S4/Huang et al. - 2022 - Seismic detection of a deep mantle discontinuity w.pdf:application/pdf},
}

@article{dannberg_entropy_2022,
	title = {An entropy method for geodynamic modelling of phase transitions: capturing sharp and broad transitions in a multiphase assemblage},
	volume = {231},
	issn = {0956-540X, 1365-246X},
	shorttitle = {An entropy method for geodynamic modelling of phase transitions},
	url = {https://academic.oup.com/gji/article/231/3/1833/6652101},
	doi = {10.1093/gji/ggac293},
	abstract = {SUMMARY
            Phase transitions play an important role for the style of mantle convection. While observations and theory agree that a substantial fraction of subducted slabs and rising plumes can move through the whole mantle at present day conditions, this behaviour may have been different throughout Earth’s history. Higher temperatures, such as in the early Earth, cause different phase transitions to be dominant, and also reduce mantle viscosity, favouring a more layered style of convection induced by phase transitions. A period of layered mantle convection in Earth’s past would have significant implications for the secular evolution of the mantle temperature and the mixing of mantle heterogeneities. The transition from layered to whole mantle convection could lead to a period of mantle avalanches associated with a dramatic increase in magmatic activity. Consequently, it is important to accurately model the influence of phase transitions on mantle convection. However, existing numerical methods generally preclude modelling phase transitions that are only present in a particular range of pressures, temperatures or compositions, and they impose an artificial lower limit on the thickness of phase transitions. To overcome these limitations, we have developed a new numerical method that solves the energy equation for entropy instead of temperature. This technique allows for robust coupling between thermodynamic and geodynamic models and makes it possible to model realistically sharp phase transitions with a wide range of properties and dynamic effects on mantle processes. We demonstrate the utility of our method by applying it in regional and global convection models, investigating the effect of individual phase transitions in the Earth’s mantle with regard to their potential for layering flow. We find that the thickness of the phase transition has a bigger influence on the style of convection than previously thought: with all other parameters being the same, a thin phase transition can induce fully layered convection where a broad phase transition would lead to whole-mantle convection. Our application of the method to convection in the early Earth illustrates that endothermic phase transitions may have induced layering for higher mantle temperatures in the Earth’s past.},
	language = {en},
	number = {3},
	urldate = {2024-01-20},
	journal = {Geophysical Journal International},
	author = {Dannberg, Juliane and Gassmöller, Rene and Li, Ranpeng and Lithgow-Bertelloni, Carolina and Stixrude, Lars},
	year = {2022},
	pages = {1833--1849},
}

@article{stixrude_melting_2014,
	title = {Melting in super-earths},
	volume = {372},
	issn = {1364-503X, 1471-2962},
	url = {https://royalsocietypublishing.org/doi/10.1098/rsta.2013.0076},
	doi = {10.1098/rsta.2013.0076},
	abstract = {We examine the possible extent of melting in rock-iron super-earths, focusing on those in the habitable zone. We consider the energetics of accretion and core formation, the timescale of cooling and its dependence on viscosity and partial melting, thermal regulation via the temperature dependence of viscosity, and the melting curves of rock and iron components at the ultra-high pressures characteristic of super-earths. We find that the efficiency of kinetic energy deposition during accretion increases with planetary mass; considering the likely role of giant impacts and core formation, we find that super-earths probably complete their accretionary phase in an entirely molten state. Considerations of thermal regulation lead us to propose model temperature profiles of super-earths that are controlled by silicate melting. We estimate melting curves of iron and rock components up to the extreme pressures characteristic of super-earth interiors based on existing experimental and
              ab initio
              results and scaling laws. We construct super-earth thermal models by solving the equations of mass conservation and hydrostatic equilibrium, together with equations of state of rock and iron components. We set the potential temperature at the core–mantle boundary and at the surface to the local silicate melting temperature. We find that ancient (∼4 Gyr) super-earths may be partially molten at the top and bottom of their mantles, and that mantle convection is sufficiently vigorous to sustain dynamo action over the whole range of super-earth masses.},
	language = {en},
	number = {2014},
	urldate = {2024-01-20},
	journal = {Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
	author = {Stixrude, Lars},
	year = {2014},
	pages = {20130076},
}

@article{labrosse_cooling_1997,
	title = {On cooling of the {Earth}'s core},
	volume = {99},
	issn = {00319201},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0031920196032074},
	doi = {10.1016/S0031-9201(96)03207-4},
	language = {en},
	number = {1-2},
	urldate = {2024-01-20},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Labrosse, Stéphane and Poirier, Jean-Paul and Le Mouël, Jean-Louis},
	year = {1997},
	pages = {1--17},
}

@article{stixrude_thermal_2021-1,
	title = {Thermal and {Tidal} {Evolution} of {Uranus} with a {Growing} {Frozen} {Core}},
	volume = {2},
	issn = {2632-3338},
	url = {https://iopscience.iop.org/article/10.3847/PSJ/ac2a47},
	doi = {10.3847/PSJ/ac2a47},
	abstract = {Abstract
            
              The origin of the very low luminosity of Uranus is unknown, as is the source of the internal tidal dissipation required by the orbits of the Uranian moons. Models of the interior of Uranus often assume that it is inviscid throughout, but recent experiments show that this assumption may not be justified; most of the interior of Uranus lies below the freezing temperature of H
              2
              O. We find that the stable solid phase of H
              2
              O, which is superionic, has a large viscosity controlled by the crystalline oxygen sublattice. We examine the consequences of finite viscosity by combining ab initio determinations of the thermal conductivity and other material properties of superionic H
              2
              O with a thermal evolution model that accounts for heat trapped in the growing frozen core. The high viscosity provides a means of trapping heat in the deep interior while also providing a source of tidal dissipation. The frozen core grows with time because its outer boundary is governed by the freezing transition rather than compositional layering. We find that the presence of a growing frozen core explains the anomalously low heat flow of Uranus. Our thermal evolution model also predicts time-varying tidal dissipation that matches the requirements of the orbits of Miranda, Ariel, and Umbriel. We make predictions that are testable by future space missions, including the tidal Love number of Uranus and the current recessional rates of its moons.},
	number = {6},
	urldate = {2024-01-20},
	journal = {The Planetary Science Journal},
	author = {Stixrude, Lars and Baroni, Stefano and Grasselli, Federico},
	year = {2021},
	pages = {222},
	file = {Full Text:/Users/dong2j/Zotero/storage/4SN239K5/Stixrude et al. - 2021 - Thermal and Tidal Evolution of Uranus with a Growi.pdf:application/pdf},
}

@article{elkins-tanton_magma_2012,
	title = {Magma {Oceans} in the {Inner} {Solar} {System}},
	volume = {40},
	issn = {0084-6597, 1545-4495},
	url = {https://www.annualreviews.org/doi/10.1146/annurev-earth-042711-105503},
	doi = {10.1146/annurev-earth-042711-105503},
	abstract = {Theory and observations point to the occurrence of magma ponds or oceans in the early evolution of terrestrial planets and in many early-accreting planetesimals. The apparent ubiquity of melting during giant accretionary impacts suggests that silicate and metallic material may be processed through multiple magma oceans before reaching solidity in a planet. The processes of magma ocean formation and solidification, therefore, strongly influence the earliest compositional differentiation and volatile content of the terrestrial planets, and they form the starting point for cooling to clement, habitable conditions and for the onset of thermally driven mantle convection and plate tectonics. This review focuses on evidence for magma oceans on planetesimals and planets and on research concerning the processes of compositional differentiation in the silicate magma ocean, distribution and degassing of volatiles, and cooling.},
	language = {en},
	number = {1},
	urldate = {2024-01-20},
	journal = {Annual Review of Earth and Planetary Sciences},
	author = {Elkins-Tanton, Linda T.},
	year = {2012},
	pages = {113--139},
}

@article{lainey_new_2017,
	title = {New constraints on {Saturn}'s interior from {Cassini} astrometric data},
	volume = {281},
	issn = {00191035},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0019103516304183},
	doi = {10.1016/j.icarus.2016.07.014},
	language = {en},
	urldate = {2024-01-20},
	journal = {Icarus},
	author = {Lainey, Valéry and Jacobson, Robert A. and Tajeddine, Radwan and Cooper, Nicholas J. and Murray, Carl and Robert, Vincent and Tobie, Gabriel and Guillot, Tristan and Mathis, Stéphane and Remus, Françoise and Desmars, Josselin and Arlot, Jean-Eudes and De Cuyper, Jean-Pierre and Dehant, Véronique and Pascu, Dan and Thuillot, William and Poncin-Lafitte, Christophe Le and Zahn, Jean-Paul},
	year = {2017},
	pages = {286--296},
	file = {Submitted Version:/Users/dong2j/Zotero/storage/CSHBZTYV/Lainey et al. - 2017 - New constraints on Saturn's interior from Cassini .pdf:application/pdf},
}

@article{nimmo_strong_2023,
	title = {Strong {Tidal} {Dissipation} at {Uranus}?},
	volume = {4},
	issn = {2632-3338},
	url = {https://iopscience.iop.org/article/10.3847/PSJ/ad0cfb},
	doi = {10.3847/PSJ/ad0cfb},
	abstract = {Abstract
            
              Geophysical estimates of paleo heat fluxes on the Uranian moons Miranda and Ariel are in the range of 25–75 mW m
              −2
              . For a canonical Uranus dissipation factor
              Q
              = 18,000, expected equilibrium tidal heating rates for these satellites are less than 6 mW m
              −2
              . At least for Ariel, this order-of-magnitude discrepancy can be resolved by positing a low Uranus
              Q
              ≈ 10
              3
              in the recent past and at the present day. Such a low
              Q
              (high dissipation) can be reconciled with an ancient origin of the Uranian satellites if
              Q
              is time-dependent, as exemplified by the “resonance-locking” hypothesis, and provides an additional constraint on the interior structure of the planet. A
              Q
              of 10
              3
              implies present-day migration rates for Miranda and Ariel of 5 and 11 cm yr
              −1
              , respectively, potentially detectable via astrometry.},
	number = {12},
	urldate = {2024-01-20},
	journal = {The Planetary Science Journal},
	author = {Nimmo, Francis},
	year = {2023},
	pages = {241},
}

@article{pou_tidal_2022,
	title = {Tidal {Constraints} on the {Martian} {Interior}},
	volume = {127},
	issn = {2169-9097, 2169-9100},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2022JE007291},
	doi = {10.1029/2022JE007291},
	abstract = {Abstract
            
              We compare several recent Martian interior models and evaluate how these are impacted by the tidal constraints provided by the Love number
              k
              2
              and the secular acceleration in longitude
              s
              of its main moon, Phobos. The expression of the latter is developed up to harmonic degree 5 to match the accuracy of the current observations. We match a number of current interior structure models to the recent measurements of the tidal parameters and derive estimations of the possible core radius, temperature profile, and attenuation in the Martian interior. Our estimation of the core radius is 1,820 ± 80 km, consistent with recent seismic measurements. The attenuation profiles in the Martian interior at the main tidal period of Phobos are similar between the considered models, giving a range for the degree‐2 bulk tidal attenuation
              Q
              2
               = 93.0 ± 8.40 but diverge at seismic frequencies. At seismic frequencies, model shear attenuation
              Q
              
                μ
              
              ranges between 100 and 4,000 in the lower mantle, so that a measurement of seismic shear attenuation could be used as an effective means for distinguishing between the models considered. Other constraints such as elastic lithosphere thickness and Chandler Wobble period favor a thicker elastic lithosphere and models with a frequency dependence
              α
              of the shear attenuation between 0.15 and 0.4. Improved constraints on the Martian interior should be possible with additional seismic and radio observations from the InSight mission.
            
          , 
            Plain Language Summary
            The largest moon of Mars, Phobos, raises tides on the red planet causing its surface to be deformed. The size of this tidal bulge depends on the elastic properties of Mars, while viscosity and anelasticity inside the planet cause the tidal bulge to be misaligned with the position of Phobos on its orbit. This misalignment between Phobos and the tidal bulge of Mars creates an acceleration in longitude for the moon, which can be measured and used with the size of the tidal bulge to constraint the interior of Mars. Both the size and orientation of the tidal bulge can be used as tidal constraints to probe the size of the core of Mars, the temperature profile in its interior, and how strong the viscous dissipation is in its mantle. Our current estimates give a wide range of possible attenuation in the Martian mantle, favoring larger core sizes with larger elastic thickness of the lithosphere, the rigid outermost layer of a solid planet. Knowledge of the Martian interior could be further improved with future seismic and radio measurements from the InSight mission.
          , 
            Key Points
            
              
                
                  We develop a formulation to calculate the secular acceleration of Phobos due to tidal dissipation in Mars
                
                
                  
                    Using the Love number
                    k
                    2
                    and the secular acceleration
                    s
                    , we obtain for Mars a core size of 1,820 ± 80 km and a bulk
                    Q
                     of 93.0 ± 8.40
                  
                
                
                  We discuss several means to distinguish between Mars models using seismological, rotational, and lithospheric observations},
	language = {en},
	number = {11},
	urldate = {2024-01-20},
	journal = {Journal of Geophysical Research: Planets},
	author = {Pou, L. and Nimmo, F. and Rivoldini, A. and Khan, A. and Bagheri, A. and Gray, T. and Samuel, H. and Lognonné, P. and Plesa, A.‐C. and Gudkova, T. and Giardini, D.},
	year = {2022},
	pages = {e2022JE007291},
	file = {Full Text:/Users/dong2j/Zotero/storage/3DHW3YD6/Pou et al. - 2022 - Tidal Constraints on the Martian Interior.pdf:application/pdf},
}

@article{stevenson_formation_1982,
	title = {Formation of the giant planets},
	volume = {30},
	issn = {00320633},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0032063382901088},
	doi = {10.1016/0032-0633(82)90108-8},
	language = {en},
	number = {8},
	urldate = {2024-01-20},
	journal = {Planetary and Space Science},
	author = {Stevenson, D.J.},
	year = {1982},
	pages = {755--764},
}

@book{liu_elements_1986,
	address = {New York},
	title = {Elements, {Oxides}, {Silicates}: {High} {Pressure} {Phases} {With} {Implications} for the {Earth}'s {Interior}},
	publisher = {Oxford   University  Press},
	author = {Liu, Lin-gun and Bassett, William A.},
	year = {1986},
}

@incollection{duffy_mineralogy_2015,
	title = {Mineralogy of {Super}-{Earth} {Planets}},
	isbn = {978-0-444-53803-1},
	url = {https://linkinghub.elsevier.com/retrieve/pii/B9780444538024000531},
	language = {en},
	urldate = {2024-01-20},
	booktitle = {Treatise on {Geophysics}},
	publisher = {Elsevier},
	author = {Duffy, T. S and Madhusudhan, N. and Lee, K.K.M.},
	year = {2015},
	doi = {10.1016/B978-0-444-53802-4.00053-1},
	pages = {149--178},
}

@phdthesis{dong_water_2023,
	address = {Cambridge, MA},
	type = {Doctoral dissertation},
	title = {Water and {Phase} {Transitions} in {Rocky} {Planetary} {Interiors}},
	url = {https://nrs.harvard.edu/URN-3:HUL.INSTREPOS:37375828},
	abstract = {This dissertation explores two fundamental aspects of rocky planetary interiors: water and phase transitions. The first two chapters investigate the deep water cycles in Earth and Mars. The research provides an estimate of the bulk water storage capacity of their mantles as a function of mantle potential temperature using thermodynamic modeling, and examines its implications for the hydrosphere of early Earth through isostatic modeling. In the third chapter, a machine learning framework is introduced for determining high-pressure phase diagrams, with a specific focus on the post-spinel transition in Mg2SiO4. The resulting nonlinear Clapeyron slope of the post-spinel transition is then used to estimate its lateral variation at the base of the Earth’s transition zone.},
	school = {Harvard University Graduate School of Arts and Sciences},
	author = {Dong, Junjie},
	year = {2023},
	file = {Dong - 2023 - Water and Phase Transitions in Rocky Planetary Int.pdf:/Users/dong2j/Zotero/storage/XZCFPLN6/Dong - 2023 - Water and Phase Transitions in Rocky Planetary Int.pdf:application/pdf},
}







%%%%%%%%%%%%%%%%%%%%
DATABASE
%%%%%%%%%%%%%%%%%%%%
@incollection{ito_theory_2007,
	title = {Theory and {Practice} – {Multianvil} {Cells} and {High}-{Pressure} {Experimental} {Methods}},
	isbn = {978-0-444-52748-6},
	url = {https://linkinghub.elsevier.com/retrieve/pii/B9780444527486000365},
	language = {en},
	urldate = {2024-01-20},
	booktitle = {Treatise on {Geophysics}},
	publisher = {Elsevier},
	author = {Ito, E.},
	year = {2007},
	doi = {10.1016/B978-044452748-6.00036-5},
	pages = {197--230},
	file = {Ito - 2007 - Theory and Practice – Multianvil Cells and High-Pr.pdf:/Users/dong2j/Zotero/storage/AQHR9RUC/Ito - 2007 - Theory and Practice – Multianvil Cells and High-Pr.pdf:application/pdf},
}

@article{mao_solids_2018,
	title = {Solids, liquids, and gases under high pressure},
	volume = {90},
	issn = {0034-6861, 1539-0756},
	url = {https://link.aps.org/doi/10.1103/RevModPhys.90.015007},
	doi = {10.1103/RevModPhys.90.015007},
	language = {en},
	number = {1},
	urldate = {2024-01-20},
	journal = {Reviews of Modern Physics},
	author = {Mao, Ho-Kwang and Chen, Xiao-Jia and Ding, Yang and Li, Bing and Wang, Lin},
	year = {2018},
	pages = {015007},
	file = {Accepted Version:/Users/dong2j/Zotero/storage/MH2I7EPP/Mao et al. - 2018 - Solids, liquids, and gases under high pressure.pdf:application/pdf},
}

@article{duffy_ultra-high_2019,
	title = {Ultra-{High} {Pressure} {Dynamic} {Compression} of {Geological} {Materials}},
	volume = {7},
	issn = {2296-6463},
	url = {https://www.frontiersin.org/article/10.3389/feart.2019.00023/full},
	doi = {10.3389/feart.2019.00023},
	urldate = {2024-01-20},
	journal = {Frontiers in Earth Science},
	author = {Duffy, Thomas S. and Smith, Raymond F.},
	year = {2019},
	pages = {23},
	file = {Full Text:/Users/dong2j/Zotero/storage/69FNXGGY/Duffy and Smith - 2019 - Ultra-High Pressure Dynamic Compression of Geologi.pdf:application/pdf},
}

@book{wentzcovitch_theoretical_2010,
	title = {Theoretical and {Computational} {Methods} in {Mineral} {Physics}: {Geophysical} {Applications}},
	isbn = {978-1-5015-0844-8},
	shorttitle = {Theoretical and {Computational} {Methods} in {Mineral} {Physics}},
	url = {https://www.degruyter.com/document/doi/10.1515/9781501508448/html},
	urldate = {2024-01-20},
	publisher = {De Gruyter},
	editor = {Wentzcovitch, Renata M. and Stixrude, Lars},
	year = {2010},
	doi = {10.1515/9781501508448},
}

%%%%%%%%%%%%%%%%%%%%
ALGORITHM
%%%%%%%%%%%%%%%%%%%%


@incollection{aoki_statistical_2000,
	edition = {1},
	title = {Statistical {Analysis} of {Phase}-{Boundary} {Observations}},
	isbn = {978-0-521-64342-9 978-0-521-08422-2 978-0-511-89659-0},
	url = {https://www.cambridge.org/core/product/identifier/CBO9780511896590A042/type/book_part},
	urldate = {2024-01-20},
	booktitle = {Physics {Meets} {Mineralogy}},
	publisher = {Cambridge University Press},
	author = {Kavner, Abby and Speed, Terry and Jeanloz, Raymond},
	editor = {Aoki, Hideo and Syono, Yasuhiko and Hemley, Russell J.},
	year = {2000},
	doi = {10.1017/CBO9780511896590.006},
	pages = {71--80},
}

@article{pedregosa_scikit-learn_2011,
	title = {Scikit-learn: {Machine} {Learning} in {Python}},
	volume = {12},
	abstract = {Scikit-learn is a Python module integrating a wide range of state-of-the-art machine learning algorithms for medium-scale supervised and unsupervised problems. This package focuses on bringing machine learning to non-specialists using a general-purpose high-level language. Emphasis is put on ease of use, performance, documentation, and API consistency. It has minimal dependencies and is distributed under the simpliﬁed BSD license, encouraging its use in both academic and commercial settings. Source code, binaries, and documentation can be downloaded from http://scikit-learn.sourceforge.net.},
	language = {en},
	author = {Pedregosa, Fabian and Varoquaux, Gaël and Gramfort, Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Dubourg, Vincent and Vanderplas, Jake and Passos, Alexandre and Cournapeau, David and Brucher, Matthieu and Perrot, Matthieu and Duchesnay, Édouard},
	year = {2011},
journal = {{J}ournal of {M}achine {L}earning {R}esearch},
	pages = {2825--2830},
	file = {Pedregosa - Scikit-learn Machine Learning in Python.pdf:/Users/dong2j/Zotero/storage/52M7F4Y8/Pedregosa - Scikit-learn Machine Learning in Python.pdf:application/pdf},
}

@book{bishop_pattern_2006,
	address = {New York},
	series = {Information science and statistics},
	title = {Pattern recognition and machine learning},
	isbn = {978-0-387-31073-2},
	publisher = {Springer},
	author = {Bishop, Christopher M.},
	year = {2006},
	keywords = {Machine learning, Pattern perception},
}

@book{james_introduction_2021,
	address = {New York, NY},
	edition = {Second edition},
	series = {Springer texts in statistics},
	title = {An introduction to statistical learning: with applications in {R}},
	isbn = {978-1-07-161417-4 978-1-07-161420-4},
	shorttitle = {An introduction to statistical learning},
	language = {eng},
	publisher = {Springer},
	author = {James, Gareth and Witten, Daniela and Hastie, Trevor and Tibshirani, Robert},
	year = {2021},
	doi = {10.1007/978-1-0716-1418-1},
	file = {Table of Contents PDF:/Users/dong2j/Zotero/storage/DX375X33/James et al. - 2021 - An introduction to statistical learning with appl.pdf:application/pdf},
}

@misc{dong_nonlinearity_2024,
	title = {Nonlinearity of the post-spinel transition and its expression in slabs and plumes worldwide},
	copyright = {Creative Commons Attribution Non Commercial No Derivatives 4.0 International},
	url = {https://arxiv.org/abs/2208.08975},
	doi = {10.48550/ARXIV.2208.08975},
	abstract = {At the interface of Earth's upper and lower mantle, the post-spinel transition boundary controls the dynamics and morphologies of downwelling slabs and upwelling plumes, and its Clapeyron slope is hence one of the most important constraints on mantle convection. In this study, we reported a new in situ experimental dataset on phase stability in Mg\$\_\{2\}\$SiO\$\_\{4\}\$ at mantle transition zone pressures from laser-heated diamond anvil cell experiments, along with a compilation of corrected in situ experimental datasets from the literature. We presented a machine learning framework for high-pressure phase diagram determination and focused on its application to constrain the location and Clapeyron slope of the post-spinel transition: ringwoodite \${\textbackslash}leftrightarrow\$ bridgmanite + periclase. We found that the post-spinel boundary is nonlinear and its Clapeyron slope varies locally from \$-2.3\_\{-1.4\}{\textasciicircum}\{+0.6\}\$ MPa/K at 1900 K, to \$-1.0\_\{-1.7\}{\textasciicircum}\{+1.3\}\$ MPa/K at 1700 K, and to \$0.0\_\{-2.0\}{\textasciicircum}\{+1.7\}\$ MPa/K at 1500 K. We applied the temperature-dependent post-spinel Clapeyron slope to estimate its lateral variation across the "660-km" seismic discontinuity in subducting slabs and hotspot-associated plumes worldwide, as well as the ambient mantle. We found that, in the present-day mantle, the average post spinel Clapeyron slope in the plumes is three times more negative than that in slabs, and we then discussed the effects of a nonlinear post-spinel transition on the dynamics of Earth's mantle.},
	urldate = {2024-01-20},
	publisher = {arXiv},
	author = {Dong, Junjie and Fischer, Rebecca A. and Stixrude, Lars and Brennan, Matthew C. and Daviau, Kierstin and Suer, Terry-Ann and Turner, Katlyn M. and Meng, Yue and Prakapenka, Vitali B.},
	year = {2024},
	note = {Publisher: arXiv
Version Number: 1},
	keywords = {FOS: Physical sciences, Geophysics (physics.geo-ph), Materials Science (cond-mat.mtrl-sci)},
	annote = {Other
42 pages, 6500 words and 5 figures in the main text, and 1 supplement with 6 texts, 5 figures, and 6 tables},
}


@article{komabayashi_thermodynamics_2014,
	title = {Thermodynamics of melting relations in the system {Fe}‐{FeO} at high pressure: {Implications} for oxygen in the {Earth}'s core},
	volume = {119},
	copyright = {http://onlinelibrary.wiley.com/termsAndConditions\#vor},
	issn = {2169-9313, 2169-9356},
	shorttitle = {Thermodynamics of melting relations in the system {Fe}‐{FeO} at high pressure},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1002/2014JB010980},
	doi = {10.1002/2014JB010980},
	abstract = {The thermodynamics of melting relations in the system Fe-FeO was investigated to the outer core–inner core boundary condition from a self-consistent thermodynamic database which was evaluated from the latest static high-pressure (P) and high-temperature (T) experiments. The evaluated database together with an existing nonideal mixing model for liquids reproduces experimental data on the eutectic composition and temperature to P = 50 GPa. On the other hand at the outer core pressures (136 to 330 GPa), employing an ideal solution model gives calculated eutectic temperatures of T = 2990–4330 K, which are also consistent with experimental data. Hence, the ideal solution model is applied to calculate the liquid property under outer core conditions and yields the eutectic compositions of Fe–7.2–9.1 wt \% O. From the Gibbs free energy for the Fe-FeO liquids, I calculated the density, sound velocity, and isentropic temperature gradient of a hypothetical oxygen-bearing outer core. Under the outer core conditions, the addition of oxygen reduces the compressional wave velocity of iron liquid, moving it away from seismologically constrained values. An overall O-rich bulk outer core model is thus excluded. Seismological observations however suggest the presence of a low-velocity layer with a thickness of 60–70 km at the top of the outer core. The origin of such a low-velocity layer can be explained by an enrichment of oxygen which might be a consequence of chemical interactions between the core and mantle.},
	language = {en},
	number = {5},
	urldate = {2024-11-24},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Komabayashi, Tetsuya},
	month = may,
	year = {2014},
	pages = {4164--4177},
	file = {Komabayashi - 2014 - Thermodynamics of melting relations in the system .pdf:/Users/jdong/Zotero/storage/V8A9PGP9/Komabayashi - 2014 - Thermodynamics of melting relations in the system .pdf:application/pdf},
}

@article{dorogokupets_thermodynamics_2017,
	title = {Thermodynamics and {Equations} of {State} of {Iron} to 350 {GPa} and 6000 {K}},
	volume = {7},
	issn = {2045-2322},
	url = {https://www.nature.com/articles/srep41863},
	doi = {10.1038/srep41863},
	abstract = {Abstract
            
              The equations of state for solid (with bcc, fcc, and hcp structures) and liquid phases of Fe were defined via simultaneous optimization of the heat capacity, bulk moduli, thermal expansion, and volume at room and higher temperatures. The calculated triple points at the phase diagram have the following parameters: bcc–fcc–hcp is located at 7.3 GPa and 820 K, bcc–fcc–liquid at 5.2 GPa and 1998 K, and fcc–hcp–liquid at 106.5 GPa and 3787 K. At conditions near the fcc–hcp–liquid triple point, the Clapeyron slope of the fcc–liquid curve is d
              T
              /d
              P
               = 12.8 K/GPa while the slope of the hcp–liquid curve is higher (d
              T
              /d
              P
               = 13.7 K/GPa). Therefore, the hcp–liquid curve overlaps the metastable fcc–liquid curve at pressures of about 160 GPa. At high-pressure conditions, the metastable bcc–hcp curve is located inside the fcc-Fe or liquid stability field. The density, adiabatic bulk modulus and P-wave velocity of liquid Fe calculated up to 328.9 GPa at adiabatic temperature conditions started from 5882 K (outer/inner core boundary) were compared to the PREM seismological model. We determined the density deficit of hcp-Fe at the inner core boundary (
              T
               = 5882 K and
              P
               = 328.9 GPa) to be 4.4\%.},
	language = {en},
	number = {1},
	urldate = {2024-11-24},
	journal = {Scientific Reports},
	author = {Dorogokupets, P. I. and Dymshits, A. M. and Litasov, K. D. and Sokolova, T. S.},
	month = mar,
	year = {2017},
	pages = {41863},
	file = {Dorogokupets et al. - 2017 - Thermodynamics and Equations of State of Iron to 3.pdf:/Users/jdong/Zotero/storage/8PRM5FIQ/Dorogokupets et al. - 2017 - Thermodynamics and Equations of State of Iron to 3.pdf:application/pdf},
}


%% MgO %%
@article{bolis_decaying_2016,
	title = {Decaying shock studies of phase transitions in {MgO}‐{SiO} $_{\textrm{2}}$ systems: {Implications} for the super‐{Earths}' interiors},
	volume = {43},
	issn = {0094-8276, 1944-8007},
	shorttitle = {Decaying shock studies of phase transitions in {MgO}‐{SiO} $_{\textrm{2}}$ systems},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1002/2016GL070466},
	doi = {10.1002/2016GL070466},
	abstract = {We report an experimental study of the phase diagrams of MgO, MgSiO3, and Mg2SiO4 at high pressures. We measured the shock compression response, including pressure-temperature Hugoniot curves of MgO, MgSiO3, and Mg2SiO4 between 0.2–1.2 TPa, 0.12–0.5 TPa, and 0.2–0.85 TPa, respectively, using laser-driven decaying shocks. A melting signature has been observed in MgO at 0.47 ± 0.04 TPa and 9860 ± 810 K, while no such phase changes were observed either in MgSiO3 or in Mg2SiO4. Increases of reﬂectivity of MgO, MgSiO3, and Mg2SiO4 liquids have been detected above 0.55 TPa (12760 K), 0.15 TPa (7540 K), 0.2 TPa (5800 K), respectively. In contrast to SiO2, melting and metallization of these compounds do not coincide, implying the presence of poorly electrically conducting liquids close to the melting lines. This has important implications for the generation of dynamos in super-Earth’s mantles.},
	language = {en},
	number = {18},
	urldate = {2024-01-01},
	journal = {Geophysical Research Letters},
	author = {Bolis, R. M. and Morard, G. and Vinci, T. and Ravasio, A. and Bambrink, E. and Guarguaglini, M. and Koenig, M. and Musella, R. and Remus, F. and Bouchet, J. and Ozaki, N. and Miyanishi, K. and Sekine, T. and Sakawa, Y. and Sano, T. and Kodama, R. and Guyot, F. and Benuzzi‐Mounaix, A.},
	month = sep,
	year = {2016},
	pages = {9475--9483},
	file = {Bolis et al. - 2016 - Decaying shock studies of phase transitions in MgO.pdf:/Users/dong2j/Zotero/storage/KJFL8XLR/Bolis et al. - 2016 - Decaying shock studies of phase transitions in MgO.pdf:application/pdf},
}

@article{hansen_melting_2021,
	title = {Melting of magnesium oxide up to two terapascals using double-shock compression},
	volume = {104},
	issn = {2469-9950, 2469-9969},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.104.014106},
	doi = {10.1103/PhysRevB.104.014106},
	language = {en},
	number = {1},
	urldate = {2024-01-01},
	journal = {Physical Review B},
	author = {Hansen, L. E. and Fratanduono, D. E. and Zhang, S. and Hicks, D. G. and Suer, T. and Sprowal, Z. K. and Huff, M. F. and Gong, X. and Henderson, B. J. and Polsin, D. N. and Zaghoo, M. and Hu, S. X. and Collins, G. W. and Rygg, J. R.},
	month = jul,
	year = {2021},
	pages = {014106},
	file = {Hansen et al. - 2021 - Melting of magnesium oxide up to two terapascals u.pdf:/Users/dong2j/Zotero/storage/CF9E5ETR/Hansen et al. - 2021 - Melting of magnesium oxide up to two terapascals u.pdf:application/pdf},
}

@article{stixrude_geophysics_2012,
	title = {Geophysics of {Chemical} {Heterogeneity} in the {Mantle}},
	volume = {40},
	issn = {0084-6597, 1545-4495},
	url = {https://www.annualreviews.org/doi/10.1146/annurev.earth.36.031207.124244},
	doi = {10.1146/annurev.earth.36.031207.124244},
	abstract = {Chemical heterogeneity, produced by the near-surface rock cycle and dominated volumetrically by subducted oceanic crust and its depleted residue, is continuously subducted into the mantle. This lithologic-scale chemical heterogeneity may survive in the mantle for as long as the age of Earth because chemical diffusion is inefficient. Estimates of rates of subduction and mantle processing over geologic history indicate that most or all of the mantle may be composed of lithologically heterogeneous material. Mineralogical models of the mantle show that chemical heterogeneity over many decades in length scale may be detectable by geophysical probes via its influence on seismic-wave propagation. Grain-scale heterogeneity influences the aggregate absolute seismic velocity and its lateral variation with temperature. The elastic-wave velocity contrast associated with lithologic-scale heterogeneity may be sufficient to produce observable scattering of short-period seismic waves.},
	language = {en},
	number = {1},
	urldate = {2024-01-21},
	journal = {Annual Review of Earth and Planetary Sciences},
	author = {Stixrude, Lars and Lithgow-Bertelloni, Carolina},
	year = {2012},
	pages = {569--595},
}

@article{mcwilliams_phase_2012,
	title = {Phase {Transformations} and {Metallization} of {Magnesium} {Oxide} at {High} {Pressure} and {Temperature}},
	volume = {338},
	issn = {0036-8075, 1095-9203},
	url = {https://www.science.org/doi/10.1126/science.1229450},
	doi = {10.1126/science.1229450},
	abstract = {Planetary Interiors Under Pressure
            
              The interiors of Earth and other rocky planets generally consist of a few common minerals. Depending largely on the size of the planet, the distribution and relative abundance of these minerals varies; for example, MgO is abundant in the mantles of Earth and large Earth-like planets, but is present in Jupiter's core. The properties of MgO also vary with planetary size as a function of temperature and pressure.
              
                McWilliams
                et al.
              
              (p.
              1330
              , published online 22 November) performed laser-shock experiments at pressures over three times higher than Earth's inner core. MgO underwent two phase transformations, first to a solid with a modified crystal structure, and then to a conductive liquid. In terrestrial planets greater than eight Earth masses, MgO in the mantle could generate a magnetic field–generating dynamo such as those that typically found in planetary cores.
            
          , 
            Mantle minerals conductive at the high pressures and temperatures of planetary interiors could induce a magnetic field.
          , 
            Magnesium oxide (MgO) is representative of the rocky materials comprising the mantles of terrestrial planets, such that its properties at high temperatures and pressures reflect the nature of planetary interiors. Shock-compression experiments on MgO to pressures of 1.4 terapascals (TPa) reveal a sequence of two phase transformations: from B1 (sodium chloride) to B2 (cesium chloride) crystal structures above 0.36 TPa, and from electrically insulating solid to metallic liquid above 0.60 TPa. The transitions exhibit large latent heats that are likely to affect the structure and evolution of super-Earths. Together with data on other oxide liquids, we conclude that magmas deep inside terrestrial planets can be electrically conductive, enabling magnetic field–producing dynamo action within oxide-rich regions and blurring the distinction between planetary mantles and cores.},
	language = {en},
	number = {6112},
	urldate = {2024-01-01},
	journal = {Science},
	author = {McWilliams, R. Stewart and Spaulding, Dylan K. and Eggert, Jon H. and Celliers, Peter M. and Hicks, Damien G. and Smith, Raymond F. and Collins, Gilbert W. and Jeanloz, Raymond},
	month = dec,
	year = {2012},
	pages = {1330--1333},
	file = {McWilliams et al. - 2012 - Phase Transformations and Metallization of Magnesi.pdf:/Users/dong2j/Zotero/storage/QYBFEFDF/McWilliams et al. - 2012 - Phase Transformations and Metallization of Magnesi.pdf:application/pdf},
}

@article{coppari_experimental_2013,
	title = {Experimental evidence for a phase transition in magnesium oxide at exoplanet pressures},
	volume = {6},
	issn = {1752-0894, 1752-0908},
	url = {https://www.nature.com/articles/ngeo1948},
	doi = {10.1038/ngeo1948},
	language = {en},
	number = {11},
	urldate = {2024-01-03},
	journal = {Nature Geoscience},
	author = {Coppari, F. and Smith, R. F. and Eggert, J. H. and Wang, J. and Rygg, J. R. and Lazicki, A. and Hawreliak, J. A. and Collins, G. W. and Duffy, T. S},
	month = nov,
	year = {2013},
	pages = {926--929},
	file = {Coppari et al. - 2013 - Experimental evidence for a phase transition in ma.pdf:/Users/dong2j/Zotero/storage/YTYNTVBL/Coppari et al. - 2013 - Experimental evidence for a phase transition in ma.pdf:application/pdf},
}

@article{speziale_quasihydrostatic_2001,
	title = {Quasi‐hydrostatic compression of magnesium oxide to 52 {GPa}: {Implications} for the pressure‐volume‐temperature equation of state},
	volume = {106},
	issn = {0148-0227},
	shorttitle = {Quasi‐hydrostatic compression of magnesium oxide to 52 {GPa}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2000JB900318},
	doi = {10.1029/2000JB900318},
	abstract = {Roomtemperatursetaticcompressioonf MgO (periclasew) asperformedunder nearlyhydrostatciconditionussingenergydispersivseynchrotroXn-raydiffractionin a diamondanvil cell with methanol-ethano(lto 10 GPa) or helium(to 52 GPa) asa pressuretransmittinmgediumH. ighlyprecisecellparameterwseredeterminewd ithanaverage relativestandarddeviation{\textless}Aa/a{\textgreater} = 0.0003 overall theexperimentapl ressurerange. FixingthebulkmodulusK0r= 160.2GPa,a fit of thedatatothethird-ordeBr irchMurnagheaqnuationfstatyeieldsV'0=74.71+0.01]i3,(•Kor/•P)=r 3.99+0.01A. fit of differenPt -V-T datasetsra, ngingto53 GPaand2500K, toa Birch-Murnaghan-Debye thermael quationof stateconstrainetdheGrtineisepnaramete)r6= 1.49+ 0.03,butnotits volumedependencqe, whichwasconstrainetdo 1.65+ 0.4bythermodynamtihceoryA. modelbasedona constanvtalueof q cannotexplaintheultrahighpressure(P = 174-203 GPa)shockcompressiodnata.We developeda modelin whichq decreasewsith compressiofrnom1.65at0.1MPato0.01at200GPa.Thismodelw, ithintheframeworkof theMie-Griineisen-Debyaessumptionssa, tisfactorildyescribetshelow-pressursetaticdata ({\textless}AV/V{\textgreater} = 0.4\% to 53 GPa)andthehigh-pressurHeugoniotdata({\textless}AV/V{\textgreater}{\textless} 1\%to 203 GPa).Averagevaluesof thethermael xpansiocnoefficienatrrangebetween14.1+ 2.8and 16.3+ 2.7x 10'6K'•atP= 174-20G3 PaT. hepressudrependenocftehemelting temperatuyrieeldsaninitialpressurdeerivativ•e\vphantom{\{}\}Tm/0P= 98K/GPa.Ouranalysisshows thatit ispossiblteodevelopa simplemodelof thevolumedependencoef theGrtineisen parametethr atcansuccessfuldlyescribteheP-V-T equationof stateof MgOfromambient conditions to 203 GPa and 3663 K.},
	language = {en},
	number = {B1},
	urldate = {2024-01-01},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Speziale, Sergio and Zha, Chang‐Sheng and Duffy, Thomas S. and Hemley, Russell J. and Mao, Ho‐kwang},
	month = jan,
	year = {2001},
	pages = {515--528},
	file = {Speziale et al. - 2001 - Quasi‐hydrostatic compression of magnesium oxide t.pdf:/Users/dong2j/Zotero/storage/8BJYQ94P/Speziale et al. - 2001 - Quasi‐hydrostatic compression of magnesium oxide t.pdf:application/pdf},
}

@article{ye_intercomparison_2017,
	title = {Intercomparison of the gold, platinum, and {MgO} pressure scales up to 140 {GPa} and 2500 {K}},
	volume = {122},
	issn = {2169-9313, 2169-9356},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1002/2016JB013811},
	doi = {10.1002/2016JB013811},
	abstract = {In order to intercalibrate the equations of state (EOSs) of the three widely used pressure standards, gold, platinum, and MgO, we have measured their unit cell volumes together in the laser-heated diamond anvil cell up to 140 GPa and 2500 K. At 300 K, three standards agree with each other within ±2.5 GPa to 135 GPa if the EOSs measured in quasi-hydrostatic media are used. We further reﬁned the EOSs at 300 K, making them consistent with each other within ±1 GPa up to 135 GPa. At high temperature (T), the three standards match the best within ±1 GPa between 40 and 140 GPa, when we use the scales by Dorogokupets and Dewaele (2007). However, a 2–3 GPa discrepancy remains at 20–40 GPa and 1500–2000 K, with gold yielding the highest pressure (P). The pressure discrepancy is likely related to steep decreases in the Grüneisen parameter, the anharmonicity, and/or the electronic eﬀects for the standards at the P-T conditions. Because gold melts near the temperatures expected for the mantle transition zone, severe anharmonic eﬀects expected under premelting conditions make gold unsuitable for determining the phase boundaries in the region. The pressure scales by Dorogokupets and Dewaele (2007) provide tighter constrains on the Clapeyron slopes of the postspinel boundary to −2.0 to −2.7 MPa/K and the postperovskite boundary to 7–10 MPa/K. The data and reﬁned EOSs presented here allow for reliable comparisons among experiments with diﬀerent pressure standards for the entire P-T conditions expected for the Earth’s lower mantle.},
	language = {en},
	number = {5},
	urldate = {2024-01-01},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Ye, Y. and Prakapenka, V. and Meng, Y. and Shim, S.‐H.},
	month = may,
	year = {2017},
	pages = {3450--3464},
	file = {Ye et al. - 2017 - Intercomparison of the gold, platinum, and MgO pre.pdf:/Users/dong2j/Zotero/storage/76E2KUUW/Ye et al. - 2017 - Intercomparison of the gold, platinum, and MgO pre.pdf:application/pdf},
}

@article{dubrovinsky_thermal_1997,
	title = {Thermal {Expansion} of {Periclase} ({MgO}) and {Tungsten} ({W}) to {Melting} {Temperatures}},
	volume = {24},
	issn = {0342-1791, 1432-2021},
	url = {http://link.springer.com/10.1007/s002690050070},
	doi = {10.1007/s002690050070},
	abstract = {In situ x-ray data on molar volumes of periclase and tungsten have been collected over the temperature range from 300 K to melting. We determine the temperature by combining the technique of spectroradiometry and electrical resistance wire heating. The thermal expansion (a) of periclase between 300 and 3100 K is given by aϭ2.6025 10Ϫ5ϩ1.3535 10Ϫ8 Tϩ6.5687 10Ϫ3 TϪ1Ϫ1.8281 TϪ2.},
	language = {en},
	number = {8},
	urldate = {2024-01-01},
	journal = {Physics and Chemistry of Minerals},
	author = {Dubrovinsky, L. S. and Saxena, S. K.},
	month = oct,
	year = {1997},
	pages = {547--550},
	file = {Dubrovinsky and Saxena - 1997 - Thermal Expansion of Periclase (MgO) and Tungsten .pdf:/Users/dong2j/Zotero/storage/PDD393L8/Dubrovinsky and Saxena - 1997 - Thermal Expansion of Periclase (MgO) and Tungsten .pdf:application/pdf},
}

@article{fei_effects_1999,
	title = {Effects of temperature and composition on the bulk modulus of ({Mg},{Fe}){O}},
	volume = {84},
	issn = {0003-004X},
	url = {https://www.degruyter.com/document/doi/10.2138/am-1999-0308/html},
	doi = {10.2138/am-1999-0308},
	abstract = {Isothermal static compression data for MgO at 300 and 1100 K were obtained by combining synchrotron X-ray diffraction techniques with an externally heated high-temperature diamond-anvil cell that is capable of achieving pressures greater than 125 GPa at temperatures up to 1100 K. The experiments at 300 K were conducted under both hydrostatic and nonhydrostatic conditions. The deviatoric stress in non-hydrostatic environment signiﬁcantly effects the measured lattice parameters. Fits to the static compression data of MgO at 300 K yield a bulk modulus of 185(7) GPa and 160(2) GPa under nonhydrostatic and hydrostatic conditions, respectively. The deviatoric stress decreases with increasing temperature, and a nearly hydrostatic condition was achieved at temperatures above 900 K when NaCl was used as a pressure-medium. The bulk modulus of MgO was determined to be 135(3) GPa at a temperature of 1100 K, yielding its temperature derivative of Ϫ0.030(3) GPa/K. Comparing these results with previous studies in the system MgO-FeO, shows that the bulk modulus of (Mg,Fe)O decreases with increasing FeO content, from 160 GPa for MgO to 146 GPa for FeO.},
	language = {en},
	number = {3},
	urldate = {2024-01-01},
	journal = {American Mineralogist},
	author = {Fei, Yingwei},
	month = mar,
	year = {1999},
	pages = {272--276},
	file = {Fei - 1999 - Effects of temperature and composition on the bulk.pdf:/Users/dong2j/Zotero/storage/EJTL5CM4/Fei - 1999 - Effects of temperature and composition on the bulk.pdf:application/pdf},
}

@article{fiquet_high-temperature_1999,
	title = {High-temperature thermal expansion of lime, periclase, corundum and spinel},
	volume = {27},
	issn = {0342-1791, 1432-2021},
	url = {http://link.springer.com/10.1007/s002690050246},
	doi = {10.1007/s002690050246},
	abstract = {The high-temperature cell parameters of lime (CaO), periclase (MgO), corundum (Al2O3), and spinel (MgAl2O4) have been determined from 300 up to 3000 K through X-ray diraction experiments with synchrotron radiation. The good agreement found with dilatometric results suggests that vacancy-type defects do not make a large contribution to thermal expansion for these oxides, even near the melting point, justifying the use of X-ray diraction for determining volume properties up to very high temperatures. Thermal expansion coecients were determined from the measured cell volumes with equations of the form a  a0 + a1T + a2/T 2. Along with available isobaric heat capacity and compressibility data, these derived coecients clearly show that anharmonic eects contribute little to the isochoric heat capacities (Cv) of CaO, MgO, and Al2O3, which do not depart appreciably from the 3nR Dulong and Petit limit.},
	language = {en},
	number = {2},
	urldate = {2024-01-01},
	journal = {Physics and Chemistry of Minerals},
	author = {Fiquet, G. and Richet, P. and Montagnac, G.},
	month = dec,
	year = {1999},
	pages = {103--111},
	file = {Fiquet et al. - 1999 - High-temperature thermal expansion of lime, pericl.pdf:/Users/dong2j/Zotero/storage/PH6DBEJW/Fiquet et al. - 1999 - High-temperature thermal expansion of lime, pericl.pdf:application/pdf},
}

@article{dewaele_pvt_2000,
	title = {P‐{V}‐{T} equation of state of periclase from synchrotron radiation measurements},
	volume = {105},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/1999JB900364},
	doi = {10.1029/1999JB900364},
	abstract = {The volumeof periclase(MgO) hasbeenmeasuredby monochromatic X-ray diffraction in a laser-heateddiamond anvil cell up to a pressureof 53 GPa and a temperature of 2500 K. The X-ray sourcewas synchrotronradiation at the EuropeanSynchrotronRadiationFacility (Grenoble,France). In addition to laser heating, the use of argon as a pressuretransmitting medium provided quasi-hydrostaticconditionsin the cell assembly.In order to take thermal pressure effect into account,pressurewas measuredusingan internal pressurecalibrant (platinum). By analysisoftheexperimentaPl -V-T datasetthe followingparameters wereobtained:at ambienttemperatureK, • = 3.94 + 0.2 whenK0 is fixedto 161 GPa (with a Birch-Murnaghanequationof state);underhightemperature, c•(P- 0,T) - (3.0+ 0.0012T)x 10-s K-I; (OKT/OT)p=-0.022(3) GPaK-1. The quasi-harmonicDebye model appearsto describecorrectlythe temperature dependenceof the volume at high pressurewithin experimental errors, with the followingparameters:ODO= 800 K, 70 = 1.45 (Griineisenparameterunderambient conditions),and q = 0.8 q- 0.5.},
	language = {en},
	number = {B2},
	urldate = {2024-01-01},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Dewaele, Agnès and Fiquet, Guillaume and Andrault, Denis and Hausermann, Daniel},
	month = feb,
	year = {2000},
	pages = {2869--2877},
	file = {Dewaele et al. - 2000 - P‐V‐T equation of state of periclase from synchrot.pdf:/Users/dong2j/Zotero/storage/EGBXK465/Dewaele et al. - 2000 - P‐V‐T equation of state of periclase from synchrot.pdf:application/pdf},
}

@article{du_highpressure_2014,
	title = {High‐pressure melting of {MgO} from ({Mg},{Fe}){O} solid solutions},
	volume = {41},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1002/2014GL061954},
	doi = {10.1002/2014GL061954},
	abstract = {Abstract
            Magnesium oxide (MgO) is a significant component of planetary interiors, particularly Earth's mantle and other rocky planets within and beyond our solar system; thus its high‐pressure, high‐temperature behavior is important to understanding the thermochemical evolution of planets. Laser‐heated diamond‐anvil cell (DAC) experiments on (Mg,Fe)O ferropericlase up to {\textasciitilde}40 GPa show that previous DAC experiments on MgO melting are too low, while previous multi‐anvil experiments yield melting temperatures too high. Instead, our quasi‐static experimental results are consistent with recent ab initio predictions as well as dynamic shock measurements. Extrapolated to the core‐mantle boundary (CMB) of the Earth, MgO is expected to melt at {\textasciitilde}8000 ± 500 K, much greater than expected geotherm temperatures.
          , 
            Key Points
            
              
                
                  Melting curve of MgO determined experimentally to 40 GPa
                
                
                  Results consistent with recent ab initio predictions and shock measurements
                
                
                  MgO‐FeO binary system is consistent with ideal solid solution model up to 40 GPa},
	language = {en},
	number = {22},
	urldate = {2024-01-01},
	journal = {Geophysical Research Letters},
	author = {Du, Zhixue and Lee, Kanani K. M.},
	month = nov,
	year = {2014},
	pages = {8061--8066},
	file = {Du and Lee - 2014 - High‐pressure melting of MgO from (Mg,Fe)O solid s.pdf:/Users/dong2j/Zotero/storage/D2V9YDJB/Du and Lee - 2014 - High‐pressure melting of MgO from (Mg,Fe)O solid s.pdf:application/pdf},
}

@article{kimura_melting_2017,
	title = {Melting temperatures of {MgO} under high pressure by micro-texture analysis},
	volume = {8},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/ncomms15735},
	doi = {10.1038/ncomms15735},
	abstract = {Abstract
            Periclase (MgO) is the second most abundant mineral after bridgmanite in the Earth’s lower mantle, and its melting behaviour under pressure is important to constrain rheological properties and melting behaviours of the lower mantle materials. Significant discrepancies exist between the melting temperatures of MgO determined by laser-heated diamond anvil cell (LHDAC) and those based on dynamic compressions and theoretical predictions. Here we show the melting temperatures in earlier LHDAC experiments are underestimated due to misjudgment of melting, based on micro-texture observations of the quenched samples. The high melting temperatures of MgO suggest that the subducted cold slabs should have higher viscosities than previously thought, suggesting that the inter-connecting textural feature of MgO would not play important roles for the slab stagnation in the lower mantle. The present results also predict that the ultra-deep magmas produced in the lower mantle are peridotitic, which are stabilized near the core–mantle boundary.},
	language = {en},
	number = {1},
	urldate = {2024-01-01},
	journal = {Nature Communications},
	author = {Kimura, T. and Ohfuji, H. and Nishi, M. and Irifune, T.},
	month = jun,
	year = {2017},
	pages = {15735},
	file = {Kimura et al. - 2017 - Melting temperatures of MgO under high pressure by.pdf:/Users/dong2j/Zotero/storage/38BV57WW/Kimura et al. - 2017 - Melting temperatures of MgO under high pressure by.pdf:application/pdf},
}

@article{zerr_constraints_1994,
	title = {Constraints on the melting temperature of the lower mantle from high-pressure experiments on {MgO} and magnesiowiistite},
	volume = {371},
    journal = {{N}ature},
	language = {en},
	author = {Zerr, A and Boehler, R},
	year = {1994},
	file = {Zerr and Boehler - 1994 - Constraints on the melting temperature of the lowe.pdf:/Users/dong2j/Zotero/storage/DVTNY7VV/Zerr and Boehler - 1994 - Constraints on the melting temperature of the lowe.pdf:application/pdf},
}

@article{zhang_melting_2008,
	title = {Melting behavior of ({Mg},{Fe}){O} solid solutions at high pressure},
	volume = {35},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2008GL034585},
	doi = {10.1029/2008GL034585},
	abstract = {High pressure melting of (Mg,Fe)O ferropericlase, the second most abundant mineral in the Earth's lower mantle, is of fundamental importance for understanding the chemical differentiation, geodynamics and thermal evolution of the Earth's interior. We report the first systematic experimental study of melting behavior in the MgO‐FeO system up to 3600 K and 7 GPa, indicating the ideal solution between solid and liquid (Mg,Fe)O in the MgO‐rich portion. The zero pressure melting slope of MgO is ∼221 K/GPa derived from our resistance heating measurements, which is several times higher than the value from the previous measurements in a CO
              2
              ‐laser heated diamond anvil cell, but consistent with the theoretically predicted melting curves. Our results combined with the previous first‐principles simulations suggest that the melting temperature of MgO‐rich (Mg,Fe)O is significantly higher than the geotherm through the lower mantle and this would place an upper bound on the solidus of the lower mantle.},
	language = {en},
	number = {13},
	urldate = {2024-01-01},
	journal = {Geophysical Research Letters},
	author = {Zhang, Li and Fei, Yingwei},
	month = jul,
	year = {2008},
	pages = {2008GL034585},
	file = {Zhang and Fei - 2008 - Melting behavior of (Mg,Fe)O solid solutions at hi.pdf:/Users/dong2j/Zotero/storage/7UBJ5KQH/Zhang and Fei - 2008 - Melting behavior of (Mg,Fe)O solid solutions at hi.pdf:application/pdf},
}

@article{soubiran_anharmonicity_2020,
	title = {Anharmonicity and {Phase} {Diagram} of {Magnesium} {Oxide} in the {Megabar} {Regime}},
	volume = {125},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.125.175701},
	doi = {10.1103/PhysRevLett.125.175701},
	language = {en},
	number = {17},
	urldate = {2024-01-01},
	journal = {Physical Review Letters},
	author = {Soubiran, François and Militzer, Burkhard},
	month = oct,
	year = {2020},
	pages = {175701},
	file = {Soubiran and Militzer - 2020 - Anharmonicity and Phase Diagram of Magnesium Oxide.pdf:/Users/dong2j/Zotero/storage/VC3UZDK6/Soubiran and Militzer - 2020 - Anharmonicity and Phase Diagram of Magnesium Oxide.pdf:application/pdf},
}

@article{li_molecular_2006,
	title = {Molecular {Dynamics} {Simulation} of {MgO} {Melting} at {High} {Pressure}},
	volume = {19},
	issn = {1674-0068, 2327-2244},
	url = {https://pubs.aip.org/cjcp/article/19/4/315/137335/Molecular-Dynamics-Simulation-of-MgO-Melting-at},
	doi = {10.1360/cjcp2006.19(4).315.4},
	abstract = {Molecular dynamics simulation was used to study the melting of MgO at high pressures. The melting temperature of MgO was accurately obtained at elevated temperature and high pressure after corrections based on the modern theory of melting. The calculated melting curve was compared with the available experimental data and other theoretical results at the pressure range of 0-135 GPa. The corrected melting temperature of MgO is in good agreement with the results from Lindemann melting equation and the twophase simulated results below 15 GPa.},
	language = {en},
	number = {4},
	urldate = {2024-01-01},
	journal = {Chinese Journal of Chemical Physics},
	author = {Li, Shou-yi and Liu, Zheng-lai and Nan, Ya-gong and Zhang, Zhi-rong},
	month = aug,
	year = {2006},
	pages = {315--318},
	file = {Li et al. - 2006 - Molecular Dynamics Simulation of MgO Melting at Hi.pdf:/Users/dong2j/Zotero/storage/WEWMFF7A/Li et al. - 2006 - Molecular Dynamics Simulation of MgO Melting at Hi.pdf:application/pdf},
}

@article{belonoshko_mgo_2010,
	title = {{MgO} phase diagram from first principles in a wide pressure-temperature range},
	volume = {81},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.81.054110},
	doi = {10.1103/PhysRevB.81.054110},
	language = {en},
	number = {5},
	urldate = {2024-01-01},
	journal = {Physical Review B},
	author = {Belonoshko, A. B. and Arapan, S. and Martonak, R. and Rosengren, A.},
	month = feb,
	year = {2010},
	pages = {054110},
	file = {Belonoshko et al. - 2010 - MgO phase diagram from first principles in a wide .pdf:/Users/dong2j/Zotero/storage/DWGXJ6T3/Belonoshko et al. - 2010 - MgO phase diagram from first principles in a wide .pdf:application/pdf},
}

@article{boates_demixing_2013,
	title = {Demixing {Instability} in {Dense} {Molten} {MgSiO} 3 and the {Phase} {Diagram} of {MgO}},
	volume = {110},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.135504},
	doi = {10.1103/PhysRevLett.110.135504},
	language = {en},
	number = {13},
	urldate = {2024-01-01},
	journal = {Physical Review Letters},
	author = {Boates, Brian and Bonev, Stanimir A.},
	month = mar,
	year = {2013},
	pages = {135504},
	file = {Boates and Bonev - 2013 - Demixing Instability in Dense Molten MgSiO 3 and t.pdf:/Users/dong2j/Zotero/storage/TYVU6KWK/Boates and Bonev - 2013 - Demixing Instability in Dense Molten MgSiO 3 and t.pdf:application/pdf},
}

@article{cebulla_ab_2014,
	title = {\textit{{Ab} initio} simulations of {MgO} under extreme conditions},
	volume = {89},
	issn = {1098-0121, 1550-235X},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.89.134107},
	doi = {10.1103/PhysRevB.89.134107},
	language = {en},
	number = {13},
	urldate = {2024-01-01},
	journal = {Physical Review B},
	author = {Cebulla, Daniel and Redmer, Ronald},
	month = apr,
	year = {2014},
	pages = {134107},
	file = {Cebulla and Redmer - 2014 - Ab initio simulations of MgO under extreme .pdf:/Users/dong2j/Zotero/storage/XVPAA457/Cebulla and Redmer - 2014 - Ab initio simulations of MgO under extreme .pdf:application/pdf},
}

@article{root_shock_2015,
	title = {Shock {Response} and {Phase} {Transitions} of {MgO} at {Planetary} {Impact} {Conditions}},
	volume = {115},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.198501},
	doi = {10.1103/PhysRevLett.115.198501},
	language = {en},
	number = {19},
	urldate = {2024-01-01},
	journal = {Physical Review Letters},
	author = {Root, Seth and Shulenburger, Luke and Lemke, Raymond W. and Dolan, Daniel H. and Mattsson, Thomas R. and Desjarlais, Michael P.},
	month = nov,
	year = {2015},
	pages = {198501},
	file = {Root et al. - 2015 - Shock Response and Phase Transitions of MgO at Pla.pdf:/Users/dong2j/Zotero/storage/AJZZCUF2/Root et al. - 2015 - Shock Response and Phase Transitions of MgO at Pla.pdf:application/pdf},
}

%% Fe %%

@article{williams_melting_1987,
	title = {The {Melting} {Curve} of {Iron} to 250 {Gigapascals}: {A} {Constraint} on the {Temperature} at {Earth}'s {Center}},
	language = {en},
	journal = {Science},
	author = {Williams, Quentin and Jeanloz, Raymond and Bass, Jay and Svendsen, Bob and Ahrens, Thomas J},
	year = {1987},
	file = {Williams et al. - The Melting Curve of Iron to 250 Gigapascals A Co.pdf:/Users/dong2j/Zotero/storage/FVT4LCY3/Williams et al. - The Melting Curve of Iron to 250 Gigapascals A Co.pdf:application/pdf},
}
@article{anzellini_melting_2013,
	title = {Melting of {Iron} at {Earth}’s {Inner} {Core} {Boundary} {Based} on {Fast} {X}-ray {Diffraction}},
	volume = {340},
	issn = {0036-8075, 1095-9203},
	url = {https://www.science.org/doi/10.1126/science.1233514},
	doi = {10.1126/science.1233514},
	abstract = {Hot Enough to Melt Iron
            
              Earth's core is divided into a fluid outer core and a solid inner core, both composed predominately of iron at extremely high pressures and temperatures. The boundary between these two regions is largely controlled by the melting point of iron at ∼330 GPa, which in turn influences heat transfer and geodynamo generation.
              
                Anzellini
                et al.
              
              (p.
              464
              , see the Perspective by
              Fei
              ) compressed iron in a laser-heated diamond anvil cell, tracking its structure and texture by using time-resolved x-ray diffraction as the pressure increased to 200 GPa. The melting curve suggests the possibility of high heat flux and partial melting at the core-mantle boundary.
            
          , 
            
              High-temperature and -pressure experiments simulate the melting behavior of metallic iron in Earth’s core.
              
                [Also see Perspective by
                Fei
                ]
              
            
          , 
            
              Earth’s core is structured in a solid inner core, mainly composed of iron, and a liquid outer core. The temperature at the inner core boundary is expected to be close to the melting point of iron at 330 gigapascal (GPa). Despite intensive experimental and theoretical efforts, there is little consensus on the melting behavior of iron at these extreme pressures and temperatures. We present static laser-heated diamond anvil cell experiments up to 200 GPa using synchrotron-based fast x-ray diffraction as a primary melting diagnostic. When extrapolating to higher pressures, we conclude that the melting temperature of iron at the inner core boundary is 6230
              ±
              500 kelvin. This estimation favors a high heat flux at the core-mantle boundary with a possible partial melting of the mantle.},
	language = {en},
	number = {6131},
	urldate = {2024-01-03},
	journal = {Science},
	author = {Anzellini, S. and Dewaele, A. and Mezouar, M. and Loubeyre, P. and Morard, G.},
	month = apr,
	year = {2013},
	pages = {464--466},
	file = {Anzellini et al. - 2013 - Melting of Iron at Earth’s Inner Core Boundary Bas.pdf:/Users/dong2j/Zotero/storage/SARSSMRB/Anzellini et al. - 2013 - Melting of Iron at Earth’s Inner Core Boundary Bas.pdf:application/pdf},
}

@article{aquilanti_melting_2015,
	title = {Melting of iron determined by {X}-ray absorption spectroscopy to 100 {GPa}},
	volume = {112},
	issn = {0027-8424, 1091-6490},
	url = {https://pnas.org/doi/full/10.1073/pnas.1502363112},
	doi = {10.1073/pnas.1502363112},
	abstract = {Significance
            There is a long-standing controversy over the melting curve of Fe at high pressure as determined from static laser heated diamond anvil cell and dynamic compression studies. X-ray absorption spectroscopy measurements are used here as a criterion to detect melting under pressure. Confronted with a diversity of obtained melting curves, this technique, used at such pressure and temperature conditions, is eligible to be at the forefront to probe Earth's deep interior. Furthermore, the experiment reported here holds promise for addressing important issues related to the structure and phase diagram of compressed melts, such as the existence of structural complexity (polyamorphism) in the liquid phase or the extent of icosahedral ordering whose investigation has been limited until now to ambient conditions.
          , 
            Temperature, thermal history, and dynamics of Earth rely critically on the knowledge of the melting temperature of iron at the pressure conditions of the inner core boundary (ICB) where the geotherm crosses the melting curve. The literature on this subject is overwhelming, and no consensus has been reached, with a very large disagreement of the order of 2,000 K for the ICB temperature. Here we report new data on the melting temperature of iron in a laser-heated diamond anvil cell to 103 GPa obtained by X-ray absorption spectroscopy, a technique rarely used at such conditions. The modifications of the onset of the absorption spectra are used as a reliable melting criterion regardless of the solid phase from which the solid to liquid transition takes place. Our results show a melting temperature of iron in agreement with most previous studies up to 100 GPa, namely of 3,090 K at 103 GPa.},
	language = {en},
	number = {39},
	urldate = {2024-01-03},
	journal = {Proceedings of the National Academy of Sciences},
	author = {Aquilanti, Giuliana and Trapananti, Angela and Karandikar, Amol and Kantor, Innokenty and Marini, Carlo and Mathon, Olivier and Pascarelli, Sakura and Boehler, Reinhard},
	month = sep,
	year = {2015},
	pages = {12042--12045},
	file = {Aquilanti et al. - 2015 - Melting of iron determined by X-ray absorption spe.pdf:/Users/dong2j/Zotero/storage/A7I3QXQR/Aquilanti et al. - 2015 - Melting of iron determined by X-ray absorption spe.pdf:application/pdf},
}

@article{assael_reference_2006,
	title = {Reference {Data} for the {Density} and {Viscosity} of {Liquid} {Aluminum} and {Liquid} {Iron}},
	volume = {35},
	language = {en},
	number = {1},
	journal = {J. Phys. Chem. Ref. Data},
	author = {Assael, Marc J and Kakosimos, Konstantinos},
	year = {2006},
	file = {Assael and Kakosimos - 2006 - Reference Data for the Density and Viscosity of Li.pdf:/Users/dong2j/Zotero/storage/2W5LFICM/Assael and Kakosimos - 2006 - Reference Data for the Density and Viscosity of Li.pdf:application/pdf},
}

@incollection{manghnani_internally-heated_1987,
	address = {Washington, D. C.},
	title = {Internally-heated diamond-anvil cell: {Phase} diagram and {P}-{V}-{T} of iron},
	volume = {39},
	isbn = {978-0-87590-066-7},
	shorttitle = {Internally-heated diamond-anvil cell},
	url = {http://doi.wiley.com/10.1029/GM039p0173},
	abstract = {In situ pressuret,emperature,and resistancemeasurements of resistivelyheatediron wiresin gasketeddiamond-anvil cellsare used to locate solid-solid and solid-liquid phase transitions with high accuracy.Pressuresaredeterminedby usingthe ruby pressurescaleand temperatures are measured by fitting a blackbody function to the spectrumof thehot wiretakenwith an opticalmultichannelanalyzer.In this mannerthe ct-7 transition line hasbeenmeasuredto 29 GPa. With a synchrotron X-ray source and resistivelyheated wires the powder diffractionpatternsof ct-,?-, andc-Fe havebeenobtainedat pressures between7 and 16GPa andtemperaturesashighas 1000K. The average volumethermal expansivityof ct-Febetween300 and 815 K at 9.5 GPa hasbeenfound to be 14+4X 10-6 K-• or about one-third of the value at atmosphericpressure.Preliminary data for ?-Fe indicatethat the molar volume decreasesby 6\% along the ct-7 transition line betweenatmosphericpressureand 9.5 GPa.},
	language = {en},
	urldate = {2024-01-03},
	booktitle = {Geophysical {Monograph} {Series}},
	publisher = {American Geophysical Union},
	author = {Boehler, R. and Nicol, M. and Johnson, M. L.},
	editor = {Manghnani, Murli H. and Syono, Yasuhiko},
	year = {1987},
	doi = {10.1029/GM039p0173},
	pages = {173--176},
	file = {Boehler et al. - 1987 - Internally-heated diamond-anvil cell Phase diagra.pdf:/Users/dong2j/Zotero/storage/K6JWIFSY/Boehler et al. - 1987 - Internally-heated diamond-anvil cell Phase diagra.pdf:application/pdf},
}

@article{boehler_melting_1990,
	title = {Melting, thermal expansion, and phase transitions of iron at high pressures},
	volume = {95},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/JB095iB13p21731},
	doi = {10.1029/JB095iB13p21731},
	abstract = {The melting curve of iron to 1.2 Mbar was remeasured in a laser‐heated diamond anvil cell. A defocused 35 W Nd∶YAG laser beam provided low‐temperature gradients which were measured within an area of 2 μm in diameter with a chromatically corrected optical geometry. Argon to 350 kbar and A1
              2
              O
              3
              to 1.2 Mbar were used as pressure media. Melting was detected by in situ measurements of optical reflectivity and electrical resistivity and by visual observation of the surface texture. At 1.2 Mbar, iron melts at 3000 ± 100 K. The same laser‐heating technique was used to measure volumes of fcc‐(γ)‐iron to 168 kbar and 2000 K using synchrotron radiation, leading to a decrease in the thermal expansion coefficient of γ‐iron represented by (∂ In α/∂ In
              V
              )
              T
              = 6.5±0.5. The α‐ε transition of iron has been studied by X ray and by the change in resistivity of a fine wire using a variety of pressure media. The hysteresis of the transition changes systematically with the shear strength of the pressure medium with an equilibrium transition pressure at 130±10 kbar.},
	language = {en},
	number = {B13},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Boehler, R. and Von Bargen, N. and Chopelas, A.},
	month = dec,
	year = {1990},
	pages = {21731--21736},
	file = {Boehler et al. - 1990 - Melting, thermal expansion, and phase transitions .pdf:/Users/dong2j/Zotero/storage/B7NNFH34/Boehler et al. - 1990 - Melting, thermal expansion, and phase transitions .pdf:application/pdf},
}

@article{boehler_temperatures_1993,
	title = {Temperatures in the {Earth}'s core from melting-point measurements of iron at high static pressures},
	volume = {363},
	issn = {0028-0836, 1476-4687},
	url = {https://www.nature.com/articles/363534a0},
	doi = {10.1038/363534a0},
	language = {en},
	number = {6429},
	urldate = {2024-01-03},
	journal = {Nature},
	author = {Boehler, R.},
	month = jun,
	year = {1993},
	pages = {534--536},
	file = {Boehler - 1993 - Temperatures in the Earth's core from melting-poin.pdf:/Users/dong2j/Zotero/storage/TV892H4B/Boehler - 1993 - Temperatures in the Earth's core from melting-poin.pdf:application/pdf},
}

@article{bundy_pressuretemperature_1965,
	title = {Pressure—{Temperature} {Phase} {Diagram} of {Iron} to 200 kbar, 900°{C}},
	volume = {36},
	issn = {0021-8979, 1089-7550},
	url = {https://pubs.aip.org/jap/article/36/2/616/347231/Pressure-Temperature-Phase-Diagram-of-Iron-to-200},
	doi = {10.1063/1.1714038},
	abstract = {The resistance changes in iron during the transitions between the α(bcc), γ(fcc), and ε(hcp) phases have been studied quantitatively in the high-compression belt apparatus. The samples were monitored by thermocouples and voltage probes. The P,T locations of the (α,γ) (α,ε), and (ε,γ) phase lines, and the (α,γ,ε) triple point were determined. The latter is placed at 110 ±3 kbar and 490 ±10°C. The changes of molar volume at the triple point are deduced to be −0.275, +0.135, and +0.140 cc/mole for the (α,ε), (ε,γ), and (γ,α) transitions, respectively. The resistivity of the α phase follows a quadratic relationship with temperature, whereas the γ and ε forms vary linearly with temperature.},
	language = {en},
	number = {2},
	urldate = {2024-01-03},
	journal = {Journal of Applied Physics},
	author = {Bundy, F. P.},
	month = feb,
	year = {1965},
	pages = {616--620},
	file = {Bundy - 1965 - Pressure—Temperature Phase Diagram of Iron to 200 .pdf:/Users/dong2j/Zotero/storage/R2QFI64K/Bundy - 1965 - Pressure—Temperature Phase Diagram of Iron to 200 .pdf:application/pdf},
}

@article{claussen_detection_1960,
	title = {Detection of the α-γ {Iron} {Phase} {Transformation} by {Differential} {Thermal} {Conductivity} {Analysis}},
	volume = {31},
	issn = {0034-6748, 1089-7623},
	url = {https://pubs.aip.org/rsi/article/31/8/878/300510/Detection-of-the-Iron-Phase-Transformation-by},
	doi = {10.1063/1.1717076},
	abstract = {A method of phase change detection in solids involving differential thermal conductivity analysis is described. This method is applied to the α-γ transformation of iron at various pressures up to 100 000 atm. This transformation temperature was found to drop continuously with increasing pressure down to 605°C at 100 000 atm.},
	language = {en},
	number = {8},
	urldate = {2024-01-03},
	journal = {Review of Scientific Instruments},
	author = {Claussen, Walter F.},
	month = aug,
	year = {1960},
	pages = {878--881},
	file = {Claussen - 1960 - Detection of the α-γ Iron Phase Transformation by .pdf:/Users/dong2j/Zotero/storage/YQ5NNP99/Claussen - 1960 - Detection of the α-γ Iron Phase Transformation by .pdf:application/pdf},
}

@article{clendenen_effect_1964,
	title = {The effect of pressure on the volume and lattice parameters of ruthenium and iron},
	volume = {25},
	issn = {00223697},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0022369764900988},
	doi = {10.1016/0022-3697(64)90098-8},
	abstract = {The volume changes and lattice parameters of ruthenium and iron have been measured to 400 kbars pressure. The compressibility of ruthenium is comparable to that of rhodium and molybdenum. c/a decreases slightly at low pressures and then increases rapidly to the highest pressures obtained.},
	language = {en},
	number = {8},
	urldate = {2024-01-03},
	journal = {Journal of Physics and Chemistry of Solids},
	author = {Clendenen, R.L. and Drickamer, H.G.},
	month = aug,
	year = {1964},
	pages = {865--868},
	file = {Clendenen and Drickamer - 1964 - The effect of pressure on the volume and lattice p.pdf:/Users/dong2j/Zotero/storage/MLVAL284/Clendenen and Drickamer - 1964 - The effect of pressure on the volume and lattice p.pdf:application/pdf},
}

@article{kaufman_lattice_1963,
	title = {The lattice stability of metals—{III}. {Iron}},
	volume = {11},
	issn = {00016160},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0001616063901573},
	doi = {10.1016/0001-6160(63)90157-3},
	language = {en},
	number = {5},
	urldate = {2024-01-03},
	journal = {Acta Metallurgica},
	author = {Kaufman, Larry and Clougherty, E.V and Weiss, R.J},
	month = may,
	year = {1963},
	pages = {323--335},
	file = {Kaufman et al. - 1963 - The lattice stability of metals—III. Iron.pdf:/Users/dong2j/Zotero/storage/KAUGDPBN/Kaufman et al. - 1963 - The lattice stability of metals—III. Iron.pdf:application/pdf},
}

@article{deng_high_2013,
	title = {High pressure and temperature electrical resistivity of iron and implications for planetary cores},
	volume = {40},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2012GL054347},
	doi = {10.1029/2012GL054347},
	abstract = {Electrical resistivity measurements of polycrystalline iron have been performed at 5, 7, and 15 GPa and in the temperature range 293–2200 K by employing a four‐wired method. The kinks in electrical resistivity associated with solid iron phase transitions and the solid to liquid transition were clearly observed upon increasing temperature. Geometry corrections due to volume variations with pressure and temperature were applied to the entire data set. High pressure and temperature thermal conductivity were calculated by fitting resistivity data through the Wiedemann‐Franz law. The temperature dependences of electrical resistivity and thermal conductivity for α, γ, and ε solid iron have been determined at high‐pressure conditions. Our study provides the first experimental constraint on the heat flux conducted at Mercury's outmost core, estimated to be 0.29–0.36 TW, assuming an adiabatic core. Extrapolations of our data to Martian outer core conditions yield a series of heat transport parameters (e.g., electrical resistivity, thermal conductivity, and heat flux), which are in reasonable comparison with various geophysical estimates.
          , 
            Key Points
            
              
                
                  High pressure and temperature electrical resistance of Fe were measured
                
                
                  Temperature dependences of thermal conductivity of Fe were determined
                
                
                  Heat flux conducted at Mercury's and Martian outmost core were estimated},
	language = {en},
	number = {1},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Deng, Liwei and Seagle, Christopher and Fei, Yingwei and Shahar, Anat},
	month = jan,
	year = {2013},
	pages = {33--37},
	file = {Deng et al. - 2013 - High pressure and temperature electrical resistivi.pdf:/Users/dong2j/Zotero/storage/K9293XTL/Deng et al. - 2013 - High pressure and temperature electrical resistivi.pdf:application/pdf},
}

@article{dubrovinsky_high-pressure_1998,
	title = {High-pressure and high-temperature in situ {X}-ray diffraction study of iron and corundum to 68 {GPa} using an internally heated diamond anvil cell},
	volume = {25},
	issn = {0342-1791, 1432-2021},
	url = {http://link.springer.com/10.1007/s002690050133},
	doi = {10.1007/s002690050133},
	language = {en},
	number = {6},
	urldate = {2024-01-03},
	journal = {Physics and Chemistry of Minerals},
	author = {Dubrovinsky, Leonid S. and Saxena, Surendra K. and Lazor, Peter},
	month = jun,
	year = {1998},
	pages = {434--441},
	file = {Dubrovinsky et al. - 1998 - High-pressure and high-temperature in situ X-ray d.pdf:/Users/dong2j/Zotero/storage/QMIKUU59/Dubrovinsky et al. - 1998 - High-pressure and high-temperature in situ X-ray d.pdf:application/pdf},
}

@article{giles_high-pressure_1971,
	title = {High-{Pressure} α⇄ε {Martensitic} {Transformation} in {Iron}},
	volume = {42},
	issn = {0021-8979, 1089-7550},
	url = {https://pubs.aip.org/jap/article/42/11/4290/4618/High-Pressure-Martensitic-Transformation-in-Iron},
	doi = {10.1063/1.1659768},
	abstract = {A study of the high-pressure transformation in iron using an opposed-anvil x-ray diffraction apparatus and high-pressure light metallography has shown that the 130-kbar transformation is martensitic. The bcc and hcp phases were found to coexist over a large pressure range, and there is a large hysteresis between the forward and reverse transformation-start pressures. A room-temperature equilibrium pressure for the bcc and hcp phases of 107 ± 8 kbar is proposed, and discrepancies in the current P-T equilibrium diagram for iron are discussed.},
	language = {en},
	number = {11},
	urldate = {2024-01-03},
	journal = {Journal of Applied Physics},
	author = {Giles, P. M. and Longenbach, M. H. and Marder, A. R.},
	month = oct,
	year = {1971},
	pages = {4290--4295},
	file = {Giles et al. - 1971 - High-Pressure α⇄ε Martensitic Transformation in Ir.pdf:/Users/dong2j/Zotero/storage/BFPEPBMI/Giles et al. - 1971 - High-Pressure α⇄ε Martensitic Transformation in Ir.pdf:application/pdf},
}

@article{hou_melting_2021,
	title = {Melting of {Iron} {Explored} by {Electrical} {Resistance} {Jump} up to 135 {GPa}},
	volume = {48},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2021GL095739},
	doi = {10.1029/2021GL095739},
	abstract = {The melting temperature (Tm) of iron at megabar pressures constrains the Earth's core temperature structure and dynamics. Previous experimental studies demonstrated large discrepancies in Tm at high pressures. We used the intrinsic resistance discontinuity across solid-liquid transition as a melting criterion to study the melting behavior of iron in laser-heated diamond anvil cells. The resistance jump is sensitive to the incipient melting, capable of detecting the emergence of less than 2 vol.\% melts. We found a high melting curve of iron at 30–135 GPa, but a relatively low-transition temperature of the slow-fast recrystallization. The determined Tm of iron is 4306(±300) K at the core-mantle boundary (CMB) pressure in good agreement with the static and shockwave experimental results by Anzellini et al. (2013, https://doi.org/10.1126/science.1233514) and Li et al. (2020, https://doi.org/10.1029/2020gl087758). The high melting point of iron implies a high and steep geothermal gradient and influences a heat flow across the CMB.},
	language = {en},
	number = {20},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Hou, Mingqiang and Liu, Jin and Zhang, Youjun and Du, Xueyan and Dong, Hongliang and Yan, Limin and Wang, Junyue and Wang, Lin and Chen, Bin},
	month = oct,
	year = {2021},
	pages = {e2021GL095739},
	file = {Hou et al. - 2021 - Melting of Iron Explored by Electrical Resistance .pdf:/Users/dong2j/Zotero/storage/G6AH5V68/Hou et al. - 2021 - Melting of Iron Explored by Electrical Resistance .pdf:application/pdf},
}

@article{jackson_melting_2013,
	title = {Melting of compressed iron by monitoring atomic dynamics},
	volume = {362},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X12006747},
	doi = {10.1016/j.epsl.2012.11.048},
	abstract = {We present a novel method for detecting the solid–liquid phase boundary of compressed iron at high temperatures using synchrotron Mo¨ ssbauer spectroscopy (SMS). Our approach is unique because the dynamics of the iron atoms are monitored. This process is described by the Lamb–Mo¨ ssbauer factor, which is related to the mean-square displacement of the iron atoms. Focused synchrotron radiation with 1 meV bandwidth passes through a laser-heated 57Fe sample inside a diamond-anvil cell, and the characteristic SMS time signature vanishes when melting occurs. At our highest compression measurement and considering thermal pressure, we ﬁnd the melting point of iron to be TM ¼30257 115 K at P ¼ 827 5 GPa. When compared with previously reported melting points for iron using static compression methods with different criteria for melting, our melting trend deﬁnes a steeper positive slope as a function of pressure. The obtained melting temperatures represent a signiﬁcant step toward a reliable melting curve of iron at Earth’s core conditions. For other terrestrial planets possessing cores with liquid portions rich in metallic iron, such as Mercury and Mars, the higher melting temperatures for compressed iron may imply warmer internal temperatures.},
	language = {en},
	urldate = {2024-01-03},
	journal = {Earth and Planetary Science Letters},
	author = {Jackson, Jennifer M. and Sturhahn, Wolfgang and Lerche, Michael and Zhao, Jiyong and Toellner, Thomas S. and Alp, E. Ercan and Sinogeikin, Stanislav V. and Bass, Jay D. and Murphy, Caitlin A. and Wicks, June K.},
	month = jan,
	year = {2013},
	pages = {143--150},
	file = {Jackson et al. - 2013 - Melting of compressed iron by monitoring atomic dy.pdf:/Users/dong2j/Zotero/storage/ZG4JJ454/Jackson et al. - 2013 - Melting of compressed iron by monitoring atomic dy.pdf:application/pdf},
}

@article{johnson_temperature_1962,
	title = {Temperature {Dependence} of {Shock}-{Induced} {Phase} {Transformations} in {Iron}},
	volume = {33},
	issn = {0021-8979, 1089-7550},
	url = {https://pubs.aip.org/jap/article/33/2/557/320852/Temperature-Dependence-of-Shock-Induced-Phase},
	doi = {10.1063/1.1702465},
	abstract = {Shock-induced phase transformations in iron have been investigated in the temperature range 78° to 1158°K. The pressure for transformation over this temperature range has been determined by a technique that depends on microstructural changes associated with a phase transformation. A discontinuity in the temperature-pressure relationship was observed at 115 kbars and 775°K. Two distinct transformation microstructures were observed. It is postulated that the results obtained above 775°K are due to the expected transformation from alpha iron to gamma iron whereas the results below 775°K are related to a transformation from alpha iron to a presently undetermined new phase.},
	language = {en},
	number = {2},
	urldate = {2024-01-03},
	journal = {Journal of Applied Physics},
	author = {Johnson, P. C. and Stein, B. A. and Davis, R. S.},
	month = feb,
	year = {1962},
	pages = {557--561},
	file = {Johnson et al. - 1962 - Temperature Dependence of Shock-Induced Phase Tran.pdf:/Users/dong2j/Zotero/storage/K47EIBIL/Johnson et al. - 1962 - Temperature Dependence of Shock-Induced Phase Tran.pdf:application/pdf},
}

@article{komabayashi_-situ_2009,
	title = {In-situ {X}-ray diffraction measurements of the γ-ε transition boundary of iron in an internally-heated diamond anvil cell},
	volume = {282},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X09001678},
	doi = {10.1016/j.epsl.2009.03.025},
	abstract = {The phase transition boundary between the γ (face-centered cubic structure) and ε (hexagonal close-packed structure) iron phases was determined up to 69 GPa by using a newly developed internally-heated diamond anvil cell, combined with in-situ synchrotron X-ray diffraction measurements. The improved experimental conﬁguration provides stable heating with reliable temperature and pressure determination and phase identiﬁcation. A simultaneous laser- and internal-heating system was also used to produce further higher temperature at higher pressures. The sample pressure at any given temperature was calculated using an established thermal equation of state for ε iron. The γ-ε transition boundary was bracketed with the normal and reversal directions and it is linear from 21 to 69 GPa with a dP/dT slope of 0.0394 GPa/K. There is no evidence for the existence of additional iron solid phase other than the γ and ε phases over the P–T range of this study. We inferred that the γ-ε-liquid triple point of iron should occur at 88 GPa and 2800 K.},
	language = {en},
	number = {1-4},
	urldate = {2024-01-03},
	journal = {Earth and Planetary Science Letters},
	author = {Komabayashi, Tetsuya and Fei, Yingwei and Meng, Yue and Prakapenka, Vitali},
	month = may,
	year = {2009},
	pages = {252--257},
	file = {Komabayashi et al. - 2009 - In-situ X-ray diffraction measurements of the γ-ε .pdf:/Users/dong2j/Zotero/storage/RCLGVHLG/Komabayashi et al. - 2009 - In-situ X-ray diffraction measurements of the γ-ε .pdf:application/pdf},
}

@article{kono_high-pressure_2015,
	title = {High-pressure viscosity of liquid {Fe} and {FeS} revisited by falling sphere viscometry using ultrafast {X}-ray imaging},
	volume = {241},
	issn = {00319201},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0031920115000229},
	doi = {10.1016/j.pepi.2015.02.006},
	abstract = {The viscosity of liquid Fe and FeS has been extensively studied, yielding results differing by almost a factor of ten (2.4–23.7 mPa s for liquid Fe, 3.6–17.9 mPa s for liquid FeS, and 7.4–35.6 mPa s for the Fe–S eutectic composition), possibly due to the low resolution of slow cameras previously employed (typically 30–60 frames/s) in falling sphere measurements using X-ray radiography. Here we revisit the viscosity of liquid Fe and FeS up to 6.4 GPa using recently developed ultrafast X-ray imaging. In this study, we imaged the falling spheres at a rate of 500 frames/s, which is around 10 times faster than previous viscosity measurements. Our measurements showed that terminal velocity is achieved only in a limited region of falling distance, and that substantial oversampling, using sufﬁciently high-speed X-ray imaging, is essential to accurately determine the terminal velocity and the resulting viscosity. We obtained a viscosity of 6.1–7.4 mPa s for liquid Fe and 4.7–5.7 mPa s for liquid FeS at pressures to 6.4 GPa along their respective melting curves. The viscosity of liquid FeS is about 25–35\% lower than that of liquid Fe between around 2 and 6.4 GPa along their respective melting curves. After correction for the effect of different melting temperatures between Fe and FeS on viscosity, we found that viscosity of liquid FeS is 31–42\% lower than that of liquid Fe at 1800 °C and 1–6 GPa, suggesting that sulfur markedly decreases viscosity in liquid Fe.},
	language = {en},
	urldate = {2024-01-03},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Kono, Yoshio and Kenney-Benson, Curtis and Shibazaki, Yuki and Park, Changyong and Shen, Guoyin and Wang, Yanbin},
	month = apr,
	year = {2015},
	pages = {57--64},
	file = {Kono et al. - 2015 - High-pressure viscosity of liquid Fe and FeS revis.pdf:/Users/dong2j/Zotero/storage/RPVW8VGQ/Kono et al. - 2015 - High-pressure viscosity of liquid Fe and FeS revis.pdf:application/pdf},
}

@article{konopkova_thermal_2011,
	title = {Thermal conductivity of hcp iron at high pressure and temperature},
	volume = {31},
	issn = {0895-7959, 1477-2299},
	url = {http://www.tandfonline.com/doi/abs/10.1080/08957959.2010.545059},
	doi = {10.1080/08957959.2010.545059},
	language = {en},
	number = {1},
	urldate = {2024-01-03},
	journal = {High Pressure Research},
	author = {Konôpková, Z. and Lazor, P. and Goncharov, A. F. and Struzhkin, V. V.},
	month = mar,
	year = {2011},
	pages = {228--236},
	file = {Konôpková et al. - 2011 - Thermal conductivity of hcp iron at high pressure .pdf:/Users/dong2j/Zotero/storage/C5FURYGD/Konôpková et al. - 2011 - Thermal conductivity of hcp iron at high pressure .pdf:application/pdf},
}

@article{kraus_measuring_2022,
	title = {Measuring the melting curve of iron at super-{Earth} core conditions},
	volume = {375},
	issn = {0036-8075, 1095-9203},
	url = {https://www.science.org/doi/10.1126/science.abm1472},
	doi = {10.1126/science.abm1472},
	abstract = {Terapascal iron-melting temperature
            
              The pressure and temperature conditions at which iron melts are important for terrestrial planets because they determine the size of the liquid metal core, an important factor for understanding the potential for generating a radiation-shielding magnetic field. Kraus
              et al
              . used laser-driven shock to determine the iron-melt curve up to a pressure of 1000 gigapascals (see the Perspective by Zhang and Lin). This value is about three times that of the Earth’s inner core boundary. The authors found that the liquid metal core lasted the longest for Earth-like planets four to six times larger in mass than the Earth. —BG
            
          , 
            Experiments constrain the occurrence and longevity of protective magnetodynamos in super-Earth exoplanets.
          , 
            The discovery of more than 4500 extrasolar planets has created a need for modeling their interior structure and dynamics. Given the prominence of iron in planetary interiors, we require accurate and precise physical properties at extreme pressure and temperature. A first-order property of iron is its melting point, which is still debated for the conditions of Earth’s interior. We used high-energy lasers at the National Ignition Facility and in situ x-ray diffraction to determine the melting point of iron up to 1000 gigapascals, three times the pressure of Earth’s inner core. We used this melting curve to determine the length of dynamo action during core solidification to the hexagonal close-packed (hcp) structure. We find that terrestrial exoplanets with four to six times Earth’s mass have the longest dynamos, which provide important shielding against cosmic radiation.},
	language = {en},
	number = {6577},
	urldate = {2024-01-03},
	journal = {Science},
	author = {Kraus, Richard G. and Hemley, Russell J. and Ali, Suzanne J. and Belof, Jonathan L. and Benedict, Lorin X. and Bernier, Joel and Braun, Dave and Cohen, R. E. and Collins, Gilbert W. and Coppari, Federica and Desjarlais, Michael P. and Fratanduono, Dayne and Hamel, Sebastien and Krygier, Andy and Lazicki, Amy and Mcnaney, James and Millot, Marius and Myint, Philip C. and Newman, Matthew G. and Rygg, James R. and Sterbentz, Dane M. and Stewart, Sarah T. and Stixrude, Lars and Swift, Damian C. and Wehrenberg, Chris and Eggert, Jon H.},
	month = jan,
	year = {2022},
	pages = {202--205},
	file = {Kraus et al. - 2022 - Measuring the melting curve of iron at super-Earth.pdf:/Users/dong2j/Zotero/storage/FH664TMN/Kraus et al. - 2022 - Measuring the melting curve of iron at super-Earth.pdf:application/pdf},
}

@article{kuwayama_phase_2008,
	title = {Phase relations of iron and iron–nickel alloys up to 300 {GPa}: {Implications} for composition and structure of the {Earth}'s inner core},
	volume = {273},
	issn = {0012821X},
	shorttitle = {Phase relations of iron and iron–nickel alloys up to 300 {GPa}},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X08004287},
	doi = {10.1016/j.epsl.2008.07.001},
	abstract = {We have investigated the phase relations of iron and iron–nickel alloys with 18 to 50 wt.\% Ni up to over 300 GPa using a laser-heated diamond-anvil cell. The synchrotron X-ray diffraction measurements show the wide stability of hcp-iron up to 301 GPa and 2000 K and 319 GPa and 300 K without phase transition to dhcp, orthorhombic, or bcc phases. On the other hand, the incorporation of nickel has a remarkable effect on expanding the stability ﬁeld of fcc phase. The geometry of the temperature–composition phase diagram of iron–nickel alloys suggests that the hcp–fcc–liquid triple point is located at 10 to 20 wt.\% Ni at the pressure of the inner core boundary. The fcc phase could crystallize depending on the nickel and silicon contents in the Earth's core, both of which are fcc stabilizer.},
	language = {en},
	number = {3-4},
	urldate = {2024-01-03},
	journal = {Earth and Planetary Science Letters},
	author = {Kuwayama, Yasuhiro and Hirose, Kei and Sata, Nagayoshi and Ohishi, Yasuo},
	month = sep,
	year = {2008},
	pages = {379--385},
	file = {Kuwayama et al. - 2008 - Phase relations of iron and iron–nickel alloys up .pdf:/Users/dong2j/Zotero/storage/NKWKVR4S/Kuwayama et al. - 2008 - Phase relations of iron and iron–nickel alloys up .pdf:application/pdf},
}

@article{kuwayama_equation_2020,
	title = {Equation of {State} of {Liquid} {Iron} under {Extreme} {Conditions}},
	volume = {124},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.124.165701},
	doi = {10.1103/PhysRevLett.124.165701},
	language = {en},
	number = {16},
	urldate = {2024-01-03},
	journal = {Physical Review Letters},
	author = {Kuwayama, Yasuhiro and Morard, Guillaume and Nakajima, Yoichi and Hirose, Kei and Baron, Alfred Q. R. and Kawaguchi, Saori I. and Tsuchiya, Taku and Ishikawa, Daisuke and Hirao, Naohisa and Ohishi, Yasuo},
	month = apr,
	year = {2020},
	pages = {165701},
	file = {Kuwayama et al. - 2020 - Equation of State of Liquid Iron under Extreme Con.pdf:/Users/dong2j/Zotero/storage/D9XV49FP/Kuwayama et al. - 2020 - Equation of State of Liquid Iron under Extreme Con.pdf:application/pdf},
}

@article{li_shock_2020,
	title = {Shock {Melting} {Curve} of {Iron}: {A} {Consensus} on the {Temperature} at the {Earth}'s {Inner} {Core} {Boundary}},
	volume = {47},
	issn = {0094-8276, 1944-8007},
	shorttitle = {Shock {Melting} {Curve} of {Iron}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2020GL087758},
	doi = {10.1029/2020GL087758},
	abstract = {The Earth's core consists of iron as the major component. The melting point of iron at the inner core boundary constrains the thermal structure and solidiﬁcation of the Earth's core. However, the current estimation of the melting temperature of iron under the core conditions has signiﬁcant variations. Here, we measured the temperatures of iron shocked up to {\textasciitilde}256 GPa using precise pyrometer and velocimeter diagnostics via a two‐stage light‐gas gun. Our results indicated that the melting temperatures of iron at the core‐mantle and inner core boundaries are 4300(250) and 5950(400) K, respectively. These temperatures are signiﬁcantly lower than some previous shock experiments but are overall consistent with the recent results determined by fast X‐ray diffraction techniques, X‐ray absorption experiments in laser‐heated diamond anvil cells, and by ab initio computations. Our iron melting curve indicates a relatively small Clapeyron slope and supports thermal models for a young inner core. Plain Language Summary Iron is the main constituent of the Earth's core, so its melting characteristics at high pressures are fundamentally crucial for understanding the thermal structure, solidiﬁcation, and evolution of the core. We determined shock temperatures of melted iron up to {\textasciitilde}256 GPa precisely by the use of a time‐resolved quasi‐spectral optical pyrometer. Our results are 1000–2000 K lower than those of some previous shock experiments. Our study reconciles the previous discrepancy in the melting temperatures of iron at pressures of 200–300 GPa and is consistent with theoretical calculations. We conclude that the melting temperature of iron at the Earth's inner core boundary is {\textasciitilde}5950(400) K. The present study indicates a relatively gentle melting slope of iron and supports a young inner core age of {\textasciitilde}0.565 Gyr inferred from paleomagnetic observations.},
	language = {en},
	number = {15},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Li, Jun and Wu, Qiang and Li, Jiabo and Xue, Tao and Tan, Ye and Zhou, Xianming and Zhang, Youjun and Xiong, Zhengwei and Gao, Zhipeng and Sekine, Toshimori},
	month = aug,
	year = {2020},
	pages = {e2020GL087758},
	file = {Li et al. - 2020 - Shock Melting Curve of Iron A Consensus on the Te.pdf:/Users/dong2j/Zotero/storage/24S8L487/Li et al. - 2020 - Shock Melting Curve of Iron A Consensus on the Te.pdf:application/pdf},
}

@article{liu_melting_1975,
	title = {The melting of iron up to 200 kbar},
	volume = {80},
	issn = {01480227},
	url = {http://doi.wiley.com/10.1029/JB080i026p03777},
	doi = {10.1029/JB080i026p03777},
	language = {en},
	number = {26},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research},
	author = {Liu, Lin-Gun and Bassett, William A.},
	month = sep,
	year = {1975},
	pages = {3777--3782},
	file = {Liu and Bassett - 1975 - The melting of iron up to 200 kbar.pdf:/Users/dong2j/Zotero/storage/AA8IL38D/Liu and Bassett - 1975 - The melting of iron up to 200 kbar.pdf:application/pdf},
}

@article{ma_situ_2004,
	title = {In situ {X}-ray diffraction studies of iron to {Earth}-core conditions},
	volume = {143-144},
	issn = {00319201},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0031920104000767},
	doi = {10.1016/j.pepi.2003.06.005},
	abstract = {The high-pressure, high-temperature behavior of iron has been investigated to 161 GPa and 3000 K by in situ synchrotron X-ray diffraction with double-side laser-heated diamond anvil cells. We found that only ␣-, ␥- and ε-Fe can be clearly veriﬁed as the stable solid phase in the P–T range studied. Only ε-Fe is observed from deep lower mantle (∼1500 km) to outer core conditions. Within the P–T range examined, we did not observe a signiﬁcant change with pressure or temperature on the c/a ratio of ε-Fe. The melting curve of iron has been determined to 105 GPa. A Lindeman law ﬁt gives a melting point of iron at the inner core boundary of 5800 (±200) K, which provides an upper bound on the temperature at that depth. We also examine numerous experimental factors that may complicate the analysis of high P–T diffraction data, and discuss the effects of sample stress on the X-ray diffraction results.},
	language = {en},
	urldate = {2024-01-03},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Ma, Yanzhang and Somayazulu, Maddury and Shen, Guoyin and Mao, Ho-kwang and Shu, Jinfu and Hemley, Russell J},
	month = jun,
	year = {2004},
	pages = {455--467},
	file = {Ma et al. - 2004 - In situ X-ray diffraction studies of iron to Earth.pdf:/Users/dong2j/Zotero/storage/I4HUMM4L/Ma et al. - 2004 - In situ X-ray diffraction studies of iron to Earth.pdf:application/pdf},
}

@article{mao_effect_1967,
	title = {Effect of {Pressure} on {Crystal} {Structure} and {Lattice} {Parameters} of {Iron} up to 300 kbar},
	volume = {38},
	issn = {0021-8979, 1089-7550},
	url = {https://pubs.aip.org/jap/article/38/1/272/3716/Effect-of-Pressure-on-Crystal-Structure-and},
	doi = {10.1063/1.1708965},
	abstract = {Lattice parameters of the bcc and hcp phases of iron have been determined as a function of pressure up to 300 kbar at 23°±3°C by means of x-ray diffraction techniques. The c/a ratio for hcp iron has been determined to be 1.603±0.001 at pressures between 80 and 300 kbar and is independent of pressure. Based upon the extrapolation of the high-pressure data using an exponential form of the Murnaghan equation of state, the volume of hcp iron at zero pressure is 6.72±0.06 cm3/mole. The volume change for the bcc-hcp transformation at 130 kbar is −0.34±0.01 cm3/mole. This value satisfies the triple point conditions for the bcc-hcp-fcc triple point when published values for the other phase transformations are used.},
	language = {en},
	number = {1},
	urldate = {2024-01-03},
	journal = {Journal of Applied Physics},
	author = {Mao, Ho-Kwang and Bassett, William A. and Takahashi, Taro},
	month = jan,
	year = {1967},
	pages = {272--276},
	file = {Mao et al. - 1967 - Effect of Pressure on Crystal Structure and Lattic.pdf:/Users/dong2j/Zotero/storage/HNEYB6QA/Mao et al. - 1967 - Effect of Pressure on Crystal Structure and Lattic.pdf:application/pdf},
}

@incollection{manghnani_experimental_1987,
	address = {Washington, D. C.},
	title = {Experimental phase relations of iron to 360 kbar, 1400°{C}, determined in an internally heated diamond-anvil apparatus},
	volume = {39},
	isbn = {978-0-87590-066-7},
	url = {http://doi.wiley.com/10.1029/GM039p0135},
	abstract = {Internalresistanceheatingexperimentswereconductedin a diamond-anvilapparatusto determinethe7-e-irontransition.Accurate valuesof thetransitiontemperatureat highpressurewereobtainedwith a diode-arrayspectrometerw, hichwasusedto measurethe blackbody emissionof theheatedironsampleat highpressureT. hetransitioncurve wasobservedin the range 190-360 kbar, 800-1375 øC. The slopeof the transition was 3.5 øC/kbar. The 7-e transition curve, if extrapolated, wouldprojectanironfieldstabilityunderconditionsof theearth'sCore.},
	language = {en},
	urldate = {2024-01-03},
	booktitle = {Geophysical {Monograph} {Series}},
	publisher = {American Geophysical Union},
	author = {Mao, H. K. and Bell, P. M. and Hadidiacos, C.},
	editor = {Manghnani, Murli H. and Syono, Yasuhiko},
	year = {1987},
	doi = {10.1029/GM039p0135},
	pages = {135--138},
	file = {Mao et al. - 1987 - Experimental phase relations of iron to 360 kbar, .pdf:/Users/dong2j/Zotero/storage/D22AD8SM/Mao et al. - 1987 - Experimental phase relations of iron to 360 kbar, .pdf:application/pdf},
}

@article{ohta_experimental_2016,
	title = {Experimental determination of the electrical resistivity of iron at {Earth}’s core conditions},
	volume = {534},
	issn = {0028-0836, 1476-4687},
	url = {https://www.nature.com/articles/nature17957},
	doi = {10.1038/nature17957},
	language = {en},
	number = {7605},
	urldate = {2024-01-03},
	journal = {Nature},
	author = {Ohta, Kenji and Kuwayama, Yasuhiro and Hirose, Kei and Shimizu, Katsuya and Ohishi, Yasuo},
	month = jun,
	year = {2016},
	pages = {95--98},
	file = {Ohta et al. - 2016 - Experimental determination of the electrical resis.pdf:/Users/dong2j/Zotero/storage/PBFKV4MI/Ohta et al. - 2016 - Experimental determination of the electrical resis.pdf:application/pdf},
}

@article{pommier_influence_2018,
	title = {Influence of sulfur on the electrical resistivity of a crystallizing core in small terrestrial bodies},
	volume = {496},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X18303157},
	doi = {10.1016/j.epsl.2018.05.032},
	language = {en},
	urldate = {2024-01-03},
	journal = {Earth and Planetary Science Letters},
	author = {Pommier, Anne},
	month = aug,
	year = {2018},
	pages = {37--46},
	file = {Pommier - 2018 - Influence of sulfur on the electrical resistivity .pdf:/Users/dong2j/Zotero/storage/6FJKIL4B/Pommier - 2018 - Influence of sulfur on the electrical resistivity .pdf:application/pdf},
}

@article{rutter_viscosity_2002,
	title = {Viscosity of liquid {Fe} at high pressure},
	volume = {66},
	issn = {0163-1829, 1095-3795},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.66.060102},
	doi = {10.1103/PhysRevB.66.060102},
	language = {en},
	number = {6},
	urldate = {2024-01-03},
	journal = {Physical Review B},
	author = {Rutter, Michael D. and Secco, Richard A. and Liu, Hongjian and Uchida, Takeyuki and Rivers, Mark L. and Sutton, Stephen R. and Wang, Yanbin},
	month = aug,
	year = {2002},
	pages = {060102},
	file = {Rutter et al. - 2002 - Viscosity of liquid Fe at high pressure.pdf:/Users/dong2j/Zotero/storage/3IMZ5XBC/Rutter et al. - 2002 - Viscosity of liquid Fe at high pressure.pdf:application/pdf},
}

@article{s_k_saxena_temperatures_1994,
	title = {Temperatures in {Earth}'s {Core} {Based} on {Melting} and {Phase} {Transformation} {Experiments} on lron},
	volume = {264},
	language = {en},
	journal = {Science},
	author = {{S. K. Saxena} and {G. Shen} and {P. Lazor}},
	year = {1994},
	file = {Boehler et al. - 1994 - REFERENCES AND NOTES.pdf:/Users/dong2j/Zotero/storage/4ZJNQJT6/Boehler et al. - 1994 - REFERENCES AND NOTES.pdf:application/pdf},
}

@article{secco_electrical_1989,
	title = {The electrical resistivity of solid and liquid {Fe} at pressures up to 7 {GPa}},
	volume = {94},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/JB094iB05p05887},
	doi = {10.1029/JB094iB05p05887},
	abstract = {The electrical resistivity of pure solid and liquid Fe has been measured at pressures up to 7 GPa in a large volume cubic anvil press. In conjunction with the four‐wired method, a novel technique of potential lead attachment was employed to measure the resistivity of 0.020‐in‐diameter Fe wire samples. Both the temperature and pressure coefficients of resistivity have been determined for solid and liquid Fe. The temperature coefficients of resistivity (TCR) in the liquid state are of the order of 10
              −4
              K
              −1
              and show an abrupt increase at approximately 5.2 GPa corresponding to the δ‐γ‐liquid triple point. We have interpreted this discontinuity in the TCR to be a reflection of local atomic structure in the liquid state which is reminiscent of the parent solid structure. By analogy, this result can be applied to the geophysically more important γ‐ε‐liquid triple point. By examining the fundamental effects of pressure and temperature on the density of states function and their ranges we arrive at an estimate of 1.2–1.5 × 10
              −6
              Ωm for the electrical resistivity of pure Fe at the pressures and temperatures expected in the Earth's core.},
	language = {en},
	number = {B5},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Secco, R. A. and Schloessin, H. H.},
	month = may,
	year = {1989},
	pages = {5887--5894},
	file = {Secco and Schloessin - 1989 - The electrical resistivity of solid and liquid Fe .pdf:/Users/dong2j/Zotero/storage/62NYZYSP/Secco and Schloessin - 1989 - The electrical resistivity of solid and liquid Fe .pdf:application/pdf},
}

@article{secco_thermal_2017,
	title = {Thermal conductivity and {Seebeck} coefficient of {Fe} and {Fe}-{Si} alloys: {Implications} for variable {Lorenz} number},
	volume = {265},
	issn = {00319201},
	shorttitle = {Thermal conductivity and {Seebeck} coefficient of {Fe} and {Fe}-{Si} alloys},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0031920116301832},
	doi = {10.1016/j.pepi.2017.01.005},
	abstract = {The Wiedemann-Franz Law is often used to calculate the thermal conductivity of Fe from experimental measurements of the electrical conductivity. It is shown by measurements of the Seebeck coefﬁcient (S) of solid and liquid Fe at pressures up to 6 GPa and temperatures up to 2100 K that the Sommerfeld value (L0 = 2.445 Â 10À8 W X KÀ2) of the Lorenz number (L) represents more than 99\% of the electronic component of the thermal conductivity of Fe. Using experimental values of electrical resistivity and thermal conductivity of Fe, L/L0 is shown to vary by as much as 1.22 in the solid state and 1.32 in the liquid state, signifying a non-negligible phonon component. An expression for the pressure dependence of L at the melting boundary up to 5 GPa is derived for electron-phonon scattering. For Fe-Si alloys, L/L0 varies more than for pure Fe and generally increases with increasing Si and state of disorder. New values for the conductive heat ﬂow in a pure Fe core of Mercury are presented.},
	language = {en},
	urldate = {2024-01-03},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Secco, Richard A.},
	month = apr,
	year = {2017},
	pages = {23--34},
	file = {Secco - 2017 - Thermal conductivity and Seebeck coefficient of Fe.pdf:/Users/dong2j/Zotero/storage/SAAEFYQ6/Secco - 2017 - Thermal conductivity and Seebeck coefficient of Fe.pdf:application/pdf},
}

@article{shen_melting_1998,
	title = {Melting and crystal structure of iron at high pressures and temperatures},
	volume = {25},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/97GL03776},
	doi = {10.1029/97GL03776},
	abstract = {High‐pressure melting, phase transitions and structures of iron have been studied to 84 GPa and 3500 K with an improved laser heated diamond anvil cell technique and
              in situ
              high P‐T x‐ray diffraction. At pressures below 60 GPa, the lower bound on the melting curve is close to those measured by
              Boehler
              [1993] and
              Saxena
              et al. [1993]; however, at pressures above 60 GPa our data indicate melting at higher temperatures than these studies, but still lower than the melting curve of
              Williams et al
              [1990]. The ε‐γ‐1 triple point is 60(±5) GPa and 2800(±200) K, based on our data of the ε‐γ phase transition and the observation of melting by
              in situ
              x‐ray diffraction. No solid phases other than ε‐Fe and γ‐Fe were observed
              in situ
              at high temperatures ({\textgreater}1000 K) and pressures to 84 GPa. However, the diffraction patterns of temperature quenched products at high pressure can be fit to other structures such as dhcp.},
	language = {en},
	number = {3},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Shen, Guoyin and Mao, Ho‐kwang and Hemley, Russell J. and Duffy, Thomas S. and Rivers, Mark L.},
	month = feb,
	year = {1998},
	pages = {373--376},
	file = {Shen et al. - 1998 - Melting and crystal structure of iron at high pres.pdf:/Users/dong2j/Zotero/storage/AJC4EKQX/Shen et al. - 1998 - Melting and crystal structure of iron at high pres.pdf:application/pdf},
}

@article{shen_structure_2004,
	title = {Structure of {Liquid} {Iron} at {Pressures} up to 58 {GPa}},
	volume = {92},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.92.185701},
	doi = {10.1103/PhysRevLett.92.185701},
	language = {en},
	number = {18},
	urldate = {2024-01-03},
	journal = {Physical Review Letters},
	author = {Shen, Guoyin and Prakapenka, Vitali B. and Rivers, Mark L. and Sutton, Stephen R.},
	month = may,
	year = {2004},
	pages = {185701},
	file = {Shen et al. - 2004 - Structure of Liquid Iron at Pressures up to 58 GPa.pdf:/Users/dong2j/Zotero/storage/5FGZJULN/Shen et al. - 2004 - Structure of Liquid Iron at Pressures up to 58 GPa.pdf:application/pdf},
}

@article{silber_electrical_2018,
	title = {Electrical resistivity of liquid {Fe} to 12 {GPa}: {Implications} for heat flow in cores of terrestrial bodies},
	volume = {8},
	issn = {2045-2322},
	shorttitle = {Electrical resistivity of liquid {Fe} to 12 {GPa}},
	url = {https://www.nature.com/articles/s41598-018-28921-w},
	doi = {10.1038/s41598-018-28921-w},
	abstract = {Abstract
            
              Electrical and thermal transport properties of liquid Fe under high pressure have important implications for the dynamics and thermal evolution of planetary cores and the geodynamo. However, electrical resistivity (
              ρ
              ) and thermal conductivity (
              k
              ) of liquid Fe at high pressure still remain contentious properties. To date, only two experimental investigations of
              ρ
              of liquid Fe in the pressure region below 7 GPa are reported in literature. Here we report the results of measurements of
              ρ
              for solid and liquid Fe (inversely proportional to
              k
              through the Wiedemann-Franz law) at pressures from 3 to 12 GPa, using a large multi-anvil press. We show that
              ρ
              of liquid Fe decreases as a function of pressure up to the δ-γ-liquid triple point at {\textasciitilde}5.2 GPa, and subsequently remains invariant from 6 to 12 GPa, which is consistent with an earlier study on liquid Ni. Our results demonstrate an important effect of solid phase on the structure and properties of liquid Fe. Our values of
              ρ
              for solid and liquid Fe are used to calculate
              k
              in Mercury’s solid inner core and along the adiabat in the liquid outer cores of Moon, Ganymede, Mercury and Mars. Our robust values of thermal conductivity place the focus on uncertainties in thermal expansion as the cause of variation in values of core conducted heat. Except for Mercury, our adiabatic heat flux values in these terrestrial cores validate the use of similar values used in several previous studies. Our high values of core adiabatic heat flux in Mercury would provide a stabilizing effect on, and lead to an increase in thickness of, the thermally stratified layer at the top of the core.},
	language = {en},
	number = {1},
	urldate = {2024-01-03},
	journal = {Scientific Reports},
	author = {Silber, Reynold E. and Secco, Richard A. and Yong, Wenjun and Littleton, Joshua A. H.},
	month = jul,
	year = {2018},
	pages = {10758},
	file = {Silber et al. - 2018 - Electrical resistivity of liquid Fe to 12 GPa Imp.pdf:/Users/dong2j/Zotero/storage/YJ3F972U/Silber et al. - 2018 - Electrical resistivity of liquid Fe to 12 GPa Imp.pdf:application/pdf},
}

@article{sinmyo_melting_2019,
	title = {Melting curve of iron to 290 {GPa} determined in a resistance-heated diamond-anvil cell},
	volume = {510},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X19300160},
	doi = {10.1016/j.epsl.2019.01.006},
	language = {en},
	urldate = {2024-01-03},
	journal = {Earth and Planetary Science Letters},
	author = {Sinmyo, Ryosuke and Hirose, Kei and Ohishi, Yasuo},
	month = mar,
	year = {2019},
	pages = {45--52},
	file = {Sinmyo et al. - 2019 - Melting curve of iron to 290 GPa determined in a r.pdf:/Users/dong2j/Zotero/storage/NHKFFLCN/Sinmyo et al. - 2019 - Melting curve of iron to 290 GPa determined in a r.pdf:application/pdf},
}

@article{strong_experimental_1959,
	title = {The experimental fusion curve of iron to 96,000 atmospheres},
	volume = {64},
	issn = {01480227},
	url = {http://doi.wiley.com/10.1029/JZ064i006p00653},
	doi = {10.1029/JZ064i006p00653},
	abstract = {The melting point of iron has been determined to 96,000 atmospheres,and the temperature for the a•y transition to 76,000 atmospheres.Simon's fusion equation, P/a-(T/To) • - 1, fits the experimentaml eltingpointswith a = 75,000arm andc = 8. Extrapolation of the melting pointsto 1.4 X 10• arm, the pressureat the boundary of the earth's core,gives 2340 4-200øC. The temperaturefor the a•y transition decreasedabout 200øC at 76,000 arm.},
	language = {en},
	number = {6},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research},
	author = {Strong, H. M.},
	month = jun,
	year = {1959},
	pages = {653--659},
	file = {Strong - 1959 - The experimental fusion curve of iron to 96,000 at.pdf:/Users/dong2j/Zotero/storage/3CSMYHNI/Strong - 1959 - The experimental fusion curve of iron to 96,000 at.pdf:application/pdf},
}

@article{strong_iron_1973,
	title = {The {Iron} {Fusion} {Curve} and {Triple} {Point}},
	language = {en},
	journal = {Metallurgical Transactions},
	author = {Strong, H M and Tuft, R E and Hanneman, R E},
	year = {1973},
	file = {Strong et al. - The Iron Fusion Curve and Triple Point.pdf:/Users/dong2j/Zotero/storage/6TB96STP/Strong et al. - The Iron Fusion Curve and Triple Point.pdf:application/pdf},
}

@article{tateno_structure_2010,
	title = {The {Structure} of {Iron} in {Earth}’s {Inner} {Core}},
	volume = {330},
	issn = {0036-8075, 1095-9203},
	url = {https://www.science.org/doi/10.1126/science.1194662},
	doi = {10.1126/science.1194662},
	abstract = {Packing the Core
            
              The packing and arrangement of atoms in Earth's solid inner core can dictate processes such as core growth and rotation. Seismology and modeling suggest the inner core is composed primarily of iron, but the structure is less clear due to anisotropic splitting of seismic waves.
              
                Tateno
                et al.
              
              (p.
              359
              ) performed static compression experiments on pure iron at the extremely high pressures and temperatures found in the inner core and saw that iron prefers a hexagonal close-packed structure, as opposed to cubic structures. The results help to explain the observed seismic anisotropy, and also suggest that individual iron crystals in the core may prefer orienting themselves with their long crystallographic axes parallel to Earth's rotation axis.
            
          , 
            Compression experiments indicate that the iron in Earth’s inner core has a hexagonal close-packed structure.
          , 
            
              Earth’s solid inner core is mainly composed of iron (Fe). Because the relevant ultrahigh pressure and temperature conditions are difficult to produce experimentally, the preferred crystal structure of Fe at the inner core remains uncertain. Static compression experiments showed that the hexagonal close-packed (hcp) structure of Fe is stable up to 377 gigapascals and 5700 kelvin, corresponding to inner core conditions. The observed weak temperature dependence of the
              c
              /
              a
              axial ratio suggests that hcp Fe is elastically anisotropic at core temperatures. Preferred orientation of the hcp phase may explain previously observed inner core seismic anisotropy.},
	language = {en},
	number = {6002},
	urldate = {2024-01-03},
	journal = {Science},
	author = {Tateno, Shigehiko and Hirose, Kei and Ohishi, Yasuo and Tatsumi, Yoshiyuki},
	month = oct,
	year = {2010},
	pages = {359--361},
	file = {Tateno et al. - 2010 - The Structure of Iron in Earth’s Inner Core.pdf:/Users/dong2j/Zotero/storage/VEV3YQ63/Tateno et al. - 2010 - The Structure of Iron in Earth’s Inner Core.pdf:application/pdf},
}

@article{terasaki_viscosity_2002,
	title = {Viscosity change and structural transition of {Molten} {Fe} at 5 {GPa}},
	volume = {29},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2001GL014321},
	doi = {10.1029/2001GL014321},
	abstract = {The in situ viscosity measurements of the pure molten Fe under high pressures were made by falling sphere X‐ray radiography method. Viscosity coefficients at about 2000 K were 15–24 mPa s at 2.7–5.0 GPa, and 4–9 mPa s at 5.0–7.0 GPa. Drastic decrease was found at around 5 GPa, at which stable solid phase below the melting temperatures change from delta (bcc) to gamma (fcc) phases. The observation indicates the possibility that the structural change in the molten Fe occurs in a narrow pressure interval (1 GPa) at the similar condition with the phase transformation in the solid.},
	language = {en},
	number = {8},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Terasaki, Hidenori and Kato, Takumi and Urakawa, S. and Funakoshi, K. and Sato, K. and Suzuki, A. and Okada, T.},
	month = apr,
	year = {2002},
	file = {Terasaki et al. - 2002 - Viscosity change and structural transition of Molt.pdf:/Users/dong2j/Zotero/storage/B8IZ6B86/Terasaki et al. - 2002 - Viscosity change and structural transition of Molt.pdf:application/pdf},
}



@article{zhang_reconciliation_2020,
	title = {Reconciliation of {Experiments} and {Theory} on {Transport} {Properties} of {Iron} and the {Geodynamo}},
	volume = {125},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.125.078501},
	doi = {10.1103/PhysRevLett.125.078501},
	language = {en},
	number = {7},
	urldate = {2024-01-03},
	journal = {Physical Review Letters},
	author = {Zhang, Youjun and Hou, Mingqiang and Liu, Guangtao and Zhang, Chengwei and Prakapenka, Vitali B. and Greenberg, Eran and Fei, Yingwei and Cohen, R. E. and Lin, Jung-Fu},
	month = aug,
	year = {2020},
	pages = {078501},
	file = {Zhang et al. - 2020 - Reconciliation of Experiments and Theory on Transp.pdf:/Users/dong2j/Zotero/storage/IDJPSFWI/Zhang et al. - 2020 - Reconciliation of Experiments and Theory on Transp.pdf:application/pdf},
}

@article{c_s_yoo_phase_1995,
	title = {Phase {Diagram} of {Iron} by in {Situ} {X}-{Ray} {Diffraction}: {Implications} for {Earth}'s {Core}},
	volume = {270},
	number = {5241},
	journal = {Science},
	author = {{C. S. Yoo} and {J. Akella} and {A. J. Campbell} and {H. K. Mao} and {R. J. Hemley}},
	month = dec,
	year = {1995},
	pages = {1473--1475},
	file = {Yoo (1995) - Phase Diagram of Iron by in Situ X-ray Diffraction.pdf:/Users/dong2j/Zotero/storage/HFNTGVNK/Yoo (1995) - Phase Diagram of Iron by in Situ X-ray Diffraction.pdf:application/pdf},
}
@article{sun_ab_2023,
	title = {\textit{{Ab} {Initio}} {Melting} {Temperatures} of {Bcc} and {Hcp} {Iron} {Under} the {Earth}’s {Inner} {Core} {Condition}},
	volume = {50},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2022GL102447},
	doi = {10.1029/2022GL102447},
	abstract = {There has been a long debate on the stable phase of iron under the Earth’s inner core conditions. Because of the solid-liquid coexistence at the inner core boundary, the thermodynamic stability of solid phases directly relates to their melting temperatures, which remains considerable uncertainty. In the present study, we utilized a semi-empirical potential fitted to high-temperature ab initio data to perform a thermodynamic integration from classical systems described by this potential to ab initio systems. This method provides a smooth path for thermodynamic integration and significantly reduces the uncertainty caused by the finite-size effect. Our results suggest the hcp phase is the stable phase of pure iron under the inner core conditions, while the free energy difference between the hcp and bcc phases is tiny, on the order of 10 s meV/atom near the melting temperature.},
	language = {en},
	number = {5},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Sun, Yang and Mendelev, Mikhail I. and Zhang, Feng and Liu, Xun and Da, Bo and Wang, Cai‐Zhuang and Wentzcovitch, Renata M. and Ho, Kai‐Ming},
	month = mar,
	year = {2023},
	pages = {e2022GL102447},
	file = {Sun et al. - 2023 - Ab Initio Melting Temperatures of Bcc and H.pdf:/Users/dong2j/Zotero/storage/77R88RT2/Sun et al. - 2023 - Ab Initio Melting Temperatures of Bcc and H.pdf:application/pdf},
}

@article{sola_melting_2009,
	title = {Melting of {Iron} under {Earth}’s {Core} {Conditions} from {Diffusion} {Monte} {Carlo} {Free} {Energy} {Calculations}},
	volume = {103},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.103.078501},
	doi = {10.1103/PhysRevLett.103.078501},
	language = {en},
	number = {7},
	urldate = {2024-01-03},
	journal = {Physical Review Letters},
	author = {Sola, Ester and Alfè, Dario},
	month = aug,
	year = {2009},
	pages = {078501},
	file = {Sola and Alfè - 2009 - Melting of Iron under Earth’s Core Conditions from.pdf:/Users/dong2j/Zotero/storage/L6MAMQYF/Sola and Alfè - 2009 - Melting of Iron under Earth’s Core Conditions from.pdf:application/pdf},
}

@article{morard_melting_2011,
	title = {The melting curve of iron at extreme pressures: {Implications} for planetary cores},
	volume = {7},
	issn = {15741818},
	shorttitle = {The melting curve of iron at extreme pressures},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S1574181811000231},
	doi = {10.1016/j.hedp.2011.02.001},
	abstract = {Exoplanets with masses similar to that of Earth have recently been discovered in extrasolar systems. A ﬁrst order question for understanding their dynamics is to know whether they possess a liquid metallic core like the Earth. However, the iron melting curve is unknown at conditions corresponding to planets several times the Earth’s mass (over 1500 GPa for planets with 10 times the Earths mass (ME)). In the density-temperature region corresponding to the core of those super-Earths, we calculate the high pressure melting curve using a ﬁrst principles approach based on density functional theory. We perform direct molecular dynamics simulations using the computer intensive two phases approach. The resulting melting exhibits a slope steeper than any calculated planetary adiabatic temperature proﬁle. This suggests that the presence of molten metallic cores is less likely as the size of terrestrial planets increases.},
	language = {en},
	number = {3},
	urldate = {2024-01-03},
	journal = {High Energy Density Physics},
	author = {Morard, G. and Bouchet, J. and Valencia, D. and Mazevet, S. and Guyot, F.},
	month = sep,
	year = {2011},
	pages = {141--144},
	file = {Morard et al. - 2011 - The melting curve of iron at extreme pressures Im.pdf:/Users/dong2j/Zotero/storage/WJBACHFM/Morard et al. - 2011 - The melting curve of iron at extreme pressures Im.pdf:application/pdf},
}

@article{gonzalez-cataldo_ab_2023,
	title = {\textit{{Ab} initio} determination of iron melting at terapascal pressures and {Super}-{Earths} core crystallization},
	volume = {5},
	issn = {2643-1564},
	url = {https://link.aps.org/doi/10.1103/PhysRevResearch.5.033194},
	doi = {10.1103/PhysRevResearch.5.033194},
	language = {en},
	number = {3},
	urldate = {2024-01-03},
	journal = {Physical Review Research},
	author = {González-Cataldo, Felipe and Militzer, Burkhard},
	month = sep,
	year = {2023},
	pages = {033194},
	file = {González-Cataldo and Militzer - 2023 - Ab initio determination of iron melting at .pdf:/Users/dong2j/Zotero/storage/XP6Q84G4/González-Cataldo and Militzer - 2023 - Ab initio determination of iron melting at .pdf:application/pdf},
}
@article{ping_solid_2013,
	title = {Solid {Iron} {Compressed} {Up} to 560 {GPa}},
	volume = {111},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.065501},
	doi = {10.1103/PhysRevLett.111.065501},
	language = {en},
	number = {6},
	urldate = {2024-01-08},
	journal = {Physical Review Letters},
	author = {Ping, Y. and Coppari, F. and Hicks, D. G. and Yaakobi, B. and Fratanduono, D. E. and Hamel, S. and Eggert, J. H. and Rygg, J. R. and Smith, R. F. and Swift, D. C. and Braun, D. G. and Boehly, T. R. and Collins, G. W.},
	month = aug,
	year = {2013},
	pages = {065501},
	file = {Ping et al. - 2013 - Solid Iron Compressed Up to 560 GPa.pdf:/Users/dong2j/Zotero/storage/9LJJWSUC/Ping et al. - 2013 - Solid Iron Compressed Up to 560 GPa.pdf:application/pdf},
}
@article{belonoshko_stabilization_2017,
	title = {Stabilization of body-centred cubic iron under inner-core conditions},
	volume = {10},
	issn = {1752-0894, 1752-0908},
	url = {https://www.nature.com/articles/ngeo2892},
	doi = {10.1038/ngeo2892},
	language = {en},
	number = {4},
	urldate = {2024-01-08},
	journal = {Nature Geoscience},
	author = {Belonoshko, Anatoly B. and Lukinov, Timofei and Fu, Jie and Zhao, Jijun and Davis, Sergio and Simak, Sergei I.},
	month = apr,
	year = {2017},
	pages = {312--316},
	file = {Belonoshko et al. - 2017 - Stabilization of body-centred cubic iron under inn.pdf:/Users/dong2j/Zotero/storage/UPVBGSJX/Belonoshko et al. - 2017 - Stabilization of body-centred cubic iron under inn.pdf:application/pdf},
}

%% SiO2 %%

@book{callen_thermodynamics_1985,
	address = {New York},
	edition = {2nd ed},
	title = {Thermodynamics and an {Introduction} to {Thermostatistics}},
	isbn = {978-0-471-86256-7},
	publisher = {Wiley},
	author = {Callen, Herbert B.},
	year = {1985},
	keywords = {Statistical mechanics, Thermodynamics},
	annote = {Rev. ed. of: Thermodynamics. 1960 Includes index},
}

@article{luo_polymorphism_2003,
	title = {Polymorphism, superheating, and amorphization of silica upon shock wave loading and release},
	volume = {108},
	copyright = {http://onlinelibrary.wiley.com/termsAndConditions\#vor},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2002JB002317},
	doi = {10.1029/2002JB002317},
	abstract = {We present a detailed and quantitative examination of the thermodynamics and phase change mechanisms (including amorphization) that occur upon shock wave loading and unloading of silica. We apply Debye‐Grüneisen theory to calculate both the Hugoniot of quartz and isentropic release paths. Quartz converts to stishovite (or a stishovite‐like phase) between 15 and 46 GPa, and persistence of the solid phase above its liquidus (i.e., superheating) is confirmed between 77 and 110 GPa. Calculations compare favorably to measurements of shock and post‐shock temperatures. For silica, the method of measuring post‐shock temperature is insensitive to predicting whether phase transitions actually occur during release. Measurements of release states in pressure‐particle velocity space are compared to computed frozen‐phase release paths. This comparison suggests transformation of a stishovite‐like phase to lower density phases including quartz, liquid, or dense amorphous glass. Transformations to liquid or glass occur upon release from peak pressure of 26 GPa and above. The isentropic release assumption appears to be approximately valid. A shock pressure‐temperature scale relating metamorphism of silica in shock‐loaded quartz is proposed. Neither recovery of coesite nor substantial quantities of crystalline stishovite‐like phases upon shock loading of quartz is predicted. Trace amounts of crystalline stishovite‐like phases from shock loading between 15 and 26 GPa are expected.},
	language = {en},
	number = {B9},
	urldate = {2025-01-30},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Luo, Sheng‐Nian and Ahrens, Thomas J. and Asimow, Paul D.},
	month = sep,
	year = {2003},
	pages = {2002JB002317},
	file = {Accepted Version:/Users/dong2j/Zotero/storage/W6B58JTY/Luo et al. - 2003 - Polymorphism, superheating, and amorphization of silica upon shock wave loading and release.pdf:application/pdf},
}

@article{hemley_pressure-induced_1988,
	title = {Pressure-induced amorphization of crystalline silica},
	volume = {334},
	copyright = {http://www.springer.com/tdm},
	issn = {0028-0836, 1476-4687},
	url = {https://www.nature.com/articles/334052a0},
	doi = {10.1038/334052a0},
	language = {en},
	number = {6177},
	urldate = {2025-01-30},
	journal = {Nature},
	author = {Hemley, R. J. and Jephcoat, A. P. and Mao, H. K. and Ming, L. C. and Manghnani, M. H.},
	month = jul,
	year = {1988},
	pages = {52--54},
}

@incollection{akaogi_calorimetric_2022,
	address = {Singapore},
	title = {Calorimetric {Experiments} and {Thermodynamic} {Calculation} of {High}-{Pressure} {Phase} {Relations}},
	isbn = {978-981-19636-2-9 978-981-19636-3-6},
	url = {https://link.springer.com/10.1007/978-981-19-6363-6_4},
	language = {en},
	urldate = {2024-08-01},
	booktitle = {High-{Pressure} {Silicates} and {Oxides}},
	publisher = {Springer Nature Singapore},
	author = {Akaogi, Masaki},
	collaborator = {Akaogi, Masaki},
	year = {2022},
	doi = {10.1007/978-981-19-6363-6_4},
	note = {Series Title: Advances in Geological Science},
	pages = {47--70},
}
@article{prakapenka_high_2004,
	title = {High pressure induced phase transformation of {SiO2} and {GeO2}: difference and similarity},
	volume = {65},
	issn = {00223697},
	shorttitle = {High pressure induced phase transformation of {SiO2} and {GeO2}},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0022369704000691},
	doi = {10.1016/j.jpcs.2003.12.019},
	language = {en},
	number = {8-9},
	urldate = {2024-01-21},
	journal = {Journal of Physics and Chemistry of Solids},
	author = {Prakapenka, V.P and Shen, Guoyin and Dubrovinsky, L.S and Rivers, M.L and Sutton, S.R},
	year = {2004},
	pages = {1537--1545},
}

@article{li_behavior_2003,
	title = {Behavior of thermocouples under high pressure in a multi-anvil apparatus},
	volume = {23},
	issn = {0895-7959, 1477-2299},
	url = {http://www.tandfonline.com/doi/abs/10.1080/0895795031000088269},
	doi = {10.1080/0895795031000088269},
	language = {en},
	number = {4},
	urldate = {2024-01-21},
	journal = {High Pressure Research},
	author = {Li, Jie and Hadidiacos, Chris and Mao, Ho-Kwang and Fei, Yingwei and Hemley, Russell J.},
	year = {2003},
	pages = {389--401},
}

@book{petrenko_physics_2002,
	title = {Physics of {Ice}},
	isbn = {978-0-19-851894-5},
	url = {http://www.oxfordscholarship.com/view/10.1093/acprof:oso/9780198518945.001.0001/acprof-9780198518945},
	urldate = {2024-01-21},
	publisher = {Oxford University Press},
	author = {Petrenko, Victor F. and Whitworth, Robert W.},
	year = {2002},
	doi = {10.1093/acprof:oso/9780198518945.001.0001},
}

@article{kechin_melting_2001,
	title = {Melting curve equations at high pressure},
	volume = {65},
	issn = {0163-1829, 1095-3795},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.65.052102},
	doi = {10.1103/PhysRevB.65.052102},
	language = {en},
	number = {5},
	urldate = {2024-01-21},
	journal = {Physical Review B},
	author = {Kechin, Vladimir V.},
	year = {2001},
	pages = {052102},
}
@article{Kechin_1995,
    doi = {10.1088/0953-8984/7/3/008},
    url = {https://dx.doi.org/10.1088/0953-8984/7/3/008},
year = {1995},
month = {jan},
publisher = {},
volume = {7},
number = {3},
pages = {531},
author = {V V Kechin},
title = {Thermodynamically based melting-curve equation},
journal = {Journal of Physics: Condensed Matter},
abstract = {An equation for the pressure dependence of the melting temperature based on thermodynamic principles has been developed, which generalizes the Simon-Glatzel equation and describes the rising and falling melting curves as well as curves with a maximum. The parameters appearing in the equation are identified in terms of the thermodynamic values. The equation accurately approximates the melting curves of different categories of substances over a large range of melting temperatures and pressures.}
}

@article{li_determination_2017,
	title = {Determination of calcium carbonate and sodium carbonate melting curves up to {Earth}'s transition zone pressures with implications for the deep carbon cycle},
	volume = {457},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X16305842},
	doi = {10.1016/j.epsl.2016.10.027},
	language = {en},
	urldate = {2024-01-21},
	journal = {Earth and Planetary Science Letters},
	author = {Li, Zeyu and Li, Jie and Lange, Rebecca and Liu, Jiachao and Militzer, Burkhard},
	year = {2017},
	pages = {395--402},
}

@article{dong_melting_2019,
	title = {Melting curve minimum of barium carbonate {BaCO3} near 5 {GPa}},
	volume = {104},
	issn = {0003-004X, 1945-3027},
	url = {https://www.degruyter.com/document/doi/10.2138/am-2019-6891/html},
	doi = {10.2138/am-2019-6891},
	language = {en},
	number = {5},
	urldate = {2024-01-21},
	journal = {American Mineralogist},
	author = {Dong, Junjie and Li, Jie and Zhu, Feng and Li, Zeyu and Farawi, Rami},
	month = may,
	year = {2019},
	pages = {671--678},
}

@article{simon_bemerkungen_1929,
	title = {Bemerkungen zur {Schmelzdruckkurve}},
	volume = {178},
	issn = {0863-1786},
	url = {https://onlinelibrary.wiley.com/doi/10.1002/zaac.19291780123},
	doi = {10.1002/zaac.19291780123},
	language = {en},
	number = {1},
	urldate = {2024-01-21},
	journal = {Zeitschrift für anorganische und allgemeine Chemie},
	author = {Simon, Franz and Glatzel, Gunther},
	year = {1929},
	pages = {309--316},
}

@article{lindemann_uber_1910,
	title = {Über die berechnung molekularer eigenfrequenzen},
	volume = {11},
	journal = {Zeitschrift für Physik},
	author = {Lindemann, Frederick A},
	year = {1910},
	pages = {609--612},
}

@article{kraut_new_1966,
	title = {New {Melting} {Law} at {High} {Pressures}},
	volume = {16},
	issn = {0031-9007},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.16.608},
	doi = {10.1103/PhysRevLett.16.608},
	language = {en},
	number = {14},
	urldate = {2024-01-21},
	journal = {Physical Review Letters},
	author = {Kraut, Edgar A. and Kennedy, George C.},
	year = {1966},
	pages = {608--609},
}



@article{akimoto_coesite-stishovite_1969,
	title = {Coesite-{Stishovite} transition},
	volume = {74},
	issn = {01480227},
	url = {http://doi.wiley.com/10.1029/JB074i006p01653},
	doi = {10.1029/JB074i006p01653},
	language = {en},
	number = {6},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research},
	author = {Akimoto, Syun-iti and Syono, Yasuhiko},
	month = mar,
	year = {1969},
	pages = {1653--1659},
	file = {Akimoto and Syono - 1969 - Coesite-Stishovite transition.pdf:/Users/dong2j/Zotero/storage/PPETLBJ6/Akimoto and Syono - 1969 - Coesite-Stishovite transition.pdf:application/pdf},
}

@article{andrault_equation_2003,
	title = {Equation of state of stishovite to lower mantle pressures},
	volume = {88},
	issn = {0003-004X},
	url = {https://www.degruyter.com/document/doi/10.2138/am-2003-2-307/html},
	doi = {10.2138/am-2003-2-307},
	abstract = {We performed new diffraction experiments to clarify the equation of state (EoS) of stishovite after we suspected systematic errors in previous experimental reports. Using diamond anvil cells, we repeated both single-crystal X-ray diffraction measurements under hydrostatic conditions and powder diffraction measurements using the laser-annealing technique and NaCl pressure medium. The major improvement is the increase in precision of the pressure determination using the quartz and NaCl equations of state. Using both sets of data, the stishovite bulk moduli were refined to K0 = 309.9(1.1) GPa and K0' = 4.59(0.23). We also reinvestigated the mechanism of the phase transformation to the CaCl2-structured polymorph of SiO2 at about 60 GPa. We confirm no volume discontinuity at the transition pressure, but the CaCl2 form appears slightly more compressible than the rutile-structured form of SiO2. This change in compression behavior is used for quantitative analyses of the spontaneous strains of the pressure-induced phase transition.},
	language = {en},
	number = {2-3},
	urldate = {2024-01-03},
	journal = {American Mineralogist},
	author = {Andrault, Denis and Angel, Ross J. and Mosenfelder, Jed L. and Le Bihan, Tristan},
	month = feb,
	year = {2003},
	pages = {301--307},
	file = {Andrault et al. - 2003 - Equation of state of stishovite to lower mantle pr.pdf:/Users/dong2j/Zotero/storage/IIIMHC4A/Andrault et al. - 2003 - Equation of state of stishovite to lower mantle pr.pdf:application/pdf},
}

@article{andrault_melting_2020,
	title = {Melting behavior of {SiO}$_{\textrm{2}}$ up to 120 {GPa}},
	volume = {47},
	issn = {0342-1791, 1432-2021},
	url = {https://link.springer.com/10.1007/s00269-019-01077-3},
	doi = {10.1007/s00269-019-01077-3},
	abstract = {The structure of liquid silicates is commonly described as a statistical mixture of various atomic entities with relative abundances that can vary with pressure, temperature, and composition. Unfortunately, this view remains largely theoretical due to scarce experimental reports on the silicate melt structure, in particular under pressure. We performed X-ray diffraction of the ­SiO2 end member to probe the melting curve up to {\textasciitilde} 120 GPa and 7000 K, and the melt structure up to {\textasciitilde} 80 GPa. We confirm the steep increase of the melting curve above {\textasciitilde} 14 GPa when stishovite becomes stable over coesite in subsolidus conditions, with a slope of about 80 K/GPa. Then, around 45 GPa and 5400 K, the melting curve flattens significantly, an effect most likely reflecting the densification of the S­ iO2 melt structure. The signal of diffuse X-ray scattering is compatible with a change of the Si coordination number from 4 to 6 along the melting curve, in agreement with previous works reporting a similar evolution during the cold compression of ­SiO2 glass. Because of the limited pressure range (within 10 to 20 GPa) in which the melting curve changes its slope, we speculate a difficult coexistence of tetrahedral S­ iO4 and octahedral ­SiO6 units in ­SiO2 melt at high pressures.},
	language = {en},
	number = {2},
	urldate = {2024-01-03},
	journal = {Physics and Chemistry of Minerals},
	author = {Andrault, D. and Morard, G. and Garbarino, G. and Mezouar, M. and Bouhifd, M. A. and Kawamoto, T.},
	month = feb,
	year = {2020},
	pages = {10},
	file = {Andrault et al. - 2020 - Melting behavior of SiO2 up to 120 GPa.pdf:/Users/dong2j/Zotero/storage/2G3QURWJ/Andrault et al. - 2020 - Melting behavior of SiO2 up to 120 GPa.pdf:application/pdf},
}

@article{andrault_comment_2022,
	title = {Comment on: {Melting} behavior of {SiO}$_{\textrm{2}}$ up to 120 {GPa} ({Andrault} et al. 2020)},
	volume = {49},
	issn = {0342-1791, 1432-2021},
	shorttitle = {Comment on},
	url = {https://link.springer.com/10.1007/s00269-021-01174-2},
	doi = {10.1007/s00269-021-01174-2},
	abstract = {The additional work we have done using our new laser heating in the diamond anvil cell system since the publication of Andrault et al. (Phys Chem Mineral 47(2), 2020) leads us to the conclusion that there was a systematic bias in the determination of temperature. First, the temperature of the W-lamp used for the calibration of the optical system was overestimated by {\textasciitilde} 22 K at 2273 K. Then, we made the assumption that hot ­SiO2 was a grey-body (constant emissivity ε(λ)), while the available measurements suggest instead that ε(λ) of ­SiO2 is similar to that of tungsten. Applying these two corrections lowers the ­SiO2 melting temperatures significantly. In LMV, we performed a new experimental determination of the S­ iO2 melting temperature, at 5000 (200) K and {\textasciitilde} 70 (4) GPa, which is well compatible with the amplitude of the correction proposed. The reevaluation of the melting temperature profile does not affect largely the interpretations or the main conclusions presented in Andrault et al. (Phys Chem Mineral 47(2), 2020). Within the stability field of stishovite, the melting curve still presents a relatively sharp change of slope at P–T recalculated as {\textasciitilde} 40 GPa and {\textasciitilde} 4800 K. It is related to a change of the melt structure. At higher pressures, the melting curve is almost flat up to the subsolidus transition from stishovite to the C­ aCl2-form around 85 GPa, where the slope of the melting curve increases again up to {\textasciitilde} 120 GPa. We present corrected figures and tables of the original publication.},
	language = {en},
	number = {2},
	urldate = {2024-01-03},
	journal = {Physics and Chemistry of Minerals},
	author = {Andrault, Denis and Pison, L. and Morard, G. and Garbarino, G. and Mezouar, M. and Bouhifd, M. A. and Kawamoto, T.},
	month = feb,
	year = {2022},
	pages = {3},
	file = {Andrault et al. - 2022 - Comment on Melting behavior of SiO2 up to 120 GPa.pdf:/Users/dong2j/Zotero/storage/ZLH94MFC/Andrault et al. - 2022 - Comment on Melting behavior of SiO2 up to 120 GPa.pdf:application/pdf},
}

@article{andrault_pressure-induced_1998,
	title = {Pressure-{Induced} {Landau}-{Type} {Transition} in {Stishovite}},
	volume = {282},
	issn = {0036-8075, 1095-9203},
	url = {https://www.science.org/doi/10.1126/science.282.5389.720},
	doi = {10.1126/science.282.5389.720},
	abstract = {A Rietveld structural analysis of stishovite, with angle-dispersive x-ray diffraction synchrotron source at the European Synchrotron Radiation Facility, confirmed a CaCl
              2
              form of stishovite distortion at 54 ± 1 gigapascals but confirmed no further phase transformation up to 120 gigapascals. The deviatoric stress that is usually encountered at such pressures was relaxed after yttrium-aluminum-garnet–laser heating. A single Birch-Murnaghan equation of state fits volumes of stishovite and a CaCl
              2
              form, showing that the tetragonal distortion occurs without a substantial change in volume. At the 54-gigapascal transition, the pressure-induced lattice modifications were similar to those found in a Landau-type temperature-induced transition. It is proposed that, above the transition pressure, the critical temperature increases above 300 kelvin, so that the lower entropy form becomes stable.},
	language = {en},
	number = {5389},
	urldate = {2024-01-03},
	journal = {Science},
	author = {Andrault, Denis and Fiquet, Guillaume and Guyot, François and Hanfland, Michael},
	month = oct,
	year = {1998},
	pages = {720--724},
	file = {Andrault et al. - 1998 - Pressure-Induced Landau-Type Transition in Stishov.pdf:/Users/dong2j/Zotero/storage/6QNNDTDZ/Andrault et al. - 1998 - Pressure-Induced Landau-Type Transition in Stishov.pdf:application/pdf},
}

@article{bohlen_quartz_1982,
	title = {The quartz ⇆ coesite transformation: {A} precise determination and the effects of other components},
	volume = {87},
	issn = {0148-0227},
	shorttitle = {The quartz ⇆ coesite transformation},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/JB087iB08p07073},
	doi = {10.1029/JB087iB08p07073},
	abstract = {Reaction reversals to within 0.2 kbar locate the quartz ⇆ coesite equilibrium at 24.6, 24.9, 25.5, 26.2, 27.0, 27.9, 28.8, and 29.7 kbar at 350, 400, 500, 600, 700, 800, 900, and 1000°C, respectively, using well‐calibrated (frictionless), 2.54‐cm diameter NaCl furnace assemblies in piston‐cylinder apparatus. The equilibrium is unaffected by the presence of H
              2
              O or jadeite, contrary to previous proposals. The positive
              dP/dT
              of the reaction at
              T
              {\textless} 500°C is inconsistent with existing thermochemical data for coesite. Numerous tight reversals provide a sound basis for use of the quartz ⇆ coesite equilibrium as a calibration of pressure in high‐pressure apparatus.},
	language = {en},
	number = {B8},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Bohlen, Steven R. and Boettcher, A. L.},
	month = aug,
	year = {1982},
	pages = {7073--7078},
	file = {Bohlen and Boettcher - 1982 - The quartz ⇆ coesite transformation A precise det.pdf:/Users/dong2j/Zotero/storage/U5V3MWRY/Bohlen and Boettcher - 1982 - The quartz ⇆ coesite transformation A precise det.pdf:application/pdf},
}

@article{buchen_equation_2018,
	title = {Equation of {State} of {Polycrystalline} {Stishovite} {Across} the {Tetragonal}‐{Orthorhombic} {Phase} {Transition}},
	volume = {123},
	issn = {2169-9313, 2169-9356},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2018JB015835},
	doi = {10.1029/2018JB015835},
	abstract = {High-pressure silica polymorphs may contribute to lithologies in Earth’s lower mantle. Stishovite, the tetragonal rutile-type polymorph of SiO2, distorts to an orthorhombic CaCl2-type structure at pressures and temperatures of the lower mantle. We compressed sintered polycrystalline stishovite and determined the unit cell parameters as a function of pressure using synchrotron X-ray diﬀraction. The compression behavior of sintered polycrystalline stishovite deviates systematically from previous results on stishovite powder and single crystals. Following an initial stiﬀening, the bulk modulus of sintered polycrystalline stishovite drops at the ferroelastic phase transition. We analyzed the observed spontaneous strains using Landau theory to predict the complete elastic behavior of sintered polycrystalline silica across the phase transition. The reduction in bulk modulus at the phase transition as derived here from the compression curve of sintered polycrystalline silica may have implications for the seismic detection of silica-rich materials in Earth’s lower mantle.},
	language = {en},
	number = {9},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Buchen, Johannes and Marquardt, Hauke and Schulze, Kirsten and Speziale, Sergio and Boffa Ballaran, Tiziana and Nishiyama, Norimasa and Hanfland, Michael},
	month = sep,
	year = {2018},
	pages = {7347--7360},
	file = {Buchen et al. - 2018 - Equation of State of Polycrystalline Stishovite Ac.pdf:/Users/dong2j/Zotero/storage/CUF9PCXT/Buchen et al. - 2018 - Equation of State of Polycrystalline Stishovite Ac.pdf:application/pdf},
}

@article{dubrovinsky_pressure-induced_2001,
	title = {Pressure-induced transformations of cristobalite},
	volume = {333},
	issn = {00092614},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0009261400011477},
	doi = {10.1016/S0009-2614(00)01147-7},
	abstract = {X-ray in situ studies in electrically and laser-heated diamond anvil cells (DACs) at pressures over 80 GPa and temperatures above 2500 K were used to determine stable silica phase at extreme conditions. We demonstrate that so far unidenti®ed phases obtained on the compression of a-cristobalite, new dense silica polymorph in the Martian Shergotty meteorite, and controversial post-stishovite phase is a-PbO2-like silica. Ó 2001 Elsevier Science B.V. All rights reserved.},
	language = {en},
	number = {3-4},
	urldate = {2024-01-03},
	journal = {Chemical Physics Letters},
	author = {Dubrovinsky, L.S and Dubrovinskaia, N.A and Saxena, S.K and Tutti, F and Rekhi, S and Le Bihan, T and Shen, Guoyin and Hu, J},
	month = jan,
	year = {2001},
	pages = {264--270},
	file = {Dubrovinsky et al. - 2001 - Pressure-induced transformations of cristobalite.pdf:/Users/dong2j/Zotero/storage/BFRKZVTI/Dubrovinsky et al. - 2001 - Pressure-induced transformations of cristobalite.pdf:application/pdf},
}

@article{fischer_equations_2018,
	title = {Equations of state and phase boundary for stishovite and {CaCl}$_{\textrm{2}}$-type {SiO}$_{\textrm{2}}$},
	volume = {103},
	issn = {0003-004X, 1945-3027},
	url = {https://www.degruyter.com/document/doi/10.2138/am-2018-6267/html},
	doi = {10.2138/am-2018-6267},
	abstract = {Silica is thought to be present in the Earth’s lower mantle in subducting plates, in addition to being a prototypical solid whose physical properties are of broad interest. It is known to undergo a phase transition from stishovite to the CaCl2-type structure at ∼50–80 GPa, but the exact location and slope of the phase boundary in pressure-temperature space is unresolved. There have been many previous studies on the equation of state of stishovite, but they span a limited range of pressures and temperatures, and there has been no thermal equation of state of CaCl2-type SiO2 measured under static conditions. We have investigated the phase diagram and equations of state of silica at 21–89 GPa and up to ∼3300 K using synchrotron X‑ray diffraction in a laser-heated diamond-anvil cell. The phase boundary between stishovite and CaCl2-type SiO2 can be approximately described as T = 64.6(49)·P – 2830(350), with temperature T in Kelvin and pressure P in GPa. The stishovite data imply K0ʹ = 5.24(9) and a quasi-anharmonic T 2 dependence of –6.0(4) × 10–6 GPa·cm3/mol/K2 for a fixed q = 1, g0 = 1.71, and K0 = 302 GPa, while for the CaCl2-type phase K0 = 341(4) GPa, K0ʹ = 3.20(16), and g0 = 2.14(4) with other parameters equal to their values for stishovite. The behaviors of the a and c axes of stishovite with pressure and temperature were also fit, indicating a much more compressible c axis with a lower thermal expansion as compared to the a axis. The phase transition between stishovite and CaCl2-type silica should occur at pressures of 68–78 GPa in the Earth, depending on the temperature in subducting slabs. Silica is denser than surrounding mantle material up to pressures of 58–68 GPa, with uncertainty due to temperature effects; at higher pressures than this, SiO2 becomes gravitationally buoyant in the lower mantle.},
	language = {en},
	number = {5},
	urldate = {2024-01-03},
	journal = {American Mineralogist},
	author = {Fischer, Rebecca A. and Campbell, Andrew J. and Chidester, Bethany A. and Reaman, Daniel M. and Thompson, Elizabeth C. and Pigott, Jeffrey S. and Prakapenka, Vitali B. and Smith, Jesse S.},
	month = may,
	year = {2018},
	pages = {792--802},
	file = {Fischer et al. - 2018 - Equations of state and phase boundary for stishovi.pdf:/Users/dong2j/Zotero/storage/AWVTAFD6/Fischer et al. - 2018 - Equations of state and phase boundary for stishovi.pdf:application/pdf},
}

@article{grocholski_stability_2013,
	title = {Stability, metastability, and elastic properties of a dense silica polymorph, seifertite},
	volume = {118},
	issn = {2169-9313, 2169-9356},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1002/jgrb.50360},
	doi = {10.1002/jgrb.50360},
	abstract = {Dense silica polymorphs with sixfold coordinated Si have been found in SNC and lunar meteorites and may be important minerals for silica‐rich components in the lower mantle. However, the stable crystal structure in the lower mantle and properties of dense silica remain controversial. Under stable heating and quasi‐hydrostatic stress conditions, we found that the CaCl
              2
              type undergoes a phase transition to the
              α
              ‐PbO
              2
              type (seifertite) at 130–140 GPa and 2500 K. Our data suggest that this phase transition occurs at a greater depth than the perovskite → postperovskite transition in the lowermost mantle. The molar volume measured at 1 bar is the smallest among the reported silica polymorphs, therefore having the highest calculated density and in excellent agreement with recent first‐principles calculations. The greater molar volume of seifertite found in the shergottite meteorite and previous experiments supports a metastable synthesis of the phase outside its stability field. Our data combined with the Hugoniots of silica polymorphs also rule out the possibility of the formation of seifertite in the meteorite within its stability field. We found very little change in bulk sound speed across the CaCl
              2
              ‐type → seifertite transition. If shear wave velocity decreases at the transition to seifertite as suggested by some computational studies, this silica transition may provide an alternative explanation for the discontinuities with a shear wave velocity decrease found at depths greater than the D
              ″
              discontinuity.
            
          , 
            Key Points
            
              
                
                  Equation of state of seifertite from 1 bar to 140 GPa
                
                
                  Silica may account for some D
                
                
                  Stability field supports metastable origin of seifertite in SNC's first‐principles},
	language = {en},
	number = {9},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Grocholski, B. and Shim, S.‐H. and Prakapenka, V. B.},
	month = sep,
	year = {2013},
	pages = {4745--4757},
	file = {Grocholski et al. - 2013 - Stability, metastability, and elastic properties o.pdf:/Users/dong2j/Zotero/storage/ISHC9PLL/Grocholski et al. - 2013 - Stability, metastability, and elastic properties o.pdf:application/pdf},
}

@article{jackson_melting_1976,
	title = {Melting of the {Silica} {Isotypes} {SiO}$_{\textrm{2}}$, {BeF}$_{\textrm{2}}$ and {GeO}$_{\textrm{2}}$2 at {Elevated} {Pressures}},
	volume = {13},
	language = {en},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Jackson, Ian},
	year = {1976},
	pages = {218--231},
	file = {Jackson - MELTING OF THE SILICA ISOTYPES Si02, BeF2 AND Ge02.pdf:/Users/dong2j/Zotero/storage/P8NXP6LC/Jackson - MELTING OF THE SILICA ISOTYPES Si02, BeF2 AND Ge02.pdf:application/pdf},
}

@article{kanzaki_melting_1990,
	title = {Melting of {Silica} up to 7 {GPa}},
	volume = {73},
	issn = {0002-7820, 1551-2916},
	url = {https://ceramics.onlinelibrary.wiley.com/doi/10.1111/j.1151-2916.1990.tb04282.x},
	doi = {10.1111/j.1151-2916.1990.tb04282.x},
	abstract = {Melting relations of SiO
              2
              were determined up to 7 GPa. The triple point of quartz‐coesite‐liquid is located at 4.5 GPa and 2450°C. The melting curve of coesite has a steep initial slope (150°C/GPa) and reaches about 2700°C at 7 GPa. Densities of the quenched glasses are also reported.},
	language = {en},
	number = {12},
	urldate = {2024-01-03},
	journal = {Journal of the American Ceramic Society},
	author = {Kanzaki, Masami},
	month = dec,
	year = {1990},
	pages = {3706--3707},
	file = {Kanzaki - 1990 - Melting of Silica up to 7 GPa.pdf:/Users/dong2j/Zotero/storage/NX4IXQHP/Kanzaki - 1990 - Melting of Silica up to 7 GPa.pdf:application/pdf},
}

@article{kuwayama_pyrite-type_2005,
	title = {The {Pyrite}-{Type} {High}-{Pressure} {Form} of {Silica}},
	volume = {309},
	url = {http://www.jstor.org/stable/3842602},
	language = {en},
	number = {5736},
	journal = {Science},
	author = {Kuwayama, Yasuhiro and Hirose, Kei and Sata, Nagayoshi and Ohishi, Yasuo},
	year = {2005},
	pages = {923--925},
	file = {Kuwayama et al. - 2005 - The Pyrite-Type High-Pressure Form of Silica.pdf:/Users/dong2j/Zotero/storage/JJXVR2YQ/Kuwayama et al. - 2005 - The Pyrite-Type High-Pressure Form of Silica.pdf:application/pdf},
}

@article{murakami_stability_2003,
	title = {Stability of {CaCl}$_{\textrm{2}}$‐type and α‐{PbO}$_{\textrm{2}}$‐type {SiO}$_{\textrm{2}}$ at high pressure and temperature determined by in‐situ {X}‐ray measurements},
	volume = {30},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2002GL016722},
	doi = {10.1029/2002GL016722},
	abstract = {Here we report the phase boundary between CaCl
              2
              ‐type and α‐PbO
              2
              ‐type silica at high pressure and temperature up to 151 GPa and 2500‐K determined by in‐situ X‐ray measurements in a laser‐heated diamond anvil cell. Amorphous silica was used as starting material, and the sample was heated for more than 1.5 hr to examine the kinetic effects. The results demonstrated that the CaCl
              2
              ‐type silica is a post‐stishovite phase and that it undergoes further transition to the α‐PbO
              2
              ‐type structure above 121 GPa at 2400‐K. Present data together with previous first‐principles calculations indicate that the phase boundary between CaCl
              2
              ‐type and α‐PbO
              2
              ‐type silica is represented by a linear equation P (GPa) = 98 + (0.0095 ± 0.0016) * T (K). The α‐PbO
              2
              ‐type silica can be present in the deep portion of the lower mantle in the silica‐saturated bulk compositions. This phase transition might contribute to the seismic wave velocity anomalies observed in the D″ region.},
	language = {en},
	number = {5},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Murakami, Motohiko and Hirose, Kei and Ono, Shigeaki and Ohishi, Yasuo},
	month = mar,
	year = {2003},
	pages = {2002GL016722},
	file = {Murakami et al. - 2003 - Stability of CaCl 2 ‐type and α‐PbO su.pdf:/Users/dong2j/Zotero/storage/MC2YNSXW/Murakami et al. - 2003 - Stability of CaCl 2 ‐type and α‐PbO su.pdf:application/pdf},
}

@article{nishihara_p-v-t_2005,
	title = {P-{V}-{T} equation of state of stishovite to the mantle transition zone conditions},
	volume = {31},
	issn = {0342-1791, 1432-2021},
	url = {http://link.springer.com/10.1007/s00269-004-0426-7},
	doi = {10.1007/s00269-004-0426-7},
	abstract = {In-situ synchrotron X-ray diﬀraction experiments were conducted using the SPEED-1500 multi-anvil press of SPring-8 on stishovite SiO2 and pressure-volume-temperature data were collected at up to 22.5 GPa and 1,073 K, which corresponds to the pressure conditions of the base of the mantle transition zone. The analysis of room-temperature data yielded V0=46.56(1) A˚ 3, KT0=296(5) GPa and K¢T=4.2(4), and these properties were consistent with the subsequent thermal equation of state (EOS) analyses. A ﬁt of the present data to high-temperature Birch-Murnaghan EOS yielded (¶KT/¶T )P=À0.046(5) GPa KÀ1 and a=a+bT with values of a=1.26(11)·10–5K–1 and b=1.29(17)·10–8 K–2. A ﬁt to the thermal pressure EOS gives a0=1.62(9)·10À5 K–1, (¶KT/¶T)V=À0.027(4) GPa KÀ1 and (¶2P/¶T 2)V=27(5)·10–7 GPa KÀ2. The lattice dynamical approach by Mie-Gru¨ neisen-Debye EOS yielded c0=1.33(6), q=6.1(8) and h0=1160(120) K. The strong volume dependence of the thermal pressure of stishovite was revealed by the analysis of present data, which was not detectable by the previous high-temperature data at lower pressures, and this yields (¶KT/ ¶T )V „ 0 and q „ 1. The analyses for the ﬁctive volume for a and c axes show that relative stiﬀness of c axis to a axis is similar both on compression and thermal expansion. Present EOS enables the accurate estimate of density of SiO2 in the deep mantle conditions.},
	language = {en},
	number = {10},
	urldate = {2024-01-03},
	journal = {Physics and Chemistry of Minerals},
	author = {Nishihara, Yu and Nakayama, Keisuke and Takahashi, Eiichi and Iguchi, Tomohiro and Funakoshi, Ken-ichi},
	month = feb,
	year = {2005},
	pages = {660--670},
	file = {Nishihara et al. - 2005 - P - V - T equation of state of stishovite to the m.pdf:/Users/dong2j/Zotero/storage/UWKCRX6C/Nishihara et al. - 2005 - P - V - T equation of state of stishovite to the m.pdf:application/pdf},
}

@article{nomura_precise_2010,
	title = {Precise determination of post-stishovite phase transition boundary and implications for seismic heterogeneities in the mid-lower mantle},
	volume = {183},
	issn = {00319201},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0031920110001585},
	doi = {10.1016/j.pepi.2010.08.004},
	abstract = {The phase transition boundary between stishovite and CaCl2-type structure in pure SiO2 was investigated at 45–75 GPa and 300–2490 K based on the in situ X-ray diffraction measurements in a laser-heated diamond-anvil cell (LHDAC). Results show that the boundary has a positive dP/dT slope of 11.1 MPa/K and the transition occurs about 70 GPa at 2200 K along the typical mantle geotherm. This corresponds to a depth of 1700 km, somewhat shallower than the previous estimate. Seismic heterogeneities have been found in a wide depth range from 800 to 1850 km in the upper to middle layers of the lower mantle. The post-stishovite phase transition is known to be ferroelastic-type, which causes a considerable reduction in shear modulus, leading to a large slow shear velocity anomaly. The almost pure SiO2 phase included in subducted crustal materials may be therefore responsible for the relatively deep mid-lower mantle seismic heterogeneities. The shallow lower mantle anomalies are possibly caused by the similar phase transition in SiO2 phase containing Al2O3 and H2O or by the phase transition in Al-bearing CaSiO3 perovskite from cubic to tetragonal structure.},
	language = {en},
	number = {1-2},
	urldate = {2024-01-03},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Nomura, Ryuichi and Hirose, Kei and Sata, Nagayoshi and Ohishi, Yasuo},
	month = nov,
	year = {2010},
	pages = {104--109},
	file = {Nomura et al. - 2010 - Precise determination of post-stishovite phase tra.pdf:/Users/dong2j/Zotero/storage/686YEDVI/Nomura et al. - 2010 - Precise determination of post-stishovite phase tra.pdf:application/pdf},
}

@article{ono_post-stishovite_2002,
	title = {Post-stishovite phase boundary in {SiO}$_{\textrm{2}}$ determined by in situ {X}-ray observations},
	volume = {197},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X0200479X},
	doi = {10.1016/S0012-821X(02)00479-X},
	abstract = {A laser heating diamond anvil cell experiment, with an angle-dispersive X-ray diffraction using synchrotron radiation source at the SPring-8, has been developed to observe the phase transition in silica (SiO2) between the P42/ mnm (rutile-type) and Pnnm (CaCl2-type) up to pressures of 100 GPa and at temperatures up to 2200 K. The transition was observed in the vicinity of 55 GPa at room temperature, and showed a positive temperature dependence of the transition pressure. The phase boundary was determined to follow the equation P (GPa) = (51 þ 2)+(0.012 þ 0.005)UT (K). Our result gives a transition pressure of near 80 GPa and a depth of 1900 km at an expected lower mantle temperature of 2000{\textasciicircum}2500 K. Therefore, this SiO2 transition is not the cause of recent observations of seismic anomalies between 800 and 1600 km depth in the mid{\textasciicircum}lower mantle. ß 2002 Elsevier Science B.V. All rights reserved.},
	language = {en},
	number = {3-4},
	urldate = {2024-01-03},
	journal = {Earth and Planetary Science Letters},
	author = {Ono, Shigeaki and Hirose, Kei and Murakami, Motohiko and Isshiki, Maiko},
	month = apr,
	year = {2002},
	pages = {187--192},
	file = {Ono et al. - 2002 - Post-stishovite phase boundary in SiO2 determined .pdf:/Users/dong2j/Zotero/storage/DMVQQC45/Ono et al. - 2002 - Post-stishovite phase boundary in SiO2 determined .pdf:application/pdf},
}

@article{ono_precise_2017,
	title = {Precise determination of the phase boundary between coesite and stishovite in {SiO}$_{\textrm{2}}$},
	volume = {264},
	issn = {00319201},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0031920116301558},
	doi = {10.1016/j.pepi.2017.01.003},
	abstract = {The phase boundary between coesite and stishovite in SiO2 was determined over the range of 1200–1700 K using a multi-anvil high-pressure apparatus combined with the synchrotron X-ray diffraction technique. The stability of each phase was determined by observing the powdered X-ray diffraction data. The transition boundary between the coesite and stishovite phases was found to occur at P (GPa) = 4.7 + 0.0031 Â T (K). The transition pressure determined in this study was in general agreement with what was observed in previous high-pressure experiments and heat capacity measurements. However, the slope of the transition, dP/dT, determined in our study was higher than that estimated in a previous study utilized with the in situ X-ray method. In contrast, the slope calculated by the heat capacity data was in good agreement with that determined in our study. The phase transition determined in our study occurs at around 10 GPa at the normal mantle geotherm, coinciding with the seismic discontinuity around 300 km depth known as the X-discontinuity.},
	language = {en},
	urldate = {2024-01-03},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Ono, Shigeaki and Kikegawa, Takumi and Higo, Yuji and Tange, Yoshinori},
	month = mar,
	year = {2017},
	pages = {1--6},
	file = {Ono et al. - 2017 - Precise determination of the phase boundary betwee.pdf:/Users/dong2j/Zotero/storage/KA9YSBGW/Ono et al. - 2017 - Precise determination of the phase boundary betwee.pdf:application/pdf},
}

@article{pigott_highpressure_2015,
	title = {High‐pressure, high‐temperature equations of state using nanofabricated controlled‐geometry {Ni}/{SiO} $_{\textrm{2}}$ /{Ni} double hot‐plate samples},
	volume = {42},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1002/2015GL066577},
	doi = {10.1002/2015GL066577},
	abstract = {We have fabricated novel controlled-geometry samples for the laser-heated diamond-anvil cell (LHDAC) in which a transparent oxide layer (SiO2) is sandwiched between two laser-absorbing layers (Ni) in a single, cohesive sample. The samples were mass manufactured ({\textgreater}104 samples) using a combination of physical vapor deposition, photolithography, and wet and plasma etching. The double hot-plate arrangement of the samples, coupled with the chemical and spatial homogeneity of the laser-absorbing layers, addresses problems of spatial temperature heterogeneities encountered in previous studies where simple mechanical mixtures of transparent and opaque materials were used. Here we report thermal equations of state (EOS) for nickel to 100 GPa and 3000 K and stishovite to 50 GPa and 2400 K obtained using the LHDAC and in situ synchrotron X-ray microdiffraction. We discuss the inner core composition and the stagnation of subducted slabs in the mantle based on our reﬁned thermal EOS.},
	language = {en},
	number = {23},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Pigott, Jeffrey S. and Ditmer, Derek A. and Fischer, Rebecca A. and Reaman, Daniel M. and Hrubiak, Rostislav and Meng, Yue and Davis, Robert J. and Panero, Wendy R.},
	month = dec,
	year = {2015},
	file = {Pigott et al. - 2015 - High‐pressure, high‐temperature equations of state.pdf:/Users/dong2j/Zotero/storage/TPJDPWRY/Pigott et al. - 2015 - High‐pressure, high‐temperature equations of state.pdf:application/pdf},
}

@article{serghiou_coesitestishovite_1995,
	title = {The {Coesite}‐{Stishovite} {Transition} in a laser‐heated diamond cell},
	volume = {22},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/94GL02692},
	doi = {10.1029/94GL02692},
	abstract = {The coesite‐stishovite phase boundary in the temperature range 2300–2630°C was examined in a CO
              2
              ‐laser heated diamond anvil cell using argon as a pressure medium. Phase identification was provided by Raman spectroscopy of the temperature quenched samples at pressure. Our results suggest a coesite‐stishovite phase boundary curve described by P(GPa) = 8.1 + 0.001T(°C) in good agreement with
              Yagi and Akimoto's
              (1976) estimate at lower temperatures. The slope of this curve is less than one half that determined recently by
              Zhang et al.
              [1993, 1994] in a multi‐anvil press.},
	language = {en},
	number = {4},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Serghiou, G. and Zerr, A. and Chudinovskikh, L. and Boehler, R.},
	month = feb,
	year = {1995},
	pages = {441--444},
	file = {Serghiou et al. - 1995 - The Coesite‐Stishovite Transition in a laser‐heate.pdf:/Users/dong2j/Zotero/storage/9RXYYG7K/Serghiou et al. - 1995 - The Coesite‐Stishovite Transition in a laser‐heate.pdf:application/pdf},
}

@article{shen_measurement_1995,
	title = {Measurement of melting temperatures of some minerals under lower mantle pressures},
	volume = {100},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/95JB01864},
	doi = {10.1029/95JB01864},
	abstract = {Meltingtemperaturme easuremenotsf sixminerals(stishovite(SiO2), corundum(A1203d),iopside(CaMgSi206),andthreeperovskite(sMgSiO3,CaSiO3, Mg3AI2Si3012)a) thighpressurewserecarriedoutin a YAG laser-heateddiamondanvilcellwith rheniummetalasan absorberof thelaserlight.A polishedor compressediscof thesamplewas in contactwith rheniumfoil andheatedby conductionM. elting wasdeterminedby plottinglaser power/samplteemperaturfeunctionandlookingfor thethermalanomalyassociatewdiththefusion of materialsA. ll thesesolidswerefoundtobehighlyrefractoryr,equiringquitehightemperatures for meltingat thelowermantlepressuresT.heexperimentaml eltingresultsshowedthatfor these mineralsm, eltingtemperatureisncreasedwithincreasingpressureO. urresultsatlow pressureasre consistenwt ith thedatadeterminedby othertechnique(spiston-cylindemr, ultianvils)T. hehighpressurme eltingof MgSiO3perovskiteagreedwiththerecentmeasuremenbtsyZerrandBoehler (1993)withinexperimentaulncertaintieMs.eltingtemperatureasndmeltingslopesof CaSiO3and Mg3AI2Si3012perovskiteswerefoundto belessthanthoseof MgSiO3perovskitei,ndicatingthat thepresenceof Ca andA1woulddecreastehemeltingtemperatureosf MgSiO3perovskitein the Earth'slowermantleandthatthiseffectwill increasewith increasingpressuresM. elting temperaturme easuremenotsnstishovitaendcorundumtopressureosf 36 GPaand25 GPa, respectivelya, rereported.},
	language = {en},
	number = {B9},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Shen, Guoyin and Lazor, Peter},
	month = sep,
	year = {1995},
	pages = {17699--17713},
	file = {Shen and Lazor - 1995 - Measurement of melting temperatures of some minera.pdf:/Users/dong2j/Zotero/storage/ZCSJPZJJ/Shen and Lazor - 1995 - Measurement of melting temperatures of some minera.pdf:application/pdf},
}

@article{shieh_x-ray_2005,
	title = {X-ray diffraction study of phase stability in {SiO}$_{\textrm{2}}$ at deep mantle conditions},
	volume = {235},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X05002165},
	doi = {10.1016/j.epsl.2005.04.004},
	abstract = {The stability of SiO2 phases were examined by X-ray diffraction at pressure up to 131 GPa and temperature N1300 K, corresponding to Earth’s deep lower mantle conditions. Three materials, stishovite, cristobalite, and silica glass were used as starting materials, and an argon pressure-transmitting medium was loaded with the sample for five out of six sets of laser-heated diamond cell experiments. X-ray fluorescent crystals were loaded with the sample to ensure alignment of X-ray beam and heating laser. Our results from three different staring materials indicate that the CaCl2-type phase is the stable phase throughout our studied P–T range. We observe the a-PbO2-type phase for cristobalite starting material at pressures greater than 48 GPa at room temperature. However, this transforms to the CaCl2-type structure upon heating between 72–113 GPa. Transition kinetics and metastability may be important in explaining differences in results reported above 75 GPa, and key experimental variables are discussed.},
	language = {en},
	number = {1-2},
	urldate = {2024-01-03},
	journal = {Earth and Planetary Science Letters},
	author = {Shieh, S and Duffy, T and Shen, G},
	month = jun,
	year = {2005},
	pages = {273--282},
	file = {Shieh et al. - 2005 - X-ray diffraction study of phase stability in SiO .pdf:/Users/dong2j/Zotero/storage/3D2YNYRY/Shieh et al. - 2005 - X-ray diffraction study of phase stability in SiO .pdf:application/pdf},
}

@article{sun_high_2019,
	title = {High {Pressure}‐{Temperature} {Study} on the {Thermal} {Equations} of {State} of {Seifertite} and {CaCl}$_{\textrm{2}}$‐{Type} {SiO}$_{\textrm{2}}$},
	volume = {124},
	issn = {2169-9313, 2169-9356},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2019JB017853},
	doi = {10.1029/2019JB017853},
	abstract = {In this study, we have determined the thermal equations of state (EoS) of CaCl2‐type SiO2 and seifertite (α‐PbO2‐type SiO2) from 55 to 147 GPa up to 3500 K using X‐ray diffraction in laser‐heated diamond anvil cells. The phase transition from stishovite to CaCl2‐type SiO2 is in good agreement with previous experimental results, whereas the transition from CaCl2‐type SiO2 to seifertite was observed to strongly rely on the starting material. For CaCl2‐type SiO2, we obtained a bulk modulus, KT0 = 245(7) GPa with a ﬁxed KT′ = 4, V0 = 48.1(2) Å3, γ0 = 1.3(3), q = 1(ﬁxed), and θD0 = 1100(400) K. Seifertite has a greater KT0 = 290(10) GPa (KT′ = 4 ﬁxed) than CaCl2‐type SiO2. Other thermoelastic parameters of seifertite are V0 = 92.3(5) Å3, γ0 = 1.6(2), q = 1 (ﬁxed), and θD0 = 1600(200) K. Using the obtained results and phase boundary in previous studies, we have found that the phase transition from stishovite to CaCl2‐type SiO2 cannot cause a noticeable change in density but can lower the bulk sound velocity (VФ) by {\textasciitilde}10\%. This phase transition in the subducted oceanic crust with 20 vol.\% SiO2 was estimated to generate a {\textasciitilde}2\% discontinuity in VФ, which could be related to the observed seismic velocity anomalies at depths of 1,400–1,800 km. At the bottom of the lower mantle, CaCl2‐type SiO2 to seifertite phase transition can lead to a 0.3\% jump in ρ and a 0.8\% jump in VΦ considering 20 vol.\% SiO2 in the subducted mid‐ocean ridge basalt, which may contribute to the formation of the D″ discontinuity above the core‐mantle boundary.},
	language = {en},
	number = {12},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Sun, Ningyu and Shi, Weigang and Mao, Zhu and Zhou, Cijin and Prakapenka, Vitali B.},
	month = dec,
	year = {2019},
	pages = {12620--12630},
	file = {Sun (2019) - Supplementary Information.doc:/Users/dong2j/Zotero/storage/S8LMJ5U9/Sun (2019) - Supplementary Information.doc:application/msword;Sun et al. - 2019 - High Pressure‐Temperature Study on the Thermal Equ.pdf:/Users/dong2j/Zotero/storage/KN7RB4M5/Sun et al. - 2019 - High Pressure‐Temperature Study on the Thermal Equ.pdf:application/pdf},
}

@article{wang_pvt_2012,
	title = {\textit{{P}}‐\textit{{V}}‐\textit{{T}} equation of state of stishovite up to mid‐lower mantle conditions},
	volume = {117},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2011JB009100},
	doi = {10.1029/2011JB009100},
	abstract = {In situ
              P
              ‐
              V
              ‐
              T
              measurements of stishovite have been performed throughout its stability field from 17 to 54 GPa and from 300 to 1700 K, by using a sintered‐diamond multianvil apparatus and synchrotron radiations. The
              P
              ‐
              V
              ‐
              T
              equation of state of stishovite was precisely determined on the basis of the Mie‐Grüneisen‐Debye model using both Morse‐Rydberg (Vinet) and third‐order Burch‐Murnaghan equations for reference isotherms. The new equation of state of stishovite gives the thermoelastic properties such as density, adiabatic bulk modulus, thermal expansivity, and isobaric heat capacity without extrapolation to mid‐lower mantle conditions, and these properties at zero pressures are consistent with those of previous measurements. The present equation of state yields a lower density and larger adiabatic modulus at lower mantle conditions compared to those obtained by extrapolate on using a previous equation of state determined at upper mantle conditions. Our new equation of state and thermoelastic properties for stishovite at lower mantle conditions is important for quantitatively modeling the fate of subducted silica‐rich rocks such as MORB and pelagic sediments, and for interpreting seismological observations.
            
          , 
            Key Points
            
              
                
                  P‐V‐T states of stishovite were measured up to 54 GPa and 1700 K
                
                
                  P‐V‐T EOS of stishovite was determined in the entire stability field
                
                
                  Thermodynamic and elastic properties of stishovite were precisely determined},
	language = {en},
	number = {B6},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Wang, Fulong and Tange, Yoshinori and Irifune, Tetsuo and Funakoshi, Ken‐ichi},
	month = jun,
	year = {2012},
	pages = {2011JB009100},
	file = {Wang et al. - 2012 - P ‐ V ‐ T equation of state o.pdf:/Users/dong2j/Zotero/storage/FDIE6CWC/Wang et al. - 2012 - P ‐ V ‐ T equation of state o.pdf:application/pdf},
}

@article{yagi_direct_1976,
	title = {Direct determination of coesite-stishovite transition by in-situ {X}-ray measurements},
	volume = {35},
	issn = {00401951},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0040195176900421},
	doi = {10.1016/0040-1951(76)90042-1},
	language = {en},
	number = {1-3},
	urldate = {2024-01-03},
	journal = {Tectonophysics},
	author = {Yagi, Takehiko and Akimoto, Syun-Iti},
	month = oct,
	year = {1976},
	pages = {259--270},
	file = {Yagi and Akimoto - 1976 - Direct determination of coesite- stishovite transi.pdf:/Users/dong2j/Zotero/storage/GNFUR8SE/Yagi and Akimoto - 1976 - Direct determination of coesite- stishovite transi.pdf:application/pdf},
}

@article{yamazaki_over_2014,
	title = {Over 1 {Mbar} generation in the {Kawai}-type multianvil apparatus and its application to compression of ({Mg}$_{\textrm{0.92}}${Fe}$_{\textrm{0.08}}$){SiO}$_{\textrm{3}}$ perovskite and stishovite},
	volume = {228},
	issn = {00319201},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0031920114000144},
	doi = {10.1016/j.pepi.2014.01.013},
	language = {en},
	urldate = {2024-01-03},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Yamazaki, D. and Ito, E. and Yoshino, T. and Tsujino, N. and Yoneda, A. and Guo, X. and Xu, F. and Higo, Y. and Funakoshi, K.},
	month = mar,
	year = {2014},
	pages = {262--267},
	file = {Yamazaki et al. - 2014 - Over 1 Mbar generation in the Kawai-type multianvi.pdf:/Users/dong2j/Zotero/storage/KGACIQ7F/Yamazaki et al. - 2014 - Over 1 Mbar generation in the Kawai-type multianvi.pdf:application/pdf},
}

@article{zhang_melting_1993,
	title = {Melting and subsolidus relations of {SiO}$_{\textrm{2}}$ at 9–14 {GPa}},
	volume = {98},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/93JB02218},
	doi = {10.1029/93JB02218},
	abstract = {Experiments were performed on amorphous silica at temperatures of 1000°–2850°C and pressures of 9–14 GPa using a 2000‐t uniaxial split‐sphere multianvil apparatus (USSA‐2000). The melting curve of coesite was extended from 8 to 13.7 GPa, and the melting temperatures indicate a slope that is almost independent of pressure. Melting of stishovite was observed at 2850°C and 14 GPa. The triple point for coexisting coesite, stishovite, and melt was located at 2800°C and 13.7 GPa. The coesite‐stishovite phase transition was determined between 2000° and 2800°C and is described by the equation
              P
              (GPa) = 5.8(4) + 0.0028(2)
              T
              (°C). The resulting
              dP/dT
              slope is more than twice that determined in the in situ X ray study of Yagi and Akimoto (1976). The present coesite‐stishovite boundary cannot be predicted by existing thermodynamic data (e.g., Fei et al., 1990), which suggests some uncertainties in the extrapolation of heat capacities of coesite and stishovite at high temperatures. Thermodynamic extrapolations of the metastable melting curves of quartz and coesite show a strongly negative slope and thus are consistent with the proposal that the room temperature amorphization of quartz and coesite results from crossing of the metastable extension of their melting curves.},
	language = {en},
	number = {B11},
	urldate = {2024-01-03},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Zhang, Jianzhong and Liebermann, Robert C. and Gasparik, Tibor and Herzberg, Claude T. and Fei, Yingwei},
	month = nov,
	year = {1993},
	pages = {19785--19793},
	file = {Zhang et al. - 1993 - Melting and subsolidus relations of SiO 2su.pdf:/Users/dong2j/Zotero/storage/L34AA4LG/Zhang et al. - 1993 - Melting and subsolidus relations of SiO 2su.pdf:application/pdf},
}

@article{zhang_situ_1996,
	title = {In situ {X}-ray observations of the coesite-stishovite transition: reversed phase boundary and kinetics},
	volume = {23},
	issn = {0342-1791, 1432-2021},
	shorttitle = {In situ {X}-ray observations of the coesite-stishovite transition},
	url = {http://link.springer.com/10.1007/BF00202987},
	doi = {10.1007/BF00202987},
	abstract = {Using a DIA-type, cubic-anvil, high-pressure apparatus (SAM-85) in conjunction with in situ X-ray diffraction, we have investigated phase relations between coesite and stishovite up to 12 GPa and 1530 {\textasciitilde} using synthetic powders of the two phases as the starting materials. The phase transition between coesite and stishovite was identified by observing the first appearance of a phase that did not already exist or by a change in the relative intensity of the two patterns. In most experiments, the diffraction patterns on samples were collected within 10 minutes after reaching a pressure and temperature condition. On this time scale, two phase boundaries associated with the coesite-stishovite transition have been determined: (1) for the stishovite-to-coesite transition, observations were made in the temperature range of 950-1530 {\textasciitilde} and (2) for the coesite-to-stishovite transition from 500 to 1300 {\textasciitilde} These observations reveal that there exists a critical temperature of about 1000 {\textasciitilde} to constrain the coesite-stishovite equilibrium phase boundary. Above this temperature, both boundaries are linear, have positive dP/dT slopes, and lie within a pressure interval of 0.4 GPa. Below this temperature, the dP/ dT slope for the stishovite-to-coesite phase boundary becomes significantly larger and that for the coesite-tostishovite phase boundary changes from positive to negative. As a result, an equilibrium phase boundary can only be determined from the results above 1000{\textasciitilde} and is described by a linear equation P(GPa)=6.1(4)+ 0.0026 (2)T ({\textasciitilde} This dP/dT slope is in good agreement with that of Zhang etal. (1993) but more than twice that of Yagi and Akimoto (1976). For the kinetics of the phase transition, preliminary rate data were obtained for the stishovite-to-coesite transition at 1160 and 1430 {\textasciitilde} and are in agreement with the simple geometric transformation model of Avrami and Cahn.},
	language = {en},
	number = {1},
	urldate = {2024-01-03},
	journal = {Physics and Chemistry of Minerals},
	author = {Zhang, Jianzhong and Li, Baosheng and Utsumi, Wataru and Liebermann, RobertC.},
	month = feb,
	year = {1996},
	file = {Zhang et al. - 1996 - In situ X-ray observations of the coesite-stishovi.pdf:/Users/dong2j/Zotero/storage/ZRKLPWEE/Zhang et al. - 1996 - In situ X-ray observations of the coesite-stishovi.pdf:application/pdf},
}

@incollection{k_suito_phase_1977,
	address = {New York},
	title = {Phase relations of pure {Mg}$_{\textrm{2}}${SiO}$_{\textrm{4}}$ up to 200 kilobars},
	booktitle = {High-{Pressure} {Research}: {Applications} in {Geophysics}},
	publisher = {Academic Press},
	author = {{K. Suito}},
	year = {1977},
	pages = {255--266},
	file = {Suito (1977) book chapter.pdf:/Users/dong2j/Zotero/storage/Z6CUWNJF/Suito (1977) book chapter.pdf:application/pdf},
}

@misc{geng_ab_2023,
	title = {Ab initio constraints on silica melting to 500 {GPa}},
	url = {http://arxiv.org/abs/2307.05444},
	abstract = {The melting curve of pure silica (SiO\$\_2\$) was determined using \{{\textbackslash}it ab initio\} density functional theory together with the solid-liquid coexisting approach, thermodynamic integration and the Z method. The melting curves are consistent with a smooth slow increase in a large region from 50 GPa (dT/dP \${\textbackslash}approx\$ 15 K/GPa) to about 500 GPa (dT/dP \${\textbackslash}approx\$ 5 K/GPa) without any abrupt changes at around 120 GPa and 300 GPa as seen in some recent experimental and computational studies. The topography of the melting curve above 50 GPa is consistent with a gradual change in the distribution of the Si coordination numbers in the liquid state and the absence of large changes in the density following solid-solid phase transitions. The pair distribution functions show that the structural correlation in the liquid is mainly short-ranged and that the Si-O bond is stiff. The densification of the melt structure with pressure above 50 GPa is therefore due to an increase in 7- and 8-fold coordinated silicon.},
	language = {en},
	urldate = {2024-01-09},
	publisher = {arXiv},
	author = {Geng, Ming and Mohn, Chris E.},
	month = nov,
	year = {2023},
	note = {arXiv:2307.05444 [cond-mat, physics:physics]},
	keywords = {Condensed Matter - Materials Science, Physics - Geophysics},
	file = {Geng and Mohn - 2023 - Ab initio constraints on silica melting to 500 GPa.pdf:/Users/dong2j/Zotero/storage/CBPC3K2L/Geng and Mohn - 2023 - Ab initio constraints on silica melting to 500 GPa.pdf:application/pdf},
}

@article{usui_ab_2010,
	title = {Ab initio two-phase molecular dynamics on the melting curve of {SiO2}},
	volume = {21},
	issn = {1674-487X, 1867-111X},
	url = {http://link.springer.com/10.1007/s12583-010-0126-9},
	doi = {10.1007/s12583-010-0126-9},
	abstract = {Ab initio two-phase molecular dynamics simulations were performed on silica at pressures of 20–160 GPa and temperatures of 2 500–6 000 K to examine its solid-liquid phase boundary. Results indicate a melting temperature (Tm) of 5 900 K at 135 GPa. This is 1 100 K higher than the temperature considered for the core-mantle boundary (CMB) of about 3 800 K. The calculated melting temperature is fairly consistent with classical MD (molecular dynamics) simulations. For liquid silica, the O-O coordination number is found to be 12 along the Tm and is almost unchanged with increasing pressure. The self-diffusion coefficients of O and Si atoms are determined to be 1.3×10-9–3.3×10-9 m2/s, and the viscosity is 0.02–0.03 Pa·s along the Tm. We find that these transport properties depend less on pressure in the wide range up of more than 135 GPa. The eutectic temperatures in the MgO-SiO2 systems were evaluated and found to be 700 K higher than the CMB temperature, though they would decrease considerably in more realistic mantle compositions.},
	language = {en},
	number = {5},
	urldate = {2024-01-09},
	journal = {Journal of Earth Science},
	author = {Usui, Yusuke and Tsuchiya, Taku},
	month = oct,
	year = {2010},
	pages = {801--810},
	file = {Usui and Tsuchiya - 2010 - Ab initio two-phase molecular dynamics on the melt.pdf:/Users/dong2j/Zotero/storage/KMRNXGWA/Usui and Tsuchiya - 2010 - Ab initio two-phase molecular dynamics on the melt.pdf:application/pdf},
}

@article{gonzalez-cataldo_melting_2016,
	title = {Melting curve of {SiO2} at multimegabar pressures: implications for gas giants and super-{Earths}},
	volume = {6},
	issn = {2045-2322},
	shorttitle = {Melting curve of {SiO2} at multimegabar pressures},
	url = {https://www.nature.com/articles/srep26537},
	doi = {10.1038/srep26537},
	abstract = {Abstract
            
              Ultrahigh-pressure phase boundary between solid and liquid SiO
              2
              is still quite unclear. Here we present predictions of silica melting curve for the multimegabar pressure regime, as obtained from first principles molecular dynamics simulations. We calculate the melting temperatures from three high pressure phases of silica (pyrite-, cotunnite-, and Fe
              2
              P-type SiO
              2
              ) at different pressures using the Z method. The computed melting curve is found to rise abruptly around 330 GPa, an increase not previously reported by any melting simulations. This is in close agreement with recent experiments reporting the
              α
              -PbO
              2
              –pyrite transition around this pressure. The predicted phase diagram indicates that silica could be one of the dominant components of the rocky cores of gas giants, as it remains solid at the core of our Solar System’s gas giants. These results are also relevant to model the interior structure and evolution of massive super-Earths.},
	language = {en},
	number = {1},
	urldate = {2024-01-21},
	journal = {Scientific Reports},
	author = {González-Cataldo, Felipe and Davis, Sergio and Gutiérrez, Gonzalo},
	year = {2016},
	pages = {26537},
	file = {Full Text:/Users/dong2j/Zotero/storage/YRVZV5HY/González-Cataldo et al. - 2016 - Melting curve of SiO2 at multimegabar pressures i.pdf:application/pdf},
}

@article{ghiorso_equation_2004,
	title = {An equation of state for silicate melts. {I}. {Formulation} of a general model},
	volume = {304},
	issn = {0002-9599},
	url = {http://www.ajsonline.org/cgi/doi/10.2475/ajs.304.8-9.637},
	doi = {10.2475/ajs.304.8-9.637},
	abstract = {A simple, empirical, volume-explicit equation of state (EOS) is developed for use in describing the volumetric properties of materials that exhibit large thermal expansivities and strongly non-linear, pressure-dependent compressibilities. Existing and commonly used EOS expressions, like the Universal and BirchMurnaghan equations, develop singularities at critical values of temperature and pressure that prevent the calculation of derived thermodynamic properties for this class of substances. The proposed EOS reduces to a simple polynomial form at low-pressure; this form is utilized in the literature to describe the properties of silicate melts at 105 Pa. At high-pressures, the proposed EOS can be parameterized to yield a ﬁnite, non-zero volume limit, unlike other formulations. Thermodynamic properties can be calculated using the proposed EOS without the need for iterative solutions and all derivative and integral representations of the equation are analytic.},
	language = {en},
	number = {8-9},
	urldate = {2024-01-09},
	journal = {American Journal of Science},
	author = {Ghiorso, M. S.},
	month = oct,
	year = {2004},
	pages = {637--678},
	file = {Ghiorso - 2004 - An equation of state for silicate melts. I. Formul.pdf:/Users/dong2j/Zotero/storage/EYTYX77V/Ghiorso - 2004 - An equation of state for silicate melts. I. Formul.pdf:application/pdf},
}

%% MgSiO3 %%

@article{angel_structure_1989,
	title = {Structure and twinning of single-crystal {MgSiO3} garnet synthesized at 17 {GPa} and 1800°{C}},
	volume = {74},
	language = {en},
	number = {3-4},
	journal = {American Mineralogist},
	author = {Angel, R. J. and Finger, L. W. and Hazen, R. M. and Kanzaki, M. and Weidner, D. J. and Liebermann, R. C. and Veblen, D. R.},
	year = {1989},
	pages = {509--512},
	file = {PDF:/Users/jdong/Zotero/storage/EM6XFE44/ANcBL et al. - Structure and twinning of single-crystalMgSiO3 garnet synthesizedat 17 GPa and 1800'C.pdf:application/pdf},
}


@article{hirose_postperovskite_2006,
	title = {Postperovskite phase transition and its geophysical implications},
	volume = {44},
	issn = {8755-1209, 1944-9208},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2005RG000186},
	doi = {10.1029/2005RG000186},
	abstract = {The stability of (Mg,Fe)SiO
              3
              perovskite in the deep lower mantle has long been uncertain. Recently, a phase transition from perovskite to postperovskite was discovered through a significant change in the X‐ray diffraction pattern at high‐pressure and high‐temperature conditions corresponding to the core‐mantle boundary region. This phase transition was also confirmed by first‐principles calculations. These suggest that (Mg,Fe)SiO
              3
              postperovskite is the predominant mineral in the lowermost mantle called the D″ layer, and phase transition from perovskite to postperovskite has significant geophysical implications for its nature and dynamics. The postperovskite phase may account for the large seismic anomalies observed in the D″ region, such as the D″ discontinuity,
              S
              wave anisotropy, and anticorrelation between the anomalies in
              S
              wave and bulk sound velocities. In addition, this phase transition is a strongly exothermic reaction. It destabilizes the thermal boundary layer at the base of the mantle and should promote the formation of high‐temperature upwelling plumes.},
	language = {en},
	number = {3},
	urldate = {2024-01-21},
	journal = {Reviews of Geophysics},
	author = {Hirose, Kei},
	year = {2006},
	pages = {2005RG000186},
}

@article{fei_melting_2021,
	title = {Melting and density of {MgSiO}$_{\textrm{3}}$ determined by shock compression of bridgmanite to {1254GPa}},
	volume = {12},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-021-21170-y},
	doi = {10.1038/s41467-021-21170-y},
	abstract = {Abstract
            
              The essential data for interior and thermal evolution models of the Earth and super-Earths are the density and melting of mantle silicate under extreme conditions. Here, we report an unprecedently high melting temperature of MgSiO
              3
              at 500 GPa by direct shockwave loading of pre-synthesized dense MgSiO
              3
              (bridgmanite) using the Z Pulsed Power Facility. We also present the first high-precision density data of crystalline MgSiO
              3
              to 422 GPa and 7200 K and of silicate melt to 1254 GPa. The experimental density measurements support our density functional theory based molecular dynamics calculations, providing benchmarks for theoretical calculations under extreme conditions. The excellent agreement between experiment and theory provides a reliable reference density profile for super-Earth mantles. Furthermore, the observed upper bound of melting temperature, 9430 K at 500 GPa, provides a critical constraint on the accretion energy required to melt the mantle and the prospect of driving a dynamo in massive rocky planets.},
	language = {en},
	number = {1},
	urldate = {2024-01-01},
	journal = {Nature Communications},
	author = {Fei, Yingwei and Seagle, Christopher T. and Townsend, Joshua P. and McCoy, Chad A. and Boujibar, Asmaa and Driscoll, Peter and Shulenburger, Luke and Furnish, Michael D.},
	month = feb,
	year = {2021},
	pages = {876},
	file = {Fei et al. - 2021 - Melting and density of MgSiO3 determined by shock .pdf:/Users/dong2j/Zotero/storage/Q6CFPA8C/Fei et al. - 2021 - Melting and density of MgSiO3 determined by shock .pdf:application/pdf},
}
%%%%%%%%
@article{zhou_sound_2021,
	title = {Sound {Velocity} of {MgSiO}$_{\textrm{3}}$ {Majorite} {Garnet} up to 18 {GPa} and 2000 {K}},
	volume = {48},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2021GL093499},
	doi = {10.1029/2021GL093499},
	abstract = {Abstract
            
              MgSiO
              3
              majorite is the most significant endmember of the Al‐deficient majorite garnets that form at depths higher than ∼400 km, in the mantle transition zone (MTZ). Here, we report elastic wave velocity measurements on polycrystalline MgSiO
              3
              majorite samples, up to 18.4 GPa and 2000 K by ultrasonic interferometry techniques combined with in situ X‐ray diffraction measurements in a multianvil apparatus. Our data show MgSiO
              3
              majorite has the lowest elastic moduli among silicate garnet endmembers, under the pressure and temperature conditions of the MTZ. These new data combined with those of other garnet endmembers allowed to estimate
              V
              
                P
              
              and
              V
              
                S
              
              of majorite with compositions relevant to the MTZ. The results suggest that variation of MgSiO
              3
              component in garnet may play a role for interpreting seismic gradients atop the 410‐km discontinuity while below ∼520 km, the velocity contrasts hold too low values to explain the discrepancy between mineral physics data and seismological observations.
            
          , 
            Plain Language Summary
            
              Majorite is an important constituent of mantle garnet that form at depths higher than ∼400 km, in the Earth's mantle transition zone. Here, we report elastic wave velocity measurements on polycrystalline MgSiO
              3
              majorite samples, up to 18.4 GPa and 2000 K by ultrasonic interferometry techniques combined with in situ X‐ray diffraction measurements in a multianvil apparatus. Our data show MgSiO
              3
              majorite has the lowest elastic moduli among other silicate garnets and therefore may play a role for interpreting the steep seismic gradients across the 410‐km discontinuity while below ∼520 km, it holds too low seismic contrast to explain the discrepancy between mineral physics data and seismological observations.
            
          , 
            Key Points
            
              
                
                  
                    Sound velocities of MgSiO
                    3
                    majorite were measured up to 18.4 GPa and 2000 K
                  
                
                
                  
                    Elastic softening increase gradually upon increasing MgSiO
                    3
                    content in mantle garnets
                  
                
                
                  
                    Pyrolite and mid‐ocean ridge basalts majorite are unlikely to explain the high
                    V
                    
                      P
                    
                    and
                    V
                    
                      S
                    
                    of the bottom mantle transition region},
	language = {en},
	number = {14},
	urldate = {2025-01-31},
	journal = {Geophysical Research Letters},
	author = {Zhou, Chunyin and Gréaux, Steeve and Liu, Zhaodong and Higo, Yuji and Arimoto, Takeshi and Irifune, Tetsuo},
	month = jul,
	year = {2021},
	pages = {e2021GL093499},
}

@article{yoshiasa_single-crystal_2013,
	title = {Single-crystal metastable high-temperature \textit{{C}} 2/ \textit{c} clinoenstatite quenched rapidly from high temperature and high pressure},
	volume = {69},
	issn = {2052-5192},
	url = {https://scripts.iucr.org/cgi-bin/paper?S2052519213028248},
	doi = {10.1107/S2052519213028248},
	language = {en},
	number = {6},
	urldate = {2024-11-16},
	journal = {Acta Crystallographica Section B Structural Science, Crystal Engineering and Materials},
	author = {Yoshiasa, Akira and Nakatsuka, Akihiko and Okube, Maki and Katsura, Tomoo},
	month = dec,
	year = {2013},
	pages = {541--546},
	file = {Screenshot 2024-11-15 at 9.03.31 PM.png:/Users/jdong/Zotero/storage/U3LMLJMH/Screenshot 2024-11-15 at 9.03.31 PM.png:image/png;Yoshiasa et al. - 2013 - Single-crystal metastable high-temperature Ci.pdf:/Users/jdong/Zotero/storage/XCE87M28/Yoshiasa et al. - 2013 - Single-crystal metastable high-temperature Ci.pdf:application/pdf},
}


@article{akimoto_pyroxenegarnet_1977,
	title = {Pyroxene—{Garnet} {Solid}-{Solution} {Equilibria} in the {Systems} {Mg}$_{\textrm{4}}${Si}$_{\textrm{4}}${O}$_{\textrm{12}}$—{Mg}$_{\textrm{3}}${Al}$_{\textrm{2}}${Si}$_{\textrm{3}}${O}$_{\textrm{12}}$ and {Fe}$_{\textrm{4}}${Si}$_{\textrm{4}}${O}$_{\textrm{12}}$—{Fe}$_{\textrm{3}}${Al}$_{\textrm{2}}${Si}$_{\textrm{3}}${O}$_{\textrm{12}}$ at {High} {Pressures} and {Temperatures}},
	volume = {15},
	language = {en},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Akimoto, S},
	year = {1977},
	pages = {90--106},
	file = {Pyroxene—Garnet Solid-Solution Equilibria in the Systems mg4si4o12—mg3ai2si3oj2 and fe4si4o12—fe3ai2s13o12 at High Pressures and Temperatures:/Users/dong2j/Zotero/storage/W83EVSW7/Akimoto - AT HIGH PRESSURES AND TEMPERATURES.pdf:application/pdf},
}

@article{chanyshev_depressed_2022,
	title = {Depressed 660-km discontinuity caused by akimotoite–bridgmanite transition},
	volume = {601},
	issn = {0028-0836, 1476-4687},
	url = {https://www.nature.com/articles/s41586-021-04157-z},
	doi = {10.1038/s41586-021-04157-z},
	abstract = {Abstract
            
              The 660-kilometre seismic discontinuity is the boundary between the Earth’s lower mantle and transition zone and is commonly interpreted as being due to the dissociation of ringwoodite to bridgmanite plus ferropericlase (post-spinel transition)
              1–3
              . A distinct feature of the 660-kilometre discontinuity is its depression to 750 kilometres beneath subduction zones
              4–10
              . However, in situ X-ray diffraction studies using multi-anvil techniques have demonstrated negative but gentle Clapeyron slopes (that is,  the ratio between pressure and temperature changes) of the post-spinel transition that do not allow a significant depression
              11–13
              . On the other hand, conventional high-pressure experiments face difficulties in accurate phase identification due to inevitable pressure changes during heating and the persistent presence of metastable phases
              1,3
              . Here we determine the post-spinel and akimotoite–bridgmanite transition boundaries by multi-anvil experiments using in situ X-ray diffraction, with the boundaries strictly based on the definition of phase equilibrium. The post-spinel boundary has almost no temperature dependence, whereas the akimotoite–bridgmanite transition has a very steep negative boundary slope at temperatures lower than ambient mantle geotherms. The large depressions of the 660-kilometre discontinuity in cold subduction zones are thus interpreted as the akimotoite–bridgmanite transition. The steep negative boundary of the akimotoite–bridgmanite transition will cause slab stagnation (a stalling of the slab’s descent) due to significant upward buoyancy
              14,15
              .},
	language = {en},
	number = {7891},
	urldate = {2024-01-01},
	journal = {Nature},
	author = {Chanyshev, Artem and Ishii, Takayuki and Bondar, Dmitry and Bhat, Shrikant and Kim, Eun Jeong and Farla, Robert and Nishida, Keisuke and Liu, Zhaodong and Wang, Lin and Nakajima, Ayano and Yan, Bingmin and Tang, Hu and Chen, Zhen and Higo, Yuji and Tange, Yoshinori and Katsura, Tomoo},
	year = {2022},
	pages = {69--73},
	file = {Chanyshev et al. - 2022 - Depressed 660-km discontinuity caused by akimotoit.pdf:/Users/dong2j/Zotero/storage/IRAPBMSR/Chanyshev et al. - 2022 - Depressed 660-km discontinuity caused by akimotoit.pdf:application/pdf},
}

@article{guignot_thermoelastic_2007,
	title = {Thermoelastic properties of post-perovskite phase {MgSiO}$_{\textrm{3}}$ determined experimentally at core–mantle boundary \textit{{P}}–\textit{{T}} conditions},
	volume = {256},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X07000416},
	doi = {10.1016/j.epsl.2007.01.025},
	abstract = {We have performed in-situ X-ray diffraction measurements on MgSiO3 up to 144.5 GPa and 2535 K to obtain a precise experimental determination of the elastic properties of the post-perovskite polymorph of MgSiO3 at high pressure and temperature. The complete dataset is comprised of 24 data points at ambient temperature and an equal number at high temperature. Fitted physical properties are the room temperature bulk modulus, the Grüneisen parameter with its volume dependency, the thermal expansion with its temperature dependency, and the linear incompressibilities as well as thermal expansions and their temperature dependency on each axis. Elastic anisotropy is observed, the structure being much more compressible along the b axis, and less compressible along the c axis, in agreement with theoretical calculations. We also demonstrate with the present study that experiments can provide precise information on the elasticity of complex materials at extreme pressure and temperature conditions. © 2007 Elsevier B.V. All rights reserved.},
	language = {en},
	number = {1-2},
	urldate = {2024-01-01},
	journal = {Earth and Planetary Science Letters},
	author = {Guignot, N and Andrault, D and Morard, G and Bolfancasanova, N and Mezouar, M},
	year = {2007},
	pages = {162--168},
	file = {Guignot et al. - 2007 - Thermoelastic properties of post-perovskite phase .pdf:/Users/dong2j/Zotero/storage/YYAGYFL5/Guignot et al. - 2007 - Thermoelastic properties of post-perovskite phase .pdf:application/pdf},
}

@article{ito_postspinel_1989,
	title = {Postspinel transformations in the system {Mg}$_{\textrm{2}}${SiO}$_{\textrm{4}}$‐{Fe}$_{\textrm{2}}${SiO}$_{\textrm{4}}$ and some geophysical implications},
	volume = {94},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/JB094iB08p10637},
	doi = {10.1029/JB094iB08p10637},
	abstract = {The high‐pressure transformation in MgSiO
              3
              and those in the spinel phases of compositions from Mg
              2
              SiO
              4
              to (Mg
              0.5
              Fe
              0.5
              )
              2
              SiO
              4
              in the Mg
              2
              SiO
              4
              ‐Fe
              2
              SiO
              4
              system were investigated using a uniaxial split‐sphere apparatus. The phase boundaries between ilmenite‐perovskite in MgSiO
              3
              and between Mg
              2
              SiO
              4
              spinel and the assemblage of MgSiO
              3
              perovskite and MgO periclase were determined to be
              P
              (GPa) = 26.8–0.0025
              T
              (°C) and
              P
              (GPa) = 27.6–0.0028
              T
              (°C), respectively, in the temperature range 1000–1600°C. The pseudobinary diagrams for the system Mg
              2
              SiO
              4
              ‐Fe
              2
              SiO
              4
              were determined at temperatures of 1100°C and 1600°C. It was demonstrated that the magnesian spinel (with Fe/Mg + Fe {\textless} 0.22 at 1100°C and {\textless}0.26 at 1600°C) dissociates into perovskite and magnesiowüstite within an extremely narrow pressure interval ({\textless}0.15 GPa at 1600°C). The dissociation pressure was found to be almost independent of iron content and to coincide to that at 670 km depth within experimental uncertainties. These experimental results indicate that the sharpness of the 670‐km discontinuity may indeed be due to this dissociation in a peridotitic or pyrolitic mantle. The current status of our understanding of deep mantle mineralogy and chemistry is discussed based on recent high‐pressure and high‐temperature experiments.},
	language = {en},
	number = {B8},
	urldate = {2024-01-01},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Ito, Eiji and Takahashi, Eiichi},
	year = {1989},
	pages = {10637--10646},
	file = {Ito and Takahashi - 1989 - Postspinel transformations in the system Mg 2.pdf:/Users/dong2j/Zotero/storage/XCAY8825/Ito and Takahashi - 1989 - Postspinel transformations in the system Mg 2.pdf:application/pdf},
}

@article{katsura_pvt_2009,
	title = {\textit{{P}}‐\textit{{V}}‐\textit{{T}} relations of {MgSiO}$_{\textrm{3}}$ perovskite determined by in situ {X}‐ray diffraction using a large‐volume high‐pressure apparatus},
	volume = {36},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2008GL035658},
	doi = {10.1029/2008GL035658},
	abstract = {The volume of MgSiO
              3
              perovskite has been precisely measured at pressures of 19 to 53 GPa and temperatures of 300 to 2300 K by means of
              in situ
              X‐ray diffraction in a multi‐anvil apparatus. The present results indicate the isothermal bulk modulus
              K
              T0
              = 256(2) GPa and its pressure derivative
              K
              ′
              T0
              = 3.8(2). The fixed Debye temperature θ
              0
              = 1030 K gives a Grüneisen parameter at ambient pressure
              γ
              0
              = 2.6(1) and its logarithmic volume dependence
              q
              = 1.7(1). The pressure derivative of the isothermal bulk modulus, Anderson‐Grüneisen parameter and thermal expansion coefficient at ambient pressure are found to be (∂
              K
              
                T
              
              /∂
              T
              )
              
                P
              
              = −0.035(2) GPa/K,
              δ
              T
              = 6.5(5),
              α
              0
              = 2.6(1) × 10
              −5
              + 1.0(1) × 10
              −8
              (
              T
              − 300)/K. Thus the thermal expansion coefficient largely becomes smaller with increasing pressure. The adiabatic geotherm would be fairly large, such as 0.41 K/km at a 660 km depth, and becoming smaller with increasing depth. The temperature and adiabatic geothermal gradient at the bottom of the D′ layer would be 2400 K and 0.14 K/km. The buoyancy‐driven mantle convection could be very small in the lower part of the lower mantle.},
	language = {en},
	number = {1},
	urldate = {2024-01-01},
	journal = {Geophysical Research Letters},
	author = {Katsura, Tomoo and Yokoshi, Sho and Kawabe, Kazuaki and Shatskiy, Anton and Manthilake, M. A. Geeth M. and Zhai, Shuangmeng and Fukui, Hiroshi and Hegoda, H. A. Chamathni I. and Yoshino, Takashi and Yamazaki, Daisuke and Matsuzaki, Takuya and Yoneda, Akira and Ito, Eiji and Sugita, Mitsuhiro and Tomioka, Naotaka and Hagiya, Kenji and Nozawa, Akifumi and Funakoshi, Ken‐ichi},
	year = {2009},
	pages = {2008GL035658},
	file = {Katsura et al. - 2009 - P‐V‐T relations of MgSiO 3 perovskite d.pdf:/Users/dong2j/Zotero/storage/AEY5N5BR/Katsura et al. - 2009 - P‐V‐T relations of MgSiO 3 perovskite d.pdf:application/pdf},
}

@article{kanzaki_orthoclinoenstatite_1991,
	title = {Ortho/clinoenstatite transition},
	volume = {17},
	issn = {0342-1791, 1432-2021},
	url = {http://link.springer.com/10.1007/BF00202244},
	doi = {10.1007/BF00202244},
	abstract = {Pressure-induced phase transformation of orthoenstatite to clinoenstatite has been studied at 710 GPa using a multi-anvil high pressure device with low stress ({\textless}10 MPa) conditions. At 1000 {\textasciitilde} clinoenstatite was stabilized at pressures above 7.5 GPa. The obtained phase boundary is consistent with natural observations and previous experimental studies performed under quasi-hydrostatic condition, suggesting that clinoenstatite is a stable high pressure phase. Large differences in dP/dT slope between this result and those of earlier studies performed with piston cylinder and belt apparatus may be attributed to large differential stress in the high pressure cells of latter studies. The present study suggests that clinoenstatite can be stabilized by either hydrostatic pressure or differential stress and that the latter tends to shift the transformation boundary defined under hydrostatic condition to lower pressure.},
	language = {en},
	number = {8},
	urldate = {2024-01-01},
	journal = {Physics and Chemistry of Minerals},
	author = {Kanzaki, Masami},
	year = {1991},
	file = {Kanzaki - 1991 - Orthoclinoenstatite transition.pdf:/Users/dong2j/Zotero/storage/AZX5VJK9/Kanzaki - 1991 - Orthoclinoenstatite transition.pdf:application/pdf},
}

@article{kuroda_determination_2000,
	title = {Determination of the phase boundary between ilmenite and perovskite in {MgSiO}$_{\textrm{3}}$ by in situ {X}-ray diffraction and quench experiments},
	volume = {27},
	issn = {0342-1791, 1432-2021},
	url = {http://link.springer.com/10.1007/s002690000096},
	doi = {10.1007/s002690000096},
	language = {en},
	number = {8},
	urldate = {2024-01-01},
	journal = {Physics and Chemistry of Minerals},
	author = {Kuroda, K. and Irifune, T. and Inoue, T. and Nishiyama, N. and Miyashita, M. and Funakoshi, K. and Utsumi, W.},
	year = {2000},
	pages = {523--532},
	file = {Kuroda et al. - 2000 - Determination of the phase boundary between ilmeni.pdf:/Users/dong2j/Zotero/storage/3G6CXHP2/Kuroda et al. - 2000 - Determination of the phase boundary between ilmeni.pdf:application/pdf},
}

@article{kulka_bridgmaniteakimotoitemajorite_2020,
	title = {The {Bridgmanite}–{Akimotoite}–{Majorite} {Triple} {Point} {Determined} in {Large} {Volume} {Press} and {Laser}-{Heated} {Diamond} {Anvil} {Cell}},
	volume = {10},
	issn = {2075-163X},
	url = {https://www.mdpi.com/2075-163X/10/1/67},
	doi = {10.3390/min10010067},
	abstract = {The bridgmanite–akimotoite–majorite (Bm–Ak–Mj or BAM) triple point in MgSiO3 has been measured in large-volume press (LVP; COMPRES 8/3 assembly) and laser-heated diamond anvil cell (LHDAC). For the LVP data, we calculated pressures from the calibration provided for the assembly. For the LHDAC data, we conducted in situ determination of pressure at high temperature using the Pt scale at synchrotron. The measured temperatures of the triple point are in good agreement between LVP and LHDAC at 1990–2000 K. However, the pressure for the triple point determined from the LVP is 3.9 ± 0.6 GPa lower than that from the LHDAC dataset. The BAM triple point determined through these experiments will provide an important reference point in the pressure–temperature space for future high-pressure experiments and will allow mineral physicists to compare the pressure–temperature conditions measured in these two different experimental methods.},
	language = {en},
	number = {1},
	urldate = {2024-01-01},
	journal = {Minerals},
	author = {Kulka, Britany L. and Dolinschi, Jonathan D. and Leinenweber, Kurt D. and Prakapenka, Vitali B. and Shim, Sang-Heon},
	year = {2020},
	pages = {67},
	file = {Kulka et al. - 2020 - The Bridgmanite–Akimotoite–Majorite Triple Point D.pdf:/Users/dong2j/Zotero/storage/59R6IPMS/Kulka et al. - 2020 - The Bridgmanite–Akimotoite–Majorite Triple Point D.pdf:application/pdf},
}

@article{ono_reaction_2017,
	title = {Reaction boundary between akimotoite and ringwoodite + stishovite in {MgSiO}$_{\textrm{3}}$},
	volume = {44},
	issn = {0342-1791, 1432-2021},
	url = {http://link.springer.com/10.1007/s00269-016-0869-7},
	doi = {10.1007/s00269-016-0869-7},
	abstract = {The phase boundary between akimotoite and ringwoodite + stishovite in ­MgSiO3 was determined using a multi-anvil high-pressure apparatus and synchrotron X-ray radiation. The phase relation was determined by observing the recovered samples using an electron microprobe analyzer. Experimental pressures were monitored by the in situ powdered X-ray diffraction data of gold, which was put in the sample chamber. The reaction boundary between akimotoite and ringwoodite + stishovite was found to occur at P (GPa) = 22.0–0.0012 × T (K). The pressure dependence of the slope of the reaction boundary, dP/dT, determined in our study was smaller than that determined by Gasparik (J Geophys Res 95:15751–15769, 1990). The triple point of ringwoodite + stishovite–wadsleyite + stishovite–akimotoite estimated in our study was at {\textasciitilde}20 GPa and {\textasciitilde}1700 K.},
	language = {en},
	number = {6},
	urldate = {2024-01-01},
	journal = {Physics and Chemistry of Minerals},
	author = {Ono, Shigeaki and Kikegawa, Takumi and Higo, Yuji},
	year = {2017},
	pages = {425--430},
	file = {Ono et al. - 2017 - Reaction boundary between akimotoite and ringwoodi.pdf:/Users/dong2j/Zotero/storage/6WY25A4Q/Ono et al. - 2017 - Reaction boundary between akimotoite and ringwoodi.pdf:application/pdf},
}

@article{ono_decomposition_2018,
	title = {Decomposition boundary from high-pressure clinoenstatite to wadsleyite + stishovite in {MgSiO}$_{\textrm{3}}$},
	volume = {103},
	issn = {0003-004X, 1945-3027},
	url = {https://www.degruyter.com/document/doi/10.2138/am-2018-6313CCBY/html},
	doi = {10.2138/am-2018-6313CCBY},
	abstract = {The reaction boundary between high-pressure clinoenstatite and wadsleyite + stishovite in MgSiO3 was investigated using a multi-anvil high-pressure apparatus and synchrotron X‑ray diffraction. Experimental pressures were monitored via in situ powdered X‑ray diffraction of gold, which was also put into the sample chamber. Stable phases at each pressure and temperature were confirmed by powdered X‑ray diffraction data and observing the recovered samples. The reaction boundary was found to occur at P (GPa) = 16.1 + 0.0064 × (T – 1250) (K), where the pressure dependence of the slope of the reaction boundary, dP/dT, is similar to that of the phase boundary between wadsleyite and ringwoodite. Thus, the stability field of wadsleyite and stishovite expands to a low-temperature region, reconciling an inconsistency recorded between previous studies regarding the phase relation in MgSiO3.},
	language = {en},
	number = {9},
	urldate = {2024-01-01},
	journal = {American Mineralogist},
	author = {Ono, Shigeaki and Kikegawa, Takumi and Higo, Yuji},
	year = {2018},
	pages = {1512--1515},
	file = {Ono et al. - 2018 - Decomposition boundary from high-pressure clinoens.pdf:/Users/dong2j/Zotero/storage/I4BR7TZ7/Ono et al. - 2018 - Decomposition boundary from high-pressure clinoens.pdf:application/pdf},
}

@article{pacalo_reversals_1990,
	title = {Reversals of the orthoenstatite‐clinoenstatite transition at high pressures and high temperatures},
	volume = {95},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/JB095iB10p15853},
	doi = {10.1029/JB095iB10p15853},
	abstract = {The MgSiO
              3
              orthoenstatite‐clinoenstatite (OEn‐CEn) phase boundary has been reversed between pressures of 70 and 110 kbar and temperatures of 900°C and 1700°C with a split‐sphere anvil apparatus (USSA‐2000). Starting materials contained PbO‐PbF
              2
              (1∶1) flux to promote equilibration of the charges and eliminate a potential effect of deviatoric stresses on the phase boundary. The phase boundary separating orthoenstatite from clinoenstatite at high pressures and temperatures can be described by the equation
              P
              (kbar) = 0.031
              T
              (°C)+50. Our results are consistent with previous unreversed determinations of the boundary at these high‐pressure, high‐temperature conditions. However, the
              dP
              /
              dT
              slope determined in the present study is much smaller than that implied by earlier experimental studies of the orthoenstatite/low clinoenstatite boundary at low pressures and temperatures. We propose that the clinoenstatite observed at high pressures and temperatures is a new high‐pressure clinoenstatite phase which is possibly an analogue of MgGeO
              3
              clinopyroxene.},
	language = {en},
	number = {B10},
	urldate = {2024-01-01},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Pacalo, R. E. G. and Gasparik, T.},
	year = {1990},
	pages = {15853--15858},
	file = {Pacalo and Gasparik - 1990 - Reversals of the orthoenstatite‐clinoenstatite tra.pdf:/Users/dong2j/Zotero/storage/IHYRSY9M/Pacalo_1990_jgr_mgsio3.pdf:application/pdf},
}

@incollection{manghnani_phase_1987,
	address = {Washington, D. C.},
	title = {Phase diagram of {MgSiO}$_{\textrm{3}}$ at pressures up to 24 {GPa} and temperatures up to 2200 °{C}: {Phase} stability and properties of tetragonal garnet},
	volume = {39},
	isbn = {978-0-87590-066-7},
	shorttitle = {Phase diagram of {MgSiO3} at pressures up to 24 {GPa} and temperatures up to 2200 °{C}},
	url = {http://doi.wiley.com/10.1029/GM039p0209},
	abstract = {T. he phasediagramfor pure MgSiO3 hasbeenobtainedat pressuresup to 24 GPa andat temperaturesup to 2200øC usinga MA8 type of high-pressureapparatus.It is found that MgSiO3 has many transformationmodesat differenttemperaturesA. t temperaturesabove 1800øC, MgSiO3hasa polymorphicsequencwe ithfivephasesin order of increasingpressureo:rthopyroxenec,linopyroxenet,etragonalgarnet, ilmenite,andperovskite.At lowertemperature,it exhibitessevenphases or phase-assemblageso:rthopyroxene,clinopyroxene,tetragonal garnet, modifiedspinelplusstishovites, pinelplusstishovitei,lmenite,and perovskite,in order of increasingdensity.All phaseboundariesare determinedby the presentexperiments,with considerationto thermodynamic constraints. The pressure-temperatureslope of the phase boundarybetweentetragonalgarnetandperovskiteisdeterminedto be positive by using parametersrepresentingwell-constrainedphase boundariesand the volumedifferencesbetweenthe relatedphases. The powder X-ray diffraction analysisof MgSiO3 with tetragonal symmetry showsthat it is isostructuralwith CaGeO3, CdGeO3, and MnSiO3;thesecompoundspossessan orderedcationicdistributionon the noequivalentsites.The unit celldimensionsof thetetragonalgarnet are a=ll.470(1) /•, c=11.398(2)/• and c/a=0.994,andthe molar volumeisabout 1\%smallerthan that estimatedfor a hypotheticalcubic garnet.Therefore tetragonalgarnetis a high-pressureand low-entropy phase.The elasticpropertiesof MgSiO3with tetragonalsymmetryare predictedfrom elasticitysystematicsb:ulk modulusK= 177 GPa and rigidity \#=101 GPa, their pressurederivatives dKs/dP=4.5 and d\#/dP= 1.44, and seismicwavevelocitiesVv=9.37 km/s and Vs=5.32 km/s.},
	language = {en},
	urldate = {2024-01-01},
	booktitle = {Geophysical {Monograph} {Series}},
	publisher = {American Geophysical Union},
	author = {Sawamoto, Hiroshi},
	editor = {Manghnani, Murli H. and Syono, Yasuhiko},
	year = {1987},
	doi = {10.1029/GM039p0209},
	pages = {209--219},
	file = {Sawamoto - 1987 - Phase diagram of MgSiO3 at pressures up to 24 GPa .pdf:/Users/dong2j/Zotero/storage/Z66UR74V/Sawamoto - 1987 - Phase diagram of MgSiO3 at pressures up to 24 GPa .pdf:application/pdf},
}

@article{shinmei_situ_1999,
	title = {In situ {X}-ray diffraction study of enstatite up to 12 {GPa} and 1473 {K} and equations of state},
	volume = {84},
	issn = {0003-004X},
	url = {https://www.degruyter.com/document/doi/10.2138/am-1999-1012/html},
	doi = {10.2138/am-1999-1012},
	language = {en},
	number = {10},
	urldate = {2024-01-01},
	journal = {American Mineralogist},
	author = {Shinmei, Toru and Tomioka, Naotaka and Fujino, Kiyoshi and Kuroda, Koji and Irifune, Tetsuo},
	year = {1999},
	pages = {1588--1594},
	file = {Shinmei et al. - 1999 - In situ X-ray diffraction study of enstatite up to.pdf:/Users/dong2j/Zotero/storage/EBD6DU8H/Shinmei et al. - 1999 - In situ X-ray diffraction study of enstatite up to.pdf:application/pdf},
}

@article{tange_pvt_2012,
	title = {\textit{{P}}‐\textit{{V}}‐\textit{{T}} equation of state of {MgSiO}$_{\textrm{3}}$ perovskite based on the {MgO} pressure scale: {A} comprehensive reference for mineralogy of the lower mantle},
	volume = {117},
	issn = {0148-0227},
	shorttitle = {\textit{{P}} ‐ \textit{{V}} ‐ \textit{{T}} equation of state of {MgSiO} $_{\textrm{3}}$ perovskite based on the {MgO} pressure scale},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2011JB008988},
	doi = {10.1029/2011JB008988},
	abstract = {In situ
              P
              ‐
              V
              ‐
              T
              measurements of MgSiO
              3
              perovskite were carried out up to 110 GPa and 2500 K, using a sintered‐diamond multianvil apparatus and a laser‐heated diamond anvil cell together with synchrotron radiation. The
              P
              ‐
              V
              ‐
              T
              data sets obtained by multianvil experiments (28–63 GPa and 300–1500 K) and diamond anvil cell experiments (52–108 GPa and 300, 1500–2430 K) are consistent with each other. The equation of state of MgSiO
              3
              perovskite was subsequently represented by a Mie‐Grüneisen‐Debye model, using the equation of state of MgO as reference for pressure determination. In this study, we provide mutually consistent and precise
              P
              ‐
              V
              ‐
              T
              equations of state of MgSiO
              3
              perovskite and MgO applicable to the bottom of the Earth's lower mantle. These
              P
              ‐
              V
              ‐
              T
              equations of state and derivative thermodynamic and elastic properties are essential for mineralogy of the lower mantle as a comprehensive reference.
            
          , 
            Key Points
            
              
                
                  P‐V‐T states of MgSiO3 perovskite were measured up to 110 GPa and 2500 K
                
                
                  Consistent P‐V‐T EOS of MgSiO3 perovskite and MgO were determined precisely
                
                
                  Thermodynamic and elastic properties of MgSiO3 perovskite and MgO are given},
	language = {en},
	number = {B6},
	urldate = {2024-01-01},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Tange, Yoshinori and Kuwayama, Yasuhiro and Irifune, Tetsuo and Funakoshi, Ken‐ichi and Ohishi, Yasuo},
	year = {2012},
	pages = {2011JB008988},
	file = {Tange et al. - 2012 - P ‐ V ‐ T equation of state o.pdf:/Users/dong2j/Zotero/storage/EHGWX3GW/Tange et al. - 2012 - P ‐ V ‐ T equation of state o.pdf:application/pdf},
}

@incollection{boyd_rhombic_1959,
	title = {The rhombic enstatite-clinoenstatite inversion},
	volume = {64},
	booktitle = {The {Carnegie} {Institution} of {Washington} {Year} {Book}},
	author = {Boyd, Francis Raymond and England, J. L.},
	year = {1959},
	pages = {117--120},
   publisher = {The {Carnegie} {Institution} of {Washington}},
	file = {boyd_1965_carnegie_year_book_mgsio3.pdf:/Users/dong2j/Zotero/storage/M9NN4CZC/boyd_1965_carnegie_year_book_mgsio3.pdf:application/pdf},
}

@article{oganov_theoretical_2004,
	title = {Theoretical and experimental evidence for a post-perovskite phase of {MgSiO}$_{\textrm{3}}$ in {Earth}’s {D}" layer},
	volume = {430},
	number = {6998},
	journal = {Nature},
	author = {Oganov, Artem R and Ono, Shigeaki},
	year = {2004},
	pages = {445--448},
	file = {oganov_2004_nature.pdf:/Users/dong2j/Zotero/storage/Q2SI8RRA/oganov_2004_nature.pdf:application/pdf},
}



@article{tateno_determination_2009,
	title = {Determination of post-perovskite phase transition boundary up to 4400 {K} and implications for thermal structure in {D}″ layer},
	volume = {277},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X08006687},
	doi = {10.1016/j.epsl.2008.10.004},
	abstract = {We have determined the post-perovskite phase transition boundary in MgSiO3 in a wide temperature range from 1640 to 4380 K at 119–171 GPa on the basis of synchrotron X-ray diffraction measurements in-situ at highpressure and -temperature in a laser-heated diamond-anvil cell (LHDAC). The results show a considerably high positive Clapeyron slope of +13.3 ± 1.0 MPa/K and a transition temperature of about 3520 ± 70 K at the core–mantle boundary (CMB) pressure. The thermal structure in D″ layer can be tightly constrained from precisely determined post-perovskite phase transition boundary and the depths of paired seismic discontinuities. These suggest that temperature at the CMB may be around 3700 K, somewhat lower than previously thought. A minimum bound on the global heat ﬂow from the core is estimated to be 6.6 ± 0.5 TW.},
	language = {en},
	number = {1-2},
	urldate = {2024-01-22},
	journal = {Earth and Planetary Science Letters},
	author = {Tateno, Shigehiko and Hirose, Kei and Sata, Nagayoshi and Ohishi, Yasuo},
	year = {2009},
	pages = {130--136},
	file = {Tateno et al. - 2009 - Determination of post-perovskite phase transition .pdf:/Users/dong2j/Zotero/storage/QREAVA3X/Tateno et al. - 2009 - Determination of post-perovskite phase transition .pdf:application/pdf},
}

%%%%%%%%
@article{eiji_ito_mgsio3_1985,
	title = {{MgSiO}$_{\textrm{3}}$ {Ilmenite}: {Calorimetry}, {Phase} {Equilibria}, and {Decomposition} at {Atmospheric} {Pressure}},
	volume = {70},
	number = {9-10},
	journal = {American Mineralogist},
	author = {{Eiji Ito} and {Alexandar Navrotsky}},
	year = {1985},
	pages = {1020--1026},
	file = {ito_1985_am_mgsio3.pdf:/Users/dong2j/Zotero/storage/UKTG4MDN/ito_1985_am_mgsio3.pdf:application/pdf},
}
@article{boyd_effects_1964,
	title = {Effects of pressure on the melting and polymorphism of enstatite, {MgSiO}$_{\textrm{3}}$},
	volume = {69},
	issn = {01480227},
	url = {http://doi.wiley.com/10.1029/JZ069i010p02101},
	doi = {10.1029/JZ069i010p02101},
	abstract = {The melting curve of enstatite, MgSiO3, has been determined in the pressure range 5 to 46 kb. The data can be fitted by a smooth curve originating at the incongruent melting point at atmospheric pressure (1557øC). Simon constants for this curve are A • 28.5 and c ----5.01. The initial slopeis 12.8 deg/kb, but it fiattens to about 6 deg/kb in the range 40 to 50 kb. The melting curve is intersectedby the polymorphictransition protoenstatite• rhombic enstatite, with rhombic enstatite as the high-pressurephase. The transition curve is approximately T \_-- 985øC -]- 84P (kb), with the triple point protoenstatite-rhombic enstatiteliquid at 1650øCand 8.0 kb. Enstatite melts congruentlyat high pressure.Experimental data showthat the pressureat which the melting changesfrom incongruentto congruent must be lessthan 5.4 kb. Thermodynamic calculationsindicate that it is probably about 2.3 kb. These data suggestthat rocks which show textural evidence of an olivine-liquid reaction relation have developed this relation at relatively shallow depth, probably less than about 9 km.},
	language = {en},
	number = {10},
	urldate = {2024-01-01},
	journal = {Journal of Geophysical Research},
	author = {Boyd, F. R. and England, J. L. and Davis, Brian T. C.},
	month = may,
	year = {1964},
	pages = {2101--2109},
	file = {Boyd et al. - 1964 - Effects of pressure on the melting and polymorphis.pdf:/Users/dong2j/Zotero/storage/ZJBTAVSP/Boyd et al. - 1964 - Effects of pressure on the melting and polymorphis.pdf:application/pdf},
}

@incollection{syono_melting_2013,
	address = {Washington, D. C.},
	title = {Melting of {Ferromagnesian} {Silicates} {Under} the {Lower} {Mantle} {Conditions}},
	isbn = {978-1-118-66392-9 978-0-87590-034-6},
	url = {http://doi.wiley.com/10.1029/GM067p0315},
	abstract = {MeltingofMgSiO3hasbeeninvestigatedin thepressurerange of 21-25 GPawith a uniaxialsplit-sphereapparatusM. gSiO3 meltscongruentlyoverthepressuresstudiedT. hemeltingcurveofMgSiO3perovskite initiatesat about2450øC and22 GPa andhasa small positiveslopeof 30 + 5 deg/GPa, which can be approximatelyexpressedby the KrautKennedyequationasTin(K)= 190011+ 5.3(Iz0 - V)/tz0].},
	language = {en},
	urldate = {2024-01-01},
	booktitle = {High-{PressureResearch}: {Application} to {Earth} and {Planetary} {Science}},
	publisher = {American Geophysical Union},
	author = {Ito, E. and Katsura, T.},
	editor = {Syono, Yasuhiko and Manghnani, Murli H.},
	month = mar,
	year = {2013},
	doi = {10.1029/GM067p0315},
	pages = {315--322},
	file = {Ito and Katsura - 2013 - Melting of Ferromagnesian Silicates Under the Lowe.pdf:/Users/dong2j/Zotero/storage/RBNC3PZN/Ito and Katsura - 2013 - Melting of Ferromagnesian Silicates Under the Lowe.pdf:application/pdf},
}

@article{kato_garnet_1985,
	title = {Garnet phase of {MgSiO}$_{\textrm{3}}$ filling the pyroxene-ilmenite gap at very high temperature},
	language = {en},
	journal = {Nature},
	author = {Kato, Takumi and Kumazawat, Mineo},
	year = {1985},
	file = {Kato and Kumazawat - 1985 - Garnet phase of MgSi03 filling the pyroxene-ilmeni.pdf:/Users/dong2j/Zotero/storage/DSWJMFHD/Kato and Kumazawat - 1985 - Garnet phase of MgSi03 filling the pyroxene-ilmeni.pdf:application/pdf},
}

@article{zerr_melting_1993,
	title = {Melting of ({Mg},{Fe}){SiO}$_{\textrm{3}}$ -{Perovskite} to 625 {Kilobars}: {Indication} of a {High} {Melting} {Temperature} in the {Lower} {Mantle}},
	volume = {262},
	issn = {0036-8075, 1095-9203},
	shorttitle = {Melting of ({Mg}, {Fe}){SiO} $_{\textrm{3}}$ -{Perovskite} to 625 {Kilobars}},
	url = {https://www.science.org/doi/10.1126/science.262.5133.553},
	doi = {10.1126/science.262.5133.553},
	language = {en},
	number = {5133},
	urldate = {2024-01-01},
	journal = {Science},
	author = {Zerr, A. and Boehler, R.},
	month = oct,
	year = {1993},
	pages = {553--555},
	file = {Zerr and Boehler - 1993 - Melting of (Mg, Fe)SiO 3 -Perovskite to.pdf:/Users/dong2j/Zotero/storage/RT6Z6K75/Zerr and Boehier - 1993 - Melting of (Mg, Fe)SiO 3 -Perovskite to.pdf:application/pdf},
}

@article{cheng-hong_chen_system_1975,
	title = {The {System} {Mg}$_{\textrm{2}}${SiO}$_{\textrm{4}}$-{SiO}$_{\textrm{2}}$ at {Pressures} {Up} to 25 {Kilobar}},
	volume = {60},
	journal = {American Mineralogist},
	author = {{Cheng-Hong Chen} and {Dean C Presnall}},
	year = {1975},
	pages = {398--406},
	file = {Chen_1975_AM_MGSIO3.pdf:/Users/dong2j/Zotero/storage/N3LXHLDJ/Chen_1975_AM_MGSIO3.pdf:application/pdf},
}

@article{dean_c_presnall_melting_1990,
	title = {Melting of {Enstatite} ({MgSiO}$_{\textrm{3}}$) {From} 10 to 16.5 {GPa} and the {Forsteritc} ({Mg}$_{\textrm{2}}${SiO}$_{\textrm{4}}$)-{Majoritc} ({MgSiO}$_{\textrm{3}}$) {Eutectic} at 16.5 {GPa}: {Implications} for the {Origin} of the {Mantle}.},
	volume = {95},
	number = {B10},
	journal = {Journal of Geophysical Research},
	author = {{Dean C Presnall} and {Tibor Gasparik}},
	month = sep,
	year = {1990},
	pages = {15771--15777},
	file = {pr90_m.pdf:/Users/dong2j/Zotero/storage/CPFLXDW3/pr90_m.pdf:application/pdf},
}
@article{niu_prediction_2015,
	title = {Prediction of novel stable compounds in the {Mg}-{Si}-{O} system under exoplanet pressures},
	volume = {5},
	issn = {2045-2322},
	url = {https://www.nature.com/articles/srep18347},
	doi = {10.1038/srep18347},
	abstract = {Abstract
            
              The Mg-Si-O system is the major Earth and rocky planet-forming system. Here, through quantum variable-composition evolutionary structure explorations, we have discovered several unexpected stable binary and ternary compounds in the Mg-Si-O system. Besides the well-known SiO
              2
              phases, we have found two extraordinary silicon oxides, SiO
              3
              and SiO, which become stable at pressures above 0.51 TPa and 1.89 TPa, respectively. In the Mg-O system, we have found one new compound, MgO
              3
              , which becomes stable at 0.89 TPa. We find that not only the (MgO)
              x
              ·(SiO
              2
              )
              y
              compounds, but also two (MgO
              3
              )
              x
              ·(SiO
              3
              )
              y
              compounds, MgSi
              3
              O
              12
              and MgSiO
              6
              , have stability fields above 2.41 TPa and 2.95 TPa, respectively. The highly oxidized MgSi
              3
              O
              12
              can form in deep mantles of mega-Earths with masses above 20 M
              ⊕
              (M
              ⊕
              :Earth’s mass). Furthermore, the dissociation pathways of pPv-MgSiO
              3
              are also clarified and found to be different at low and high temperatures. The low-temperature pathway is MgSiO
              3
              ⇒ Mg
              2
              SiO
              4
              + MgSi
              2
              O
              5
              ⇒ SiO
              2
              + Mg
              2
              SiO
              4
              ⇒ MgO + SiO
              2
              , while the high-temperature pathway is MgSiO
              3
              ⇒ Mg
              2
              SiO
              4
              + MgSi
              2
              O
              5
              ⇒ MgO + MgSi
              2
              O
              5
              ⇒ MgO + SiO
              2
              . Present results are relevant for models of the internal structure of giant exoplanets and for understanding the high-pressure behavior of materials.},
	language = {en},
	number = {1},
	urldate = {2024-01-21},
	journal = {Scientific Reports},
	author = {Niu, Haiyang and Oganov, Artem R. and Chen, Xing-Qiu and Li, Dianzhong},
	year = {2015},
	pages = {18347},
	file = {Full Text:/Users/dong2j/Zotero/storage/32NYJV5Y/Niu et al. - 2015 - Prediction of novel stable compounds in the Mg-Si-.pdf:application/pdf},
}

@article{umemoto_phase_2017,
	title = {Phase transitions in {MgSiO3} post-perovskite in super-{Earth} mantles},
	volume = {478},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X1730479X},
	doi = {10.1016/j.epsl.2017.08.032},
	language = {en},
	urldate = {2024-01-09},
	journal = {Earth and Planetary Science Letters},
	author = {Umemoto, Koichiro and Wentzcovitch, Renata M. and Wu, Shunqing and Ji, Min and Wang, Cai-Zhuang and Ho, Kai-Ming},
	year = {2017},
	pages = {40--45},
	file = {Umemoto et al. - 2017 - Phase transitions in MgSiO3 post-perovskite in sup.pdf:/Users/dong2j/Zotero/storage/X2ZMH8WF/Umemoto et al. - 2017 - Phase transitions in MgSiO3 post-perovskite in sup.pdf:application/pdf},
}

@article{tsuchiya_prediction_2011,
	title = {Prediction of a hexagonal {SiO} $_{\textrm{2}}$ phase affecting stabilities of {MgSiO} $_{\textrm{3}}$ and {CaSiO} $_{\textrm{3}}$ at multimegabar pressures},
	volume = {108},
	issn = {0027-8424, 1091-6490},
	url = {https://pnas.org/doi/full/10.1073/pnas.1013594108},
	doi = {10.1073/pnas.1013594108},
	abstract = {Ultrahigh-pressure phase relationship of SiO
              2
              silica in multimegabar pressure condition is still quite unclear. Here, we report a theoretical prediction on a previously uncharacterized stable structure of silica with an unexpected hexagonal Fe
              2
              P-type form. This phase, more stable than the cotunnite-type structure, a previously postulated postpyrite phase, was discovered to stabilize at 640 GPa through a careful structure search by means of ab initio density functional computations over various structure models. This is the first evidential result of the pressure-induced phase transition to the Fe
              2
              P-type structure among all dioxide compounds. The crystal structure consists of closely packed, fairly regular SiO
              9
              tricapped trigonal prisms with a significantly compact lattice. Additional investigation further elucidates large effects of this phase change in SiO
              2
              on the stability of MgSiO
              3
              and CaSiO
              3
              at multimegabar pressures. A postperovskite phase of MgSiO
              3
              breaks down at 1.04 TPa along an assumed adiabat of super-Earths and yields Fe
              2
              P-type SiO
              2
              and CsCl (B2)-type MgO. CaSiO
              3
              perovskite, on the other hand, directly dissociates into SiO
              2
              and metallic CaO, skipping a postperovskite polymorph. Predicted ultrahigh-pressure and temperature phase diagrams of SiO
              2
              , MgSiO
              3
              , and CaSiO
              3
              indicate that the Fe
              2
              P-type SiO
              2
              could be one of the dominant components in the deep mantles of terrestrial exoplanets and the cores of gas giants.},
	language = {en},
	number = {4},
	urldate = {2024-01-21},
	journal = {Proceedings of the National Academy of Sciences},
	author = {Tsuchiya, Taku and Tsuchiya, Jun},
	year = {2011},
	pages = {1252--1255},
	file = {Full Text:/Users/dong2j/Zotero/storage/5E7QMVPR/Tsuchiya and Tsuchiya - 2011 - Prediction of a hexagonal SiO 2 phase a.pdf:application/pdf},
}


@article{deng_melting_2023,
	title = {Melting of {MgSiO}$_{\textrm{3}}$ determined by machine learning potentials},
	volume = {107},
	issn = {2469-9950, 2469-9969},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.107.064103},
	doi = {10.1103/PhysRevB.107.064103},
	language = {en},
	number = {6},
	urldate = {2024-01-09},
	journal = {Physical Review B},
	author = {Deng, Jie and Niu, Haiyang and Hu, Junwei and Chen, Mingyi and Stixrude, Lars},
	month = feb,
	year = {2023},
	pages = {064103},
	file = {Deng et al. - 2023 - Melting of MgSi O 3 determined by machine learning.pdf:/Users/dong2j/Zotero/storage/CVWWG8FB/Deng et al. - 2023 - Melting of MgSi O 3 determined by machine learning.pdf:application/pdf},
}

###IMPLICATION###

@article{schlichting_chemical_2022,
	title = {Chemical Equilibrium between Cores, Mantles, and Atmospheres of Super-Earths and Sub-Neptunes and Implications for Their Compositions, Interiors, and Evolution},
	volume = {3},
	issn = {2632-3338},
	url = {https://iopscience.iop.org/article/10.3847/PSJ/ac68e6},
	doi = {10.3847/PSJ/ac68e6},
	abstract = {Abstract
            
              We investigate the equilibrium chemistry between molten metal and silicate and a hydrogen-rich envelope using 18 independent reactions among 25 phase components for sub-Neptune-like exoplanets. Both reactive and unreactive metal sequestered in an isolated core are modeled. The overarching effects of equilibration are oxidation of the envelope and reduction of the mantle and core. Hydrogen and oxygen typically comprise significant fractions of metal cores at chemical equilibrium, leading to density deficits that offer a possible alternative explanation for the low densities of the Trappist-1 planets. Reactions with the magma ocean produce significant amounts of {SiO} and H
              2
              O in the envelopes directly above the magma ocean. Molar concentrations in the envelopes of planets with reactive metal are H
              2
              {\textgreater} {SiO} {\textgreater} {CO} ∼ Na ∼ Mg {\textgreater} H
              2
              O ≫ {CO}
              2
              ∼ {CH}
              4
              ≫ O
              2
              , while for the unreactive metal case, H
              2
              O becomes the second most abundant species, after H
              2
              , providing an arbiter for the two scenarios amenable to observation. The water abundances in the atmospheres exceed those in the mantles by at least an order of magnitude in both scenarios. The water concentrations in the silicate mantles are ∼0.01 and ∼0.1 wt\% in the reactive and unreactive metal core cases, respectively, limiting the H
              2
              O that might be outgassed in a future super-Earth. Less dissolved water in the reactive core case is due to sequestration of H and O in the Fe-rich metal. The total hydrogen budget of most sub-Neptunes can, to first order, be estimated from their atmospheres alone, as the atmospheres typically contain more than 90\% of all H.},
	pages = {127},
	number = {5},
	journaltitle = {The Planetary Science Journal},
	shortjournal = {Planet. Sci. J.},
	author = {Schlichting, Hilke E. and Young, Edward D.},
	urldate = {2024-02-20},
	date = {2022},
	file = {Full Text:/Users/jdong/Zotero/storage/H9FLXHV4/Schlichting and Young - 2022 - Chemical Equilibrium between Cores, Mantles, and A.pdf:application/pdf},
}


%%%%%%%%%%%%%%
appx
%%%%%%%%%%%%%%




@article{saxena_temperatures_1994,
	title = {Temperatures in {Earth}'s {Core} {Based} on {Melting} and {Phase} {Transformation} {Experiments} on lron},
	volume = {264},
	language = {en},
	journal = {Science},
	author = {Saxena, S. K. and Shen, G. and Lazor, P.},
	year = {1994},
	file = {Boehler et al. - 1994 - REFERENCES AND NOTES.pdf:/Users/jdong/Zotero/storage/4ZJNQJT6/Boehler et al. - 1994 - REFERENCES AND NOTES.pdf:application/pdf},
}





@article{yoo_phase_1995,
	title = {Phase {Diagram} of {Iron} by in {Situ} {X}-{Ray} {Diffraction}: {Implications} for {Earth}'s {Core}},
	volume = {270},
	number = {5241},
	journal = {Science},
	author = {Yoo, C. S. and Akella, J. and Campbell, A. J. and Mao, H. K. and Hemley, R. J.},
	month = dec,
	year = {1995},
	pages = {1473--1475},
	file = {Yoo (1995) - Phase Diagram of Iron by in Situ X-ray Diffraction.pdf:/Users/jdong/Zotero/storage/HFNTGVNK/Yoo (1995) - Phase Diagram of Iron by in Situ X-ray Diffraction.pdf:application/pdf},
}


@article{zhang_temperature_2016,
	title = {Temperature of {Earth}'s core constrained from melting of {Fe} and {Fe0}.{9Ni0}.1 at high pressures},
	volume = {447},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X16301984},
	doi = {10.1016/j.epsl.2016.04.026},
	language = {en},
	urldate = {2024-01-03},
	journal = {Earth and Planetary Science Letters},
	author = {Zhang, Dongzhou and Jackson, Jennifer M. and Zhao, Jiyong and Sturhahn, Wolfgang and Alp, E. Ercan and Hu, Michael Y. and Toellner, Thomas S. and Murphy, Caitlin A. and Prakapenka, Vitali B.},
	month = aug,
	year = {2016},
	pages = {72--83},
	file = {Zhang et al. - 2016 - Temperature of Earth's core constrained from melti.pdf:/Users/jdong/Zotero/storage/LSHBSPR6/Zhang et al. - 2016 - Temperature of Earth's core constrained from melti.pdf:application/pdf},
}




@article{morard_solving_2018,
	title = {Solving {Controversies} on the {Iron} {Phase} {Diagram} {Under} {High} {Pressure}},
	volume = {45},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2018GL079950},
	doi = {10.1029/2018GL079950},
	abstract = {As the main constituent of planetary cores, pure iron phase diagram under high pressure and temperature is of fundamental importance in geophysics and planetary science. However, previously reported iron-melting curves show large discrepancies (up to 1000 K at the Earth’s core–mantle boundary, 136 GPa), resulting in persisting high uncertainties on the solid-liquid phase boundary. Here we unambiguously show that the observed differences commonly attributed to the nature of the used melting diagnostic are due to a carbon contamination of the sample as well as pressure overestimation at high temperature. The high melting temperature of pure iron under core-mantle boundary (4250 ± 250 K), here determined by X-ray absorption experiments at the Fe K-edge, indicates that volatile light elements such as sulfur, carbon, or hydrogen are required to lower the crystallization temperature of the Earth’s liquid outer core in order to prevent extended melting of the surrounding silicate mantle. Plain Language Summary Iron is the main constituent of planetary cores; however, there are still large controversies regarding its melting temperature and phase diagram under planetary interior conditions. The present study reconciles different experimental approaches using laser-heated diamond anvil cell with different in situ X-ray diagnostics (absorption, diffraction, and Mossbauer spectroscopy). The main reason of discrepancies (over 1000 K at core-mantle boundary conditions) is attributed to carbon contamination from the diamond anvils and metrology issues related to thermal pressure overestimation. A high-melting temperature for iron at core-mantle boundary pressure would imply the presence of volatile elements in the liquid outer core, such as sulfur, carbon, or hydrogen, in order to lower its crystallization temperature and avoid extended melting of the surrounding silicate mantle.},
	language = {en},
	number = {20},
	urldate = {2024-01-03},
	journal = {Geophysical Research Letters},
	author = {Morard, Guillaume and Boccato, Silvia and Rosa, Angelika D. and Anzellini, Simone and Miozzi, Francesca and Henry, Laura and Garbarino, Gaston and Mezouar, Mohamed and Harmand, Marion and Guyot, François and Boulard, Eglantine and Kantor, Innokenty and Irifune, Tetsuo and Torchio, Raffaella},
	month = oct,
	year = {2018},
	file = {Morard et al. - 2018 - Solving Controversies on the Iron Phase Diagram Un.pdf:/Users/jdong/Zotero/storage/B3323MS2/Morard et al. - 2018 - Solving Controversies on the Iron Phase Diagram Un.pdf:application/pdf},
}

@article{yong_iron_2019,
	title = {The {Iron} {Invariance}: {Implications} for {Thermal} {Convection} in {Earth}'s {Core}},
	volume = {46},
	issn = {0094-8276, 1944-8007},
	shorttitle = {The {Iron} {Invariance}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2019GL084485},
	doi = {10.1029/2019GL084485},
	abstract = {Abstract
            Convection of the liquid iron (Fe) outer core and electrical properties of Fe are responsible for the geodynamo that generates the geomagnetic field. Recent results showed the thermal conductivity of the core and related conductive heat flux may be much larger than previously accepted, suggesting that thermal convection would not be an energy source to power the geodynamo. Here we report experimental measurements of the electrical resistivity of solid and liquid Fe which show invariant values along the melting boundary at pressures up to 24 GPa. The observed resistivity invariance was extrapolated to Earth's predominantly Fe solid inner core and liquid outer core conditions and, using the Wiedemann‐Franz law, the thermal conductivity was calculated. We calculate a conductive core heat flow of 8–9 TW at the core‐mantle boundary. These results provide strong support for thermal convection as a geodynamo energy source.
          , 
            Plain Language Summary
            Earth's magnetic field is produced by a dynamo in the core that requires motion of the fluid Fe alloy. Both thermal convection, arising from the transport of heat in excess of conducted heat, and compositional convection, arising from light element exsolution at the freezing inner core boundary, are suggested as energy sources. The contribution of thermal convection (possibly ranging from nothing to significant) depends on thermal conductivity of the outer core. Our experimental measurements of electrical resistivity of solid and liquid Fe at high pressures show that resistivity is constant along the pressure‐dependent melting boundary of Fe. Using our derived thermal conductivity value at the inner core (freezing) boundary, we calculate the heat conducted in the liquid outer core and find that thermal convection is needed to carry additional heat through the outer core to match the heat extracted through the core‐mantle boundary.
          , 
            Key Points
            
              
                
                  Experimental measurements of electrical resistivity of solid and liquid Fe up to 24 GPa in multianvil press are reported
                
                
                  Electrical resistivity is constant along the melting boundary
                
                
                  Derived electronic thermal conductivity and calculated adiabatic heat flow provide support for thermal convection as a geodynamo energy source},
	language = {en},
	number = {20},
	urldate = {2024-07-19},
	journal = {Geophysical Research Letters},
	author = {Yong, Wenjun and Secco, Richard A. and Littleton, Joshua A. H. and Silber, Reynold E.},
	month = oct,
	year = {2019},
	pages = {11065--11070},
}

@incollection{kennedy_solid-liquid_1963,
	address = {New York},
	title = {Solid-liquid and solid-solid phase transitions in some metals at high temperatures and pressures},
	booktitle = {Solids {Under} {Pressure}},
	publisher = {McGraw-Hill Book Co.},
	author = {Kennedy, G. C. and Newton, R. C.},
	year = {1963},
pages = {11065--11070},
}

%%%MgO%%%
@article{mcnally_laboratory_1961,
	title = {Laboratory {Furnace} for {Studies} in {Controlled} {Atmospheres}; {Melting} {Points} of {MgO} in a {N2} {Atmosphere} and of {Cr2O3} in {N2} and in {Air} {Atmospheres}},
	volume = {44},
	copyright = {http://doi.wiley.com/10.1002/tdm\_license\_1.1},
	issn = {0002-7820, 1551-2916},
	url = {https://onlinelibrary.wiley.com/doi/10.1111/j.1151-2916.1961.tb13711.x},
	doi = {10.1111/j.1151-2916.1961.tb13711.x},
	language = {en},
	number = {10},
	urldate = {2024-11-25},
	journal = {Journal of the American Ceramic Society},
	author = {McNally, R. N. and Peters, F. I. and Ribbe, P. H.},
	month = oct,
	year = {1961},
	pages = {491--493},
	file = {McNALLY et al. - 1961 - Laboratory Furnace for Studies in Controlled Atmos.pdf:/Users/jdong/Zotero/storage/YQ6PNRIB/McNALLY et al. - 1961 - Laboratory Furnace for Studies in Controlled Atmos.pdf:application/pdf},
}

@article{ronchi_melting_2001,
	title = {Melting point of {MgO}},
	volume = {90},
	issn = {0021-8979, 1089-7550},
	url = {https://pubs.aip.org/jap/article/90/7/3325/292189/Melting-point-of-MgO},
	doi = {10.1063/1.1398069},
	abstract = {Despite large commercial production of MgO-based ceramics for a wide gamut of applications, the melting point of magnesia remained uncertain for almost one century. This article shows that a number of problems must be solved to attain experimental conditions where the solid–liquid phase transition of magnesia can be unambiguously detected, and the temperature be measured with sufficient accuracy. The method adopted in the reported work is based on controlled laser pulse heating. The solidification point was measured by the thermal arrest occurring during cooldown from the melt. The measurement of temperature, a most delicate problem for pyrometry applications in semitransparent materials, was obtained by using combined brightness and spectral pyrometers. The experimental and analytical methods are described in some detail. The resulting melting point of MgO is 3250±20 K, which is approximately 150 K higher than the value currently recommended.},
	language = {en},
	number = {7},
	urldate = {2024-11-25},
	journal = {Journal of Applied Physics},
	author = {Ronchi, Claudio and Sheindlin, Mikhail},
	month = oct,
	year = {2001},
	pages = {3325--3331},
	file = {Ronchi and Sheindlin - 2001 - Melting point of MgO.pdf:/Users/jdong/Zotero/storage/J7VEY63H/Ronchi and Sheindlin - 2001 - Melting point of MgO.pdf:application/pdf},
}

@article{riley_determination_1966,
	title = {Determination of melting points at temperatures above 2000 degrees {Celcius}},
	volume = {3},
	journal  = {Revue internationale des hautes températures et des réfractaires},
	author = {Riley, B.},
	year = {1966},
	pages = {327},
}

@article{alfe_melting_2005,
	title = {Melting {Curve} of {MgO} from {First}-{Principles} {Simulations}},
	volume = {94},
	copyright = {http://link.aps.org/licenses/aps-default-license},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.94.235701},
	doi = {10.1103/PhysRevLett.94.235701},
	language = {en},
	number = {23},
	urldate = {2024-11-25},
	journal = {Physical Review Letters},
	author = {Alfè, Dario},
	month = jun,
	year = {2005},
	pages = {235701},
	file = {Submitted Version:/Users/jdong/Zotero/storage/28BR2S9Z/Alfè - 2005 - Melting Curve of MgO from First-Principles Simulat.pdf:application/pdf},
}

@article{taniuchi_melting_2018,
	title = {The melting points of {MgO} up to 4 {TPa} predicted based on \textit{ab initio} thermodynamic integration molecular dynamics},
	volume = {30},
	issn = {0953-8984, 1361-648X},
	url = {https://iopscience.iop.org/article/10.1088/1361-648X/aaac96},
	doi = {10.1088/1361-648X/aaac96},
	number = {11},
	urldate = {2024-11-25},
	journal = {Journal of Physics: Condensed Matter},
	author = {Taniuchi, Takashi and Tsuchiya, Taku},
	month = mar,
	year = {2018},
	pages = {114003},
}

@article{musella_physical_2019,
	title = {Physical properties of {MgO} at deep planetary conditions},
	volume = {99},
	issn = {2469-9950, 2469-9969},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.99.064110},
	doi = {10.1103/PhysRevB.99.064110},
	language = {en},
	number = {6},
	urldate = {2024-11-25},
	journal = {Physical Review B},
	author = {Musella, R. and Mazevet, S. and Guyot, F.},
	month = feb,
	year = {2019},
	pages = {064110},
	file = {Full Text:/Users/jdong/Zotero/storage/Q4CIYXKK/Musella et al. - 2019 - Physical properties of MgO at deep planetary condi.pdf:application/pdf},
}

@article{wisesa_machine-learning_2023,
	title = {Machine-{Learning} {Accelerated} {First}-{Principles} {Accurate} {Modeling} of the {Solid}–{Liquid} {Phase} {Transition} in {MgO} under {Mantle} {Conditions}},
	volume = {14},
	copyright = {https://doi.org/10.15223/policy-029},
	issn = {1948-7185, 1948-7185},
	url = {https://pubs.acs.org/doi/10.1021/acs.jpclett.3c02424},
	doi = {10.1021/acs.jpclett.3c02424},
	language = {en},
	number = {39},
	urldate = {2024-11-25},
	journal = {The Journal of Physical Chemistry Letters},
	author = {Wisesa, Pandu and Andolina, Christopher M. and Saidi, Wissam A.},
	month = oct,
	year = {2023},
	pages = {8741--8748},
}

@article{fatyanov_melting_2024,
	title = {Melting of {B1}-phase {MgO} from simultaneous true radiative shock temperature and sound speed measurements to 250 {GPa} on samples preheated to 2300 {K}},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Fat’yanov, O. V. and Asimow, P. D.},
	year = {2024},
	annote = {accepted

},
}

@article{chernyshev_thermal_1993,
	title = {Thermal radiative properties of magnesium oxide at high temperatures},
	volume = {218},
	copyright = {https://www.elsevier.com/tdm/userlicense/1.0/},
	issn = {00406031},
	url = {https://linkinghub.elsevier.com/retrieve/pii/0040603193804227},
	doi = {10.1016/0040-6031(93)80422-7},
	abstract = {Results are given, obtained from measurements of the normalhemispherical reflectivity of pure magnesium oxide at wavelengths of 0.488; 0.6328; 1.15; 3.39 and 5,4 pm during its heating in air bY COZ laser radiation from room temperature up to intensive evaporation temperatures and during subsequent cooling. It was found that when there is a molten layer about 100 wrn thick on the surface, an optically infinite layer is realized in the melt for the entire studied spectral range, and the value of the reflectivity is determined only by the refractive index. Comparison of the MgO radiation spectra in the wavelength range of O-4-1.5 pm, measured during heating and cooling, and the radiation spectra of a blackbody model made it possible to calculate the "effective" brightness temperatures. This information enabled the nature of the spectral and temperature dependence of the absorption coefficient of MgO in both the solid and the liquid phase to be appraised. The brightness temperatures measured by a pyrometer at wavelengths of 0.55 and 0.72 Ctrnduring the course of melting indicated a substantial change in the absorption coefficient. The possible influence of radiation scattering by MgO condensate particles near the sample on the results of measuring radiative characteristics has been considered. This influence can be very appreciable in the visible and the nearest infrared region of the spectrum.},
	language = {en},
	urldate = {2024-11-25},
	journal = {Thermochimica Acta},
	author = {Chernyshev, A.P. and Petrov, V.A. and Titov, V.E. and Vorobyev, A.Yu.},
	month = may,
	year = {1993},
	pages = {195--209},
	file = {Chernyshev et al. - 1993 - Thermal radiative properties of magnesium oxide at.pdf:/Users/jdong/Zotero/storage/6SEAT8BA/Chernyshev et al. - 1993 - Thermal radiative properties of magnesium oxide at.pdf:application/pdf},
}

@article{wicks_b1-b2_2024,
	title = {B1-{B2} transition in shock-compressed {MgO}},
	volume = {10},
	issn = {2375-2548},
	url = {https://www.science.org/doi/10.1126/sciadv.adk0306},
	doi = {10.1126/sciadv.adk0306},
	abstract = {Magnesium oxide (MgO) is a major component of the Earth’s mantle and is expected to play a similar role in the mantles of large rocky exoplanets. At extreme pressures, MgO transitions from the NaCl
              B
              1 crystal structure to a CsCl
              B
              2 structure, which may have implications for exoplanetary deep mantle dynamics. In this study, we constrain the phase diagram of MgO with laser-compression along the shock Hugoniot, with simultaneous measurements of crystal structure, density, pressure, and temperature. We identify the
              B
              1 to
              B
              2 phase transition between 397 and 425 gigapascal (around 9700 kelvin), in agreement with recent theory that accounts for phonon anharmonicity. From 425 to 493 gigapascal, we observe a mixed-phase region of B1 and B2 coexistence. The transformation follows the Watanabe-Tokonami-Morimoto mechanism. Our data are consistent with
              B
              2-liquid coexistence above 500 gigapascal and complete melting at 634 gigapascal. This study bridges the gap between previous theoretical and experimental studies, providing insights into the timescale of this phase transition.
            
          , 
            High-pressure properties of an important planetary component, magnesium oxide, are measured under laser shock compression.},
	language = {en},
	number = {23},
	urldate = {2024-11-25},
	journal = {Science Advances},
	author = {Wicks, June K. and Singh, Saransh and Millot, Marius and Fratanduono, Dayne E. and Coppari, Federica and Gorman, Martin G. and Ye, Zixuan and Rygg, J. Ryan and Hari, Anirudh and Eggert, Jon H. and Duffy, Thomas S. and Smith, Raymond F.},
	month = jun,
	year = {2024},
	pages = {eadk0306},
	file = {Wicks et al. - 2024 - B1-B2 transition in shock-compressed MgO.pdf:/Users/jdong/Zotero/storage/3B9JU3RP/Wicks et al. - 2024 - B1-B2 transition in shock-compressed MgO.pdf:application/pdf},
}

@article{FU20181,
title = {Melting behavior of the lower-mantle ferropericlase across the spin crossover: Implication for the ultra-low velocity zones at the lowermost mantle},
journal = {Earth and Planetary Science Letters},
volume = {503},
pages = {1-9},
year = {2018},
issn = {0012-821X},
doi = {https://doi.org/10.1016/j.epsl.2018.09.014},
url = {https://www.sciencedirect.com/science/article/pii/S0012821X1830551X},
author = {Suyu Fu and Jing Yang and Youjun Zhang and Jiachao Liu and Eran Greenberg and Vitali B. Prakapenka and Takuo Okuchi and Jung-Fu Lin},
keywords = {melting behavior, ferropericlase, spin crossover, lower mantle},
abstract = {Preferential iron partitioning into melt during melting and crystallization of lower mantle minerals – bridgmanite and ferropericlase – can play a critical role in our understanding of the origin of the early Earth and its evolution to form chemically and seismically distinct regions in the present lowermost mantle. Of particular interest is the consequence of iron spin crossover in ferropericlase on the physical and chemical properties of the molten materials under relevant pressure–temperature (P–T) conditions of the lowermost mantle. However, the spin crossover in liquid (Mg, Fe)O and its effects on melting curves, iron partitioning, melt density – and thus the evolution of an early basal magma ocean – remain poorly studied. Here we conducted high P–T melting experiments on ferropericlase with a starting composition of (Mg0.86Fe0.14)O using synchrotron X-ray diffraction up to ∼120 GPa and ∼5400 K in laser-heated diamond anvil cells, together with chemical analyses on quenched samples using focused ion beam and energy dispersive spectroscopy technique. An ideal solid solution model could be satisfactorily used to fit the experimental data of the liquidus and solidus of (Mg, Fe)O for pure high-spin (HS, below ∼83 GPa), and low-spin (LS, above ∼120 GPa) states, respectively. The experimental solidus and liquidus at 99 GPa and ∼4000–5200 K strongly deviate from ideal solid solution behavior for pure HS and LS states alone, but can be qualitatively explained using a thermodynamics model for a mixture of HS and LS states across the spin crossover. We found that LS (Mg, Fe)O exhibits ∼6–8% lower solidus and liquidus temperature than its HS counterpart. Furthermore, our results show that iron preferentially partitions into melt within the spin crossover to generate iron-rich LS melt. Such iron-rich LS (Mg, Fe)O is ∼27(±5)% denser than materials expected for lowermost mantle and could potentially persist as residual melt in the lowermost mantle at the late stage of magma ocean crystallization. Modeled results indicate that the existence of the dense, iron-rich LS (Mg, Fe)O melt in the lowermost mantle could provide plausible explanations for characteristic seismological signatures of ultra-low velocity zones (ULVZs).}
}

@incollection{manghnani_volume_1998,
	address = {Washington, D. C.},
	title = {Volume measurement of {MgO} at high pressures and high temperatures},
	volume = {101},
	isbn = {978-0-87590-083-4},
	url = {http://doi.wiley.com/10.1029/GM101p0327},
	language = {en},
	urldate = {2024-07-19},
	booktitle = {Geophysical {Monograph} {Series}},
	publisher = {American Geophysical Union},
	author = {Utsumi, Wataru and Weidner, Donald J. and Liebermann, Robert C.},
	editor = {Manghnani, Murli H. and Yagi, Takehiko},
	year = {1998},
	doi = {10.1029/GM101p0327},
	pages = {327--333},
}

%%%SIO2%%%
@article{boyd_quartz-coesite_1960,
	title = {The quartz-coesite transition},
	volume = {65},
	doi = {10.1029/JZ065i002p00749},
	number = {2},
	journal = {Journal of Geophysical Research},
	author = {Boyd, F. R. and England, J. L.},
	year = {1960},
	pages = {749--756},
}

@article{lewis_h_cohen_high-low_1967,
	title = {High-low quartz inversion: {Determination} to 35 kilobars},
	volume = {72},
	doi = {https://doi.org/10.1029/JZ072i016p04245},
	number = {16},
	journal = {Journal of Geophysical Research},
	author = {{Lewis H. Cohen} and {William Klement}},
	year = {1967},
	pages = {4245--4251},
	file = {Journal of Geophysical Research  1896-1977 - 15 August 1967 - Cohen - High%E2%80%90low quartz inversion  Determination to 35-2:/Users/jdong/Zotero/storage/MQ46P9DQ/Journal of Geophysical Research  1896-1977 - 15 August 1967 - Cohen - High%E2%80%90low quartz inversion  Determination to 35-2.pdf:application/pdf},
}

@article{mirwald_lowhigh_1980,
	title = {The low‐high quartz and quartz‐coesite transition to 40 kbar between 600° and 1600°{C} and some reconnaissance data on the effect of {NaAlO}$_{\textrm{2}}$ component on the low quartz‐coesite transition},
	volume = {85},
	copyright = {http://onlinelibrary.wiley.com/termsAndConditions\#vor},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/JB085iB12p06983},
	doi = {10.1029/JB085iB12p06983},
	abstract = {The phase relations of low quartz, high quartz, and coesite were reinvestigated using extremely pure SiO
              2
              . The study was conducted with a piston‐cylinder apparatus employing low‐friction cells. While the low quartz‐coesite transition between 600° and 1100°C was determined by conventional quench techniques, the greater portion of this study relied on in situ methods (differential thermal analysis and a volumetric method referred to as differential pressure analysis). The agreement with previous results is good; however, the precision of present data is considerably higher. A comparison of our salt‐cell data with the raw data of previous studies shows a pressure loss due to friction of about 10\% for talc cells. A discussion of thermochemical aspects of the low quartz‐coesite transition indicates improved agreement between thermodynamic and experimental data. Reconnaissance data on the influence of the NaAlO
              2
              component show above 600°C in the absence of H
              2
              O a considerable shift of the quartz‐coesite boundary toward higher pressure (4 kbar at 1100°C). In the presence of H
              2
              O a partial liquid is formed, and the shift is reversed; the transition boundary is reduced 3 kbar and lies between 680° and 1000°C at even lower pressure than that of the pure SiO
              2
              modifications.},
	language = {en},
	number = {B12},
	urldate = {2025-01-28},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Mirwald, Peter W. and Massonne, H.‐J.},
	month = dec,
	year = {1980},
	pages = {6983--6990},
}

@article{bose_quartz-coesite_1995,
	title = {Quartz-coesite transition revisited; reversed experimental determination at 500-1200 degrees {C} and retrieved thermochemical properties},
	volume = {80},
	issn = {0003-004X},
	url = {https://pubs.geoscienceworld.org/ammin/article/80/3-4/231-238/42968},
	doi = {10.2138/am-1995-3-404},
	language = {en},
	number = {3-4},
	urldate = {2025-01-28},
	journal = {American Mineralogist},
	author = {Bose, Kunal and Ganguly, Jibamitra},
	month = apr,
	year = {1995},
	pages = {231--238},
}

@article{hudon_melting_2002,
	title = {Melting of β-quartz up to 2.0 {GPa} and thermodynamic optimization of the silica liquidus up to 6.0 {GPa}},
	volume = {130},
	copyright = {https://www.elsevier.com/tdm/userlicense/1.0/},
	issn = {00319201},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0031920102000055},
	doi = {10.1016/S0031-9201(02)00005-5},
	language = {en},
	number = {3-4},
	urldate = {2025-01-28},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Hudon, Pierre and Jung, In-Ho and Baker, Don R.},
	month = apr,
	year = {2002},
	pages = {159--174},
}


@incollection{suito_phase_1977,
	address = {New York},
	title = {Phase relations of pure {Mg}$_{\textrm{2}}${SiO}$_{\textrm{4}}$ up to 200 kilobars},
	booktitle = {High-{Pressure} {Research}: {Applications} in {Geophysics}},
	publisher = {Academic Press},
	author = {Suito, K.},
	year = {1977},
	pages = {255--266},
	file = {Suito (1977) book chapter.pdf:/Users/jdong/Zotero/storage/Z6CUWNJF/Suito (1977) book chapter.pdf:application/pdf},
}

@article{andrault_melting_2020,
	title = {Melting behavior of {SiO}$_{\textrm{2}}$ up to 120 {GPa}},
	volume = {47},
	issn = {0342-1791, 1432-2021},
	url = {https://link.springer.com/10.1007/s00269-019-01077-3},
	doi = {10.1007/s00269-019-01077-3},
	abstract = {The structure of liquid silicates is commonly described as a statistical mixture of various atomic entities with relative abundances that can vary with pressure, temperature, and composition. Unfortunately, this view remains largely theoretical due to scarce experimental reports on the silicate melt structure, in particular under pressure. We performed X-ray diffraction of the ­SiO2 end member to probe the melting curve up to {\textasciitilde} 120 GPa and 7000 K, and the melt structure up to {\textasciitilde} 80 GPa. We confirm the steep increase of the melting curve above {\textasciitilde} 14 GPa when stishovite becomes stable over coesite in subsolidus conditions, with a slope of about 80 K/GPa. Then, around 45 GPa and 5400 K, the melting curve flattens significantly, an effect most likely reflecting the densification of the S­ iO2 melt structure. The signal of diffuse X-ray scattering is compatible with a change of the Si coordination number from 4 to 6 along the melting curve, in agreement with previous works reporting a similar evolution during the cold compression of ­SiO2 glass. Because of the limited pressure range (within 10 to 20 GPa) in which the melting curve changes its slope, we speculate a difficult coexistence of tetrahedral S­ iO4 and octahedral ­SiO6 units in ­SiO2 melt at high pressures.},
	language = {en},
	number = {2},
	urldate = {2024-01-03},
	journal = {Physics and Chemistry of Minerals},
	author = {Andrault, D. and Morard, G. and Garbarino, G. and Mezouar, M. and Bouhifd, M. A. and Kawamoto, T.},
	month = feb,
	year = {2020},
	pages = {10},
	file = {Andrault et al. - 2020 - Melting behavior of SiO2 up to 120 GPa.pdf:/Users/jdong/Zotero/storage/2G3QURWJ/Andrault et al. - 2020 - Melting behavior of SiO2 up to 120 GPa.pdf:application/pdf},
}


@article{geng_ab_2024,
	title = {\textit{{Ab} initio} constraints on the melting of silica at high pressures up to 500 {GPa}},
	volume = {109},
	issn = {2469-9950, 2469-9969},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.109.024106},
	doi = {10.1103/PhysRevB.109.024106},
	language = {en},
	number = {2},
	urldate = {2024-07-19},
	journal = {Physical Review B},
	author = {Geng, Ming and Mohn, Chris E.},
	month = jan,
	year = {2024},
	pages = {024106},
	file = {Submitted Version:/Users/jdong/Zotero/storage/W4RFMFSF/Geng and Mohn - 2024 - Ab initio constraints on the melting of sil.pdf:application/pdf},
}
%%%mgsio3%%%
@article{PIERRU2022117770,
title = {Solidus melting of pyrolite and bridgmanite: Implication for the thermochemical state of the Earth's interior},
journal = {Earth and Planetary Science Letters},
volume = {595},
pages = {117770},
year = {2022},
issn = {0012-821X},
doi = {https://doi.org/10.1016/j.epsl.2022.117770},
url = {https://www.sciencedirect.com/science/article/pii/S0012821X2200406X},
author = {Rémy Pierru and Laure Pison and Antoine Mathieu and Emmanuel Gardés and Gaston Garbarino and Mohamed Mezouar and Louis Hennet and Denis Andrault},
keywords = {Earth's lower mantle, melting properties},
abstract = {Melting properties of the deep mantle remain controversial due to experimental difficulties; e.g., reports of solidus temperatures of mantle-relevant compositions span over ∼700 K at 2000 km depth. This situation limits our understanding of the thermochemical state of the Earth's interior. Using the laser heated diamond anvil cell (LH-DAC), we performed new experimental determination of the solidus profile of ultra-dry pyrolite and the solidus of two compositions of (Mg,Fe)(Si,Al)O3 bridgmanite (Bg). Melting was detected (i) from -the correlation between laser power and sample temperature, -changes of sample texture and -the level of visible light absorption, for all samples, (ii) using X-ray diffraction, for the MgSiO3 composition and (iii) after scanning electron microscope observations, for selected Fe-bearing samples. Special care was given to using ultra-dry experimental chambers and to determination of sample temperature. In particular, we discuss the wavelength-dependent thermal emission of silicate samples, which lowers the solidus by 100 to 300 K, compared to the grey-body assumption. The solidus of MgSiO3-Bg is in good agreement with previous reports using ab initio calculations and shock wave experiments. We observe a net decrease in the solid-liquid Clapeyron slope at 60(3) GPa and 4400(200) K, which can be related to rapid pressure-induced coordination change of Si in the melt. (Mg0.955,Fe0.045)(Si0.993,Al0.007)O3 Bg melts 600–800 K lower than MgSiO3-Bg. Its solidus evolves smoothly with pressure, suggesting progressive Si coordination change in the melt. In the pressure range investigated (24–135 GPa) Clapeyron slopes suggest rapid decrease of the volume of fusion, from 14 to 2% for MgSiO3 and from 9 to 3% for (Fe,Al)-bearing Bg, assuming congruent melting. By comparing the solidii of various silicates, it appears that the higher the number of cations, the less pronounced is the curvature of the solidus. This observation suggests that the relatively ordered structure of simple liquid compositions with a limited number of distinct network-modifying cations frustrates the coexistence of tetrahedrally and octahedrally coordinated Si polyhedral. The solidus of pyrolite presents a smooth evolution from 2200(100) K to 3950(200) K in the same pressure interval. This is very similar to our previous work on chondritic-type mantle. The new solidus is 200–300 K lower than that of KLB-1 peridotite, which can be related to more incompatible elements in pyrolite. It remains problematic that our solidus plots several 100 K higher than other recent measurements performed on pyrolite; we discuss the possibility of a higher water content in previous samples, compared to our experiments. Assuming a dry lowermost mantle, our results imply a core-mantle boundary temperature lower than 3950(200) K. Modeling the melting diagram at the core-mantle boundary suggests a pseudo-eutectic melt significantly depleted in SiO2, compared to the composition of the mean mantle.}
}
@article{okuda_electrical_2024,
	title = {Electrical {Conductivity} of {Dense} {MgSiO3} {Melt} {Under} {Static} {Compression}},
	volume = {51},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1029/2024GL109741},
	doi = {https://doi.org/10.1029/2024GL109741},
	abstract = {Abstract The magnetic fields of terrestrial planets are created by core convection. Molten silicate mantles could also generate magnetic fields through their convective motion, known as a silicate dynamo. Recent computational studies have suggested that silicate melts may exhibit high electrical conductivity (EC) at temperatures above 4000 K due to strong electronic conduction, which could activate a silicate dynamo. We determined the EC of dense molten MgSiO3 up to 71 GPa and 4490 K by static compression experiments. It jumped by one order of magnitude upon melting, but 57(27) S/m at 4490 K is much lower than previous predictions, suggesting that molten MgSiO3 carries charge via ions rather than predicted electronic conduction. Nevertheless, the strong temperature dependence of the ionic conductivity found in this study suggests that super-Earths’ hotter magma ocean with larger-scale convection could power a dynamo that drives magnetic fields, which plays key roles in sustaining planetary surface environments.},
	number = {12},
	journal = {Geophysical Research Letters},
	author = {Okuda, Yoshiyuki and Hirose, Kei and Ohta, Kenji and Kawaguchi-Imada, Saori and Oka, Kenta},
	year = {2024},
	note = {\_eprint: https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1029/2024GL109741},
	keywords = {electrical conductivity, high pressure, MgSiO3 melt, silicate dynamo},
	pages = {e2024GL109741},
	annote = {e2024GL109741 2024GL109741},
}

@article{akashi_orthoenstatiteclinoenstatite_2009,
	title = {Orthoenstatite/clinoenstatite phase transformation in {MgSiO}$_{\textrm{3}}$ at high‐pressure and high‐temperature determined by in situ {X}‐ray diffraction: {Implications} for nature of the {X} discontinuity},
	volume = {114},
	issn = {0148-0227},
	shorttitle = {Orthoenstatite/clinoenstatite phase transformation in {MgSiO} $_{\textrm{3}}$ at high‐pressure and high‐temperature determined by in situ {X}‐ray diffraction},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2008JB005894},
	doi = {10.1029/2008JB005894},
	abstract = {In the upper mantle, the X discontinuity at the depths of 240 to 340 km is observed in many localities, but its origin is under debate. The phase transformation of (Mg,Fe)SiO
              3
              from orthopyroxene to high‐pressure clinopyroxene has been proposed to cause this discontinuity. In this study, in situ X‐ray diffraction experiments were performed, and the orthoenstatite/high‐pressure clinoenstatite (
              C
              2/
              c
              ) phase boundary in the MgSiO
              3
              system was determined. All the experiments were carried out using a Kawai‐type multianvil apparatus installed at BL04B1 in SPring‐8, Hyogo, Japan. Two types of experiments were carried out: (1) “phase observation experiments” at varying pressures and temperatures and (2) “quench experiments” at fixed pressure and temperature. The phase boundary, determined precisely by integrating the results of both sets of experiments, was found to be
              P
              (GPa) = 0.0035
              T
              (°C) + 3.7, using a recent MgO pressure scale. The orthoenstatite/high‐pressure clinoenstatite phase boundary at 1400°C determined here is 0.7–1.0 GPa lower than previous reports based on quench experiments. The phase transformation of orthopyroxene is expected to occur at 260 km depth along a typical mantle geotherm, and the shallower part of the observed X discontinuity can be explained by this phase transformation.},
	language = {en},
	number = {B4},
	urldate = {2024-01-01},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Akashi, Akihiko and Nishihara, Yu and Takahashi, Eiichi and Nakajima, Yoichi and Tange, Yoshinori and Funakoshi, Ken‐ichi},
	year = {2009},
	pages = {2008JB005894},
	file = {Akashi et al. - 2009 - Orthoenstatiteclinoenstatite phase transformation.pdf:/Users/jdong/Zotero/storage/IPZRUIJA/Akashi et al. - 2009 - Orthoenstatiteclinoenstatite phase transformation.pdf:application/pdf},
}

@article{ono_situ_2005,
	title = {In situ observations of phase transition between perovskite and {CaIrO}$_{\textrm{3}}$-type phase in {MgSiO}$_{\textrm{3}}$ and pyrolitic mantle composition},
	volume = {236},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X05003547},
	doi = {10.1016/j.epsl.2005.06.001},
	abstract = {In situ observations of the perovskite–CaIrO3 phase transition in MgSiO3 and in pyrolitic compositions were carried out using a laser-heated diamond anvil cell interfaced with a synchrotron radiation source. For pure MgSiO3, the phase boundary between the orthorhombic Mg-perovskite and CaIrO3-type phases in the temperature range of 1300–3100 K was determined to be P (GPa) = 130 (F 3) + 0.0070 (F 0.0030) Â (T À 2500) (K) using platinum as a pressure calibrant. We confirmed that the CaIrO3-type phase remained stable up to pressures of at least 156 GPa and temperatures of 2600 K. The consistency of our results with previous theoretical calculations leads us to conclude that the 2700 km seismic discontinuity at the bottom of the lower mantle can be attributed to a phase transition to the CaIrO3-type phase. The phase change from an orthorhombic Mgperovskite to a CaIrO3-type bearing assemblage in a pyrolitic mantle composition was also observed at P = 125 GPa, which corresponds to the same mantle depth as the seismic discontinuity. The phase boundary between the orthorhombic Mgperovskite and CaIrO3-type bearing assemblage was determined to be P (GPa) = 124 (F 4) + 0.008 (F 0.005) Â (T À 2500) (K) using gold as a pressure calibrant. This transition boundary indicates that the temperature at a depth of 2700 km is about 2600 K, and the adiabatic temperature gradient in the lower mantle is estimated to be 0.31 K/km. The partition coefficients and the effect of some elements on the phase equilibrium between the orthorhombic MgSiO3 perovskite and CaIrO3-type MgSiO3 were estimated from ab initio calculations. Our experimental and theoretical results indicate that the DW layer consists of a CaIrO3-type bearing assemblage which is likely to have significant effect on the chemical and thermal evolution of the Earth’s mantle.},
	language = {en},
	number = {3-4},
	urldate = {2024-01-01},
	journal = {Earth and Planetary Science Letters},
	author = {Ono, S and Oganov, A},
	year = {2005},
	pages = {914--932},
	file = {Ono and Oganov - 2005 - In situ observations of phase transition between p.pdf:/Users/jdong/Zotero/storage/2AXTQGZE/Ono and Oganov - 2005 - In situ observations of phase transition between p.pdf:application/pdf;shen_1995_jgr.pdf:/Users/jdong/Zotero/storage/RGUEF4W2/shen_1995_jgr.pdf:application/pdf},
}

@article{ono_situ_2001,
	title = {\textit{{In} situ} {Observation} of ilmenite‐perovskite phase transition in {MgSiO}$_{\textrm{3}}$ using synchrotron radiation},
	volume = {28},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/1999GL008446},
	doi = {10.1029/1999GL008446},
	abstract = {In situ observationsof the ilmenite-perovskite transition in MgSiO3 were carried out in a multianvil high-pressuraepparatusinterfacedwith synchrotrornadiation. The phaseboundarybetweenilmeniteand perovskitein the temperaturerangeof 1300-1600K was determinedto be P (GPa) = 28.4(ñ0.4) - 0.0029(ñ0.0020)T (K) based on Jamieson'sequationof stateof gold [Jamiesonet al., 1982] andP (GPa)= 27.3(ñ0.4)- 0.0035(ñ0.0024)T (K) basedon Anderson'sequationof stateof gold[Andersonet al., 1989]. The consistencyof our results,usingJamieson'sequationof state,with previousstudiesobtainedby quenchmethodsleads us to concludethat the 660 km seismicdiscontinuityin the mantlecanbe attributeda phasetransitionto perovskitephase. However, the phase boundary based on the Anderson's equationof stateimpliesthatthedepthof the 660-km seismic discontinuitydoesnot matchthepressureof thistransition.},
	language = {en},
	number = {5},
	urldate = {2024-01-01},
	journal = {Geophysical Research Letters},
	author = {Ono, S. and Katsura, T. and Ito, E. and Kanzaki, M. and Yoneda, A. and Walter, M. J. and Urakawa, S. and Utsumi, W. and Funakoshi, K.},
	year = {2001},
	pages = {835--838},
	file = {Ono et al. - 2001 - In situ Observation of ilmenite‐perovskite .pdf:/Users/jdong/Zotero/storage/EZXY79EK/Ono et al. - 2001 - In situ Observation of ilmenite‐perovskite .pdf:application/pdf;tateno_2009_epsl_mgsio3.pdf:/Users/jdong/Zotero/storage/A63ZRSY8/tateno_2009_epsl_mgsio3.pdf:application/pdf},
}

@article{ono_equation_2006,
	title = {Equation of state of {CaIrO}$_{\textrm{3}}$-type {MgSiO}$_{\textrm{3}}$ up to 144 {GPa}},
	volume = {91},
	issn = {0003-004X},
	url = {https://www.degruyter.com/document/doi/10.2138/am.2006.2118/html},
	doi = {10.2138/am.2006.2118},
	abstract = {The structure and equation of state for CaIrO3-type MgSiO3 were determined using high-pressure powder X-ray diffraction from 116 to 144 GPa. The CaIrO3-type phase remained stable over this entire pressure range. At each pressure increment, the sample was heated with a laser to relax the deviatoric stress in the sample. Pressure-volume data could be ﬁtted to the Birch-Murnaghan equation of state with K0 = 237(1) GPa using Anderson’s gold pressure standard, when K0' and V0 were set to 4 and 162.86 Å3, respectively. This indicates that the bulk modulus of MgSiO3 decreases when the phase transition occurs, because the bulk modulus of perovskite-type MgSiO3 is 250–260 GPa. The b axis of the unit-cell parameter was more compressive than the a and c axes. The unit-cell volumes at high pressures, observed in high-pressure experiments, were slightly smaller than those predicted by theoretical studies.},
	language = {en},
	number = {2-3},
	urldate = {2024-01-01},
	journal = {American Mineralogist},
	author = {Ono, S.},
	year = {2006},
	pages = {475--478},
	file = {Ono - 2006 - Equation of state of CaIrO3-type MgSiO3 up to 144 .pdf:/Users/jdong/Zotero/storage/5T66IGNZ/ono_2006_am.pdf:application/pdf},
}


@article{ito_mgsio3_1985,
	title = {{MgSiO}$_{\textrm{3}}$ {Ilmenite}: {Calorimetry}, {Phase} {Equilibria}, and {Decomposition} at {Atmospheric} {Pressure}},
	volume = {70},
	number = {9-10},
	journal = {American Mineralogist},
	author = {Ito, Eiji and Navrotsky, Alexandar},
	year = {1985},
	pages = {1020--1026},
	file = {ito_1985_am_mgsio3.pdf:/Users/jdong/Zotero/storage/UKTG4MDN/ito_1985_am_mgsio3.pdf:application/pdf},
}

@article{presnall_melting_1990,
	title = {Melting of enstatite ({MgSiO} $_{\textrm{3}}$ ) from 10 to 16.5 {GPa} and the forsterite ({Mg} $_{\textrm{2}}$ {SiO} $_{\textrm{4}}$ )‐majorite ({MgSiO} $_{\textrm{3}}$ ) eutectic at 16.5 {GPa}: {Implications} for the origin of the mantle},
	volume = {95},
	copyright = {http://onlinelibrary.wiley.com/termsAndConditions\#vor},
	issn = {0148-0227},
	shorttitle = {Melting of enstatite ({MgSiO} $_{\textrm{3}}$ ) from 10 to 16.5 {GPa} and the forsterite ({Mg} $_{\textrm{2}}$ {SiO} $_{\textrm{4}}$ )‐majorite ({MgSiO} $_{\textrm{3}}$ ) eutectic at 16.5 {GPa}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/JB095iB10p15771},
	doi = {10.1029/JB095iB10p15771},
	abstract = {A split sphere multianvil apparatus (USSA 2000) has been used to determine the melting curve of enstatite (MgSiO
              3
              ) from 10 to 16.5 GPa and the forsterite (Mg
              2
              SiO
              4
              )‐majorite (MgSiO
              3
              ) eutectic at 16.5 GPa. Use of a new capsule material, rhenium, allowed long runs of up to 2 hours at temperatures up to 2380°C with no observed contamination of the sample and with stable temperature control. Melting temperatures of enstatite are up to 160°C higher than those of Kato and Kumazawa (1986a). Two invariant points have been located, one for orthoenstatite+clinoenstatite+liquid at 2230°C, 11.9 GPa, and one for clinoenstatite+majorite+liquid at 2370°C, 16.4 GPa. Forsterite melts incongruently at 2350°C, 16.5 GPa to liquid and AnhB (Mg
              14
              Si
              5
              O
              24
              ). In the system Mg
              2
              SiO
              4
              ‐MgSiO
              3
              at 16.5 GPa, the forsterite‐majorite eutectic has been located at 34 wt \% Mg
              2
              SiO
              4
              , a composition similar to that determined by Kato and Kumazawa (1986a) at 20 GPa but much lower in Mg
              2
              SiO
              4
              than several previous estimates based on melting experiments on mantle peridotite compositions. This forsterite‐poor location for the eutectic is in apparent conflict with the suggestion that the peridotitic upper mantle is a crystallized eutectic‐like liquid formed at about 16 GPa.},
	language = {en},
	number = {B10},
	urldate = {2024-07-20},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Presnall, D. C. and Gasparik, T.},
	month = sep,
	year = {1990},
	pages = {15771--15777},
}
@incollection{syono_melting_1992,
	address = {Washington, D. C.},
	series = {Geophysical {Monograph} {Series}},
	title = {Melting of {Ferromagnesian} {Silicates} {Under} the {Lower} {Mantle} {Conditions}},
	isbn = {978-1-118-66392-9 978-0-87590-034-6},
	url = {http://doi.wiley.com/10.1029/GM067p0315},
	urldate = {2024-07-20},
	booktitle = {High-{Pressure} {Research}: {Application} to {Earth} and {Planetary} {Sciences}},
	publisher = {American Geophysical Union},
	author = {Ito, E. and Katsura, T.},
	editor = {Syono, Yasuhiko and Manghnani, Murli H.},
	year = {1992},
	doi = {10.1029/GM067p0315},
	pages = {315--322},
}

@article{hinkel_stellar_2014,
	title = {{STELLAR} {ABUNDANCES} {IN} {THE} {SOLAR} {NEIGHBORHOOD}: {THE} {HYPATIA} {CATALOG}},
	volume = {148},
	copyright = {http://iopscience.iop.org/info/page/text-and-data-mining},
	issn = {0004-6256, 1538-3881},
	shorttitle = {{STELLAR} {ABUNDANCES} {IN} {THE} {SOLAR} {NEIGHBORHOOD}},
	url = {https://iopscience.iop.org/article/10.1088/0004-6256/148/3/54},
	doi = {10.1088/0004-6256/148/3/54},
	number = {3},
	urldate = {2024-07-22},
	journal = {The Astronomical Journal},
	author = {Hinkel, Natalie R. and Timmes, F.X. and Young, Patrick A. and Pagano, Michael D. and Turnbull, Margaret C.},
	month = aug,
	year = {2014},
	pages = {54},
	file = {Full Text:/Users/jdong/Zotero/storage/ZVNSN7PU/Hinkel et al. - 2014 - STELLAR ABUNDANCES IN THE SOLAR NEIGHBORHOOD THE .pdf:application/pdf},
}
@article{buder_galah_2021,
	title = {The {GALAH}+ survey: {Third} data release},
	volume = {506},
	copyright = {https://academic.oup.com/journals/pages/open\_access/funder\_policies/chorus/standard\_publication\_model},
	issn = {0035-8711, 1365-2966},
	shorttitle = {The {GALAH}+ survey},
	url = {https://academic.oup.com/mnras/article/506/1/150/6270919},
	doi = {10.1093/mnras/stab1242},
	abstract = {ABSTRACT
            The ensemble of chemical element abundance measurements for stars, along with precision distances and orbit properties, provides high-dimensional data to study the evolution of the Milky Way. With this third data release of the Galactic Archaeology with HERMES (GALAH) survey, we publish 678 423 spectra for 588 571 mostly nearby stars (81.2 per cent of stars are within \&lt;2 kpc), observed with the HERMES spectrograph at the Anglo-Australian Telescope. This release (hereafter GALAH+ DR3) includes all observations from GALAH Phase 1 (bright, main, and faint survey, 70 per cent), K2-HERMES (17 per cent), TESS-HERMES (5 per cent), and a subset of ancillary observations (8 per cent) including the bulge and \&gt;75 stellar clusters. We derive stellar parameters Teff, log g, [Fe/H], vmic, vbroad, and vrad using our modified version of the spectrum synthesis code Spectroscopy Made Easy (sme) and 1D marcs model atmospheres. We break spectroscopic degeneracies in our spectrum analysis with astrometry from Gaia DR2 and photometry from 2MASS. We report abundance ratios [X/Fe] for 30 different elements (11 of which are based on non-LTE computations) covering five nucleosynthetic pathways. We describe validations for accuracy and precision, flagging of peculiar stars/measurements and recommendations for using our results. Our catalogue comprises 65 per cent dwarfs, 34 per cent giants, and 1 per cent other/unclassified stars. Based on unflagged chemical composition and age, we find 62 per cent young low-\${\textbackslash}alpha\$, 9 per cent young high-\${\textbackslash}alpha\$, 27 per cent old high-\${\textbackslash}alpha\$, and 2 per cent stars with [Fe/H] ≤ −1. Based on kinematics, 4 per cent are halo stars. Several Value-Added-Catalogues, including stellar ages and dynamics, updated after Gaia eDR3, accompany this release and allow chrono-chemodynamic analyses, as we showcase.},
	language = {en},
	number = {1},
	urldate = {2024-07-22},
	journal = {Monthly Notices of the Royal Astronomical Society},
	author = {Buder, Sven and Sharma, Sanjib and Kos, Janez and Amarsi, Anish M and Nordlander, Thomas and Lind, Karin and Martell, Sarah L and Asplund, Martin and Bland-Hawthorn, Joss and Casey, Andrew R and De Silva, Gayandhi M and D’Orazi, Valentina and Freeman, Ken C and Hayden, Michael R and Lewis, Geraint F and Lin, Jane and Schlesinger, Katharine J and Simpson, Jeffrey D and Stello, Dennis and Zucker, Daniel B and Zwitter, Tomaž and Beeson, Kevin L and Buck, Tobias and Casagrande, Luca and Clark, Jake T and Čotar, Klemen and Da Costa, Gary S and de Grijs, Richard and Feuillet, Diane and Horner, Jonathan and Kafle, Prajwal R and Khanna, Shourya and Kobayashi, Chiaki and Liu, Fan and Montet, Benjamin T and Nandakumar, Govind and Nataf, David M and Ness, Melissa K and Spina, Lorenzo and Tepper-García, Thor and Ting(丁源森), Yuan-Sen and Traven, Gregor and Vogrinčič, Rok and Wittenmyer, Robert A and Wyse, Rosemary F G and Žerjal, Maruša and {GALAH Collaboration}},
	month = jul,
	year = {2021},
	pages = {150--201},
	file = {Accepted Version:/Users/jdong/Zotero/storage/YRNSE3BA/Buder et al. - 2021 - The GALAH+ survey Third data release.pdf:application/pdf},
}

@article{tateno_melting_2014,
	title = {Melting experiments on peridotite to lowermost mantle conditions},
	volume = {119},
	copyright = {http://onlinelibrary.wiley.com/termsAndConditions\#vor},
	issn = {2169-9313, 2169-9356},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1002/2013JB010616},
	doi = {10.1002/2013JB010616},
	abstract = {Abstract
            
              Melting experiments on a pyrolitic mantle material were performed in a pressure range from 34 to 179 GPa based on laser‐heated diamond‐anvil cell (DAC) techniques. The textural and chemical characterizations of quenched samples were made by using field‐emission‐type electron microprobe (FE‐EPMA). Melts formed by 46 to 77 wt.\% partial melting in this study were ultrabasic in composition and became more depleted in SiO
              2
              and more enriched in FeO with increasing pressure. Melting textures indicate that the liquidus phase changed from ferropericlase to MgSiO
              3
              ‐rich perovskite at least above 34 GPa and further to post‐perovskite. The first phase to melt (disappear) changed from CaSiO
              3
              perovskite to (Mg,Fe)O ferropericlase between 68 and 82 GPa. The stability of ferropericlase above solidus temperature shrinks with increasing pressure (melting last below 34 GPa and first 82 GPa), resulting in higher (MgO + FeO)/SiO
              2
              ratio in partial melt at higher pressure. Additionally, the Fe‐Mg distribution coefficients (
              K
              D
              ) between perovskite/post‐perovskite and melt decreased considerably with increasing pressure, leading to strong Fe‐enrichment in partial melts. It supports dense partial melts in a deep lower mantle, which migrate downward to the core mantle boundary (CMB).
            
          , 
            Key Points
            
              
                
                  Melting relations and chemical compositions of melt and solid to CMB conditions
                
                
                  Partial melt become more ultrabasic with increasing pressure
                
                
                  Strong Fe enrichment in partial melts formed at deep lower mantle},
	language = {en},
	number = {6},
	urldate = {2024-07-31},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Tateno, Shigehiko and Hirose, Kei and Ohishi, Yasuo},
	month = jun,
	year = {2014},
	pages = {4684--4694},
	file = {Full Text:/Users/dong2j/Zotero/storage/2EUN5J2P/Tateno et al. - 2014 - Melting experiments on peridotite to lowermost man.pdf:application/pdf},
}
@article{dragulet_partitioning_2024,
	title = {Partitioning of {Iron} {Between} ({Mg},{Fe}){SiO} $_{\textrm{3}}$ {Liquid} and {Bridgmanite}},
	volume = {51},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2023GL107979},
	doi = {10.1029/2023GL107979},
	abstract = {Abstract
            
              The evolution of the magma ocean that occupied the early Earth is influenced by the buoyancy of crystals in silicate liquid. At lower mantle pressures, silicate crystals are denser than the iso‐chemical liquid, but heavy elements like iron can cause crystals to float if they partition into the liquid phase. Crystal flotation allows for a basal magma ocean, which might explain geochemical anomalies in mantle‐derived magmas, seismic anomalies in the lower mantle, and the source of the Earth's early magnetic field. To examine whether a basal magma ocean is gravitationally stable, we investigate the degree of iron partitioning between (Mg,Fe)SiO
              3
              liquid and bridgmanite. By utilizing ab initio molecular dynamics simulations coupled with thermodynamic integration, we find that iron partitions into the liquid, and increasingly so with increasing pressure. Bridgmanite crystals are found to be buoyant at lower mantle conditions, stabilizing the basal magma ocean.
            
          , 
            Plain Language Summary
            The early Earth may have been in a completely molten state, and its evolution during this stage depends on whether crystals float or sink in magma. While crystals typically sink in magma near the Earth's surface, we find that crystals float in the deep Earth. This is because liquid at greater depths is enriched in iron, making it denser than the crystals. This suggests that there once was a stable magma layer below the solid mantle and above the core, which might explain several properties of the Earth's deep interior.
          , 
            Key Points
            
              
                
                  
                    The Fe‐Mg distribution coefficient between bridgmanite and (Mg,Fe)SiO
                    3
                    liquid is computed using ab‐initio simulations
                  
                
                
                  Iron is incompatible in bridgmanite and partitions into silicate liquid
                
                
                  Bridgmanite crystals are buoyant in the lower mantle, allowing for a basal magma ocean to be gravitationally stable},
	language = {en},
	number = {12},
	urldate = {2024-07-31},
	journal = {Geophysical Research Letters},
	author = {Dragulet, Francis and Stixrude, Lars},
	month = jun,
	year = {2024},
	pages = {e2023GL107979},
}
@article{stixrude_silicate_2020,
	title = {A silicate dynamo in the early {Earth}},
	volume = {11},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-020-14773-4},
	doi = {10.1038/s41467-020-14773-4},
	abstract = {Abstract
            The Earth’s magnetic field has operated for at least 3.4 billion years, yet how the ancient field was produced is still unknown. The core in the early Earth was surrounded by a molten silicate layer, a basal magma ocean that may have survived for more than one billion years. Here we use density functional theory-based molecular dynamics simulations to predict the electrical conductivity of silicate liquid at the conditions of the basal magma ocean: 100–140 GPa, and 4000–6000 K. We find that the electrical conductivity exceeds 10,000 S/m, more than 100 times that measured in silicate liquids at low pressure and temperature. The magnetic Reynolds number computed from our results exceeds the threshold for dynamo activity and the magnetic field strength is similar to that observed in the Archean paleomagnetic record. We therefore conclude that the Archean field was produced by the basal magma ocean.},
	language = {en},
	number = {1},
	urldate = {2024-07-31},
	journal = {Nature Communications},
	author = {Stixrude, Lars and Scipioni, Roberto and Desjarlais, Michael P.},
	month = feb,
	year = {2020},
	pages = {935},
	file = {Full Text:/Users/dong2j/Zotero/storage/WTCWUHL3/Stixrude et al. - 2020 - A silicate dynamo in the early Earth.pdf:application/pdf},
}
@article{helled_fuzzy_2024,
	title = {The {Fuzzy} {Cores} of {Jupiter} and {Saturn}},
	volume = {5},
	issn = {2576-604X, 2576-604X},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2024AV001171},
	doi = {10.1029/2024AV001171},
	abstract = {Abstract
            New interior models of Jupiter and Saturn suggest that both planets have “fuzzy cores.” These cores should be viewed as central regions that are enriched with heavy elements but are not distinct from the rest of the deep interior. These cores may contain large amounts of hydrogen and helium though small pure heavy‐element cores may also exist. New measurements along with advanced planetary modeling have revolutionized the way we think about the interiors of giant planets and provide important constraints for planet formation and evolution theories. These developments are also relevant for the characterization of giant exoplanets.
          , 
            Plain Language Summary
            For decades giant planets were assumed to have distinct heavy‐element cores in their deep interiors overlain by an envelope of hydrogen and helium. Measurements from the Juno and the Cassini missions strongly indicate that the internal structure of Jupiter and Saturn is much more complex, including inhomogeneities in composition and “fuzzy” cores. In Jupiter, this dilution might extend to more than one hundred Earth masses, while in Saturn it is less, though both planets have a diluted region that extends to many tens of percent of total radius. In both cases, a small central core composed of pure heavy elements may exist. These structures pose challenges for our understanding of giant planet formation and evolution.
          , 
            Key Points
            
              
                
                  The interiors of Jupiter and Saturn are complex, they include inhomogeneities in composition and “fuzzy” cores
                
                
                  The origin of the “fuzzy cores” is unknown, but is probably linked to the planetary formation process
                
                
                  Many open questions remain. Future modeling, observations, experiments, and links to exoplanet science can improve our understanding of the gas giants},
	language = {en},
	number = {2},
	urldate = {2024-07-31},
	journal = {AGU Advances},
	author = {Helled, Ravit and Stevenson, David J.},
	month = apr,
	year = {2024},
	pages = {e2024AV001171},
	file = {Full Text:/Users/dong2j/Zotero/storage/HQECTLNK/Helled and Stevenson - 2024 - The Fuzzy Cores of Jupiter and Saturn.pdf:application/pdf},
}
@article{muller_challenge_2020,
	title = {The challenge of forming a fuzzy core in {Jupiter}},
	volume = {638},
	copyright = {http://creativecommons.org/licenses/by/4.0},
	issn = {0004-6361, 1432-0746},
	url = {https://www.aanda.org/10.1051/0004-6361/201937376},
	doi = {10.1051/0004-6361/201937376},
	abstract = {Recent structure models of Jupiter that match Juno gravity data suggest that the planet harbours an extended region in its deep interior that is enriched with heavy elements: a so-called dilute or fuzzy core. This finding raises the question of what possible formation pathways could have lead to such a structure. We modelled Jupiter’s formation and long-term evolution, starting at late-stage formation before runaway gas accretion. The formation scenarios we considered include both primordial composition gradients, as well as gradients that are built as proto-Jupiter rapidly acquires its gaseous envelope. We then followed Jupiter’s evolution as it cools down and contracts, with a particular focus on the energy and material transport in the interior. We find that none of the scenarios we consider lead to a fuzzy core that is compatible with interior structure models. In all the cases, most of Jupiter’s envelope becomes convective and fully mixed after a few million years at most. This is true even when we considered a case where the gas accretion leads to a cold planet, and large amounts of heavy elements are accreted. We therefore conclude that it is very challenging to explain Jupiter’s dilute core from standard formation models. We suggest that future works should consider more complex formation pathways as well as the modelling of additional physical processes that could lead to Jupiter’s current-state internal structure.},
	urldate = {2024-07-31},
	journal = {Astronomy \& Astrophysics},
	author = {Müller, Simon and Helled, Ravit and Cumming, Andrew},
	month = jun,
	year = {2020},
	pages = {A121},
	file = {Full Text:/Users/dong2j/Zotero/storage/GLXCBTM6/Müller et al. - 2020 - The challenge of forming a fuzzy core in Jupiter.pdf:application/pdf},
}
@article{vazan_new_2022,
	title = {A {New} {Perspective} on the {Interiors} of {Ice}-rich {Planets}: {Ice}–{Rock} {Mixture} {Instead} of {Ice} on {Top} of {Rock}},
	volume = {926},
	issn = {0004-637X, 1538-4357},
	shorttitle = {A {New} {Perspective} on the {Interiors} of {Ice}-rich {Planets}},
	url = {https://iopscience.iop.org/article/10.3847/1538-4357/ac458c},
	doi = {10.3847/1538-4357/ac458c},
	abstract = {Abstract
            
              Ice-rich planets are formed exterior to the water ice line and thus are expected to contain a substantial amount of ice. The high ice content leads to unique conditions in the interior, under which the structure of a planet is affected by ice interaction with other metals. We apply experimental data of ice–rock interaction at high pressure, and calculate detailed thermal evolution for possible interior configurations of ice-rich planets, in the mass range of super-Earth to Neptunes (5–15
              M
              ⊕
              ). We model the effect of migration inward on the ice-rich interior by including the influences of stellar flux and envelope mass loss. We find that ice and rock are expected to remain mixed, due to miscibility at high pressure, in substantial parts of the planetary interior for billions of years. We also find that the deep interior of planetary twins that have migrated to different distances from the star are usually similar, if no mass loss occurs. Significant mass loss results in separation of the water from the rock on the surface and emergence of a volatile atmosphere of less than 1\% of the planet’s mass. The mass of the atmosphere of water/steam is limited by the ice–rock interaction. We conclude that when ice is abundant in planetary interiors the planet structure may differ significantly from the standard layered structure of a water shell on top of a rocky core. Similar structure is expected in both close-in and further-out planets.},
	number = {2},
	urldate = {2024-07-31},
	journal = {The Astrophysical Journal},
	author = {Vazan, Allona and Sari, Re’em and Kessel, Ronit},
	month = feb,
	year = {2022},
	pages = {150},
	file = {Full Text:/Users/dong2j/Zotero/storage/7JXVLGHD/Vazan et al. - 2022 - A New Perspective on the Interiors of Ice-rich Pla.pdf:application/pdf},
}
@incollection{guillot_interior_2006,
	address = {Cambridge},
	series = {Cambridge {Planetary} {Science}},
	title = {The {Interior} of {Jupiter}},
	isbn = {978-0-521-03545-3},
	booktitle = {Jupiter: the planet, satellites and magnetosphere},
	publisher = {Cambridge University Press},
	author = {Guillot, T. and Stevenson, D. J. and Hubbard, W. B. and Saumon, D.},
	year = {2006},
}


@article{li_ultrahigh-pressure_2022,
	title = {Ultrahigh-{Pressure} {Magnesium} {Hydrosilicates} as {Reservoirs} of {Water} in {Early} {Earth}},
	volume = {128},
	issn = {0031-9007, 1079-7114},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.128.035703},
	doi = {10.1103/PhysRevLett.128.035703},
	language = {en},
	number = {3},
	urldate = {2024-07-31},
	journal = {Physical Review Letters},
	author = {Li, Han-Fei and Oganov, Artem R. and Cui, Haixu and Zhou, Xiang-Feng and Dong, Xiao and Wang, Hui-Tian},
	month = jan,
	year = {2022},
	pages = {035703},
	file = {Submitted Version:/Users/dong2j/Zotero/storage/47T7AH6H/Li et al. - 2022 - Ultrahigh-Pressure Magnesium Hydrosilicates as Res.pdf:application/pdf},
}
@article{mankovich_diffuse_2021,
	title = {A diffuse core in {Saturn} revealed by ring seismology},
	volume = {5},
	issn = {2397-3366},
	url = {https://www.nature.com/articles/s41550-021-01448-3},
	doi = {10.1038/s41550-021-01448-3},
	language = {en},
	number = {11},
	urldate = {2024-08-01},
	journal = {Nature Astronomy},
	author = {Mankovich, Christopher R. and Fuller, Jim},
	month = aug,
	year = {2021},
	pages = {1103--1109},
	file = {Accepted Version:/Users/dong2j/Zotero/storage/EVZLT8U4/Mankovich and Fuller - 2021 - A diffuse core in Saturn revealed by ring seismolo.pdf:application/pdf},
}
@techreport{hofstadter_uranus_2024,
	address = {Pasadena, CA},
	title = {Uranus {Study} {Report}},
	institution = {W. M. Keck Institute for Space Studies (KISS)},
	author = {Hofstadter, Mark and Helled, Ravit and Stevenson, David},
	year = {2024},
	file = {Uranus_KISS.pdf:/Users/jdong/Zotero/storage/CK35H6F5/Uranus_KISS.pdf:application/pdf},
}
@article{nettelmann_uranus_2016,
	title = {Uranus evolution models with simple thermal boundary layers},
	volume = {275},
	issn = {00191035},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0019103516300537},
	doi = {10.1016/j.icarus.2016.04.008},
	language = {en},
	urldate = {2024-08-02},
	journal = {Icarus},
	author = {Nettelmann, N. and Wang, K. and Fortney, J.J. and Hamel, S. and Yellamilli, S. and Bethkenhagen, M. and Redmer, R.},
	month = sep,
	year = {2016},
	pages = {107--116},
	file = {Submitted Version:/Users/jdong/Zotero/storage/P7SERRN3/Nettelmann et al. - 2016 - Uranus evolution models with simple thermal bounda.pdf:application/pdf},
}
@article{swain_planet_2024,
	title = {Planet {Mass} and {Metallicity}: {The} {Exoplanets} and {Solar} {System} {Connection}},
	volume = {220},
	issn = {0038-6308, 1572-9672},
	shorttitle = {Planet {Mass} and {Metallicity}},
	url = {https://link.springer.com/10.1007/s11214-024-01098-7},
	doi = {10.1007/s11214-024-01098-7},
	language = {en},
	number = {6},
	urldate = {2025-01-20},
	journal = {Space Science Reviews},
	author = {Swain, Mark R. and Hasegawa, Yasuhiro and Thorngren, Daniel P. and Roudier, Gaël M.},
	month = sep,
	year = {2024},
	pages = {61},
	file = {Full Text:/Users/jdong/Zotero/storage/M8QHDW4L/Swain et al. - 2024 - Planet Mass and Metallicity The Exoplanets and So.pdf:application/pdf},
}
@article{liebske_melting_2012,
	title = {Melting phase relations in the {MgO}–{MgSiO3} system between 16 and {26GPa}: {Implications} for melting in {Earth}'s deep interior},
	volume = {345-348},
	copyright = {https://www.elsevier.com/tdm/userlicense/1.0/},
	issn = {0012821X},
	shorttitle = {Melting phase relations in the {MgO}–{MgSiO3} system between 16 and {26GPa}},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X12003226},
	doi = {10.1016/j.epsl.2012.06.038},
	language = {en},
	urldate = {2025-01-22},
	journal = {Earth and Planetary Science Letters},
	author = {Liebske, Christian and Frost, Daniel J.},
	month = sep,
	year = {2012},
	pages = {159--170},
}

@article{de_koker_thermodynamics_2013,
	title = {Thermodynamics of the {MgO}–{SiO2} liquid system in {Earth}'s lowermost mantle from first principles},
	volume = {361},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X12006449},
	doi = {10.1016/j.epsl.2012.11.026},
	language = {en},
	urldate = {2025-01-22},
	journal = {Earth and Planetary Science Letters},
	author = {De Koker, Nico and Karki, Bijaya B. and Stixrude, Lars},
	month = jan,
	year = {2013},
	pages = {58--63},
}


@article{ohnishi_melting_2017,
	title = {Melting relations in the {MgO}–{MgSiO3} system up to 70 {GPa}},
	volume = {44},
	issn = {0342-1791, 1432-2021},
	url = {http://link.springer.com/10.1007/s00269-017-0871-8},
	doi = {10.1007/s00269-017-0871-8},
	language = {en},
	number = {6},
	urldate = {2025-03-12},
	journal = {Physics and Chemistry of Minerals},
	author = {Ohnishi, Satoka and Kuwayama, Yasuhiro and Inoue, Toru},
	month = jun,
	year = {2017},
	pages = {445--453},
	file = {PDF:/Users/dong2j/Zotero/storage/4JNJ2N8R/Ohnishi et al. - 2017 - Melting relations in the MgO–MgSiO3 system up to 70 GPa.pdf:application/pdf},
}

@article{ozawa_experimental_2018,
	title = {Experimental {Determination} of {Eutectic} {Liquid} {Compositions} in the {MgO}‐{SiO}$_{\textrm{2}}$ {System} to the {Lowermost} {Mantle} {Pressures}},
	volume = {45},
	issn = {0094-8276, 1944-8007},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2018GL079313},
	doi = {10.1029/2018GL079313},
	abstract = {We have performed melting experiments on the MgO-SiO2 binary system to 139 GPa in a diamond anvil cell. Both MgO-MgSiO3 and MgSiO3-SiO2 eutectic compositions were examined by textural/chemical characterizations of recovered samples. Results demonstrate that the MgO-MgSiO3 eutectic becomes more enriched in MgO with increasing pressure and is close in composition to Mg2SiO4 at the core-mantle boundary (CMB) pressure. On the other hand, the MgSiO3-SiO2 eutectic is more SiO2-rich at higher pressure and exhibits SiO2/(MgO + SiO2) = 0.66 at the CMB. These have profound implications for a large-scale compositional stratiﬁcation possibly formed upon solidiﬁcation of a magma ocean. The MgO-MgSiO3 eutectic liquid being more MgO-rich than previously predicted suggests that only bridgmanite crystallizes up to 60 wt\% solidiﬁcation from a fully molten state of a pyrolitic lowermost mantle. In contrast, an SiO2 layer may develop when melting/crystallization occurs in rocky objects with silica-rich enstatite-chondritic compositions. Plain Language Summary MgO-SiO2 is the most important binary system to understand melting/crystallization processes in the Earth’s crust and mantle as well as those in other rocky objects. Its melting phase relations, in particular, eutectic compositions, also have profound implications for a large-scale compositional stratiﬁcation possibly formed upon solidiﬁcation of a magma ocean. However, the eutectic compositions in the MgO-MgSiO3 and MgSiO3-SiO2 systems have not been examined experimentally at the deep lower mantle conditions yet. Here we performed melting experiments and determined both of these eutectic compositions to 135 GPa, corresponding to the pressure at the bottom of the mantle, by a combination of high-pressure-temperature generation in a laser-heated diamond anvil cell and textural/compositional characterization of recovered samples. The results demonstrate that the MgO-MgSiO3 eutectic liquid is more MgO-rich than previously predicted. It suggests that a large volume of MgSiO3 bridgmanite-dominant-layer may have formed during crystallization of a deep magma ocean and is possibly still preserved up to the present in the Earth’s lower mantle. On the other hand, the MgSiO3-SiO2 eutectic liquid implies that an SiO2-phase-rich layer could develop when extensive melting occurs in rocky objects with silica-rich enstatite-chondritic compositions.},
	language = {en},
	number = {18},
	urldate = {2025-03-12},
	journal = {Geophysical Research Letters},
	author = {Ozawa, Keisuke and Anzai, Miyuki and Hirose, Kei and Sinmyo, Ryosuke and Tateno, Shigehiko},
	month = sep,
	year = {2018},
	pages = {9552--9558},
	file = {PDF:/Users/dong2j/Zotero/storage/QDJQ2DNQ/Ozawa et al. - 2018 - Experimental Determination of Eutectic Liquid Compositions in the MgO‐SiO2 System to the.pdf:application/pdf},
}

@article{baron_experimental_2017,
	title = {Experimental constraints on melting temperatures in the {MgO}–{SiO2} system at lower mantle pressures},
	volume = {472},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X17302807},
	doi = {10.1016/j.epsl.2017.05.020},
	language = {en},
	urldate = {2025-03-12},
	journal = {Earth and Planetary Science Letters},
	author = {Baron, Marzena A. and Lord, Oliver T. and Myhill, Robert and Thomson, Andrew R. and Wang, Weiwei and Trønnes, Reidar G. and Walter, Michael J.},
	month = aug,
	year = {2017},
	pages = {186--196},
	file = {PDF:/Users/dong2j/Zotero/storage/HAC54KUP/Baron et al. - 2017 - Experimental constraints on melting temperatures in the MgO–SiO2 system at lower mantle pressures.pdf:application/pdf},
}

@book{bowen_evolution_1928,
	address = {Princeton, N.J.},
	title = {The {Evolution} of the {Igneous} {Rocks}},
	publisher = {Princeton University Press},
	author = {Bowen, Norman Levi},
	year = {1928},
}
@article{miyazaki_timescale_2019,
	title = {On the {Timescale} of {Magma} {Ocean} {Solidification} and {Its} {Chemical} {Consequences}: 1. {Thermodynamic} {Database} for {Liquid} at {High} {Pressures}},
	volume = {124},
	issn = {2169-9313, 2169-9356},
	shorttitle = {On the {Timescale} of {Magma} {Ocean} {Solidification} and {Its} {Chemical} {Consequences}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2018JB016932},
	doi = {10.1029/2018JB016932},
	abstract = {We present a new method to construct an internally consistent thermodynamic model using a compilation of high-pressure melting experiments. The steepest descent method and Monte Carlo sampling are combined to constrain all model parameters simultaneously instead of determining each parameter sequentially from relevant experiments. Our approach is applied to the published melting experiments on mantle materials to obtain the thermodynamic parameters of the MgO-FeO-SiO2 ternary system. Inversion with the subsets of experimental data is conducted as well to investigate the source of discrepancy among existing studies, and the key parameters are found to be the thermal expansivity of SiO2 and the excess volume of mixing between MgO and SiO2. Mixing between FeO and SiO2 is only constrained with large uncertainty, which could also imply that oxides with low concentrations have minimal effects on melting. Constraining the thermodynamics of MgO and SiO2 will be important for a better understanding of mantle melting at high pressures.},
	language = {en},
	number = {4},
	urldate = {2025-03-13},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Miyazaki, Yoshinori and Korenaga, Jun},
	month = apr,
	year = {2019},
	pages = {3382--3398},
	file = {PDF:/Users/jdong/Zotero/storage/GNQF3G6G/Miyazaki and Korenaga - 2019 - On the Timescale of Magma Ocean Solidification and Its Chemical Consequences 1. Thermodynamic Datab.pdf:application/pdf},
}

@article{boukare_thermodynamics_2015,
	title = {Thermodynamics of the {MgO}‐{FeO}‐{SiO}$_{\textrm{2}}$ system up to 140 {GPa}: {Application} to the crystallization of {Earth}'s magma ocean},
	volume = {120},
	copyright = {http://onlinelibrary.wiley.com/termsAndConditions\#vor},
	issn = {2169-9313, 2169-9356},
	shorttitle = {Thermodynamics of the {MgO}‐{FeO}‐{SiO}$_{\textrm{2}}$ system up to 140 {GPa}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1002/2015JB011929},
	doi = {10.1002/2015JB011929},
	abstract = {Abstract
            
              At the end of Earth's accretion and after the core‐mantle segregation, the existence of a basal magma ocean at the top of the core‐mantle boundary (CMB) depends on the physical properties of mantle materials at relevant pressure and temperature. Present‐day deep mantle structures such as ultralow‐velocity zones and low‐shear velocity provinces might be directly linked to the still ongoing crystallization of a primordial magma ocean. We provide the first steps toward a self‐consistent thermodynamic model of magma ocean crystallization at high pressure. We build a solid‐liquid thermodynamic database for silicates in the MgO‐FeO‐SiO
              2
              system from 20 GPa to 140 GPa. We use already published chemical potentials for solids, liquid MgO, and SiO
              2
              . We derive standard state chemical potential for liquid FeO and mixing relations from various indirect observations. Using this database, we compute the ternary phase diagram in the MgO‐FeO‐SiO
              2
              system as a function of temperature and pressure. We confirm that the melt is lighter than the solid of same composition for all mantle conditions but at thermodynamic equilibrium, the iron‐rich liquid is denser than the solid in the deep mantle. We compute a whole fractional crystallization sequence of the mantle and show that an iron‐rich and fusible layer should be left above the CMB at the end of the crystallization.
            
          , 
            Key Points
            
              
                
                  We construct a thermodynamic database for solid and liquid silicates at HP/HT
                
                
                  We compute crystallization sequences of simplified peridotite composition
                
                
                  We show that a gravitationally stable melt layer at the CMB should form},
	language = {en},
	number = {9},
	urldate = {2025-03-13},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Boukaré, C.‐E. and Ricard, Y. and Fiquet, G.},
	month = sep,
	year = {2015},
	pages = {6085--6101},
	file = {Full Text:/Users/jdong/Zotero/storage/TKHJZ2J6/Boukaré et al. - 2015 - Thermodynamics of the MgO‐FeO‐SiO2 system up to 140 GPa Application to the crystallizati.pdf:application/pdf},
}

@article{yao_lower_2021,
	title = {Lower {Mantle} {Melting}: {Experiments} and {Thermodynamic} {Modeling} in the {System} {MgO}‐{SiO}$_{\textrm{2}}$},
	volume = {126},
	issn = {2169-9313, 2169-9356},
	shorttitle = {Lower {Mantle} {Melting}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2021JB022568},
	doi = {10.1029/2021JB022568},
	abstract = {Abstract
            
              Characterizing and modeling melting relations in the system MgO‐SiO
              2
              at lower mantle pressures rely on the location of the eutectic points for MgO‐MgSiO
              3
              and MgSiO
              3
              ‐SiO
              2
              . While at an uppermost lower mantle pressure there is general consensus on the eutectic composition in the former, large discrepancies exist for MgSiO
              3
              ‐SiO
              2
              from experiments in the diamond anvil cell, ab‐initio simulations and models built on them. In order to address this discrepancy, we have performed multi‐anvil press experiments at
              
              GPa for Mg
              4
              Si
              6
              O
              16
              and Mg
              3
              Si
              7
              O
              17
              at temperatures of
              
              K and
              
              K. In the experiments at
              
              K, we observe the presence of partial melt. The recovered Mg
              4
              Si
              6
              O
              16
              sample shows SiO
              2
              stishovite as the liquidus phase, and electron microprobe analysis of the quenched melt determines
              
              as the eutectic composition. We fit a thermodynamic model to describe the melting relations in the MgO‐SiO
              2
              system, and extrapolate to core‐mantle boundary pressure. At 136 GPa, we predict that the eutectic points have moved further away from enstatite composition, and solidus temperatures remain similar for MgO‐MgSiO
              3
              and MgSiO
              3
              ‐SiO
              2
              .
            
          , 
            Plain Language Summary
            
              Melting of rock in the Earth's deep interior is an important process that has shaped its geological history, and continues to do so to date. However, melting processes at high pressure have not been fully characterized to date, and here we perform experiments that help to better describe models for it. We do so for compositions in the MgSiO
              3
              ‐SiO
              2
              system that complement prior work for MgO‐MgSiO
              3
              ; combined, these experiments put important constraints on melting for the most important chemical components in the Earth's mantle, MgO‐SiO
              2
              . We find that when silicate melts crystallize, they do form the dominant lowermost mantle mineral, MgSiO
              3
              bridgmanite, only for a limited composition range in terms of the SiO
              2
              /MgO ratio; otherwise, MgO or SiO
              2
              form first, and generally at much higher temperatures. Melts in both the MgO‐MgSiO
              3
              and MgSiO
              3
              ‐SiO
              2
              systems become fully crystallized at very similar temperatures which suggests that a prior idea that the occurrence of partial melts in the Earth's deepest mantle is associated with different chemical composition does not hold if only the MgO‐SiO
              2
              system is considered.
            
          , 
            Key Points
            
              
                
                  
                    Multi‐anvil press experiments in the system MgSiO
                    3
                    ‐SiO
                    2
                    at 24 GPa located the eutectic at 53 mol\% SiO
                    2
                    and 2750 K
                  
                
                
                  
                    We build a thermodynamic model for MgO‐SiO
                    2
                    based on the data and other constraints that allows extrapolation to the core‐mantle boundary
                  
                
                
                  
                    Based on melting curves of MgO and SiO
                    2
                    and their liquid interaction parameter, the model predicts eutectic temperatures and compositions},
	language = {en},
	number = {12},
	urldate = {2025-01-22},
	journal = {Journal of Geophysical Research: Solid Earth},
	author = {Yao, Jie and Frost, Daniel J. and Steinle‐Neumann, Gerd},
	month = dec,
	year = {2021},
	pages = {e2021JB022568},
	file = {Full Text:/Users/jdong/Zotero/storage/R54CVPIC/Yao et al. - 2021 - Lower Mantle Melting Experiments and Thermodynami.pdf:application/pdf},
}
@article{dutta_high-pressure_2023,
	title = {High-pressure order-disorder transition in {Mg} 2 {Si} {O} 4 : {Implications} for super-{Earth} mineralogy},
	volume = {107},
	issn = {2469-9950, 2469-9969},
	shorttitle = {High-pressure order-disorder transition in {Mg} 2 {Si} {O} 4},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.107.184112},
	doi = {10.1103/PhysRevB.107.184112},
	language = {en},
	number = {18},
	urldate = {2025-01-24},
	journal = {Physical Review B},
	author = {Dutta, Rajkrishna and Tracy, Sally J. and Cohen, R. E.},
	month = may,
	year = {2023},
	pages = {184112},
	file = {Submitted Version:/Users/jdong/Zotero/storage/EZB8CGVR/Dutta et al. - 2023 - High-pressure order-disorder transition in Mg 2 Si.pdf:application/pdf},
}

@article{dutta_ultrahigh-pressure_2022,
	title = {Ultrahigh-pressure disordered eight-coordinated phase of {Mg}$_{\textrm{2}}$ {GeO}$_{\textrm{4}}$ : {Analogue} for super-{Earth} mantles},
	volume = {119},
	issn = {0027-8424, 1091-6490},
	shorttitle = {Ultrahigh-pressure disordered eight-coordinated phase of {Mg}$_{\textrm{2}}$ {GeO}$_{\textrm{4}}$},
	url = {https://pnas.org/doi/full/10.1073/pnas.2114424119},
	doi = {10.1073/pnas.2114424119},
	abstract = {Significance
            
              This work presents experimental evidence for the formation of a phase with eightfold coordination of germanium by oxygen in Mg
              2
              GeO
              4
              , a well-known analogue of Mg
              2
              SiO
              4
              at extreme pressure and temperatures. Using both experiments and theoretical computations, we have determined the structure, equation of state, and phase stability of this phase at pressures above 200 GPa. The existence of this phase in the silicate counterpart may play an important role in the structure and dynamics of the deep interiors of large, rocky exoplanets.
            
          , 
            
              Mg
              2
              GeO
              4
              is important as an analog for the ultrahigh-pressure behavior of Mg
              2
              SiO
              4
              , a major component of planetary interiors. In this study, we have investigated magnesium germanate to 275 GPa and over 2,000 K using a laser-heated diamond anvil cell combined with in situ synchrotron X-ray diffraction and density functional theory (DFT) computations. The experimental results are consistent with the formation of a phase with disordered Mg and Ge, in which germanium adopts eightfold coordination with oxygen: the cubic, Th
              3
              P
              4
              -type structure. DFT computations suggest partial Mg-Ge order, resulting in a tetragonal
              
                
                  
                    I
                    
                      4
                      ¯
                    
                    2
                    d
                  
                
              
              structure indistinguishable from
              
                
                  
                    I
                    
                      4
                      ¯
                    
                    3
                    d
                  
                
              
              Th
              3
              P
              4
              in our experiments. If applicable to silicates, the formation of this highly coordinated and intrinsically disordered phase may have important implications for the interior mineralogy of large, rocky extrasolar planets.},
	language = {en},
	number = {8},
	urldate = {2025-01-24},
	journal = {Proceedings of the National Academy of Sciences},
	author = {Dutta, Rajkrishna and Tracy, Sally June and Cohen, R. E. and Miozzi, Francesca and Luo, Kai and Yang, Jing and Burnley, Pamela C. and Smith, Dean and Meng, Yue and Chariton, Stella and Prakapenka, Vitali B. and Duffy, Thomas S.},
	month = feb,
	year = {2022},
	pages = {e2114424119},
	file = {Full Text:/Users/jdong/Zotero/storage/HQQXTMI7/Dutta et al. - 2022 - Ultrahigh-pressure disordered eight-coordinated ph.pdf:application/pdf},
}

@article{zurkowski_synthesis_2022,
	title = {Synthesis and {Stability} of an {Eight}‐{Coordinated} {Fe}$_{\textrm{3}}$ {O}$_{\textrm{4}}$ {High}‐{Pressure} {Phase}: {Implications} for the {Mantle} {Structure} of {Super}‐{Earths}},
	volume = {127},
	issn = {2169-9097, 2169-9100},
	shorttitle = {Synthesis and {Stability} of an {Eight}‐{Coordinated} {Fe}$_{\textrm{3}}$ {O}$_{\textrm{4}}$ {High}‐{Pressure} {Phase}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2022JE007344},
	doi = {10.1029/2022JE007344},
	abstract = {Abstract
            
              Super‐Earths ranging up to 10 Earth masses (M
              E
              ) with Earth‐like density are common among the observed exoplanets thus far, but their measured masses and radii do not uniquely elucidate their internal structure. Exploring the phase transitions in the Mg‐silicates that define the mantle‐structure of super‐Earths is critical to characterizing their interiors, yet the relevant terapascal conditions are experimentally challenging for direct structural analysis. Here we investigated the crystal chemistry of Fe
              3
              O
              4
              as a low‐pressure analog to Mg
              2
              SiO
              4
              between 45–115 GPa and up to 3000 K using powder and single crystal X‐ray diffraction in the laser‐heated diamond anvil cell. Between 60–115 GPa and above 2000 K, Fe
              3
              O
              4
              adopts an 8‐fold coordinated Th
              3
              P
              4
              ‐type structure (
              I
              ‐43d,
              Z
               = 4) with disordered Fe
              2+
              and Fe
              3+
              into one metal site. This Fe‐oxide phase is isostructural with that predicted for Mg
              2
              SiO
              4
              above 500 GPa in super‐Earth mantles and suggests that Mg
              2
              SiO
              4
              can incorporate both ferric and ferrous iron at these conditions. The pressure‐volume behavior observed in this 8‐fold coordinated Fe
              3
              O
              4
              indicates a maximum 4\% density increase across the 6‐ to 8‐fold coordination transition in the analog Mg‐silicate. Reassessment of the FeO—Fe
              3
              O
              4
              fugacity buffer considering the Fe
              3
              O
              4
              phase relationships identified in this study reveals that increasing pressure and temperature to 120 GPa and 3000 K in Earth and planetary mantles drives iron toward oxidation.
            
          , 
            Plain Language Summary
            
              Thousands of exoplanets have been discovered so far, and a sizable portion of them, known as “super‐Earths,” are much more massive than Earth but have an Earth‐like density. In order to accurately model super‐Earth interiors, their high pressure‐temperature mineralogy must be determined. Previous studies have predicted that an ultra‐dense Mg
              2
              SiO
              4
              phase becomes stable above 500 GPa and is the predominant mineral in the mantles of super‐Earths. The stability of this phase would mark the onset of 8‐fold Si–O coordination—a critical densification boundary. Here we have identified that Fe
              3
              O
              4
              undergoes an analogous 6 – to 8 – fold coordination transition and adopts the same structure above 60 GPa and 2000 K. We have employed powder and single‐crystal X‐ray diffraction to explore the stability and structural properties of this 8‐fold coordinated Fe
              3
              O
              4
              phase and the results suggest that the analog silicate is likely an iron‐bearing phase and that the onset of its stability is associated with approximately a 4\% density increase in super‐Earth mantles.
            
          , 
            Key Points
            
              
                
                  
                    Fe
                    3
                    O
                    4
                    was explored to 115 GPa and 3000 K using powder and single‐crystal X‐ray diffraction as an analog to Mg
                    2
                    SiO
                    4
                    in super‐Earth mantles
                  
                
                
                  
                    Above 60 GPa and 2000 K, Fe
                    3
                    O
                    4
                    transitions to an 8‐fold coordinated, Th
                    3
                    P
                    4
                    ‐related structure
                  
                
                
                  The analog coordination increase in silicates would result in a ∼4\% density increase in super‐Earth mantles},
	language = {en},
	number = {8},
	urldate = {2025-01-24},
	journal = {Journal of Geophysical Research: Planets},
	author = {Zurkowski, C. C. and Yang, J. and Chariton, S. and Prakapenka, V. B. and Fei, Y.},
	month = aug,
	year = {2022},
	pages = {e2022JE007344},
	file = {Full Text PDF:/Users/jdong/Zotero/storage/2TB8MHNH/Zurkowski et al. - 2022 - Synthesis and Stability of an Eight‐Coordinated Fe3 O4 High‐Pressure Phase Im.pdf:application/pdf},
}

@article{tonks_magma_1993,
	title = {Magma ocean formation due to giant impacts},
	volume = {98},
	copyright = {http://onlinelibrary.wiley.com/termsAndConditions\#vor},
	issn = {0148-0227},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/92JE02726},
	doi = {10.1029/92JE02726},
	abstract = {Current understanding of the last stages of planetary accretion suggests that mass and energy accumulation are dominated by a few large impacts. An important thermal consequence of such impacts is melting and formation of a large melt pond. If the planet's isostatic adjustment time scale is short compared to the magma pond's cooling time scale, the melt may be extruded onto the surface and form a magma ocean of approximately uniform depth. Although a giant impact striking at 10–15 km s
              −1
              deposits enough energy to melt the entire planet, the distribution of that energy is important in determining the thermal outcome of the collision. We examine the thermal effects of giant impacts by estimating the melt volume generated by the initial shock wave and corresponding magma ocean depths. Additionally, we examine the effects of the planet's initial temperature on the generated melt volume. The Hugoniot curve plotted in pressure‐entropy space is used to determine the shock pressure required to completely melt the material. For room temperature dunite, this pressure is about 150 GPa and the partial melt region is narrow. For dunite initially at the solidus temperature, this pressure is about 115 GPa. The partial melt region extends throughout the planet. Once the melting pressure is known, an impact melting model based on the second Hugoniot equation, the linear shock‐particle velocity relationship, and the empirical particle velocity‐distance relationship is used to estimate the radial distance melting occurred from the impact site. Once the distance is found, the melt region's geometry determines the associated melt volume. Partial melt volume is also estimated. The melt fraction that is not excavated during crater formation is estimated and magma ocean depths resulting from both excavated and retained melt are calculated. The model is also used to estimate the fraction of a planet melted by the initial shock wave. Nominal conditions of the Moon‐forming giant impact (projectile/planet mass = 0.14, impact speed = 15 km s
              −1
              ) generate melting of 30–65\% of the planet depending on its initial temperature. Whole planet melting requires projectile/planet mass ratios of {\textgreater} 0.4 for a 15 km s
              −1
              impact if the planet was near its solidus before the impact. Isostatic relaxation may generate a significant volume of additional melting.},
	language = {en},
	number = {E3},
	urldate = {2025-01-24},
	journal = {Journal of Geophysical Research: Planets},
	author = {Tonks, W. Brian and Melosh, H. Jay},
	month = mar,
	year = {1993},
	pages = {5319--5333},
}

@article{nakajima_scaling_2021,
	title = {Scaling laws for the geometry of an impact-induced magma ocean},
	volume = {568},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X21002429},
	doi = {10.1016/j.epsl.2021.116983},
	language = {en},
	urldate = {2025-01-24},
	journal = {Earth and Planetary Science Letters},
	author = {Nakajima, Miki and Golabek, Gregor J. and Wünnemann, Kai and Rubie, David C. and Burger, Christoph and Melosh, Henry J. and Jacobson, Seth A. and Manske, Lukas and Hull, Scott D.},
	month = aug,
	year = {2021},
	pages = {116983},
	file = {Submitted Version:/Users/jdong/Zotero/storage/DVBLVMZU/Nakajima et al. - 2021 - Scaling laws for the geometry of an impact-induced magma ocean.pdf:application/pdf},
}

@article{lherm_thermal_2024,
	title = {Thermal and magnetic evolution of an {Earth}-like planet with a basal magma ocean},
	volume = {356},
	issn = {00319201},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0031920124001250},
	doi = {10.1016/j.pepi.2024.107267},
	language = {en},
	urldate = {2025-01-24},
	journal = {Physics of the Earth and Planetary Interiors},
	author = {Lherm, Victor and Nakajima, Miki and Blackman, Eric G.},
	month = nov,
	year = {2024},
	pages = {107267},
}
@incollection{newsom_fluid_1990,
	title = {Fluid {Dynamics} {Of} {Core} {Formation}},
	isbn = {978-0-19-506619-7 978-0-19-770971-9},
	url = {https://academic.oup.com/book/53843/chapter/422184173},
	abstract = {Abstract
            Past discussions of core formation are incorrect or incomplete because they assume that metallic iron­ rich liquid is able to migrate through a mostly solid silicate matrix by percolation, prior to macrosegregation and diapiric descent. Experimental and theoretical considerations suggest that percolation is largely prevented because of the high surface tension of iron. Two alternative views of core formation are offered. One assumes that percolation is possible in the deep mantle ( where perovskite is the major phase). Iron is then supplied to the deep mantle by Rayleigh-Taylor instabilities of a silicate­ iron suspension in the shallow mantle, and drains efficiently from the deepest mantle into the core by Darcy flow. The other model assumes complete or nearly complete melting of all or part of the mantle. Despite vigorous convection, iron droplets approximately one centimeter in radius are predicted and settle rapidly by Stokes flow, either to the core or into a layer or ponds that provide iron-rich diapirs that can descend to the core. These stories generally suggest very efficient core formation in the sense that the t\vphantom{\{}\}pical residence time of metallic iron in the mantle is orders of magnitude shorter tban the formation time of Earth (-108 years). Good chemical equilibrium between mantle and core phases is also predicted in many cases. Geochemical constraints and implications relevant to these scenarios are discussed but are largely inconclusive. The tentative inference of rapid core formation on Mars suggests a magma ocean and iron rainout.},
	language = {en},
	urldate = {2025-01-24},
	booktitle = {Origin of the {Earth}},
	publisher = {Oxford University PressNew York, NY},
	author = {Stevenson, D J},
	editor = {Newsom, Horton E and Jones, John H},
	month = oct,
	year = {1990},
	doi = {10.1093/oso/9780195066197.003.0014},
	pages = {231--249},
}

@incollection{newsom_heat_1990,
	title = {Heat {And} {Mass} {Transport} {In} {The} {Early} {Earth}},
	isbn = {978-0-19-506619-7 978-0-19-770971-9},
	url = {https://academic.oup.com/book/53843/chapter/422184157},
	abstract = {Abstract
            Mass transport was responsible for establishing the main stratification of the Earth ( core, mantle, and crust) and also was the dominant means of heat transport through most of the Earth’s history. During early accretion, impacts supplied the heat input and also enhanced heat loss by stirring the near-surface. Initial core segregation probably began catastrophically when the Earth was about half of its present radius and homogenized the temperature near the melting temperature of the C. Thereafter, core segregation would have been rate-limited by accretion. Subsequent thermal evolution would have depended on whether the surface was insulated by a thick atmosphere or a buoyant crust, either of which might have pertnitted a magma ocean to accumulate. Magma extruding onto a cold slllface is a potent heat removal mechanism: In this case accretion in much less than 1 m.y. would have been required for a magma ocean to accumulate, and a magma ocean generated by a late giant impact would cool to a mush in about 1000 years. Solid-state mantle convection would have begun soon after initial core segregation ( or upon establishment of a cool surface). Mantle convection would have been enhanced by continuing core segregation and melt extraction of heat. At a mean temperature perhaps 100°C higher than at present, the mantle would have entered a regime in which a further increase by 100°C would have required increasing the heat input by one or two orders of magnitude because of heat extraction by melt. In the latter regime, intrasilicate density differences may have played an important role. A substantial magma ocean seems likely only in the cases of an insulated slllface or a late giant impact. As the Earth cooled, there may have been one or more transitions in tectonic style, but how these might relate to the accumulation, chemistry, and structural style of the preserved continental crust is still not clear. The lack of clear evidence for any compositional stratification in the present mantle cautions against models involving substantial early stratification.},
	language = {en},
	urldate = {2025-01-24},
	booktitle = {Origin of the {Earth}},
	publisher = {Oxford University PressNew York, NY},
	author = {Davies, G F},
	editor = {Newsom, Horton E and Jones, John H},
	month = oct,
	year = {1990},
	doi = {10.1093/oso/9780195066197.003.0011},
	pages = {175--194},
}

@incollection{newsom_physics_1990,
	title = {The {Physics} {Of} {Crystal} {Settling} {And} {Suspension} {In} {A} {Turbulent} {Magma} {Ocean}},
	isbn = {978-0-19-506619-7 978-0-19-770971-9},
	url = {https://academic.oup.com/book/53843/chapter/422184152},
	abstract = {Abstract
            It is widely assumed that a magma ocean on either the Earth or the Moon would necessarily differentiate by fractional crystallization. Geochemists and petrologists making this ption, however, have so Jar fulled to take into account the physics of crystal suspension in a planetary-scale convecting system. In the first part of this paper we show that convective velocities in a deep ultramafic magma ocean on either the Earth or the Moon are sufficiently rapid to suspend large crystals. 1bis demonstration involves aspects of convective theory and the mechanics of suspension that may be unfamiliar to most planetary scientists. Indeed, the problem has more affinities to aeolian transport in a deep planetary atmosphere than to traditional studies of magma convection. A vigorously convecting system can be divided into three distinct regions: an upper conductive boundary layer, a sublayer dominated byviscous forces, and a volume of turbulent fluid whose flow is controlled by inertial forces. 1bis inertial flow zone, which does not exist in the more familiar subsolidus convection, supports large-scale turbulent eddies that are analogous to gusty winds in a planetary atmospheric convective system. The criterion for suspension is derived from empirical studies of sediment transport and is given by the Rouse number, which is the ratio between the tenninal velocity of the crystals and the turbulent friction velocity. Settling ( or flotation) only takes place for Rouse numbers greater than about. We present several studies of magma ocean evolution with realistic rheological properties and cooling histories. The results show that on both the Earth and Moon crystals up to 1-2 cm in diameter can be suspended from the onset of cooling. In the later stages of cooling, as viscosity increases, crystals of 10 cm to more than I m in diameter may be suspended A surprising feature of our analysis is that the ability of a magma ocean to suspend crystals is only weakly dependent on gravity and depth: Viscosity is the major factor determining suspension. 1bis result raises a serious problem for the lunar magma ocean hypothesis, because the differentiation of an anorthositic crust strongly suggests that crystal fractionation did occur. We offer an explanation for this apparent anomaly by appealing to the low lunar gravity. Since pressure in the Moon increases only slowly with depth, the solidus and liquidus temperatures are · nearly independent of depth. In a convecting magma ocean on the Moon adiabats lie between the solidus and liquidus at all depths, so that growing crystals circulate through the ocean for long periods of time without dissolving. Under these circumstances they may grow large enough to settle out, resulting in the observed differentiation. In contrast, on the Earth the liquidus and solidus profiles are steeper than an adiabat so crystallization only takes place over a restricted depth range near the bottom of the ocean. Convective velocities are so high that crystals liti lciiting in this zone do not have time to grow larger than a few microns and are thus incapable of settling out. In this way even a totally molten initial Earth may have fulled to differentiate by fractional crystallization.},
	language = {en},
	urldate = {2025-01-24},
	booktitle = {Origin of the {Earth}},
	publisher = {Oxford University PressNew York, NY},
	author = {Tonks, W B and Melosh, H J},
	editor = {Newsom, Horton E and Jones, John H},
	month = oct,
	year = {1990},
	doi = {10.1093/oso/9780195066197.003.0010},
	pages = {151--174},
}

@article{dong_nonlinearity_2025,
	title = {Nonlinearity of the post-spinel transition and its expression in slabs and plumes worldwide},
	volume = {16},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-025-56231-z},
	doi = {10.1038/s41467-025-56231-z},
	abstract = {Abstract
            Phase transitions in the mantle control its internal dynamics and structure. The post-spinel transition marks the upper–lower mantle boundary, where ringwoodite dissociates into bridgmanite plus ferropericlase, and its Clapeyron slope regulates mantle flow across it. This interaction has previously been assumed to have no lateral spatial variations, based on the assumption of a linear post-spinel boundary in pressure and temperature. Here we present laser-heated diamond anvil cell experiments with synchrotron X-ray diffraction to better constrain this boundary, especially at higher temperatures. Combining our data with results from the literature, and using a global analysis based on machine learning, we find a pronounced nonlinearity in the post-spinel boundary, with its slope ranging from –4 MPa/K at 2100 K, to –2 MPa/K at 1950 K, and to 0 MPa/K at 1600 K. Changes in temperature over time and space can therefore cause the post-spinel transition to have variable effects on mantle convection and the movement of subducting slabs and upwelling plumes.},
	language = {en},
	number = {1},
	urldate = {2025-01-30},
	journal = {Nature Communications},
	author = {Dong, Junjie and Fischer, Rebecca A. and Stixrude, Lars P. and Brennan, Matthew C. and Daviau, Kierstin and Suer, Terry-Ann and Turner, Katlyn M. and Meng, Yue and Prakapenka, Vitali B.},
	month = jan,
	year = {2025},
	pages = {1039},
}
@article{faccenda_role_2017,
	title = {The role of solid–solid phase transitions in mantle convection},
	volume = {268-271},
	issn = {00244937},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0024493716303930},
	doi = {10.1016/j.lithos.2016.11.007},
	language = {en},
	urldate = {2025-02-07},
	journal = {Lithos},
	author = {Faccenda, Manuele and Dal Zilio, Luca},
	month = jan,
	year = {2017},
	pages = {198--224},
}

@article{tackley_mantle_2013,
	title = {Mantle dynamics in super-{Earths}: {Post}-perovskite rheology and self-regulation of viscosity},
	volume = {225},
	copyright = {https://www.elsevier.com/tdm/userlicense/1.0/},
	issn = {00191035},
	shorttitle = {Mantle dynamics in super-{Earths}},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0019103513001231},
	doi = {10.1016/j.icarus.2013.03.013},
	language = {en},
	number = {1},
	urldate = {2025-02-07},
	journal = {Icarus},
	author = {Tackley, P.J. and Ammann, M. and Brodholt, J.P. and Dobson, D.P. and Valencia, D.},
	month = jul,
	year = {2013},
	pages = {50--61},
	file = {Submitted Version:/Users/jdong/Zotero/storage/XFTHM3VA/Tackley et al. - 2013 - Mantle dynamics in super-Earths Post-perovskite rheology and self-regulation of viscosity.pdf:application/pdf},
}

@article{shahnas_focused_2021,
	title = {Focused {Penetrative} {Plumes}: {A} {Possible} {Consequence} of the {Dissociation} {Transition} of {Post}‐{Perovskite} at ∼0.9 {TPa} in {Massive} {Rocky} {Super}‐{Earths}},
	volume = {22},
	issn = {1525-2027, 1525-2027},
	shorttitle = {Focused {Penetrative} {Plumes}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2021GC009910},
	doi = {10.1029/2021GC009910},
	abstract = {Abstract
            
              Based on the standard view of depth‐increasing viscosity in the mantle of rocky planets, convection in the deep mantle of these planets is expected to become less likely as the size of planet increases. However, a recent theoretical study suggests that above 100 GPa pressure, the mantle viscosity can instead decrease with pressure at higher depths. We explore the potential impact of this type of viscosity structure on the nature of mantle convection in a super‐Earth planet of size GJ 876 d with a mass of ∼7.33 M
              ⊕
              (M
              ⊕
              : Earth's mass). The pressures at the bottom of the mantle of GJ 876 d allow MgSiO
              3
              post‐perovskite to dissociate into magnesium oxide (MgO) and relatively highly oxidized magnesium silicate MgSi
              2
              O
              5
              at 0.9 TPa with highly negative Clapeyron slope. Our 3D‐spherical numerical model results suggest that for sufficiently low values of viscosity at the transition depth, a vigorous layered mantle convection may develop at the bottom of GJ 876 d‐size super‐Earth. Focused penetrative plumes originating from the deep mantle layered region can survive and stabilize over very long geological timescales and reach to the surface, which may induce unique circumstances of volcanism and tectonic activity.
            
          , 
            Plain Language Summary
            
              A planet is made habitable by a suitable atmosphere, evolving at a right distance from the host star, a protective magnetic field shielding the planet from solar and cosmic harmful radiations, and proper elements required for life such as carbon, oxygen, and water. A further key element is plate tectonics as driven by mantle convection, in order to help regulate the composition and temperature of the atmosphere. Here we study more about the poorly understood processes of mantle convection in a super‐Earth sized planet: GJ 876 d with a mass of ∼7.33 M
              ⊕
              . The predicted dissociation transition of minerals MgSiO
              3
              ‐post‐perovskite into magnesium oxide (MgO) and magnesium silicate MgSi
              2
              O
              5
              at 0.9 TPa likely occurs near the bottom of the planet's mantle. Our 3D‐control volume numerical model results suggest that with the theoretically predicted dissociation transition and new theoretical estimations of the mantle viscosity at high pressures, a layered convection may occur above the core‐mantle boundary (CMB). Model results suggest that massive penetrative superplumes may originate from the top boundary of the layered region at about 500 km from the CMB and approach to the surface. Such mantle superplumes may sustain volcanism and plate tectonics for very long geological timescales.
            
          , 
            Key Points
            
              
                
                  The pPv‐dissociation transition may cause deep mantle layering in the large super‐Earth planets from which superplumes may originate},
	language = {en},
	number = {8},
	urldate = {2025-02-07},
	journal = {Geochemistry, Geophysics, Geosystems},
	author = {Shahnas, M. H. and Pysklywec, R. N.},
	month = aug,
	year = {2021},
	pages = {e2021GC009910},
	file = {Full Text:/Users/jdong/Zotero/storage/NPMIQCH4/Shahnas and Pysklywec - 2021 - Focused Penetrative Plumes A Possible Consequence of the Dissociation Transition of Post‐Perovskite.pdf:application/pdf},
}

@article{miyagoshi_thermal_2015,
	title = {Thermal convection and the convective regime diagram in super-{Earths}: {REGIMES} {OF} {CONVECTION} {IN} {SUPER}-{EARTHS}},
	volume = {120},
	copyright = {http://doi.wiley.com/10.1002/tdm\_license\_1.1},
	issn = {21699097},
	shorttitle = {Thermal convection and the convective regime diagram in super-{Earths}},
	url = {http://doi.wiley.com/10.1002/2015JE004793},
	doi = {10.1002/2015JE004793},
	language = {en},
	number = {7},
	urldate = {2025-02-07},
	journal = {Journal of Geophysical Research: Planets},
	author = {Miyagoshi, Takehiro and Kameyama, Masanori and Ogawa, Masaki},
	month = jul,
	year = {2015},
	pages = {1267--1278},
}

@article{shahnas_penetrative_2018,
	title = {Penetrative {Convection} in {Super}‐{Earth} {Planets}: {Consequences} of {MgSiO}$_{\textrm{3}}$ {Postperovskite} {Dissociation} {Transition} and {Implications} for {Super}‐{Earth} {GJ} 876 d},
	volume = {123},
	issn = {2169-9097, 2169-9100},
	shorttitle = {Penetrative {Convection} in {Super}‐{Earth} {Planets}},
	url = {https://agupubs.onlinelibrary.wiley.com/doi/10.1029/2018JE005633},
	doi = {10.1029/2018JE005633},
	abstract = {Abstract
            
              Theoretical studies suggest that MgSiO
              3
              postperovskite dissociates into MgO and MgSi
              2
              O
              5
              at 0.9 TPa, and MgSi
              2
              O
              5
              dissociates into MgO and SiO
              2
              at 2.1 TPa, both with negative Clapeyron slopes. In addition, unlike a conventional view, the viscosity in super‐Earth planets is proposed to decrease with pressure when pressure exceeds {\textasciitilde}0.1 TPa. Employing 2‐D‐axisymmtric and 3‐D‐spherical control volume compressible models, we perform an investigation on the impact of deep mantle dissociation of postperovskite into oxides, in conjunction with variations of the mantle viscosity, on the degree of the deep mantle layering, and the consequences of this layering on cooling of the rocky planets similar to super‐Earth GJ 876 d. Small‐scale convection in a layer of thickness {\textasciitilde}500 km from which penetrative plumes originate, develops above the core‐mantle boundary (CMB) in the models for which the viscosity at the dissociation transition depth and below is less than {\textasciitilde}10
              23
               Pa·s. Due to the buffering effect of this deep mantle layering, while the mean mantle temperature above the layer decreases, resulting in a viscosity increase above the layer, it increases in the layered region above the CMB. This leads to a further reduction in viscosity at the bottom of the mantle. The effect is enhanced with increasing the CMB temperature and the contrast in thermal expansivity. The cooling rate of the planet decreases in the layered models due to the buffering effect of this deep mantle transition, as well as the influence of the viscosity increase above transition depth.
            
          , 
            Key Points
            
              
                
                  
                    MgSiO
                    3
                    postperovskite dissociation into MgO and MgSi
                    2
                    O
                    5
                    at 0.9 TP may cause deep mantle layering in super‐Earth planets
                  
                
                
                  The postperovskite dissociation transition‐induced layer above the CMB can reduce the cooling rate of the super‐Earth planet
                
                
                  Penetrative convection flows may originate from the pPv dissociation transition‐induced layer above the CMB in super‐Earth planets},
	language = {en},
	number = {8},
	urldate = {2025-02-07},
	journal = {Journal of Geophysical Research: Planets},
	author = {Shahnas, M. H. and Pysklywec, R. N. and Yuen, D. A.},
	month = aug,
	year = {2018},
	pages = {2162--2177},
}
@article{thomson_experimental_2014,
	title = {Experimental determination of melting in the systems enstatite-magnesite and magnesite-calcite from 15 to 80 {GPa}},
	volume = {99},
	issn = {0003-004X},
	url = {https://www.degruyter.com/document/doi/10.2138/am.2014.4735/html},
	doi = {10.2138/am.2014.4735},
	language = {en},
	number = {8-9},
	urldate = {2025-02-08},
	journal = {American Mineralogist},
	author = {Thomson, A. R. and Walter, M. J. and Lord, O. T. and Kohn, S. C.},
	month = aug,
	year = {2014},
	pages = {1544--1554},
}
@article{stixrude_structure_2005,
	title = {Structure and {Freezing} of {MgSiO}$_{\textrm{3}}$ {Liquid} in {Earth}'s {Lower} {Mantle}},
	volume = {310},
	issn = {0036-8075, 1095-9203},
	url = {https://www.science.org/doi/10.1126/science.1116952},
	doi = {10.1126/science.1116952},
	abstract = {First-principles molecular-dynamics simulations show that over the pressure regime of Earth's mantle the mean silicon-oxygen coordination number of magnesium metasilicate liquid changes nearly linearly from 4 to 6. The density contrast between liquid and crystal decreases by a factor of nearly 5 over the mantle pressure regime and is 4\% at the core-mantle boundary. The ab initio melting curve, obtained by integration of the Clausius-Clapeyron equation, yields a melting temperature at the core-mantle boundary of 5400 ± 600 kelvins.},
	language = {en},
	number = {5746},
	urldate = {2025-02-08},
	journal = {Science},
	author = {Stixrude, Lars and Karki, Bijaya},
	month = oct,
	year = {2005},
	pages = {297--299},
}
@article{insixiengmay_mgo_2025,
	title = {{MgO} miscibility in liquid iron},
	volume = {654},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X2500041X},
	doi = {10.1016/j.epsl.2025.119242},
	language = {en},
	urldate = {2025-02-10},
	journal = {Earth and Planetary Science Letters},
	author = {Insixiengmay, Leslie and Stixrude, Lars},
	month = mar,
	year = {2025},
	pages = {119242},
	file = {Submitted Version:/Users/jdong/Zotero/storage/CRMKHFBD/Insixiengmay and Stixrude - 2025 - MgO miscibility in liquid iron.pdf:application/pdf},
}

@article{wahl_high-temperature_2015,
	title = {High-temperature miscibility of iron and rock during terrestrial planet formation},
	volume = {410},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X14007067},
	doi = {10.1016/j.epsl.2014.11.014},
	language = {en},
	urldate = {2025-02-10},
	journal = {Earth and Planetary Science Letters},
	author = {Wahl, Sean M. and Militzer, Burkhard},
	month = jan,
	year = {2015},
	pages = {25--33},
	file = {Submitted Version:/Users/jdong/Zotero/storage/7WBASZCG/Wahl and Militzer - 2015 - High-temperature miscibility of iron and rock during terrestrial planet formation.pdf:application/pdf},
}

@incollection{solomatov_magma_2007,
	title = {Magma {Oceans} and {Primordial} {Mantle} {Differentiation}},
	copyright = {https://www.elsevier.com/tdm/userlicense/1.0/},
	isbn = {978-0-444-52748-6},
	url = {https://linkinghub.elsevier.com/retrieve/pii/B9780444527486001413},
	language = {en},
	urldate = {2025-02-10},
	booktitle = {Treatise on {Geophysics}},
	publisher = {Elsevier},
	author = {Solomatov, V.},
	year = {2007},
	doi = {10.1016/B978-044452748-6.00141-3},
	pages = {91--119},
}
@article{fischer_equation_2011,
	title = {Equation of state and phase diagram of {FeO}},
	volume = {304},
	issn = {0012821X},
	url = {https://linkinghub.elsevier.com/retrieve/pii/S0012821X11000963},
	doi = {10.1016/j.epsl.2011.02.025},
	language = {en},
	number = {3-4},
	urldate = {2025-02-11},
	journal = {Earth and Planetary Science Letters},
	author = {Fischer, Rebecca A. and Campbell, Andrew J. and Shofner, Gregory A. and Lord, Oliver T. and Dera, Przemyslaw and Prakapenka, Vitali B.},
	month = apr,
	year = {2011},
	pages = {496--502},
	file = {Submitted Version:/Users/dong2j/Zotero/storage/4XHIWISE/Fischer et al. - 2011 - Equation of state and phase diagram of FeO.pdf:application/pdf},
}

@article{lindsley_ferrosilite_1964,
	title = {Ferrosilite ({FeSiO}$_{\textrm{3}}$): {Synthesis} at {High} {Pressures} and {Temperatures}},
	volume = {144},
	issn = {0036-8075, 1095-9203},
	shorttitle = {Ferrosilite ({FeSiO}$_{\textrm{3}}$ )},
	url = {https://www.science.org/doi/10.1126/science.144.3614.73},
	doi = {10.1126/science.144.3614.73},
	abstract = {The FeSiO
              3
              (ferrosilite) end member of the pyroxene series is not known as a pure mineral in nature and cannot be synthesized at atmospheric pressure. It is readily synthesized, however, at pressures from 18 to 45 kb and temperatures from 1150° to 1400°C. Its refractive indices approach those predicted for ferrosilite and it melts incongruently to an Fe
              2
              SiO
              4
              -rich liquid plus quartz.},
	language = {en},
	number = {3614},
	urldate = {2025-02-11},
	journal = {Science},
	author = {Lindsley, D. H. and Davis, B. T.C. and Macgregor, I. D.},
	month = apr,
	year = {1964},
	pages = {73--74},
}
@article{kingma_transformation_1995,
	title = {Transformation of stishovite to a denser phase at lower-mantle pressures},
	volume = {374},
	copyright = {http://www.springer.com/tdm},
	issn = {0028-0836, 1476-4687},
	url = {https://www.nature.com/articles/374243a0},
	doi = {10.1038/374243a0},
	language = {en},
	number = {6519},
	urldate = {2025-02-11},
	journal = {Nature},
	author = {Kingma, Kathleen J. and Cohen, Ronald E. and Hemley, Russell J. and Mao, Ho-kwang},
	month = mar,
	year = {1995},
	pages = {243--245},
}

